All Byzantine Agreement Problems are Expensive

Byzantine agreement, arguably the most fundamental problem in distributed computing, operates among n processes, out of which t < n can exhibit arbitrary failures. The problem states that all correct (non-faulty) processes must eventually decide (termination) the same value (agreement) from a set of admissible values defined by the proposals of the processes (validity). Depending on the exact version of the validity property, Byzantine agreement comes in different forms, from Byzantine broadcast to strong and weak consensus, to modern variants of the problem introduced in today's blockchain systems. Regardless of the specific flavor of the agreement problem, its communication cost is a fundamental metric whose improvement has been the focus of decades of research. The Dolev-Reischuk bound, one of the most celebrated results in distributed computing, proved 40 years ago that, at least for Byzantine broadcast, no deterministic solution can do better than Omega(t^2) exchanged messages in the worst case. Since then, it remained unknown whether the quadratic lower bound extends to seemingly weaker variants of Byzantine agreement. This paper answers the question in the affirmative, closing this long-standing open problem. Namely, we prove that any non-trivial agreement problem requires Omega(t^2) messages to be exchanged in the worst case. To prove the general lower bound, we determine the weakest Byzantine agreement problem and show, via a novel indistinguishability argument, that it incurs Omega(t^2) exchanged messages.

==> depricated/introduction.tex <==
\section{Introduction}

% \iffalse

% \section{Introduction}
% % \jovan{Work in progress}\manuel{continuing...}

% Consensus~\cite{LSP82},  a fundamental problem in
% distributed computing, stands as the cornerstone of state machine replication (SMR)~\cite{CL02,adya2002farsite,abd2005fault,kotla2004high,veronese2011efficient,amir2006scaling,kotla2007zyzzyva,malkhi2019flexible,momose2021multi} as well as certain cryptographic protocols~\cite{ben2019completeness,galil1987cryptographic}.
% Consensus has received a lot of attention recently with the advent of blockchain systems~\cite{abraham2016solida,chen2016algorand,abraham2016solidus,luu2015scp,correia2019byzantine,CGL18,buchman2016tendermint}.
% % Recently, the interest for the consensus problem has reemerged due to the advent of blockchain systems~\cite{abraham2016solida,chen2016algorand,abraham2016solidus,luu2015scp,correia2019byzantine,CGL18,buchman2016tendermint}. 
% % Thus, it comes as no surprise that Byzantine consensus is one of the most studied problems in the literature.

% Essentially, the consensus problem is posed in a system of $n$ processes, 
% out of which $t < n$ can be faulty and the rest are correct. 
% Correct processes propose each a value and seek to decide the same value.
% We consider 
% "Byzantine" consensus where a faulty process can behave in an arbitrary manner.
% While the exact definition of consensus might vary, two properties 
% typically remain identical: (1) \emph{termination}, requiring correct  processes to eventually decide, and (2) \emph{agreement}, preventing them from deciding different values.
% Satisfying only these two properties is straightforward: 
% any correct process decides the same, predetermined value.
% To preclude such trivial solutions and make consensus useful, 
% an additional property is necessary: \emph{validity}, defining which decisions are admissible.
% Naturally, different validity properties yield different variants of the problem.
% %In this paper, we study the validity property of the Byzantine consensus problem in the standard partially synchronous setting~\cite{DLS88}.

% % Due to the advent of blockchain, interest in Byzantine consensus has reignited.
% % This has lead numerous new advances in the last decade alone, culminating in the first message and communication optimal solutions (and the closure of a 40-year old problem).
% % However, these optimal solutions only concern the best understood variant of the problem: Byzantine Consensus with \emph{Strong Validity}.

% \paragraph{Background on validity.}
% Not all validity properties have been equally studied in the literature.
% One of the best understood properties is \emph{Strong Validity}~\cite{civit2022byzantine,CGL18,KMM03,abraham2017brief}, 
% stipulating that, if all correct processes propose the same value, 
% only that value can be decided.
% Another common property is \emph{Weak Validity}~\cite{civit2022byzantine,CGG21,yin2019hotstuff}, 
% affirming that if all processes are correct and 
% propose the same value, that value must be decided.
% In fact, several other validity properties can be defined~\cite{fitzi2003efficient,siu1998reaching,stolz2016byzantine,melnyk2018byzantine}.
% {\bf Rachid: we need to cite here more validity properties.}
% \jovan{I added the citations. Do you want me to expand on them?}


% While validity may appear as an inconspicuous property, 
% its exact definition has a big impact on the Byzantine consensus problem, and its solutions.
% For example, the seminal Dolev-Reischuk bound~\cite{dolev1985bounds} 
% shows that any solution to the Byzantine consensus problem with \emph{Strong Validity} incurs a quadratic number of messages; this bound is tight as recently shown by Civit \emph{et al.}~\cite{civit2022byzantine} and Lewis-Pye~\cite{lewis2022quadratic}.
% % is one of the few properties foxr which lower-bounds on message and communication complexity are known (i.e., the seminal Dolev-Reischuk bound \cite{dolev1985bounds}), as well as optimal upper-bounds (the recent work by Civit et al \cite{civit2022byzantine}).
% By contrast, while there have been several improvements to the performance of Byzantine consensus with \emph{Weak Validity} over the last 40 years (e.g., \cite{yin2019hotstuff, lewis2022quadratic, civit2022byzantine}), the (tight) lower bound on message complexity has remained unknown.
% (Although the bound is conjectured to be the same as for \emph{Strong Validity}, to the best of our knowledge, it has not been formally proven.)
% % \emph{External Validity}, which states that a value is admissible only if it satisfies a given boolean predicate, is a validity property of critical importance to blockchain systems.
% Moreover, many other fundamental questions remain unanswered:
% \begin{compactitem}
% \item What does it take for a specific validity property to make consensus solvable? 

% \item What are the (best) upper and lower bounds on the message complexity for the consensus problem given a specific validity property?

% \item Is there a hierarchy of validity properties (e.g., a ``strongest'' validity property)?
% \end{compactitem}
% As far as we are aware, no general, in-depth study of the validity property has ever been conducted, despite its importance and the growing interest from the research community~\cite{aboutvalidity}.

% % \paragraph{Technical overview.}
% % We mathematically define a validity property as a function which maps assignments of proposals to correct processes into admissible decisions.
% % The aforementioned assignments of proposals are named \emph{input configurations}.




% \paragraph{Contributions.}
% This paper studies the impact of the validity property on the solvability and complexity of Byzantine consensus in a partially synchronous setting.
% We start by providing a generic and precise formalism for the analysis of validity properties.
% In our formalism, a validity property is defined as a function which maps assignments of proposals to correct processes into admissible decisions.
% Moreover, we say that a validity property is \emph{solvable} if it makes Byzantine consensus solvable.
% This simple yet expressive model allows us to define key relations between proposal assignments, namely \emph{similarity} and \emph{compatibility}, which have general implications on all validity properties: by building on these relations we are able to capture fundamental concepts, such as those of \emph{indistinguishability} and \emph{partitioning attacks}, and summarily apply them to any validity property.
% %(This is perhaps best exemplified by our main intermediate result, \emph{canonical similarity}, which we re-use extensively throughout this paper.)


% \fi

%\iffalse
\section{Introduction}
% \jovan{Work in progress}\manuel{continuing...}

Consensus~\cite{LSP82} is the cornerstone of state machine replication (SMR)~\cite{CL02,adya2002farsite,abd2005fault,kotla2004high,veronese2011efficient,amir2006scaling,kotla2007zyzzyva,malkhi2019flexible,momose2021multi}, as well as various distributed algorithms~\cite{GS01, ben2019completeness,galil1987cryptographic, gilbert2010rambo}.
Recently, it has received a lot of attention with the advent of blockchain systems~\cite{abraham2016solida,chen2016algorand,abraham2016solidus,luu2015scp,correia2019byzantine,CGL18,buchman2016tendermint}.
The consensus problem is posed in a system of $n$ processes, out of which $t < n$ can be \emph{faulty}, and the rest are \emph{correct}.
Each correct process proposes a value, and consensus enables correct processes to decide on a common value.
In this paper, we consider Byzantine~\cite{LSP82} consensus, where faulty processes can behave arbitrarily.
% , in the partially synchronous setting~\cite{DLS88}.
% , where faulty processes can behave in an arbitrary manner.
While the exact definition of the problem might vary, two properties are always present: (1) \emph{termination}, requiring correct  processes to eventually decide, and (2) \emph{agreement}, preventing them from deciding different values.
It is not hard to devise an algorithm that satisfies only these two properties: 
every correct process decides the same, predetermined value. 
However, this algorithm is vacuous. 
To preclude such trivial solutions and render consensus meaningful, 
an additional property is required -- \emph{validity} -- defining which decisions are admissible.
%Naturally, different validity properties yield different variants of the problem.
% %In this paper, we study the validity property of the Byzantine consensus problem in the standard partially synchronous setting~\cite{DLS88}.

% is a fundamental problem of distributed computing.
% Since its emergence, it has been one of the most studied problems in the field.
% Today, it stands as the cornerstone of state machine replication (SMR)~\cite{CL02,adya2002farsite,abd2005fault,kotla2004high,veronese2011efficient,amir2006scaling,kotla2007zyzzyva,malkhi2019flexible,momose2021multi}, certain cryptographic protocols~\cite{ben2019completeness,galil1987cryptographic}, as well as blockchain systems~\cite{abraham2016solida,chen2016algorand,abraham2016solidus,luu2015scp,correia2019byzantine,CGL18,buchman2016tendermint}.
% Recently, the interest for the consensus problem has reemerged due to the advent of blockchain systems~\cite{abraham2016solida,chen2016algorand,abraham2016solidus,luu2015scp,correia2019byzantine,CGL18,buchman2016tendermint}. 
% Thus, it comes as no surprise that Byzantine consensus is one of the most studied problems in the literature.

% Essentially, Byzantine consensus allows $n$ processes to agree on a common value despite up to $t < n$ arbitrary process failures. While the exact definition of consensus might vary, two properties typically remain identical: (1) \emph{termination}, requiring correct (non-faulty) processes to eventually decide, and (2) \emph{agreement}, preventing them from deciding different values. Notice that satisfying just these two properties is straightforward: any correct process decides the same, predetermined value. To preclude trivial solutions and make consensus useful, an additional property is necessary: \emph{validity}, defining which decisions are admissible. Naturally, different validity properties yield different variants of the problem. In this paper, we study the influence validity properties have on the Byzantine consensus problem in the classical partially synchronous setting~\cite{DLS88}.

% Due to the advent of blockchain, interest in Byzantine consensus has reignited.
% This has lead numerous new advances in the last decade alone, culminating in the first message and communication optimal solutions (and the closure of a 40-year old problem).
% However, these optimal solutions only concern the best understood variant of the problem: Byzantine Consensus with \emph{Strong Validity}.

\paragraph{The many faces of validity.}
The literature contains many flavors of validity~\cite{AbrahamAD04,civit2022byzantine,CGL18,abraham2017brief,KMM03,CGG21,yin2019hotstuff,fitzi2003efficient,siu1998reaching,stolz2016byzantine,melnyk2018byzantine}.
% Not all validity properties have received equal attention in the literature.
% in the literature.
One of the most studied properties is \emph{Strong Validity}~\cite{civit2022byzantine,CGL18,KMM03,abraham2017brief}, stipulating that, if all correct processes propose the same value, only that value can be decided.
Another common property is \emph{Weak Validity}~\cite{civit2022byzantine,CGG21,yin2019hotstuff}, affirming that, if all processes are correct and propose the same value, that value must be decided. 
In fact, many other variants of the property have been considered~\cite{fitzi2003efficient,siu1998reaching,stolz2016byzantine,melnyk2018byzantine}.
While validity may appear as an inconspicuous property, its exact definition has a big impact on our understanding of consensus algorithms.
For example, the seminal Dolev-Reischuk bound~\cite{dolev1985bounds} states that any solution to consensus with \emph{Strong Validity} incurs a quadratic number of messages;  it was recently proven that the bound is tight~\cite{Momose2021,civit2022byzantine,lewis2022quadratic}.
% this bound is tight as recently shown by in~\cite{civit2022byzantine} and~\cite{lewis2022quadratic}.
% is one of the few properties foxr which lower-bounds on message and communication complexity are known (i.e., the seminal Dolev-Reischuk bound \cite{dolev1985bounds}), as well as optimal upper-bounds (the recent work by Civit et al \cite{civit2022byzantine}).
In contrast, while there have been several improvements to the performance of consensus with \emph{Weak Validity} over the last 40 years~\cite{yin2019hotstuff, lewis2022quadratic, civit2022byzantine}, the (tight) lower bound on message complexity remains unknown.
(Although the bound is conjectured to be the same as for \emph{Strong Validity}, this has yet to be formally proven.)
% \emph{External Validity}, which states that a value is admissible only if it satisfies a given boolean predicate, is a validity property of critical importance to blockchain systems.
Many other fundamental questions remain unanswered:
\begin{compactitem}
\item What does it take for a specific validity property to make consensus solvable? 

\item What are the (best) upper and lower bounds on the message complexity of consensus with any specific validity property?

\item Is there a hierarchy of validity properties (e.g., a ``strongest'' validity property)?
\end{compactitem}
To the best of our knowledge, no in-depth study of the validity property has ever been conducted, despite its importance and the emerging interest from the research community~\cite{aboutvalidity,CKN21}.

% \paragraph{Technical overview.}
% We mathematically define a validity property as a function which maps assignments of proposals to correct processes into admissible decisions.
% The aforementioned assignments of proposals are named \emph{input configurations}.




\paragraph{Contributions.}
% This paper studies the impact of the validity property on the solvability and complexity of Byzantine consensus in a partially synchronous setting.
%If a validity property makes Byzantine consensus solvable, we say that the property itself is \emph{solvable}.
%In this paper, we present the following contributions:
We propose a precise mathematical formalism for the analysis of validity properties.
We define a validity property as a mapping from assignments of proposals into admissible decisions.
Although simple, our formalism enables us to determine the exact impact of validity on the solvability and complexity of consensus in the classical partially synchronous model~\cite{DLS88}, and answer the aforementioned open questions.
Namely, we provide the following contributions:
\begin{compactitem} 
    \item We classify all validity properties into solvable and unsolvable ones.
    (If a validity property makes consensus solvable, we say that the property itself is \emph{solvable}.)
    % \jovan{Why indulgent? Indulgent algorithms tolerate "wrong" failure detectors (if I am not mistaken). But, in the Byzantine case, we do not have failure detectors.}
    Specifically, for $n \leq 3t$, we show that only \emph{trivial} validity properties (for which there exists an always-admissible decision) are solvable.
    In the case of $n > 3t$, we define the \emph{similarity condition}, which we prove to be necessary and sufficient for a validity property to be solvable.
    
    \item
    We prove that all non-trivial (and solvable) validity properties require $\Omega(t^2)$ exchanged messages.
    This result extends the Dolev-Reischuk bound~\cite{dolev1985bounds}, proven only for \emph{Strong Validity}, to \emph{all} ``reasonable'' validity properties.
    
    \item 
    Finally, we present \general, a general consensus algorithm for all solvable (and non-trivial) validity properties.
    % \jovan{Why do we cite indulgent algorithms? If we should, I think we need to explain it; otherwise, it might be confusing.}
    Assuming a threshold signature scheme, \general exchanges $O(n^2)$ messages.
    % complexity.
    Thus, together with our lower bound, \general implies a fundamental result in partial synchrony: given $t \in \Omega(n)$, all (non-trivial) consensus variants have $\Theta(n^2)$ message complexity.
    \Cref{fig:classification_landscape} summarizes our findings.
\end{compactitem}

\iffalse
We start by providing a generic and precise formalism for the analysis of validity properties.
In our formalism, a validity property is defined as a function which maps assignments of proposals to correct processes into admissible decisions.
Moreover, we say that a validity property is \emph{solvable} if it makes Byzantine consensus solvable.
We present the following contributions (summarized in \Cref{fig:classification_landscape}):

% In this paper, we provide a generic and precise formalism for the analysis of validity properties, and present the following contributions (summarized in \Cref{fig:classification_landscape}):

\emph{(i)} For $n \leq 3t$, we prove that a validity property is solvable only if it is \emph{trivial} (there exists an always-admissible decision).

% that Byzantine consensus can only be solved with a \emph{trivial} validity property (there exists an always-admissible decision).
% a validity property is solvable only if it is \emph{trivial}, i.e., there exists an ``always-admissible'' decision.
% which is always admissible.
% Our proof employs a non-trivial adaptation of the traditional partitioning argument.

\emph{(ii)} We define the \emph{similarity condition}, and prove that, if $n > 3t$, a validity property is solvable if and only if it satisfies the similarity condition.

% Byzantine consensus with a specific validity property can be solved if and only if the property satisfies the similarity condition.
% we define the \emph{similarity condition}, which we prove to be necessary and sufficient for solvable validity properties.
% % a validity property to be solvable.
% Intuitively, the similarity condition stipulates that there must exist a \emph{common} admissible decision for executions which are indistinguishable to any correct process.

\emph{(iii)} We show that any solution to the Byzantine consensus with a non-trivial validity property incurs $\Omega(t^2)$ messages.
By doing so, we extend the celebrated Dolev-Reischuk bound~\cite{dolev1985bounds} to \emph{all} non-trivial (and solvable) validity properties. 


\emph{(iv)} We introduce \general, a general Byzantine consensus algorithm for \emph{any} non-trivial (and solvable) validity property.
Our algorithm incurs $O(n^2)$ message complexity, which makes it optimal (with $t \in \Omega(n)$) according to our new lower bound.
As for the communication complexity, \general exchanges $O(n^3)$ bits.
\fi
% Furthermore, the design of our general algorithm suggests a \emph{strongest} validity property.
% Namely, we prove that a solution to any solvable validity property can be obtained from a solution of the \emph{Vector Validity} property.

% In the optional appendix, we 

\begin{figure}[ht]
    \centering
    \includegraphics[scale = 0.45]{figures/classification_wider.pdf}
    \caption{Illustration of our results: (1) with $n \leq 3t$, all solvable validity properties are trivial; (2) the exact set of solvable validity properties (as determined by our necessary and sufficient conditions); (3) all non-trivial (and solvable) validity properties require $\Omega(t^2)$ exchanged messages; (4) for any non-trivial (and solvable) validity property, there exists a consensus algorithm with $O(n^2)$ message complexity.}
    \label{fig:classification_landscape}
\end{figure}

\paragraph{Technical overview.}
% We mathematically define a validity property as a function which maps assignments of proposals to correct processes into admissible decisions.
In our formalism, we use the notion of an \emph{input configuration} that denotes an 
assignment of proposals to correct processes.
% The aforementioned assignments of proposals to correct processes are named \emph{input configurations}.
For example, $\big[ (P_1, v), (P_2, v), (P_3, v) \big]$ represents an input configuration by which (1) only processes $P_1$, $P_2$, and $P_3$ are correct, and (2) processes $P_1$, $P_2$, and $P_3$ propose $v$.

First, we define a similarity relation between input configurations: two input configurations are similar if and only if (1) they have (at least) one process in common, and (2) for every common process, the process's proposal is identical in both input configurations.
For example, an input configuration $c = \big[ (P_1, 0), (P_2, 1) \big]$ is similar to $c' = \big[ (P_1, 0), (P_3, 0) \big]$, but not to $\big[ (P_1, 0), (P_2, 0) \big]$.
We observe that all similar input configurations must have an admissible value in common; we call this \emph{canonical similarity}.
Let us illustrate why a common admissible value must exist.
Consider the aforementioned similar input configurations $c = \big[ (P_1, 0), (P_2, 1) \big]$ and $c' = \big[ (P_1, 0), (P_3, 0) \big]$.
If there is no common admissible value for $c$ and $c'$, consensus cannot be solved: process $P_1$ cannot distinguish (1) an execution in which $P_2$ is correct, and $P_3$ is faulty and silent, from (2) an execution in which $P_2$ is faulty, but behaves correctly, and $P_3$ is correct, but slow.
Thus, $P_1$ cannot conclude whether it needs to decide an admissible value for $c$ or for $c'$.
Canonical similarity is a critical intermediate result that we use extensively throughout the paper (even if it does not directly imply any of our results).

% The two most technically challenging results are the proof of triviality if $n \leq 3t$, as well as the proof of the general lower bound.
In our proof of triviality with $n \leq 3t$, we intertwine the classical partitioning argument~\cite{lamport2019byzantine} with our canonical similarity result.
Namely, we show that, for any input configuration, there exists an execution in which the same value $x$ is decided, making $x$ an always-admissible value. 
% to show that there exists an always-admissible decision.
% value which is admissible for any input configuration.
For our lower bound, while following the idea of the original proof~\cite{dolev1985bounds,DBLP:conf/podc/AbrahamCDNP0S19}, we rely on canonical similarity to prove the bound for all solvable and non-trivial validity properties.
% we present a novel mechanism for showing the lower bound on the message complexity.
% In both results, canonical similarity greatly improved the conciseness and presentation of the proofs.
Finally, we design \general by relying on vector consensus~\cite{neves2005solving,vaidya2013byzantine,Doudou1998,correia2006consensus}, a problem in which processes agree on the proposals of $n - t$ processes: when a correct process decides a vector $\mathit{vec}$ of $n - t$ proposals (from vector consensus), it decides (from \general) the common admissible value for all input configurations similar to $\mathit{vec}$.
For example, consider an execution which corresponds to an input configuration $c$.
If, in this execution, a correct process decides a vector $\mathit{vec}$ from vector consensus, it is guaranteed that $\mathit{vec}$ is similar to $c$ (the proposals of correct processes are identical in $c$ and in $\mathit{vec}$).
Hence, deciding (from \general) the common admissible value for all input configurations similar to $\mathit{vec}$ guarantees that the decided value is admissible according to $c$.


%, in which we employ a significant modification to the classical partitioning argument~\cite{lamport2019byzantine}, as well as the 
%We underline that, although it lies in the core of our results, canonical similarity does not directly imply any of them.
%For example, proving that, if $n \leq 3t$, consensus can only be solved with a trivial validity property required us to employ a significant modification to the classical partitioning argument~\cite{lamport2019byzantine}.
%Similarly, while following the idea of the original proof~\cite{dolev1985bounds,DBLP:conf/podc/AbrahamCDNP0S19}, we present a novel mechanism for showing the lower bound on the message complexity.




% First, we observe that, if two input configurations assign the same proposal to all ``common'' processes, there must exist a common admissible decision; we call this result \emph{canonical similarity}.
% The reason is that correct processes cannot distinguish slow, correct processes from live, faulty ones.


\paragraph{Roadmap.}
We provide an overview of related work in \Cref{section:related_work}.
In \Cref{section:preliminaries}, we specify the system model (\Cref{subsection:computational_model_main}), define the consensus problem (\Cref{subsection:byzantine_consensus}), describe our formalism for validity properties (\Cref{subsection:specifying_validity}), and present canonical similarity (\Cref{subsection:similarity}).
% , a predominant intermediate result.
% In \Cref{section:similarity}, we present canonical similarity, a predominant intermediate result.
We define the necessary conditions for the solvability of validity properties in \Cref{section:classification}.
In \Cref{section:lower_upper_bounds}, we prove a quadratic lower bound on message complexity for all non-trivial (and solvable) validity properties (\Cref{subsection:lower_bound}), and introduce \general, a general consensus algorithm for any solvable (and non-trivial) validity property (\Cref{subsection:general_algorithm}).
% In \Cref{section:extended_formalism_main}, we extend our formalism to accommodate for blockchain-specific validity properties.
We conclude the paper in \Cref{section:conclusion}.
The appendix contains (1) omitted proofs and algorithms, and (2) a proposal for how to extend our formalism to accommodate for blockchain-specific validity properties.
% The appendix contains (1) detailed proofs of our results, (2) omitted algorithms, and (3) a proposal for how to extend our formalism to accommodate for blockchain-specific validity properties.
% Detailed proofs and an extension of our formalism to accommodate for blockchain-specific validity properties can be found in the optional appendix.

% \iffalse
% Consensus is a fundamental agreement problem which allows processes to agree on a common value despite failures.
% The application of consensus ranges from state machine replication (SMR) to blockchain and decentralized cloud computing.
% Formally, consensus is defined as a coordination problem among $n$ processes out of which $f$ can fail by crashing.
% Processes that fail are said to be \emph{faulty}; other processes are \emph{correct}.
% Each process starts with an \emph{input} value (its proposal) and should eventually irrevocably produce an \emph{output} value (its decision).
% Consensus requires the following properties to be satisfied:
% \begin{compactitem}
%     \item \emph{Agreement:} No two processes decide different values.
    
%     \item \emph{Termination:} All correct processes eventually decide.
% \end{compactitem}

% It is not hard to see a straightforward solution to the consensus problem defined with the aforementioned two properties: all processes decide $0$.
% In order to preclude such trivial solutions, consensus requires a ``connection'' between proposed and decided values.
% For example, the ``usual'' validity property requires any decided value to have been proposed.
% Importantly, there is no ``the validity property''; any function that maps the initial proposals into permitted decisions can be considered as a legitimate validity property.
% % Indeed, many different validity properties are considered in the literature of the consensus problem in the Byzantine failure model.
% The natural question is whether \emph{all} validity properties can be satisfied. 
% Are there any validity properties for which we cannot design consensus protocols?

% \paragraph{Warm-up: Let $\mathit{val} =$ ``If the specific process $P$ is correct, then only $P$'s proposal can be decided.'' be a validity property.
% Then, $\mathit{val}$ cannot be satisfied in partial synchrony.} 
% The $\mathit{val}$ property cannot be satisfied in partial synchrony due to the fact that $P$'s messages can be arbitrarily delayed.
% Let us elaborate.
% Consider an execution $e_1$ in which $P$ crashes at the very beginning; processes decide some value $v$ in $e_1$ by some time $T_1$.
% Now, we can construct another execution $e_2$ which is identical to $e_1$, except (1) $P$ is correct and it proposes $v' \neq v$, and (2) all messages sent by $P$ are delayed until $T_1$.
% Hence, no process (other than $P$) can distinguish $e_2$ from $e_1$, which means that $v \neq v'$ is decided in $e_2$, even though $P$ is correct and its proposal was $v'$.

% \paragraph{Our contribution.}
% In this paper, we study the \emph{satisfiability} of validity properties.
% % in the crash-stop and Byzantine case.
% Specifically, we present the following contributions:
% \begin{compactitem}
%     \item We define conditions $C_1$, $C_2$ and $C_3$ and show that (1) conditions $C_1$ and $C_2$ must be satisfied by any satisfiable validity property, and (2) conditions $C_1$, $C_2$ and $C_3$ must be satisfied by any validity property satisfiable in partial synchrony.
%     Moreover, we show that these three conditions are sufficient: if a validity property satisfies $C_1$ and $C_2$ (resp., $C_1$, $C_2$ and $C_3$), the validity property is satisfiable (resp., satisfiable in partial synchrony).
    
%     % Similarly, we define conditions $B_1$, $B_2$ and $B_3$ for the Byzantine failure model.
%     % We show that (1) conditions $B_1$ and $B_2$ are necessary for a validity property to be satisfied in a Byzantine setting, and (2) conditions $B_1$, $B_2$ and $B_3$ are necessary for a validity property to be satisfied in a partially synchronous Byzantine setting.
%     % Furthermore, we show that these conditions are sufficient for a validity property to be satisfiable in a Byzantine setting: if a validity property satisfies $B_1$ and $B_2$ (resp., $B_1$, $B_2$ and $B_3$), the validity property is satisfiable (resp., satisfiable in partial synchrony).
    
%     \item We give a generic and simple algorithm that solves consensus for \emph{any} satisfiable validity property.
%     Moreover, we show that the ``traditional'' validity property which requires the decided value to have been proposed is the \emph{strongest} validity property, i.e., any satisfiable validity property can be reduced to this validity property.
% \end{compactitem}
% \fi

% \iffalse
% Byzantine consensus, a fundamental problem in distributed computing, is at the heart of state machine replication (SMR), the classical way to ensure digital trust.
% % in data centers and blockchain  systems.Therefore, it comes as no surprise that consensus has been one of the most studied problems in the literature, both in the past and today.
% In essence, Byzantine consensus consists for a set of $n$ processes to agree on a common value despite (at most) $t$ of them behaving in an arbitrary manner (Byzantine).
% Byzantine consensus is usually defined with three properties: (1) every correct (non-Byzantine) process eventually decides (termination), (2) correct processes do not decide on different values (agreement), and (3) correct processes decide on an admissible value  (validity).
% Whereas termination and agreement are easy to define, validity is not. What is indeed an admissible value?
% Clearly, having processes systematically agree on some default value, say 0, would clearly satisfy termination and agreement. But the resulting consensus solution would not be very useful. In state machine replication, processes use consensus to agree on an ordered set of commands (operations) to execute on the replicated state machine and this set cannot come out of thin air: it is typically a set proposed by processes (invoked by some clients to be executed on the machine). 

% Several validity properties deem different decision values admissible. 
% % Two such properties have been widely studied. 
% A property called \emph{strong validity} stipulates that, if all processes are correct and propose the same value, only that value is admissible.
% Another one called \emph{weak validity} states that, if all correct processes propose the same value, only that value is admissible.
% None of these properties however prevents an arbitrary value to be decided in case correct processes propose differently. 
% Another, more generic, property has been proposed recently 
% in blockchain-based systems: \cite{Cachin2001}.
% % \cite{external validity}. 
%  % Given their large scale,  it is very seldom to have situations where all processes are correct:  deciding any value would  lead to a useless consensus. 
%  Essentially, a specific boolean "validity function" is defined by the application and a value can only be decided if the function returns true for that value, e.g., only if the value has been signed by correct clients. 

% The motivation of our work is to study the precise impact of a validity property on the solvability of Byzantine consensus. 
% It was shown that Byzantine consensus with strong validity 
% %\pierre{Weak Validity, no ? DLS88, p306, theorem 4.4 } \jovan{Yes, of course. We just focused on strong validity as we have a lot of already-proven results on it.} 
%  requires correct processes to exchange $\Theta(n^2)$ messages and to constitute more than two third of the entire system. 
% However, other validity properties are not nearly as studied. The space of validity properties is vast and the impact on the consensus problem remains unclear.

% % Can we classify all validity properties into solvable and unsolvable? What is the lower bound on message complexity for each solvable validity property? These questions remain unanswered.

% In this paper, we study the impact of the validity property on the solvability and complexity of Byzantine consensus considering a partially synchronous distributed system (some of our results apply directly to a synchronous setting as we explain in the paper).
% % We are interested in \emph{solvability} of validity properties: given a validity property, is there a Byzantine consensus algorithm which satisfies it? Moreover, we study the message complexity each solvable validity property requires.

% %\paragraph{Warm-up: Not all validity properties are solvable.}



% % A process is either correct or faulty; a correct process follows the predetermined algorithm, whereas a faulty process can arbitrarily deviate from it.
% % Each correct process \emph{proposes} a value, and should eventually \emph{decide} a value.
% % The following properties are guaranteed:
% %\begin{compactitem}
% %    \item \emph{Agreement:} No two correct processes decide different values.
    
% %    \item \emph{Termination:} All correct processes eventually decide.
% %\end{compactitem}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[scale = 0.3]{figures/classification_3.png}
%     \caption{Landscape of validity properties given our results, summarily $(i)$ solvability conditions, $(ii)$ triviality when $n \leq 3t$, $(iii)$ generalized lower bound, and $(iv)$ general message-optimal solution (upper bound).}
%     \label{fig:state_diagram}
% \end{figure}


% % Byzantine consensus is a fundamental problem of distributed computing. It is defined among $n$ processes, out of which $t < n$ can be Byzantine.
% % defined among $n$ processes, out of which $t < n$ can be Byzantine.  Byzantine consensus is typically characterized by three properties: (1) termination, requiring correct processes to eventually reach a decision, (2) agreement, preventing them from deciding different values, and (3) validity, ensuring reasonable decisions. However, what defines a reasonable decision?  Different applications may require different validity properties. Some validity properties stipulate that the decided value should have been proposed by a correct process; others stipulate that, if all correct processes propose the same value, then this value should be decided. 

% %This paper studies the validity properties of partially synchronous Byzantine consensus in a general manner. Specifically, we are interested in solvability (and its cost) of validity properties.
% We present the following contributions:

% \emph{(i)} For $n > 3t$, we define the \emph{similarity} and \emph{knowledge} conditions, which we prove are necessary and sufficient for a validity property to be solvable.

% \emph{(ii)} For $n \leq 3t$, we prove that a validity property is solvable if and only if it is \emph{trivial}, i.e., there exists a value which is always admissible.
% Our proof employs a non-trivial adaptation of the classical partitioning argument.

% % \emph{(i)} We prove that, if $n \leq 3t$, \emph{any} solvable validity property is trivial (requires no communication).
% % % A validity property is solvable if and only if there exists a partially synchronous Byzantine consensus algorithm with this specific validity property.
% % Our proof employs a non-trivial adaptation of the classical partitioning arguments.
% % % which cannot be directly applied due to the breadth of all possible validity properties.

% % \emph{(ii)} For $n > 3t$, we provide necessary and sufficient conditions for a validity property to be solvable.
% % A validity property is solvable if and only if there exists a partially synchronous algorithm solving the Byzantine consensus problem with this specific validity property.
% % , i.e., to make Byzantine consensus solvable. This goes through a precise definition of validity as a mapping from proposals of correct processes into admissible decisions.

% % \emph{(ii)} We prove that, if $n \leq 3t$, \emph{any} solvable validity property is trivial (requires no communication).
% % Our proof employs a non-trivial adaptation of classical partitioning arguments which cannot be directly applied due to the breadth of all possible validity properties.

% \emph{(iii)} We show that any non-trivial (and solvable) validity property requires $\Omega(t^2)$ messages. 
% By doing so, we generalize the celebrated Dolev-Reischuk bound to all non-trivial (and solvable) validity properties. 
% This includes all classical validity properties, for most of which a lower bound had never been proven.

% % (which generalizes the Dolev-Reischuk bound).

% \emph{(iv)} We give a general Byzantine consensus algorithm for any non-trivial (and solvable) validity property. 
% Our algorithm incurs $O(n^2)$ message complexity, which makes it optimal (with $t \in \Omega(n)$).
% Furthermore, the design of our general algorithm suggests a \emph{strongest} validity property.
% Namely, we prove that a solution to any solvable validity property can be obtained from a solution of the \emph{Interactive-Consistency Validity} property.

% % \fi
% \iffalse
% Byzantine consensus is a fundamental problem of distributed computing.
% Its application ranges from state machine replication (SMR) to blockchain and decentralized cloud computing.
% In essence, Byzantine consensus enables processes to decide on a common value despite arbitrary (Byzantine) failures.
% The following guarantees are provided: (1) every correct (non-Byzantine) process eventually decides (termination), (2) correct processes do not decide on different values (agreement), and (3) correct processes decide on an admissible value (validity).
% In this paper, we focus on the validity property of partially synchronous Byzantine consensus.

% In the literature, we can find various validity properties.
% \emph{Strong Validity}, a classical validity property, stipulates that, if all correct processes propose the same value $v$, only value $v$ is admissible.
% \emph{Weak Validity}, another well-established validity property, states that, if all processes are correct and they all propose the same value $v'$, only value $v'$ can be decided.
% In fact, the space of validity properties is vast, and the impact on the consensus problem remains unclear.
% We ask which validity properties make the Byzantine consensus problem solvable, and at what cost.

% This paper presents the following contributions:
% \begin{compactenum}
%     \item We classify all validity properties into \emph{solvable} and \emph{unsolvable} ones.
%     Namely, we define the \emph{similarity} and \emph{knowledge} conditions, which, as we prove, are necessary conditions for a validity property to be solvable.
%     Moreover, when $n > 3t$, we show that these conditions are sufficient.

%     \item In the case $n \leq 3t$, we determine an even stronger necessary condition for solvable validity properties.
%     That is, if a validity property is solvable with $n \leq 3t$, the property is trivial, i.e., there exists a decision which is always admissible (irrespectively of the proposals).

%     \item We prove that all non-trivial (and solvable) validity properties require $\Omega(t^2)$ messages to be sent by correct processes.
%     Therefore, we extend the well-known Dolev-Reischuk bound on the message complexity, which was shown for \emph{Strong Validity}, to all non-trivial and solvable validity properties.

%     \item We present \textsc{Complete}, a Byzantine consensus algorithm for \emph{any} solvable validity property.
%     Importantly, the message complexity of \textsc{Complete} is $O(n^2)$, which matches our lower bound (when $t \in \Omega(n)$).
% \end{compactenum}
% \fi
% \fi

==> sections/alternative_anton_proof.tex <==
\section{Lower Bound on Message Complexity of Weak Consensus (Alternative Proof)}

This section proves the following theorem:

\begin{theorem} \label{theorem:lower_bound_weak_validity_alternative}
Any algorithm which solves WBC has $\Omega(t^2)$ message complexity.
\end{theorem}

Due to space constraints, we formally prove \Cref{theorem:lower_bound_weak_validity_alternative} in \Cref{section:lower_bound_formal}.
In this section, we provide an informal (but complete) proof of the lower bound.
Namely, to prove \Cref{theorem:lower_bound_weak_validity_alternative}, we show a strictly stronger lower bound for the omission failure model in which processes can only fail by ``dropping'' some messages they send or receive, but not by behaving maliciously.

\paragraph{Omission failures.}
In (only) this section, we consider \emph{omission} failures.
A static adversary corrupts up to $t$ ($0 < t < n$) processes before each execution.
A corrupted process can commit:
\begin{compactitem}
    \item \emph{send-omission} faults by not sending some messages it is supposed to send, or

    \item \emph{receive-omission} faults by not receiving some messages it is suppose to receive.
\end{compactitem}
Note that a faulty process cannot misbehave in an arbitrary manner, i.e., it acts according to its state machine at all times.
Moreover, corrupted processes are not aware of the fact that they are corrupted, i.e., they do not know if or when they omitted some messages.
Corrupted processes are said to be \emph{faulty}, whereas non-corrupted processes are said to be \emph{correct}.
(The formal proof of \Cref{theorem:lower_bound_weak_validity_alternative} in \Cref{section:lower_bound_formal} includes a precise definition of the omission failure model.)

\paragraph{Notation \& remarks.}
Given any set of processes $G$, $\bar{G} = \Pi \setminus{G}$.
If a faulty process omits sending (resp., receiving) some message $m$, we say that the process \emph{send-omits} (resp., \emph{receive-omits}) $m$.
Note that, in the omission failure model, it is reasonable to make claims about the behaviors of faulty processes as they always behave according to their state machine; recall that faulty processes do not know if or when they have omitted some messages.
% Thus, throughout our proof, we do make some claims concerned with the faulty processes.

\paragraph{Proof of \Cref{theorem:lower_bound_weak_validity_alternative}.}
As mentioned, we prove \Cref{theorem:lower_bound_weak_validity_alternative} by proving the following result:

\begin{restatable}{lemma}{lowerboundomission}\label{lemma:lower_bound_omission_alternative}
Any algorithm which solves WBC with omission failures has $\Omega(t^2)$ message complexity.
\end{restatable}

We prove \Cref{lemma:lower_bound_omission_alternative} by contradiction.
Thus, let there exist an algorithm $\mathcal{A}$ which (1) solves WBC with up to $t$ omission failures, and (2) has $o(t^2)$ message complexity.
% \footnote{Observe that any lower bound for authenticated algorithms trivially extends to unauthenticated algorithms.}
As $\mathcal{A}$'s message complexity is $o(t^2)$, correct processes send less than $\frac{t^2}{32}$ messages in \emph{every} execution of $\mathcal{A}$.
Before presenting the proof of \Cref{lemma:lower_bound_omission_alternative}, we define a concept of \emph{isolation}.

\begin{definition} [Isolation] \label{definition:isolation_alternative}
A group $G \subsetneq \Pi$ of $|G| \leq t$ processes is \emph{isolated from some round $k \in \mathbb{N}$} in an execution $\mathcal{E}$ of $\mathcal{A}$ if and only if, for every process $p_G \in G$, the following holds:
\begin{compactitem}
    \item $p_G$ is faulty in $\mathcal{E}$, and

    \item $p_G$ does not send-omit any message in $\mathcal{E}$, and

    \item for every message $m$ sent by any process $p_m$ to $p_G$ in any round $k' \in \mathbb{N}$ of $\mathcal{E}$, $p_G$ receive-omits $m$ in $\mathcal{E}$ if and only if (1) $p_m \in \bar{G}$, and (2) $k' \geq k$.
\end{compactitem}
\end{definition}

Intuitively, a group $G$ is isolated from some round $k$ if and only if no process $p_G \in G$ receives any message from outside of $G$ in any round $k' \geq k$, i.e., $p_G$ only receives messages sent by processes in $G$ from round $k$ onward; other than these receive-omission faults, $p_G$ commits no other faults.

\iffalse
\begin{figure}[ht]
    \centering
    \begin{minipage}{1\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/isolation.pdf}
        \caption{Illustration of \Cref{definition:isolation}.
        The colors represent the local behaviors of processes (including the messages sent).
        Execution $\mathcal{E}_0$ has no faults.
        Execution $\mathcal{E}_0^{X(R)}$ proceeds identically to $\mathcal{E}_0$, sending the same messages (green color) up until round $R$ (inclusive).
        However, group $X$ is \emph{isolated} at round $R$, causing it to miss all messages from group $\overline{X}$ from then on.
        This (potentially) changes $X$'s sending behavior from round $R+1$ onward (red color).
        By propagation, group $\overline{X}$ is then (potentially) affected by $X$'s new sending behavior (red color), causing $\overline{X}$ to deviate from $\mathcal{E}_0$ from round $R+2$ onward (blue color).
        }
        \label{figure:helper_isolation_illustration}
    \end{minipage}
\end{figure}
\fi


Let us start our proof by providing a general result which we reuse throughout the entire section.

\begin{restatable}{lemma}{generic_isolation_alternative} \label{lemma:lower_bound_helper_alternative}
Let $(X, Y, Z)$ represent any partition of $\Pi$ such that (1) $|X| = n - |Y| - |Z|$, (2) $|Y| = \frac{t}{4}$, and (3) $|Z| \leq \frac{t}{4}$.
Moreover, let $\mathcal{E}$ be any infinite execution of $\mathcal{A}$ such that:
\begin{compactitem}
    \item processes from $X$ are correct in $\mathcal{E}$ and agree on some bit $b_X \in \{0,1\}$, whereas processes from $Y \cup Z$ are faulty in $\mathcal{E}$; and

    \item group $Y$ is isolated from some round $k \in \mathbb{N}$ in $\mathcal{E}$.
\end{compactitem}
Then, there exists a set $Y' \subset Y$, such that (a) $|Y'|>\frac{|Y|}{2}$ and (b) every process in $Y'$ decide $b_X$.
%for every process $P_i \in Y'$, there exists a process $P_{x_i} \in X$ and an infinite execution $\mathcal{E}_i$ of $\mathcal{A}$ such that (1) $P_{x_i}$ and $P_i$ are correct in $\mathcal{E}_i$, and (2) $\mathcal{E}_i$ is indistinguishable from $\mathcal{E}$ to both $P_{x_i}$ and $P_i$.
\end{restatable}
\begin{sketch}
We will prove the existence of a set $Y' \subset Y$, such that (a) $|Y'|>\frac{|Y|}{2}$ and (b') for every process $P_i \in Y'$, there exists a process $P_{x_i} \in X$ and an infinite execution $\mathcal{E}_i$ of $\mathcal{A}$ such that (1) $P_{x_i}$ and $P_i$ are correct in $\mathcal{E}_i$, and (2) $\mathcal{E}_i$ is indistinguishable from $\mathcal{E}$ to both $P_{x_i}$ and $P_i$.

For every process $p \in Y$, let $\mathcal{M}_{X \to p}$ denote the set of all messages which are (1) sent by any process $p' \in X$ in $\mathcal{E}$, and (2) receive-omitted by $p$ in $\mathcal{E}$; as $p \in Y$ and group $Y$ is isolated from round $k \in \mathbb{N}$ in $\mathcal{E}$, every message $m \in \mathcal{M}_{X \to p}$ is sent in some round $k' \geq k$.
Let $\mathcal{M}_{X \to Y''} = \bigcup\limits_{p \in Y''} \mathcal{M}_{X \to p}$ for any $Y'' \subset Y$.
As correct processes (i.e., processes from $X$) send less than $\frac{t^2}{32}$ messages in $\mathcal{E}$, $|\mathcal{M}_{X \to Y}| < \frac{t^2}{32}$. Thus, there is no subset $Y'' \subset Y$, such that $|Y''| > \frac{|Y|}{2} \geq \frac{t}{8}$ and for every processes $p$ in $Y''$, $|\mathcal{M}_{X \to p}| \geq \frac{t}{2}$.
Thus, there exists a subset $Y' \subset Y$, such that $|Y'| > \frac{|Y|}{2}$ and for every processes $p$ in $Y'$, $|\mathcal{M}_{X \to p}\}| \leq \frac{t}{2}$.
%Thus, by pigeonhole principle, there exists a process $p_{Y'} \in Y'$ such that $|\mathcal{M}_{X \to p_{Y'}}| < \frac{t}{2}$.
Let $p_i \in Y'$
Let $\mathcal{S}_i$ denote the set of all processes whose messages $p_{i}$ receive-omits in (any round $k' \geq k$ of) $\mathcal{E}$; note that $|\mathcal{S}_i \cap X| < \frac{t}{2}$ (since $|\mathcal{M}_{X \to p_{i}}| < \frac{t}{2}$) and $\mathcal{S}_i \subsetneq X \cup Z$.
Let us construct another infinite execution $\mathcal{E}'_i$ of $\mathcal{A}$ following the (sequentially-executed) steps below:
\begin{compactenum}
    \item Processes in $\mathcal{S}_i \cup Y \cup Z \setminus{\{ p_{i} \}}$ are faulty in $\mathcal{E}'_i$, whereas all other processes are correct.

    \item Then, we set $\mathcal{E}'_i \gets \mathcal{E}$: every process (at first) behaves in the same manner as in $\mathcal{E}$.

    \item For every message $m$ such that $p_{i}$ receive-omits $m$ in $\mathcal{E}$, $m$ is send-omitted in $\mathcal{E}'_i$.
    That is, the sender of $m$ is responsible for $p_{i}$ not receiving $m$ in $\mathcal{E}'_i$.
\end{compactenum}
Observe that $p_{i}$ is indeed correct in $\mathcal{E}'_i$ as (1) $p_{i}$ does not commit any send-omission faults (since $p_{i}$ does not commit those faults in $\mathcal{E}$), and (2) $p_{i}$ does not commit any receive-omission faults (since every message which is receive-omitted in $\mathcal{E}$ is send-omitted in $\mathcal{E}'_i$).
Moreover, there are $|\mathcal{S}_i \cup Y \cup Z \setminus{\{p_{i}\}}| = |(\mathcal{S}_i \cap X) \cup Y \cup Z \setminus{\{p_{i}\}}| < \frac{t}{2} + \frac{t}{4} + \frac{t}{4} - 1 < t$ faulty processes in $\mathcal{E}'_i$.
Furthermore, there exists a process $p_{x_i} \in X$ which is correct in $\mathcal{E}_i'$ as $|\mathcal{S}_i \cap X| < \frac{t}{2}$, $|X| \geq n - \frac{t}{2}$ and $n > t$.
Thus, processes $p_{i}$ and $p_{x_i}$ must agree on the same bit $b_i' \in \{0,1\}$ in $\mathcal{E}'_i$ by correctness of $\mathcal{A}$
Finally, neither $p_{i}$ nor $p_{x_i}$ can distinguish $\mathcal{E}'_i$ from $\mathcal{E}$ as their behaviors in $\mathcal{E}'_i$ and $\mathcal{E}$ are identical. Thus, processes $p_{i}$ and $p_{x_i}$ must decide $b_i'$ by indistinguishability, which means $b_i' = b_X$.
Hence, every process in $Y'$ decide $b_X$, which concludes the lemma.
% \Cref{figure:helper_lemma_illustration} provides an illustration of the proof.
\end{sketch}


% \begin{figure}[ht]
%     \centering
%     % \begin{minipage}{.2\textwidth}
%     %     \centering
%     %     %\vspace{.4cm}
%     %     \includegraphics[width=.85\linewidth]{figures/legend.pdf}
%     %     %\vspace{.95cm}
%     %     \caption{Legend}
%     %     \label{figure:legend}
%     % \end{minipage}%
%     \begin{minipage}{1\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/generic_lemma.pdf}
%         \caption{Illustration of \Cref{lemma:lower_bound_helper}.
%         % For simplicity, consider $|X| = n - \frac{t}{2}, |Y| = \frac{t}{4}$, and $|Z| = \frac{t}{4}$.
%         % $S$ denotes the senders of $p_{Y'}$ for which $p_{Y'}$ committed a receive-omission in $\mathcal{E}$.
%         % Messages that $p_{Y'}$ receive-omits in $\mathcal{E}$ are instead send-omitted in $\mathcal{E'}$ by $S$.
%         % \jovan{Maybe we can simplify the caption to just the main trick behind our proof. Here, it would be that the messages are send-omitted instead of being receive-omitted.}
%         % \manuel{Agreed. I kind of wrote a quick caption just to have a placeholder.}
%         }
%         \label{figure:helper_lemma_illustration}
%     \end{minipage}
% \end{figure}

\iffalse

The following lemma shows that, in any infinite execution of $\mathcal{A}$ in which the group of all faulty processes is isolated from some round $k \in \mathbb{N}$, at least a quarter of the faulty processes decide the same value.
Otherwise, \Cref{lemma:lower_bound_helper_alternative} would allow us to prove that $\mathcal{A}$ does not satisfy \emph{Termination}.

\begin{restatable}{lemma}{isolation} \label{lemma:x_isolated_main}
Let $\mathcal{E}$ be any infinite execution of $\mathcal{A}$ such that (1) some group $G$ of $|G| = \frac{t}{4}$ processes is isolated from some round $k \in \mathbb{N}$, and (2) all processes in $\bar{G}$ are correct.
Then, at least $\frac{|G|}{4} = \frac{t}{16}$ processes from the group $G$ decide the same value in $\mathcal{E}$.
\end{restatable}
\begin{sketch}
As only possible decisions are $0$ and $1$, it suffices to show that at least $\frac{|G|}{2} = \frac{t}{8}$ processes from the group $G$ decide some value in $\mathcal{E}$.
By contradiction, suppose that there exists a group $G' \subseteq G$ of $|G'| \geq \frac{t}{8}$ processes such that no process $p_{G'} \in G'$ decides in $\mathcal{E}$.
Given the partition $(\bar{G}, G, \emptyset)$ of $\Pi$ and a group $G' \subseteq G$, \Cref{lemma:lower_bound_helper} yields an infinite execution $\mathcal{E}'$ of $\mathcal{A}$ and a process $p_{G'} \in G'$ such that (1) $p_{G'}$ is correct in $\mathcal{E}'$, and (2) $p_{G'}$ does not distinguish $\mathcal{E}'$ from $\mathcal{E}$.
Therefore, $p_{G'}$ does not decide in $\mathcal{E}'$, which represents a contradiction with the fact that $\mathcal{A}$ satisfies \emph{Termination}.

\end{sketch}
\fi

In the rest of the proof, we fix the following:

\begin{table} [h]
    \begin{tabular}{|c|m{8.5cm}|}
    \hline
        $(A, B, C)$ & any partition of $\Pi$ such that (1) $|A| = n - \frac{t}{2}$, (2) $|B| = \frac{t}{4}$, and (3) $|C| = \frac{t}{4}$
         \\ \hline
        $\mathcal{E}_0$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, and (2) all processes are correct \\ \hline
        $\mathcal{E}_0^{B(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup C$ are correct, and (3) group $B$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup B$ are correct, and (3) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{B(k_1), C(k_2)}, k_1,k_2 \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k_1$, and (4) group $C$ is isolated from round $k_2$ \\ \hline
        %$\mathcal{E}_0^{B(k + 1), C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k + 1$, and (4) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_1^{C(1)}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $1$, (2) processes from  $A \cup B$ are correct, and (3) group $C$ is isolated from round $1$  \\ \hline
    \end{tabular}
    % \caption{Fixed parameters}
    \label{tab:fixed_parameters}
\end{table}


In the next lemma, we prove that processes in $A$ agree on the same bit in both $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$.

\begin{restatable}{lemma}{either_alternative}
\label{lemma:either_or_alternative}
Processes in $A$ agree on the same bit in both $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$.
\end{restatable}
\begin{sketch}
Let us note $b^0_A$ and $b^1_A$ the bit on which processes in $A$ agree in $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$ respectively.
By \Cref{lemma:lower_bound_helper_alternative} applied to partition $(A \cup C, B, \emptyset)$ and execution $\mathcal{E}^{B(1)}_0$ (resp. $(A \cup B, C, \emptyset)$ and execution $\mathcal{E}^{C(1)}_1$), there exists a set $B' \subseteq B$ of $|B'| > \frac{|B|}{2}$ (resp. $C' \subseteq C$ of $|C'| > \frac{|C|}{2}$) processes which decide the same bit $b^0_A$ in $\mathcal{E}^{B(1)}_0$ (resp. $b^1_A$ in $\mathcal{E}^{C(1)}_1$).

We construct another infinite execution $\mathcal{E}^{*}$ of $\mathcal{A}$ following the steps below:
\begin{compactenum}
    \item Processes from $A$ are correct and agree on a common bit $b^{*}_A$, whereas processes from $B \cup C$ are faulty.
    
    \item All processes from $A \cup B$ propose $0$, whereas all processes from group $C$ propose $1$.

    \item Every process $p_B \in B$ (resp. $p_C \in C$) behaves in the same manner as in $\mathcal{E}^{B(1)}_0$ (resp., $\mathcal{E}^{C(1)}_1$).
    Note that this step of construction is valid as, from round $1$ onward, every process $p_B \in B$ (resp. $p_c \in C$) receives messages only from other processes in group $B$ (resp., $C$).
    Moreover, this step ensures that both groups $B$ and $C$ are isolated from round $1$ in $\mathcal{E}'$.

    \item Every process $p_A \in A$ behaves correctly, i.e., commits no omission faults, and eventually agree on $b^{*}_A$.
\end{compactenum}
In $\mathcal{E}^{*}$, there are $|B \cup C| < t$ faulty processes, which implies that $\mathcal{E}^{*}$ is indeed a valid infinite execution in $\mathcal{A}$.
Moreover, in $\mathcal{E}^{*}$, groups $B$ and $C$ are isolated from round $1$.
Furthermore, as no process $p_B \in B$ (resp. $p_C \in C$) distinguishes $\mathcal{E}^{*}$ from $\mathcal{E}^{B(1)}_0$ (resp. $\mathcal{E}^{C(1)}_1$), processes from the group $B'$ (resp. $C'$) decide $b^0_A$ (resp. $b^1_A$) in $\mathcal{E}^{*}$.

In parallel, By \Cref{lemma:lower_bound_helper_alternative} applied to partition $(A, B, C)$ (resp. $(A, C, B$) and execution $\mathcal{E}^{*}$, there exists a set $B'' \subseteq B$ of $|B''| > \frac{|B|}{2}$ (resp. $C'' \subseteq C$ of $|C''| > \frac{|C|}{2}$) processes which decide the same bit $b^{*}_A$ in $\mathcal{E}^{*}$ (resp. $b^{*}_A$ in $\mathcal{E}^{*}$).

Crucially, $B' \cap B'' = \emptyset$ (resp. $C' \cap C'' = \emptyset$) since $|B'|> \frac{|B|}{2}$ and $|B''|> \frac{|B|}{2}$ (resp. $|C'|> \frac{|C|}{2}$ and $|C''|> \frac{|C|}{2}$), which means $b^{*}_A = b^{0}_A$ (resp. $b^{*}_A = b^{1}_A$).
Hence, $b^0_A = b^1_A$, which concludes the lemma.
\end{sketch}

Without the loss of generality, we assume that processes in $A$ agree on $1$ in $\mathcal{E}_0^{B(1)}$.
The next lemma proves an existence of a round $R \in \mathbb{N}$.

\begin{restatable}{lemma}{criticalround} \label{lemma:R_alternative}
There exists a round $R \in \mathbb{N}$ such that (1) processes in $A$ agree on $1$ in $\mathcal{E}_0^{B(R)}$, and (2) processes in $A$ agree on $0$ in $\mathcal{E}_0^{B(R + 1)}$.
\end{restatable}
\begin{proof}
For every round $k \in \mathbb{N}$, $A$ agree on the bit $b^k$ in $\mathcal{E}_0^{B(k)}$, to satisfy \emph{Termination} and \emph{Agreement}.
We have fixed $b^1 = 1$.
Let $R_{\mathit{max}} \in \mathbb{N}$ denote the round before which every process decides $0$ in $\mathcal{E}_0$ in order to satisfy \emph{Termination} and \emph{Weak Validity}, i.e. $b^{R_{\mathit{max}}} = 0$.
there exists a round $R \in [1, R_{\mathit{max}})$ which satisfies $b^{R} = 1$ and $b^{R+1} = 0$, that is the statement of the lemma. 
\end{proof}

%%%%%%%%%%


Finally, we prove that there exists an inconsistent execution of $\mathcal{A}$, which contradicts \Cref{lemma:no_execution_main_alternative}.
Thus, the following lemma proves \Cref{lemma:lower_bound_omission_alternative}, which directly implies \Cref{theorem:lower_bound_weak_validity_alternative}.

\begin{restatable}{lemma}{lemmafinal} \label{lemma:final_alternative}
There exists an inconsistent execution of $\mathcal{A}$.
\end{restatable}
\begin{sketch}
According to \Cref{lemma:R_alternative}, there exists a round $R \in \mathbb{N}$ such that (1) processes in $A$ agree on $1$ in $\mathcal{E}_0^{B(R)}$, and (2) processes in $A$ agree on $0$ in $\mathcal{E}_0^{B(R + 1)}$.
By correctness of $\mathcal{A}$, processes in $A$ agree on some bit $b_C \in \{0,1\}$ in $\mathcal{E}_0^{C(R)}$.
By \Cref{lemma:lower_bound_helper_alternative} applied to partition $(A \cup B, C, \emptyset)$ and execution $\mathcal{E}_0^{C(R)}$, there exists a subset $C' \subset C$ of $|C'| >\frac{|C|}{2}$ processes that agree on bit $b_C$ in $\mathcal{E}_0^{C(R)}$. Similarly, By \Cref{lemma:lower_bound_helper_alternative} applied to partition $(A \cup C, B, \emptyset)$ and execution to $\mathcal{E}_0^{B(R)}$ and $\mathcal{E}_0^{B(R+1)}$ respectively,
there exists a subset $B_1' \subset B$ of $|B_1'| >\frac{|B|}{2}$ processes that agree on $1$ in $\mathcal{E}_0^{B(R)}$ and there exists a subset $B_0' \subset B$ of $|B_0'| >\frac{|B|}{2}$ processes that agree on $0$ in $\mathcal{E}_0^{B(R+1)}$.
Let us consider two possible scenarios:
\begin{compactitem}
    \item Let $b_C = 0$.
    We construct an inconsistent execution $\mathcal{E}$ in the following manner:
    \begin{compactenum}
        \item Processes from $A$ are correct, and eventually agree on a bit $b^{*}_A$, whereas processes from $B \cup C$ are faulty.

        \item All processes propose $0$.

        \item Every process $p_B \in B$ (resp., $p_C \in C$) behaves in the same manner as in $\mathcal{E}_0^{B(R)}$ (resp., $\mathcal{E}_0^{C(R)}$).
        This step of construction is valid as (1) executions $\mathcal{E}_0^{B(R)}$ and $\mathcal{E}_0^{C(R)}$ are identical until (and excluding) round $R$, and (2) from round $R$ onward, $p_B$ (resp., $p_C$ receives messages only from processes in group $B$ (resp., $C$).

        \item Every process $p_A \in A$ behaves correctly, i.e., commits no omission faults.
        Note that $p_A$'s behavior in $\mathcal{E}$ until (and excluding) round $R$ is identical to $p_A$'s behavior until (and excluding) round $R$ in both $\mathcal{E}_0^{B(R)}$ and $\mathcal{E}_0^{C(R)}$.
    \end{compactenum}
    In $\mathcal{E}$, there are $|B \cup C| < t$ faulty processes; thus, $\mathcal{E}$ is a valid infinite execution of $\mathcal{A}$.
    Moreover, groups $B$ and $C$ are isolated from round $R$ in $\mathcal{E}$.
    Furthermore, as no process $p_B \in B$ (resp., $p_C \in C$) distinguishes $\mathcal{E}$ from $\mathcal{E}_0^{B(R)}$ (resp., $\mathcal{E}_0^{C(R)}$),  processes from group $B_1'$ (resp., $C'$) decide $1$ (resp., $0$). 

    In parallel, By \Cref{lemma:lower_bound_helper_alternative} applied to partition $(A, B, C)$ (resp. $(A, C, B)$) and execution $\mathcal{E}$, there exists a set $B'' \subseteq B$ of $|B''| > \frac{|B|}{2}$ (resp. $C'' \subseteq C$ of $|C''| > \frac{|C|}{2}$) processes which decide the same bit $b^{*}_A$ in $\mathcal{E}^{*}$.

Crucially, $B'_1 \cap B'' = \emptyset$ (resp. $C' \cap C'' = \emptyset$) since $|B'_1|> \frac{|B|}{2}$ and $|B''|> \frac{|B|}{2}$ (resp. $|C'|> \frac{|C|}{2}$ and $|C''|> \frac{|C|}{2}$), which means $b^{*}_A = 1$ (resp. $b^{*}_A = 0$).
Hence, we reached a contradiction for case $b_C = 0$

    \item Let $b_C = 1$.
    We construct an inconsistent execution $\mathcal{E}$ in the following way:
    \begin{compactenum}
        \item Processes from $A$ are correct and eventually agree on a bit $b^{*}_A$, whereas processes from $B \cup C$ are faulty.

        \item All processes propose $0$.

        \item Every process $p_C \in C$ behaves in the same manner as in $\mathcal{E}_0^{C(R)}$.

        \item Every process $p_B \in B$ behaves in the same manner as in $\mathcal{E}_0^{B(R + 1)}$.

        \item Every process $p_A \in A$ behaves correctly, i.e., commits no omission faults.
        Note that $p_A$'s behavior in $\mathcal{E}$ until (and excluding) round $R$ is identical to $p_A$'s behavior until (and excluding) round $R$ in both $\mathcal{E}_0^{B(R + 1)}$ and $\mathcal{E}_0^{C(R)}$.
    \end{compactenum}
    Note that the third and fourth steps of the construction above are valid as (1) executions $\mathcal{E}_0^{B(R + 1)}$ and $\mathcal{E}_0^{C(R)}$ are identical until (and excluding) round $R$, (2) the same set of messages is sent in round $R$ of both $\mathcal{E}_0^{B(R + 1)}$ and $\mathcal{E}_0^{C(R)}$, and (3) from round $R + 1$ (resp., $R$) onward, every process $p_B \in B$ (resp., $p_c \in C$) receives messages only from processes in group $B$ (resp., $C$).
    There are $|B \cup C| < t$ faulty processes in $\mathcal{E}$, which implies that $\mathcal{E}$ is a valid infinite execution.
    Furthermore, group $B$ (resp., $C$) is isolated from round $R + 1$ (resp., $R$) in $\mathcal{E}$.
    Lastly, as no process $p_B \in B$ (resp., $p_C \in C$) distinguishes $\mathcal{E}$ from $\mathcal{E}_0^{B(R + 1)}$ (resp., $\mathcal{E}_0^{C(R)}$), processes from the group $B'_0$ (resp., $C'$) decide $0$ (resp., $1$).%, with necessarily either $b^{*}_A \neq 0$ or $b^{*}_A \neq 1$. 
    %Thus, $\mathcal{E}$ is an inconsistent execution of $\mathcal{A}$.
    In parallel, By \Cref{lemma:lower_bound_helper_alternative} applied to partition $(A, B, C)$ (resp. $(A, C, B)$) and execution $\mathcal{E}$, there exists a set $B'' \subseteq B$ of $|B''| > \frac{|B|}{2}$ (resp. $C'' \subseteq C$ of $|C''| > \frac{|C|}{2}$) processes which decide the same bit $b^{*}_A$ in $\mathcal{E}^{*}$.

Crucially, $B'_0 \cap B'' = \emptyset$ (resp. $C' \cap C'' = \emptyset$) since $|B_0'|> \frac{|B|}{2}$ and $|B''|> \frac{|B|}{2}$ (resp. $|C'|> \frac{|C|}{2}$ and $|C''|> \frac{|C|}{2}$), which means $b^{*}_A = 0$ (resp. $b^{*}_A = 1$).
Hence, we reached a contradiction for case $b_C = 1$.
\end{compactitem}
As the statement of the lemma holds in both possible cases, the proof is concluded.
\end{sketch}

%%%%%%%%%%

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% VERSION OF TUESDAY 02/11/23 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Lower Bound on Message Complexity of Weak Consensus (Alternative Proof)}

This section proves the following theorem:

\begin{theorem} \label{theorem:lower_bound_weak_validity_alternative}
Any algorithm which solves WBC has $\Omega(t^2)$ message complexity.
\end{theorem}

Due to space constraints, we formally prove \Cref{theorem:lower_bound_weak_validity_alternative} in \Cref{section:lower_bound_formal}.
In this section, we provide an informal (but complete) proof of the lower bound.
Namely, to prove \Cref{theorem:lower_bound_weak_validity_alternative}, we show a strictly stronger lower bound for the omission failure model in which processes can only fail by ``dropping'' some messages they send or receive, but not by behaving maliciously.

\paragraph{Omission failures.}
In (only) this section, we consider \emph{omission} failures.
A static adversary corrupts up to $t$ ($0 < t < n$) processes before each execution.
A corrupted process can commit:
\begin{compactitem}
    \item \emph{send-omission} faults by not sending some messages it is supposed to send, or

    \item \emph{receive-omission} faults by not receiving some messages it is suppose to receive.
\end{compactitem}
Note that a faulty process cannot misbehave in an arbitrary manner, i.e., it acts according to its state machine at all times.
Moreover, corrupted processes are not aware of the fact that they are corrupted, i.e., they do not know if or when they omitted some messages.
Corrupted processes are said to be \emph{faulty}, whereas non-corrupted processes are said to be \emph{correct}.
(The formal proof of \Cref{theorem:lower_bound_weak_validity_alternative} in \Cref{section:lower_bound_formal} includes a precise definition of the omission failure model.)

\paragraph{Notation \& remarks.}
Given any set of processes $G$, $\bar{G} = \Pi \setminus{G}$.
If a faulty process omits sending (resp., receiving) some message $m$, we say that the process \emph{send-omits} (resp., \emph{receive-omits}) $m$.
Note that, in the omission failure model, it is reasonable to make claims about the behaviors of faulty processes as they always behave according to their state machine; recall that faulty processes do not know if or when they have omitted some messages.
% Thus, throughout our proof, we do make some claims concerned with the faulty processes.

\paragraph{Proof of \Cref{theorem:lower_bound_weak_validity_alternative}.}
As mentioned, we prove \Cref{theorem:lower_bound_weak_validity_alternative} by proving the following result:

\begin{restatable}{lemma}{lowerboundomission}\label{lemma:lower_bound_omission_alternative}
Any algorithm which solves WBC with omission failures has $\Omega(t^2)$ message complexity.
\end{restatable}

We prove \Cref{lemma:lower_bound_omission_alternative} by contradiction.
Thus, let there exist an algorithm $\mathcal{A}$ which (1) solves WBC with up to $t$ omission failures, and (2) has $o(t^2)$ message complexity.
% \footnote{Observe that any lower bound for authenticated algorithms trivially extends to unauthenticated algorithms.}
As $\mathcal{A}$'s message complexity is $o(t^2)$, correct processes send less than $\frac{t^2}{32}$ messages in \emph{every} execution of $\mathcal{A}$.
Before presenting the proof of \Cref{lemma:lower_bound_omission_alternative}, we define a concept of \emph{isolation}.

\begin{definition} [Isolation] \label{definition:isolation_alternative}
A group $G \subsetneq \Pi$ of $|G| \leq t$ processes is \emph{isolated from some round $k \in \mathbb{N}$} in an execution $\mathcal{E}$ of $\mathcal{A}$ if and only if, for every process $p_G \in G$, the following holds:
\begin{compactitem}
    \item $p_G$ is faulty in $\mathcal{E}$, and

    \item $p_G$ does not send-omit any message in $\mathcal{E}$, and

    \item for every message $m$ sent by any process $p_m$ to $p_G$ in any round $k' \in \mathbb{N}$ of $\mathcal{E}$, $p_G$ receive-omits $m$ in $\mathcal{E}$ if and only if (1) $p_m \in \bar{G}$, and (2) $k' \geq k$.
\end{compactitem}
\end{definition}

Intuitively, a group $G$ is isolated from some round $k$ if and only if no process $p_G \in G$ receives any message from outside of $G$ in any round $k' \geq k$, i.e., $p_G$ only receives messages sent by processes in $G$ from round $k$ onward; other than these receive-omission faults, $p_G$ commits no other faults.

\iffalse
\begin{figure}[ht]
    \centering
    \begin{minipage}{1\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/isolation.pdf}
        \caption{Illustration of \Cref{definition:isolation}.
        The colors represent the local behaviors of processes (including the messages sent).
        Execution $\mathcal{E}_0$ has no faults.
        Execution $\mathcal{E}_0^{X(R)}$ proceeds identically to $\mathcal{E}_0$, sending the same messages (green color) up until round $R$ (inclusive).
        However, group $X$ is \emph{isolated} at round $R$, causing it to miss all messages from group $\overline{X}$ from then on.
        This (potentially) changes $X$'s sending behavior from round $R+1$ onward (red color).
        By propagation, group $\overline{X}$ is then (potentially) affected by $X$'s new sending behavior (red color), causing $\overline{X}$ to deviate from $\mathcal{E}_0$ from round $R+2$ onward (blue color).
        }
        \label{figure:helper_isolation_illustration}
    \end{minipage}
\end{figure}
\fi


Let us start our proof by providing a general result which we reuse throughout the entire section.

\begin{restatable}{lemma}{generic_isolation_alternative} \label{lemma:lower_bound_helper_alternative}
Let $(X, Y, Z)$ represent any partition of $\Pi$ such that (1) $|X| = n - |Y| - |Z|$, (2) $|Y| = \frac{t}{4}$, and (3) $|Z| \leq \frac{t}{4}$.
Moreover, let $\mathcal{E}$ be any infinite execution of $\mathcal{A}$ such that:
\begin{compactitem}
    \item processes from $X$ are correct in $\mathcal{E}$, whereas processes from $Y \cup Z$ are faulty in $\mathcal{E}$; and

    \item group $Y$ is isolated from some round $k \in \mathbb{N}$ in $\mathcal{E}$.
\end{compactitem}
Then, there exists a set $Y' \subset Y$, such that (a) $|Y'|>\frac{|Y|}{2}$ and (b) for every process $P_i \in Y'$, there exists a process $P_{x_i} \in X$ and an infinite execution $\mathcal{E}_i$ of $\mathcal{A}$ such that (1) $P_{x_i}$ and $P_i$ are correct in $\mathcal{E}_i$, and (2) $\mathcal{E}_i$ is indistinguishable from $\mathcal{E}$ to both $P_{x_i}$ and $P_i$.
\end{restatable}
\begin{sketch}
For every process $p \in Y$, let $\mathcal{M}_{X \to p}$ denote the set of all messages which are (1) sent by any process $p' \in X$ in $\mathcal{E}$, and (2) receive-omitted by $p$ in $\mathcal{E}$; as $p \in Y$ and group $Y$ is isolated from round $k \in \mathbb{N}$ in $\mathcal{E}$, every message $m \in \mathcal{M}_{X \to p}$ is sent in some round $k' \geq k$.
Let $\mathcal{M}_{X \to Y''} = \bigcup\limits_{p \in Y''} \mathcal{M}_{X \to p}$ for any $Y'' \subset Y$.
As correct processes (i.e., processes from $X$) send less than $\frac{t^2}{32}$ messages in $\mathcal{E}$, $|\mathcal{M}_{X \to Y}| < \frac{t^2}{32}$. Thus, there is no subset $Y'' \subset Y$, such that $|Y''| > \frac{|Y|}{2} \geq \frac{t}{8}$ and for every processes $p$ in $Y''$, $|\mathcal{M}_{X \to p}| \geq \frac{t}{2}$.
Thus, there exists a subset $Y' \subset Y$, such that $|Y'| > \frac{|Y|}{2}$ and for every processes $p$ in $Y'$, $|\mathcal{M}_{X \to p}\}| \leq \frac{t}{2}$.
%Thus, by pigeonhole principle, there exists a process $p_{Y'} \in Y'$ such that $|\mathcal{M}_{X \to p_{Y'}}| < \frac{t}{2}$.
Let $p_i \in Y'$
Let $\mathcal{S}_i$ denote the set of all processes whose messages $p_{i}$ receive-omits in (any round $k' \geq k$ of) $\mathcal{E}$; note that $|\mathcal{S}_i \cap X| < \frac{t}{2}$ (since $|\mathcal{M}_{X \to p_{i}}| < \frac{t}{2}$) and $\mathcal{S}_i \subsetneq X \cup Z$.
Let us construct another infinite execution $\mathcal{E}'_i$ of $\mathcal{A}$ following the (sequentially-executed) steps below:
\begin{compactenum}
    \item Processes in $\mathcal{S}_i \cup Y \cup Z \setminus{\{ p_{i} \}}$ are faulty in $\mathcal{E}'_i$, whereas all other processes are correct.

    \item Then, we set $\mathcal{E}'_i \gets \mathcal{E}$: every process (at first) behaves in the same manner as in $\mathcal{E}$.

    \item For every message $m$ such that $p_{i}$ receive-omits $m$ in $\mathcal{E}$, $m$ is send-omitted in $\mathcal{E}'_i$.
    That is, the sender of $m$ is responsible for $p_{i}$ not receiving $m$ in $\mathcal{E}'_i$.
\end{compactenum}
Observe that $p_{i}$ is indeed correct in $\mathcal{E}'_i$ as (1) $p_{i}$ does not commit any send-omission faults (since $p_{i}$ does not commit those faults in $\mathcal{E}$), and (2) $p_{i}$ does not commit any receive-omission faults (since every message which is receive-omitted in $\mathcal{E}$ is send-omitted in $\mathcal{E}'_i$).
Moreover, there are $|\mathcal{S}_i \cup Y \cup Z \setminus{\{p_{i}\}}| = |(\mathcal{S}_i \cap X) \cup Y \cup Z \setminus{\{p_{i}\}}| < \frac{t}{2} + \frac{t}{4} + \frac{t}{4} - 1 < t$ faulty processes in $\mathcal{E}'_i$.
Furthermore, there exists a process $p_{x_i} \in X$ which is correct in $\mathcal{E}_i'$ as $|\mathcal{S}_i \cap X| < \frac{t}{2}$, $|X| \geq n - \frac{t}{2}$ and $n > t$.
Finally, neither $p_{i}$ nor $p_{x_i}$ can distinguish $\mathcal{E}'_i$ from $\mathcal{E}$ as their behaviors in $\mathcal{E}'_i$ and $\mathcal{E}$ are identical.
% \Cref{figure:helper_lemma_illustration} provides an illustration of the proof.
\end{sketch}


% \begin{figure}[ht]
%     \centering
%     % \begin{minipage}{.2\textwidth}
%     %     \centering
%     %     %\vspace{.4cm}
%     %     \includegraphics[width=.85\linewidth]{figures/legend.pdf}
%     %     %\vspace{.95cm}
%     %     \caption{Legend}
%     %     \label{figure:legend}
%     % \end{minipage}%
%     \begin{minipage}{1\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/generic_lemma.pdf}
%         \caption{Illustration of \Cref{lemma:lower_bound_helper}.
%         % For simplicity, consider $|X| = n - \frac{t}{2}, |Y| = \frac{t}{4}$, and $|Z| = \frac{t}{4}$.
%         % $S$ denotes the senders of $p_{Y'}$ for which $p_{Y'}$ committed a receive-omission in $\mathcal{E}$.
%         % Messages that $p_{Y'}$ receive-omits in $\mathcal{E}$ are instead send-omitted in $\mathcal{E'}$ by $S$.
%         % \jovan{Maybe we can simplify the caption to just the main trick behind our proof. Here, it would be that the messages are send-omitted instead of being receive-omitted.}
%         % \manuel{Agreed. I kind of wrote a quick caption just to have a placeholder.}
%         }
%         \label{figure:helper_lemma_illustration}
%     \end{minipage}
% \end{figure}

\iffalse

The following lemma shows that, in any infinite execution of $\mathcal{A}$ in which the group of all faulty processes is isolated from some round $k \in \mathbb{N}$, at least a quarter of the faulty processes decide the same value.
Otherwise, \Cref{lemma:lower_bound_helper_alternative} would allow us to prove that $\mathcal{A}$ does not satisfy \emph{Termination}.

\begin{restatable}{lemma}{isolation} \label{lemma:x_isolated_main}
Let $\mathcal{E}$ be any infinite execution of $\mathcal{A}$ such that (1) some group $G$ of $|G| = \frac{t}{4}$ processes is isolated from some round $k \in \mathbb{N}$, and (2) all processes in $\bar{G}$ are correct.
Then, at least $\frac{|G|}{4} = \frac{t}{16}$ processes from the group $G$ decide the same value in $\mathcal{E}$.
\end{restatable}
\begin{sketch}
As only possible decisions are $0$ and $1$, it suffices to show that at least $\frac{|G|}{2} = \frac{t}{8}$ processes from the group $G$ decide some value in $\mathcal{E}$.
By contradiction, suppose that there exists a group $G' \subseteq G$ of $|G'| \geq \frac{t}{8}$ processes such that no process $p_{G'} \in G'$ decides in $\mathcal{E}$.
Given the partition $(\bar{G}, G, \emptyset)$ of $\Pi$ and a group $G' \subseteq G$, \Cref{lemma:lower_bound_helper} yields an infinite execution $\mathcal{E}'$ of $\mathcal{A}$ and a process $p_{G'} \in G'$ such that (1) $p_{G'}$ is correct in $\mathcal{E}'$, and (2) $p_{G'}$ does not distinguish $\mathcal{E}'$ from $\mathcal{E}$.
Therefore, $p_{G'}$ does not decide in $\mathcal{E}'$, which represents a contradiction with the fact that $\mathcal{A}$ satisfies \emph{Termination}.

\end{sketch}
\fi

In the rest of the proof, we fix the following:

\begin{table} [h]
    \begin{tabular}{|c|m{8.5cm}|}
    \hline
        $(A, B, C)$ & any partition of $\Pi$ such that (1) $|A| = n - \frac{t}{2}$, (2) $|B| = \frac{t}{4}$, and (3) $|C| = \frac{t}{4}$
         \\ \hline
        $\mathcal{E}_0$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, and (2) all processes are correct \\ \hline
        $\mathcal{E}_0^{B(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup C$ are correct, and (3) group $B$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup B$ are correct, and (3) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{B(k_1), C(k_2)}, k_1,k_2 \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k_1$, and (4) group $C$ is isolated from round $k_2$ \\ \hline
        %$\mathcal{E}_0^{B(k + 1), C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k + 1$, and (4) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_1^{C(1)}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $1$, (2) processes from  $A \cup B$ are correct, and (3) group $C$ is isolated from round $1$  \\ \hline
    \end{tabular}
    % \caption{Fixed parameters}
    \label{tab:fixed_parameters}
\end{table}

Before we continue with the proof, we define \emph{inconsistent} executions.

\begin{definition} [Inconsistent execution] \label{definition:inconsistent_execution_alternative}
An infinite execution $\mathcal{E}$ of $\mathcal{A}$ is \emph{inconsistent} if:
\begin{compactitem}
    \item group $B$ is isolated from some round $k_B \in \mathbb{N}$ in $\mathcal{E}$, and

    \item group $C$ is isolated from some round $k_C \in \mathbb{N}$ in $\mathcal{E}$, and

    \item all processes from group $A$ are correct in $\mathcal{E}$ and agree on bit $b_A$, and 

    \item One of this true statement is true: either
    \begin{compactitem}

    \item strictly more than $\frac{|B|}{2}$ processes from group $B$ do not decide $b_A$ in $\mathcal{E}$, or

    \item strictly more than $\frac{|C|}{2}$ processes from group $C$ do not decide $b_A$ in $\mathcal{E}$.
    \end{compactitem}
    
\end{compactitem}
\end{definition}

The following lemma proves that no inconsistent execution of $\mathcal{A}$ exists.
% as, otherwise, \Cref{lemma:lower_bound_helper} would allow us to prove that $\mathcal{A}$ does not satisfy \emph{Consistency}.

\begin{restatable}{lemma}{noexecution}\label{lemma:no_execution_main_alternative}
No inconsistent execution of $\mathcal{E}$ exists.
\end{restatable}
\begin{sketch}
We prove the lemma by contradiction.
Thus, let us assume that an (infinite) inconsistent execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ exists; recall that correct processes (i.e., processes from $A$) send less than $\frac{t^2}{32}$ messages in $\mathcal{E}$.
We denote by $B' \subseteq B$ (resp., $C' \subseteq C$) the set of strictly more $\frac{|B|}{2}$ (resp. $\frac{|C|}{2}$) processes from group $B$ (resp., group $C$) that do not decide $b_A$ in $\mathcal{E}$.

Given the partition $(A, B, C)$ of $\Pi$, \Cref{lemma:lower_bound_helper_alternative} proves existence of $(B'',C'') \subset B \times C$, s.t. $B'' > \frac{|B|}{2}$, $C'' > \frac{|C|}{2}$ and for every process in $P_{\ell} \in B'' \cup C''$, there exists a valid execution $\mathcal{E}_{\ell}'$, indistinguishable from $\mathcal{E}$, such that both $P_{\ell}$ and another process $P_{x_{\ell}} \in A$ are correct in $\mathcal{E}_{\ell}'$.
Crucially, $B' \cap B'' \neq \emptyset$ (resp. $C' \cap C'' \neq \emptyset$) since $|B'|>\frac{|B|}{2}$, and $|B''|>\frac{|B|}{2}$ (resp. $|C'|>\frac{|C|}{2}$, and $|C''|>\frac{|C|}{2}$).
Let $P_i \in B' \cap B''$ (resp. $P_j \in C' \cap C''$). There exists a valid execution $\mathcal{E}_i'$ (resp. $\mathcal{E}_j'$), indistinguishable from $\mathcal{E}$, such that both $P_{i}$ (resp. $P_{j}$) and another process $P_{x_{i}} \in A$ (resp. $P_{x_{j}} \in A$) are correct in $\mathcal{E}_{i}'$ (resp. $\mathcal{E}_{j}'$). By correctness of $\mathcal{A}$, both $P_{i}$ (resp. $P_{j}$) and $P_{x_{i}}$ (resp. $P_{x_{j}}$) agree on the same bit $b_i$ (resp. $b_j$) in $\mathcal{E}_{i}'$ (resp. $\mathcal{E}_{j}'$). By indistinguishability, $b_i = b_A$ (resp. $b_j=b_A$). Hence, we reach a contradiction with the fact that $P_i$ (resp. $P_j$) does not decide $b_A$ since $P_i \in B'$ (resp. $P_j \in C'$).
\end{sketch}


In the next lemma, we prove that processes in $A$ agree on the same bit in both $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$.

\begin{restatable}{lemma}{either_alternative}
\label{lemma:either_or_alternative}
Processes in $A$ agree on the same bit in both $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$.
\end{restatable}
\begin{sketch}
Let us note $b^0_A$ and $b^v_A$ the bit on which processes in $A$ agree in $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$ respectively.
By \Cref{lemma:no_execution_main_alternative}, there exists a set $B' \subseteq B$ of $|B'| > \frac{|B|}{2}$ (resp. $C' \subseteq C$ of $|C'| > \frac{|C|}{2}$) processes which decide the same bit $b^0_A$ in $\mathcal{E}^{B(1)}_0$ (resp. $b^1_A$ in $\mathcal{E}^{C(1)}_1$).

We construct another infinite execution $\mathcal{E}^{*}$ of $\mathcal{A}$ following the steps below:
\begin{compactenum}
    \item Processes from $A$ are correct, whereas processes from $B \cup C$ are faulty.
    
    \item All processes from $A \cup B$ propose $0$, whereas all processes from group $C$ propose $1$.

    \item Every process $p_B \in B$ (resp., $p_C \in C$) behaves in the same manner as in $\mathcal{E}^{B(1)}_0$ (resp., $\mathcal{E}^{C(1)}_1$).
    Note that this step of construction is valid as, from round $1$ onward, every process $p_B \in B$ (resp., $p_c \in C$) receives messages only from other processes in group $B$ (resp., $C$).
    Moreover, this step ensures that both groups $B$ and $C$ are isolated from round $1$ in $\mathcal{E}'$.

    \item Every process $p_A \in A$ behaves correctly, i.e., commits no omission faults, and eventually agree on $b^{*}_A$.
\end{compactenum}
In $\mathcal{E}^{*}$, there are $|B \cup C| < t$ faulty processes, which implies that $\mathcal{E}^{*}$ is indeed a valid infinite execution in $\mathcal{A}$.
Moreover, in $\mathcal{E}^{*}$, groups $B$ and $C$ are isolated from round $1$.
Furthermore, as no process $p_B \in B$ (resp., $p_C \in C$) distinguishes $\mathcal{E}^{*}$ from $\mathcal{E}^{B(1)}_0$ (resp., $\mathcal{E}^{C(1)}_1$), processes from the group $B'$ (resp., $C'$) decide $b^0_A$ (resp., $b^1_A$) in $\mathcal{E}^{*}$.
By \Cref{lemma:no_execution_main_alternative}, $\mathcal{E}^{*}$ cannot be an inconsistent execution, which means $b^0_A = b^1_A$ and concludes the proof of this lemma.
\end{sketch}

Without the loss of generality, we assume that processes in $A$ agree on $1$ in $\mathcal{E}_0^{B(1)}$.
The next lemma proves an existence of a round $R \in \mathbb{N}$.

\begin{restatable}{lemma}{criticalround} \label{lemma:R_alternative}
There exists a round $R \in \mathbb{N}$ such that (1) processes in $A$ agree on $1$ in $\mathcal{E}_0^{B(R)}$, and (2) processes in $A$ agree on $0$ in $\mathcal{E}_0^{B(R + 1)}$.
\end{restatable}
\begin{proof}
For every round $k \in \mathbb{N}$, $A$ agree on the bit $b^k$ in $\mathcal{E}_0^{B(k)}$, to satisfy \emph{Termination} and \emph{Agreement}.
We have fixed $b^1 = 1$.
Let $R_{\mathit{max}} \in \mathbb{N}$ denote the round before which every process decides $0$ in $\mathcal{E}_0$ in order to satisfy \emph{Termination} and \emph{Weak Validity}, i.e. $b^{R_{\mathit{max}}} = 0$.
there exists a round $R \in [1, R_{\mathit{max}})$ which satisfies $b^{R} = 1$ and $b^{R+1} = 0$, that is the statement of the lemma. 
\end{proof}

%%%%%%%%%%


Finally, we prove that there exists an inconsistent execution of $\mathcal{A}$, which contradicts \Cref{lemma:no_execution_main_alternative}.
Thus, the following lemma proves \Cref{lemma:lower_bound_omission_alternative}, which directly implies \Cref{theorem:lower_bound_weak_validity_alternative}.

\begin{restatable}{lemma}{lemmafinal} \label{lemma:final_alternative}
There exists an inconsistent execution of $\mathcal{A}$.
\end{restatable}
\begin{sketch}
According to \Cref{lemma:R_alternative}, there exists a round $R \in \mathbb{N}$ such that (1) processes in $A$ agree on $1$ in $\mathcal{E}_0^{B(R)}$, and (2) processes in $A$ agree on $0$ in $\mathcal{E}_0^{B(R + 1)}$.
By correctness of $\mathcal{A}$, processes in $A$ agree on some bit $b_c \in \{0,1\}$ in $\mathcal{E}_0^{C(R)}$.
Due to \Cref{lemma:no_execution_main_alternative}, there exists a subset $C' \subset C$ of $|C'| >\frac{|C|}{2}$ processes that agree on bit $b_c$ in $\mathcal{E}_0^{C(R)}$. Similarly, there exists a subset $B_1' \subset B$ of $|B_1'| >\frac{|B|}{2}$ processes that agree on $1$ in $\mathcal{E}_0^{B(R)}$ and there exists a subset $B_0' \subset B$ of $|B_0'| >\frac{|B|}{2}$ processes that agree on $0$ in $\mathcal{E}_0^{B(R+1)}$.
Let us consider two possible scenarios:
\begin{compactitem}
    \item Let $b_C = 0$.
    We construct an inconsistent execution $\mathcal{E}$ in the following manner:
    \begin{compactenum}
        \item Processes from $A$ are correct, and eventually agree on a bit $b^{*}_A$, whereas processes from $B \cup C$ are faulty.

        \item All processes propose $0$.

        \item Every process $p_B \in B$ (resp., $p_C \in C$) behaves in the same manner as in $\mathcal{E}_0^{B(R)}$ (resp., $\mathcal{E}_0^{C(R)}$).
        This step of construction is valid as (1) executions $\mathcal{E}_0^{B(R)}$ and $\mathcal{E}_0^{C(R)}$ are identical until (and excluding) round $R$, and (2) from round $R$ onward, $p_B$ (resp., $p_C$ receives messages only from processes in group $B$ (resp., $C$).

        \item Every process $p_A \in A$ behaves correctly, i.e., commits no omission faults.
        Note that $p_A$'s behavior in $\mathcal{E}$ until (and excluding) round $R$ is identical to $p_A$'s behavior until (and excluding) round $R$ in both $\mathcal{E}_0^{B(R)}$ and $\mathcal{E}_0^{C(R)}$.
    \end{compactenum}
    In $\mathcal{E}$, there are $|B \cup C| < t$ faulty processes; thus, $\mathcal{E}$ is a valid infinite execution of $\mathcal{A}$.
    Moreover, groups $B$ and $C$ are isolated from round $R$ in $\mathcal{E}$.
    Furthermore, as no process $p_B \in B$ (resp., $p_C \in C$) distinguishes $\mathcal{E}$ from $\mathcal{E}_0^{B(R)}$ (resp., $\mathcal{E}_0^{C(R)}$),  processes from group $B'$ (resp., $C'$) decide $1$ (resp., $0$), with necessarilly either $b^{*}_A \neq 0$ or $b^{*}_A \neq 1$. 
    Thus, $\mathcal{E}$ is an inconsistent execution of $\mathcal{A}$.

    \item Let $b_C = 1$.
    We construct an inconsistent execution $\mathcal{E}$ in the following way:
    \begin{compactenum}
        \item Processes from $A$ are correct and eventually agree on a bit $b^{*}_A$, whereas processes from $B \cup C$ are faulty.

        \item All processes propose $0$.

        \item Every process $p_C \in C$ behaves in the same manner as in $\mathcal{E}_0^{C(R)}$.

        \item Every process $p_B \in B$ behaves in the same manner as in $\mathcal{E}_0^{B(R + 1)}$.

        \item Every process $p_A \in A$ behaves correctly, i.e., commits no omission faults.
        Note that $p_A$'s behavior in $\mathcal{E}$ until (and excluding) round $R$ is identical to $p_A$'s behavior until (and excluding) round $R$ in both $\mathcal{E}_0^{B(R + 1)}$ and $\mathcal{E}_0^{C(R)}$.
    \end{compactenum}
    Note that the third and fourth steps of the construction above are valid as (1) executions $\mathcal{E}_0^{B(R + 1)}$ and $\mathcal{E}_0^{C(R)}$ are identical until (and excluding) round $R$, (2) the same set of messages is sent in round $R$ of both $\mathcal{E}_0^{B(R + 1)}$ and $\mathcal{E}_0^{C(R)}$, and (3) from round $R + 1$ (resp., $R$) onward, every process $p_B \in B$ (resp., $p_c \in C$) receives messages only from processes in group $B$ (resp., $C$).
    There are $|B \cup C| < t$ faulty processes in $\mathcal{E}$, which implies that $\mathcal{E}$ is a valid infinite execution.
    Furthermore, group $B$ (resp., $C$) is isolated from round $R + 1$ (resp., $R$) in $\mathcal{E}$.
    Lastly, as no process $p_B \in B$ (resp., $p_C \in C$) distinguishes $\mathcal{E}$ from $\mathcal{E}_0^{B(R + 1)}$ (resp., $\mathcal{E}_0^{C(R)}$), processes from the group $B'$ (resp., $C$) decide $0$ (resp., $1$), with necessarily either $b^{*}_A \neq 0$ or $b^{*}_A \neq 1$. 
    Thus, $\mathcal{E}$ is an inconsistent execution of $\mathcal{A}$.
\end{compactitem}
As the statement of the lemma holds in both possible cases, the proof is concluded.
\end{sketch}
\iffalse
\fi
%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% END VERSION OF TUESDAY 02/11/23 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

==> sections/alternative_proof_formal.tex <==
\section{Lower Bound on Message Complexity of Weak Consensus (Alternative Proof Formal)}

\begin{lemma}[Sub-majority isolation] \label{lemma:lower_bound_helper}
Let $(X, Y, Z)$ represent any partition of $\Pi$ such that (1) $|X| = n - |Y| - |Z|$, (2) $|Y| = \frac{t}{4}$, and (3) $|Z| \leq \frac{t}{4}$.
Moreover, let $\mathcal{E}$ be any infinite execution of $\mathcal{A}$ such that:
\begin{compactitem}
    \item processes from $X$ are correct in $\mathcal{E}$ and agree on some bit $b_X \in \{0,1\}$, whereas processes from $Y \cup Z$ are faulty in $\mathcal{E}$; and

    \item group $Y$ is isolated from some round $k \in \mathbb{N}$ in $\mathcal{E}$.
\end{compactitem}
Then, there exists a set $Y' \subset Y$, such that (a) $|Y'|>\frac{|Y|}{2}$ and (b) every process in $Y'$ decide $b_X$.
%for every process $P_i \in Y'$, there exists a process $P_{x_i} \in X$ and an infinite execution $\mathcal{E}_i$ of $\mathcal{A}$ such that (1) $P_{x_i}$ and $P_i$ are correct in $\mathcal{E}_i$, and (2) $\mathcal{E}_i$ is indistinguishable from $\mathcal{E}$ to both $P_{x_i}$ and $P_i$.
\end{lemma}
\begin{proof}
We will prove the existence of a set $Y' \subset Y$, such that (a) $|Y'|>\frac{|Y|}{2}$ and (b') for every process $P_i \in Y'$, there exists a process $P_{x_i} \in X$ and an infinite execution $\mathcal{E}_i$ of $\mathcal{A}$ such that (1) $P_{x_i}$ and $P_i$ are correct in $\mathcal{E}_i$, and (2) $\mathcal{E}_i$ is indistinguishable from $\mathcal{E}$ to both $P_{x_i}$ and $P_i$.
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Due to the statement of the lemma, $\mathcal{F} = Y \cup Z$.
Moreover, no process in $X \cup Y$ commits any send-omission failure in $\mathcal{E}$: for every process $P_i \in X \cup Y$ and every round $j \in \mathbb{N}^+ \cup \{+\infty\}$, $\mathsf{send\_omitted}(\mathcal{B}_i, j) = \emptyset$.

For every set of processes $U$, we note $M_{U} = \bigcup\limits_{P_i \in U} \big( \bigcup\limits_{k' \geq k}  \fmsgs{\mathcal{B}_i}{k'} \big)$ to denote the set of messages sent by processes in $U$ from (and including) round $k$ onward in $\mathcal{E}$.

For every pair of sets of processes $(U, V)$, we define $M_{U \to V}$ as the set containing all messages sent to a process in $V$ by processes in $U$ from (and including) round $k$ onward of $\mathcal{E}$:
\begin{equation*}
    M_{U \to V} = \{ m \,|\, m \in M_{U} \land m.\mathsf{receiver} \in V \}.
\end{equation*}
Note that, for every $P_i \in Y$, each message $m \in M_{(X \cup Z) \to \{P_i\}}$ is receive-omitted in $\mathcal{B}_i$.

First, we will prove by contradiction that $\exists Y' \subset Y$, $|Y'| > \frac{|Y|}{2}$, such that every process in $Y'$ receives less than $t_S = \lfloor \frac{t}{2} \rfloor$ messages in $\mathcal{E}$ from processes in $X$. Therefore, assume that there exists a subset $Y'' \subseteq Y$ of $|Y''| \geq \lceil \frac{|Y|}{2} \rceil$ processes which receive more than $t_S$ messages in $\mathcal{E}$ from processes in $X$.
As $\mathcal{A}$ sends less than $\frac{t^2}{32}$ messages in execution $\mathcal{E}$, less than $\frac{t^2}{32}$ messages are sent in $\mathcal{E}$ by correct processes (i.e., processes in $X$), which implies $|M_{X \to Y''}| < \frac{t^2}{32} < \lceil \frac{|Y|}{2} \rceil \cdot \lfloor \frac{t}{2} \rfloor$, thus we reach a contradiction. Hence, $\exists Y' \subset Y$, $|Y'| > \frac{|Y|}{2}$, such that every process in $Y'$ receive less than $t_S = \lfloor \frac{t}{2} \rfloor$ messages in $\mathcal{E}$ from processes in $X$, i.e. $\forall P_i \in Y', |M_{X \to \{P_i\}}| \leq t_S$.

Let $P_i \in Y'$.
Let $S_i$ denote the set of processes in $X$ whose messages $P_i$ receive-omits from (and including) round $k$ onward in $\mathcal{B}_i$:
\begin{equation*}
    S_i = \{ P_s \in X \,|\, \exists k' \in [k, \infty], \exists m \in \fmsgro{\mathcal{B}_i}{k'}: m.\mathsf{sender} = P_s \}.
\end{equation*}
Note that $P_i \notin S_i$ (as no process ever sends messages to itself).
Moreover, as $|M_{X \to \{P_i\}}| \leq t_S$, $|S_i| \leq t_S$.
We now create another execution $\mathcal{E}'_i = [\mathcal{F}', \mathcal{B}_1', ..., \mathcal{B}_n'] = \fswitcho{\mathcal{E}}{\tilde{M}_i}$ where $\tilde{M}_i = M_{(X \cup Z) \to \{P_i\}}$.
We can observe that $P_i$ is correct in $\mathcal{E}'_i$.
Hence, $\mathcal{F}' \subseteq S_i \cup Z \cup (Y \setminus{\{ P_i \}})$ which means  $|\mathcal{F}'| \leq t$. 

By \Cref{lemma:switch_omission}, $\mathcal{E}'_i$ is a valid execution of $\mathcal{A}$, indistinguishable from $\mathcal{E}$.
Since $|X|>t_S$ and $|S_i|\leq t_S$, then $\exists P_{x_i} \in X \setminus S_i \neq \emptyset$, that is both $P_i$ and $P_{x_i}$ are correct in $\mathcal{E}'_i$.

Thus, processes $p_{i}$ and $p_{x_i}$ must agree on the same bit $b_i' \in \{0,1\}$ in $\mathcal{E}'_i$ by correctness of $\mathcal{A}$
Finally, neither $p_{i}$ nor $p_{x_i}$ can distinguish $\mathcal{E}'_i$ from $\mathcal{E}$ as their behaviors in $\mathcal{E}'_i$ and $\mathcal{E}$ are identical. Thus, processes $p_{i}$ and $p_{x_i}$ must decide $b_i'$ by indistinguishability, which means $b_i' = b_X$.
Hence, every process in $Y'$ decide $b_X$, which concludes the lemma.
\end{proof}



In the rest of the proof, we fix the following:

\begin{table} [h]
    \begin{tabular}{|c|m{8.5cm}|}
    \hline
        $(A, B, C)$ & any partition of $\Pi$ such that (1) $|A| = n - \frac{t}{2}$, (2) $|B| = \frac{t}{4}$, and (3) $|C| = \frac{t}{4}$
         \\ \hline
        $\mathcal{E}_0$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, and (2) all processes are correct \\ \hline
        $\mathcal{E}_0^{B(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup C$ are correct, and (3) group $B$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup B$ are correct, and (3) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{B(k_1), C(k_2)}, k_1,k_2 \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k_1$, and (4) group $C$ is isolated from round $k_2$ \\ \hline
        %$\mathcal{E}_0^{B(k + 1), C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k + 1$, and (4) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_1^{C(1)}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $1$, (2) processes from  $A \cup B$ are correct, and (3) group $C$ is isolated from round $1$  \\ \hline
    \end{tabular}
    % \caption{Fixed parameters}
    \label{tab:fixed_parameters}
\end{table}

\begin{lemma}[Majority of $B$ and $C$ must agree with $A$]\label{lemma:majority_agreement}
    Let $\mathcal{E}$ be an infinite execution of $\mathcal{A}$ such that processes in $A$ agree on bit $b'_A \in \{0,1\}$ (by correctness of $\mathcal{A}$), while $B$ is correct or receive-isolated from some round and $C$ is correct or receive-isolated from some (potentially different) round.
    Then, $\exists (B',C') \subset B \times C$ with $|B'| > \frac{|B|}{2}$ and $|C'| > \frac{|C|}{2}$ such that every process in $B' \cup C'$ decides $b'_A$.
\end{lemma}

\begin{proof}
    By \Cref{lemma:lower_bound_helper} applied to $\mathcal{E}$ and $(X,Y,Z)$, with either $(X,Y,Z) = (A,B,C)$, or $(X,Y,Z) = (A \cup B,C,\emptyset)$ or $(X,Y,Z) = (A \cup C,B,\emptyset)$.
\end{proof}

\begin{lemma}\label{lemma:merge_and_isolation}
    Let $k^{u}, k^{v} \in \mathbb{N}^{>0}$ and $b^{u}, b^{v} \in \{0,1\}$.
    Let $\mathcal{E}^u = \mathcal{E}^{B(k^u)}_{b^{u}} = [\mathcal{F}^{u}, \mathcal{B}^{u}_1, ...,  \mathcal{B}^{u}_n]$ and $\mathcal{E}^v = \mathcal{E}^{C(k^v)}_{b^{v}} = [\mathcal{F}^{v}, \mathcal{B}^{v}_1, ...,  \mathcal{B}^{v}_n]$ be two infinite executions such that either (1) $k^{u} = k^{v} = 1$ or (2) $|k^{u} - k^{v}| \leq 1$ and $b^{u} = b^{v}$.
Then $A$ agree on the same bit $\tilde{b}_A \in \{0,1\}$  in both $\mathcal{E}^u$ and $\mathcal{E}^v$.
\end{lemma}

\begin{proof}
    By correctness of $\mathcal{A}$, $A$ agree on the bit $\tilde{b}^{u}_A \in \{0,1\}$ in $\mathcal{E}^u$ and on the bit $\tilde{b}^{v}_A \in \{0,1\}$ in $\mathcal{E}^v$.
    Let $\mathcal{E}^{w} = \mathsf{merge}(\mathcal{E}^u,\mathcal{E}^v)$. By \Cref{lemma:merge}, $\mathcal{E}^{w}$ is a valid execution indistinguishable from $\mathcal{E}^u$ (resp. $\mathcal{E}^v$) for processes in $B$ (resp. processes in $B$).   By correctness of $\mathcal{A}$, $A$ agree on the same bit $\tilde{b}^{w}_A \in \{0,1\}$ in $\mathcal{E}^{w}$.
    
    By \Cref{lemma:majority_agreement}, $\exists (B_u',C_u'), (B_v',C_v'), (B_w',C_w') \subset B \times C$ with $B_u',B_v',B_w' > \frac{|B|}{2}$ and $C_u',C_v',C_w' > \frac{|C|}{2}$ such that every process in $B_u' \cup C_u'$ decides $\tilde{b}^{u}_A$, every process in $B_v' \cup C_v'$ decides $\tilde{b}^{v}_A$, and every process in $B_w' \cup C_w'$ decides $\tilde{b}^{w}_A$.

    Crucially, $B_u' \cap B_w' \neq \emptyset$ and $C_v' \cap C_w' \neq \emptyset$. We note $P_i \in B_u' \cap B_w'$ and $P_j \in C_v' \cap C_w'$.
    By indistinguishability, $P_i$ (resp. $P_j$) decide the same bit in both $\mathcal{E}^{w}$ and $\mathcal{E}^u$ (resp. $\mathcal{E}^v$), that is $\tilde{b}^{w}_A = \tilde{b}^{u}_A$ and $\tilde{b}^{w}_A = \tilde{b}^{v}_A$, which means $\tilde{b}^{u}_A = \tilde{b}^{v}_A$.    
\end{proof}

\begin{lemma}
    Processes in $A$ agree on the same bit $\tilde{b}_A \in \{0,1\}$ in both $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$
\end{lemma}

\begin{proof}
    By direct application of case (1) of \Cref{lemma:majority_agreement}.
\end{proof}

Without the loss of generality, we assume that $A$ agree on bit $1$ in both $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$
The next lemma proves an existence of a critical round $R \in \mathbb{N}$, where processes in $A$ modify their decision in $\mathcal{E}_0^{B(R)}$ and $\mathcal{E}_0^{B(R + 1)}$.

\begin{lemma}[Critical round] \label{lemma:critical_round}
There exists a round $R \in \mathbb{N}$ such that (1) $A$ agree on the bit $1$ in $\mathcal{E}_0^{B(R)}$, and (2) $A$ agree on the bit $0$ in $\mathcal{E}_0^{B(R + 1)}$.
\end{lemma}
\begin{proof}
For every round $k \in \mathbb{N}$, $A$ agree on the bit $b^k$ in $\mathcal{E}_0^{B(k)}$, to satisfy \emph{Termination} and \emph{Agreement}.
We have fixed $b^1 = 1$.
Let $R_{\mathit{max}} \in \mathbb{N}$ denote the round before which every process decides $0$ in $\mathcal{E}_0$ in order to satisfy \emph{Termination} and \emph{Weak Validity}, i.e. $b^{R_{\mathit{max}}} = 0$.
there exists a round $R \in [1, R_{\mathit{max}})$ which satisfies $b^{R} = 1$ and $b^{R+1} = 0$, that is the statement of the lemma. 
\end{proof}

Finally, we prove a contradiction.
Thus, the following lemma proves \Cref{lemma:lower_bound_omission}, which directly implies \Cref{theorem:lower_bound_weak_validity}.

\lowerboundomission*

\begin{proof}
    According to \Cref{lemma:critical_round}, there exists a round $R \in \mathbb{N}$ such that (1) $A$ agree on the bit $1$ in $\mathcal{E}_0^{B(R)}$, and (2) $A$ agree on the bit $0$ in $\mathcal{E}_0^{B(R + 1)}$.
    By correctness of $\mathcal{A}$, processes in $A$ agree on the same bit $b_c$ in $\mathcal{E}_0^{C(R)}$.
    By case (2) of \Cref{lemma:merge_and_isolation} applied to both the pair $(\mathcal{E}_0^{B(R)}, \mathcal{E}_0^{C(R)})$ and the pair $(\mathcal{E}_0^{B(R+1)}, \mathcal{E}_0^{C(R)})$, $b_c = 1$ and $b_c = 0$, thus the contradiction. The entire proof is concluded.
\end{proof}

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% version tuesday 02/11/23 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Sub-majority isolation] \label{lemma:lower_bound_helper}
Let $(X, Y, Z)$ represent any partition of $\Pi$ such that (1) $|X| = n - |Y| - |Z|$, (2) $|Y| = \frac{t}{4}$, and (3) $|Z| \leq \frac{t}{4}$.
Moreover, let $\mathcal{E}$ be any infinite execution of $\mathcal{A}$ such that:
\begin{compactitem}
    \item processes from $X$ are correct in $\mathcal{E}$, whereas processes from $Y \cup Z$ are faulty in $\mathcal{E}$; and

    \item group $Y$ is isolated from some round $k \in \mathbb{N}$ in $\mathcal{E}$.
\end{compactitem}
Then, there exists a set $Y' \subset Y$, such that (a) $|Y'|>\frac{|Y|}{2}$ and (b) for every process $P_i \in Y'$, there exists a process $P_{x_i} \in X$ and an infinite execution $\mathcal{E}_i$ of $\mathcal{A}$ such that (1) $P_{x_i}$ and $P_i$ are correct in $\mathcal{E}_i$, and (2) $\mathcal{E}_i$ is indistinguishable from $\mathcal{E}$ to both $P_{x_i}$ and $P_i$.
\end{lemma}

\begin{proof}[formal proof]
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Due to the statement of the lemma, $\mathcal{F} = Y \cup Z$.
Moreover, no process in $X \cup Y$ commits any send-omission failure in $\mathcal{E}$: for every process $P_i \in X \cup Y$ and every round $j \in \mathbb{N}^+ \cup \{+\infty\}$, $\mathsf{send\_omitted}(\mathcal{B}_i, j) = \emptyset$.

For every set of processes $U$, we note $M_{U} = \bigcup\limits_{P_i \in U} \big( \bigcup\limits_{k' \geq k}  \fmsgs{\mathcal{B}_i}{k'} \big)$ to denote the set of messages sent by processes in $U$ from (and including) round $k$ onward in $\mathcal{E}$.

For every pair of sets of processes $(U, V)$, we define $M_{U \to V}$ as the set containing all messages sent to a process in $V$ by processes in $U$ from (and including) round $k$ onward of $\mathcal{E}$:
\begin{equation*}
    M_{U \to V} = \{ m \,|\, m \in M_{U} \land m.\mathsf{receiver} \in V \}.
\end{equation*}
Note that, for every $P_i \in Y$, each message $m \in M_{(X \cup Z) \to \{P_i\}}$ is receive-omitted in $\mathcal{B}_i$.

First, we will prove by contradiction that $\exists Y' \subset Y$, $|Y'| > \frac{|Y|}{2}$, such that every process in $Y'$ receives less than $t_S = \lfloor \frac{t}{2} \rfloor$ messages in $\mathcal{E}$ from processes in $X$. Therefore, assume that there exists a subset $Y'' \subseteq Y$ of $|Y''| \geq \lceil \frac{|Y|}{2} \rceil$ processes which receive more than $t_S$ messages in $\mathcal{E}$ from processes in $X$.
As $\mathcal{A}$ sends less than $\frac{t^2}{32}$ messages in execution $\mathcal{E}$, less than $\frac{t^2}{32}$ messages are sent in $\mathcal{E}$ by correct processes (i.e., processes in $X$), which implies $|M_{X \to Y''}| < \frac{t^2}{32} < \lceil \frac{|Y|}{2} \rceil \cdot \lfloor \frac{t}{2} \rfloor$, thus we reach a contradiction. Hence, $\exists Y' \subset Y$, $|Y'| > \frac{|Y|}{2}$, such that every process in $Y'$ receive less than $t_S = \lfloor \frac{t}{2} \rfloor$ messages in $\mathcal{E}$ from processes in $X$, i.e. $\forall P_i \in Y', |M_{X \to \{P_i\}}| \leq t_S$.

Let $P_i \in Y'$.
Let $S_i$ denote the set of processes in $X$ whose messages $P_i$ receive-omits from (and including) round $k$ onward in $\mathcal{B}_i$:
\begin{equation*}
    S_i = \{ P_s \in X \,|\, \exists k' \in [k, \infty], \exists m \in \fmsgro{\mathcal{B}_i}{k'}: m.\mathsf{sender} = P_s \}.
\end{equation*}
Note that $P_i \notin S_i$ (as no process ever sends messages to itself).
Moreover, as $|M_{X \to \{P_i\}}| \leq t_S$, $|S_i| \leq t_S$.
We now create another execution $\mathcal{E}'_i = [\mathcal{F}', \mathcal{B}_1', ..., \mathcal{B}_n'] = \fswitcho{\mathcal{E}}{\tilde{M}_i}$ where $\tilde{M}_i = M_{(X \cup Z) \to \{P_i\}}$.
We can observe that $P_i$ is correct in $\mathcal{E}'_i$.
Hence, $\mathcal{F}' \subseteq S_i \cup Z \cup (Y \setminus{\{ P_i \}})$ which means  $|\mathcal{F}'| \leq t$. 

By \Cref{lemma:switch_omission}, $\mathcal{E}'_i$ is a valid execution of $\mathcal{A}$, indistinguishable from $\mathcal{E}$.
Since $|X|>t_S$ and $|S_i|\leq t_S$, then $\exists P_{x_i} \in X \setminus S_i \neq \emptyset$, that is both $P_i$ and $P_{x_i}$ are correct in $\mathcal{E}'_i$.
Hence, the lemma holds.
\end{proof}



In the rest of the proof, we fix the following:

\begin{table} [h]
    \begin{tabular}{|c|m{8.5cm}|}
    \hline
        $(A, B, C)$ & any partition of $\Pi$ such that (1) $|A| = n - \frac{t}{2}$, (2) $|B| = \frac{t}{4}$, and (3) $|C| = \frac{t}{4}$
         \\ \hline
        $\mathcal{E}_0$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, and (2) all processes are correct \\ \hline
        $\mathcal{E}_0^{B(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup C$ are correct, and (3) group $B$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup B$ are correct, and (3) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{B(k_1), C(k_2)}, k_1,k_2 \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k_1$, and (4) group $C$ is isolated from round $k_2$ \\ \hline
        %$\mathcal{E}_0^{B(k + 1), C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k + 1$, and (4) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_1^{C(1)}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $1$, (2) processes from  $A \cup B$ are correct, and (3) group $C$ is isolated from round $1$  \\ \hline
    \end{tabular}
    % \caption{Fixed parameters}
    \label{tab:fixed_parameters}
\end{table}

\begin{lemma}[Majority of $B$ and $C$ must agree with $A$]\label{lemma:majority_agreement}
    Let $\mathcal{E}$ be an infinite execution of $\mathcal{A}$ such that processes in $A$ agree on bit $b'_A \in \{0,1\}$ (by correctness of $\mathcal{A}$), while $B$ and $C$ are receive-isolated from rounds $k_B \in \mathbb{N}^{>0}$ and $k_C \in \mathbb{N}^{>0}$ respectively Then, $\exists (B',C') \subset B \times C$ with $|B'| > \frac{|B|}{2}$ and $|C'| > \frac{|C|}{2}$ such that every process in $B' \cup C'$ decides $b'_A$.
\end{lemma}

\begin{proof}
    By former lemma, with $(X,Y,Z) = (A,B,C)$, $\exists (B',C') \subset B \times C$ with $B' > \frac{|B|}{2}$ and $C' > \frac{|C|}{2}$ such that for every process $P_i \in B' \cup C'$, there exists a process $P_{x_i} \in A$ and a valid execution $\mathcal{E}'_i$ indistinguishable from $\mathcal{E}$ such that both $P_i$ and $P_{x_i}$ are correct. By correctness of $\mathcal{A}$, $P_i$ and $P_{x_i}$ decide a common bit $b^{i}$. By indistinguishability, $P_i$ and $P_{x_i}$ decide $b^{i}$ in $\mathcal{E}'_i$. Hence, $b^{i} = b'_A$. Thus, the lemma holds. 
\end{proof}

\begin{lemma}\label{lemma:merge_and_isolation}
    Let $k^{u}, k^{v} \in \mathbb{N}^{>0}$ and $b^{u}, b^{v} \in \{0,1\}$.
    Let $\mathcal{E}^u = \mathcal{E}^{B(k^u)}_{b^{u}} = [\mathcal{F}^{u}, \mathcal{B}^{u}_1, ...,  \mathcal{B}^{u}_n]$ and $\mathcal{E}^v = \mathcal{E}^{C(k^v)}_{b^{v}} = [\mathcal{F}^{v}, \mathcal{B}^{v}_1, ...,  \mathcal{B}^{v}_n]$ be two infinite executions such that either (1) $k^{u} = k^{v} = 1$ or (2) $|k^{u} - k^{v}| \leq 1$ and $b^{u} = b^{v}$.
Then $A$ agree on the same bit $\tilde{b}_A \in \{0,1\}$  in both $\mathcal{E}^u$ and $\mathcal{E}^v$.
\end{lemma}

\begin{proof}
    By correctness of $\mathcal{A}$, $A$ agree on the bit $\tilde{b}^{u}_A \in \{0,1\}$ in $\mathcal{E}^u$ and on the bit $\tilde{b}^{v}_A \in \{0,1\}$ in $\mathcal{E}^v$.
    Let $\mathcal{E}^{w} = \mathsf{merge}(\mathcal{E}^u,\mathcal{E}^v)$. By \Cref{lemma:merge}, $\mathcal{E}^{w}$ is a valid execution indistinguishable from $\mathcal{E}^u$ (resp. $\mathcal{E}^v$) for processes in $B$ (resp. processes in $B$).   By correctness of $\mathcal{A}$, $A$ agree on the same bit $\tilde{b}^{w}_A \in \{0,1\}$ in $\mathcal{E}^{w}$.
    
    By \Cref{lemma:majority_agreement}, $\exists (B_u',C_u'), (B_v',C_v'), (B_w',C_w') \subset B \times C$ with $B_u',B_v',B_w' > \frac{|B|}{2}$ and $C_u',C_v',C_w' > \frac{|C|}{2}$ such that every process in $B_u' \cup C_u'$ decides $\tilde{b}^{u}_A$, every process in $B_v' \cup C_v'$ decides $\tilde{b}^{v}_A$, and every process in $B_w' \cup C_w'$ decides $\tilde{b}^{w}_A$.

    Crucially, $B_u' \cap B_w' \neq \emptyset$ and $C_v' \cap C_w' \neq \emptyset$. We note $P_i \in B_u' \cap B_w'$ and $P_j \in C_v' \cap C_w'$.
    By indistinguishability, $P_i$ (resp. $P_j$) decide the same bit in both $\mathcal{E}^{w}$ and $\mathcal{E}^u$ (resp. $\mathcal{E}^v$), that is $\tilde{b}^{w}_A = \tilde{b}^{u}_A$ and $\tilde{b}^{w}_A = \tilde{b}^{v}_A$, which means $\tilde{b}^{u}_A = \tilde{b}^{v}_A$.    
\end{proof}

\begin{lemma}
    Processes in $A$ agree on the same bit $\tilde{b}_A \in \{0,1\}$ in both $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$
\end{lemma}

\begin{proof}
    By direct application of case (1) of \Cref{lemma:majority_agreement}.
\end{proof}

Without the loss of generality, we assume that $A$ agree on bit $1$ in both $\mathcal{E}^{B(1)}_0$ and $\mathcal{E}^{C(1)}_1$
The next lemma proves an existence of a critical round $R \in \mathbb{N}$, where processes in $A$ modify their decision in $\mathcal{E}_0^{B(R)}$ and $\mathcal{E}_0^{B(R + 1)}$.

\begin{lemma}[Critical round] \label{lemma:critical_round}
There exists a round $R \in \mathbb{N}$ such that (1) $A$ agree on the bit $1$ in $\mathcal{E}_0^{B(R)}$, and (2) $A$ agree on the bit $0$ in $\mathcal{E}_0^{B(R + 1)}$.
\end{lemma}
\begin{proof}
For every round $k \in \mathbb{N}$, $A$ agree on the bit $b^k$ in $\mathcal{E}_0^{B(k)}$, to satisfy \emph{Termination} and \emph{Agreement}.
We have fixed $b^1 = 1$.
Let $R_{\mathit{max}} \in \mathbb{N}$ denote the round before which every process decides $0$ in $\mathcal{E}_0$ in order to satisfy \emph{Termination} and \emph{Weak Validity}, i.e. $b^{R_{\mathit{max}}} = 0$.
there exists a round $R \in [1, R_{\mathit{max}})$ which satisfies $b^{R} = 1$ and $b^{R+1} = 0$, that is the statement of the lemma. 
\end{proof}

Finally, we prove a contradiction.
Thus, the following lemma proves \Cref{lemma:lower_bound_omission}, which directly implies \Cref{theorem:lower_bound_weak_validity}.

\lowerboundomission*

\begin{proof}
    According to \Cref{lemma:critical_round}, there exists a round $R \in \mathbb{N}$ such that (1) $A$ agree on the bit $1$ in $\mathcal{E}_0^{B(R)}$, and (2) $A$ agree on the bit $0$ in $\mathcal{E}_0^{B(R + 1)}$.
    By correctness of $\mathcal{A}$, processes in $A$ agree on the same bit $b_c$ in $\mathcal{E}_0^{C(R)}$.
    By case (2) of \Cref{lemma:merge_and_isolation} applied to both the pair $(\mathcal{E}_0^{B(R)}, \mathcal{E}_0^{C(R)})$ and the pair $(\mathcal{E}_0^{B(R+1)}, \mathcal{E}_0^{C(R)})$, $b_c = 1$ and $b_c = 0$, thus the contradiction. The entire proof is concluded.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end version tuesday 02/11/23 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

%%%%%%%%%%%%%
%% figures %%
%%%%%%%%%%%%%

\begin{figure}[!t]
\centering
\includegraphics[width=9cm]{figures/alternative/generic_isolation.eps}
\caption{Isolation}
\label{figure:isolation_alternative}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=9cm]{figures/alternative/merge_init.eps}
\caption{Some default value ($0$ or $1$) exists}
\label{figure:merge_init_alternative}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=9cm]{figures/alternative/merge_final_R.eps}
\caption{Inconsistency occurs when $b_C = 0$}
\label{figure:merge_final_R_alternative}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=9cm]{figures/alternative/merge_final_R_p_1.eps}
\caption{Inconsistency occurs when $b_C = 1$}
\label{figure:merge_final_R_p_1_alternative}
\end{figure}


==> sections/alternative_proof_with_abstract_merging.tex <==
\section{Lower Bound on Message Complexity of Weak Consensus (With 1 lemma for all the merging operations)}

To prove our general lower bound, we first show a quadratic lower bound for weak consensus:

\begin{theorem} \label{theorem:lower_bound_weak_validity_am}
Any weak consensus algorithm achieves $\Omega(t^2)$ message complexity.
\end{theorem}

A formal proof of \Cref{theorem:lower_bound_weak_validity_am} is relegated to \Cref{section:lower_bound_formal}.
In this section, we provide an informal (but comprehensive) proof of the lower bound.
Concretely, to prove \Cref{theorem:lower_bound_weak_validity_am}, we show a strictly stronger lower bound for the omission failure model in which processes can only fail by ``dropping'' some messages they send or receive, but not by behaving maliciously.

\paragraph{Omission failures.}
In (only) this section, we consider \emph{omission failures}.
A static adversary corrupts up to $t$ processes, for any $t \in [1, n - 1]$, before each execution.
A corrupted process can commit:
\begin{compactitem}
    \item \emph{send-omission} faults, by not sending some messages it is supposed to send, or

    \item \emph{receive-omission} faults, by not receiving some messages it is suppose to receive.
\end{compactitem}
Note that a faulty process cannot misbehave in an arbitrary manner, i.e., it acts according to its state machine at all times.
Moreover, corrupted processes are not aware of the fact that they are corrupted, i.e., they do not know if or when they omitted some messages.
Corrupted processes are said to be \emph{faulty}, whereas non-corrupted processes are said to be \emph{correct}.
(\Cref{section:lower_bound_formal_am} includes a precise definition of the omission failure model.)

\paragraph{Notation \& remarks.}
Given any set of processes $G$, $\bar{G} = \Pi \setminus{G}$.
If a faulty process omits sending (resp., omits receiving) some message $m$, we say that the process \emph{send-omits} (resp., \emph{receive-omits}) $m$.
Note that, in the omission failure model, it is reasonable to make claims about the behaviors of faulty processes as they always behave according to their state machine; recall that faulty processes do not know if or when they have omitted some messages.
Finally, observe that any weak consensus algorithm provides guarantees \emph{only} to correct processes, i.e., it is possible for faulty processes to not terminate or to disagree (among themselves or with correct processes).
% Thus, throughout our proof, we do make some claims concerned with the faulty processes.

\subsection{Proof of \Cref{theorem:lower_bound_weak_validity_am}}
% \paragraph{Proof of \Cref{theorem:lower_bound_weak_validity}.}

As previously mentioned, we prove a quadratic lower bound for weak consensus by showing that the problem requires $\Omega(t^2)$ in the worst-case even with omission failures:

\begin{restatable}{lemma}{lowerboundomissionam}\label{lemma:lower_bound_omission_am}
Any omission-resilient weak consensus algorithm achieves $\Omega(t^2)$ message complexity.
\end{restatable}

We prove \Cref{lemma:lower_bound_omission_am} by contradiction.
Thus, we fix any weak consensus algorithm $\mathcal{A}$ which (1) tolerates up to $t$ omission failures, for any $t \in [1, n - 1]$, and (2) achieves $o(t^2)$ message complexity.
As $\mathcal{A}$'s message complexity is $o(t^2)$, correct processes send fewer than $\frac{t^2}{32}$ messages in \emph{every} execution of $\mathcal{A}$.
First, let us introduce the concept of \emph{isolation}, which we extensively use.

\begin{definition} [Isolation] \label{definition:isolation_am}
A group $G \subsetneq \Pi$ of $|G| \leq t$ processes is \emph{isolated from some round $k \in \mathbb{N}$} in an execution $\mathcal{E}$ of $\mathcal{A}$ if and only if, for every process $p_G \in G$, the following holds:
\begin{compactitem}
    \item $p_G$ is faulty in $\mathcal{E}$; and
    
    \item $p_G$ does not send-omit any message in $\mathcal{E}$; and

    \item for every message $m$ sent by any process $p_m$ to $p_G$ in any round $k' \in \mathbb{N}$ of $\mathcal{E}$, $p_G$ receive-omits $m$ in $\mathcal{E}$ if and only if (1) $p_m \in \bar{G}$, and (2) $k' \geq k$.
\end{compactitem}
\end{definition}

Intuitively, a group $G$ is isolated from some round $k$ if and only if no process $p_G \in G$ receives any message from outside of $G$ in any round $k' \geq k$, i.e., $p_G$ only receives messages sent by processes in $G$ from round $k$ onward; other than these receive-omission faults, $p_G$ commits no other faults.

\begin{figure}[ht]
    \centering
    \begin{minipage}{1\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/isolation.pdf}
        \caption{Illustration of \Cref{definition:isolation_am}.
        The colors represent the local behaviors of processes (including the messages sent).
        Execution $\mathcal{E}_0$ has no faults.
        Execution $\mathcal{E}_0^{X(R)}$ proceeds identically to $\mathcal{E}_0$, sending the same messages (green color) up until round $R$ (inclusive).
        However, group $X$ is \emph{isolated} at round $R$, causing it to miss all messages from group $\overline{X}$ from then on.
        This (potentially) changes $X$'s sending behavior from round $R+1$ onward (red color).
        By propagation, group $\overline{X}$ is then (potentially) affected by $X$'s new sending behavior (red color), causing $\overline{X}$ to deviate from $\mathcal{E}_0$ from round $R+2$ onward (blue color).
        }
        \label{figure:helper_isolation_illustration_am}
    \end{minipage}
\end{figure}

Consider any partition $(X, Y, Z)$ of $\Pi$.
The following lemma proves that, in any infinite execution $\mathcal{E}$ of $\mathcal{A}$ in which processes from $X$ are correct and processes from $Y \cup Z$ are faulty, at least half of processes from $Y$ decide the same bit as processes from $X$.
If this was not the case, we could construct an execution which proves that $\mathcal{A}$ is not a correct weak consensus algorithm.


\begin{restatable}{lemma}{genericisolationam}\label{lemma:lower_bound_helper_am}
Let $(X, Y, Z)$ be any partition of $\Pi$ such that (1) $|Y| = \frac{t}{4}$, and (2) $|Z| \leq \frac{t}{4}$ (naturally, $|X| = n - |Y| - |Z|$).
% Let $Y'$ be any group of processes such that (1) $Y' \subseteq Y$, and (2) $|Y'| \geq \frac{|Y|}{4} = \frac{t}{16}$. 
Moreover, let $\mathcal{E}$ be any infinite execution of $\mathcal{A}$ such that:
\begin{compactitem}
    \item processes from $X$ are correct in $\mathcal{E}$, whereas processes from $Y \cup Z$ are faulty in $\mathcal{E}$; and

    \item all processes from $X$ decide the same bit $b_X$ (to satisfy \emph{Termination} and \emph{Agreement}); and 

    \item group $Y$ is isolated from some round $k \in \mathbb{N}$ in $\mathcal{E}$.
\end{compactitem}
Then, there exists a set $Y' \subseteq Y$ of $|Y'| > \frac{|Y|}{2}$ processes such that all processes in $Y'$ decide $b_X$ in $\mathcal{E}$.
\end{restatable}
\begin{proof}
For every process $p \in Y$, let $\mathcal{M}_{X \to p}$ denote the set of all messages which are (1) sent by any process $p' \in X$ in $\mathcal{E}$, and (2) receive-omitted by $p$ in $\mathcal{E}$; as $p \in Y$ and group $Y$ is isolated from round $k$ in $\mathcal{E}$, every message $m \in \mathcal{M}_{X \to p}$ is sent in some round $k' \geq k$.
For every set $Y'' \subseteq Y$, let $\mathcal{M}_{X \to Y''} = \bigcup\limits_{p \in Y''} \mathcal{M}_{X \to p}$.
As correct processes (i.e., processes from group $X$) send fewer than $\frac{t^2}{32}$ messages in $\mathcal{E}$, $|\mathcal{M}_{X \to Y}| < \frac{t^2}{32}$.
Therefore, there does not exist any set $Y^* \subseteq Y$ of $|Y^*| \geq \frac{|Y|}{2}$ processes such that, for every process $p_{Y^*} \in Y^*$, $|\mathcal{M}_{X \to p_{Y^*}}| \geq \frac{t}{2}$.
This implies that there exists a set $Y' \subseteq Y$ of $|Y'| > \frac{|Y|}{2}$ processes such that, for every process $p_{Y'} \in Y'$, $|\mathcal{M}_{X \to p_{Y'}}| < \frac{t}{2}$.

Fix any process $p_{Y'} \in Y'$.
By contradiction, suppose that $p_{Y'}$ does not decide $b_X$ in $\mathcal{E}$.
Let $\mathcal{S}$ denote the set of all processes whose messages $p_{Y'}$ receive-omits in (any round $k' \geq k$ of) $\mathcal{E}$; note that $|\mathcal{S} \cap X| < \frac{t}{2}$ (since $|\mathcal{M}_{X \to p_{Y'}}| < \frac{t}{2}$) and $\mathcal{S} \subsetneq X \cup Z$.
Let us construct another infinite execution $\mathcal{E}'$ of $\mathcal{A}$ following the (sequentially-executed) steps below:
\begin{compactenum}
    \item Processes in $\mathcal{S} \cup Y \cup Z \setminus{\{ p_{Y'} \}}$ are faulty in $\mathcal{E}'$, whereas all other processes are correct.

    \item Then, we set $\mathcal{E}' \gets \mathcal{E}$: every process (at first) behaves in the same manner as in $\mathcal{E}$.

    \item For every message $m$ such that $p_{Y'}$ receive-omits $m$ in $\mathcal{E}$, $m$ is send-omitted in $\mathcal{E}'$.
    That is, the sender of $m$ is responsible for $p_{Y'}$ not receiving $m$ in $\mathcal{E}'$.
\end{compactenum}
Observe that $p_{Y'}$ is indeed correct in $\mathcal{E}'$ as (1) $p_{Y'}$ does not commit any send-omission faults (since $p_{Y'}$ does not commit those faults in $\mathcal{E}$), and (2) $p_{Y'}$ does not commit any receive-omission faults (since every message which is receive-omitted in $\mathcal{E}$ is send-omitted in $\mathcal{E}'$).
Moreover, there are $|\mathcal{S} \cup Y \cup Z \setminus{\{p_{Y'}\}}| = |(\mathcal{S} \cap X) \cup Y \cup Z \setminus{\{p_{Y'}\}}| < \frac{t}{2} + \frac{t}{4} + \frac{t}{4} - 1 < t$ faulty processes in $\mathcal{E}'$.
Furthermore, there exists a process $p_X \in X$ which is correct in $\mathcal{E}'$ as $|\mathcal{S} \cap X| < \frac{t}{2}$, $|X| \geq n - \frac{t}{2}$ and $n > t$.
Finally, neither $p_{Y'}$ nor $p_X$ can distinguish $\mathcal{E}'$ from $\mathcal{E}$ as their behaviors in $\mathcal{E}'$ and $\mathcal{E}$ are identical.
Therefore, either \emph{Termination} (if $p_{Y'}$ does not decide) or \emph{Agreement} (if $p_{Y'}$ decides $1 - b_X$) is violated in $\mathcal{E}'$, which contradicts the fact that $\mathcal{A}$ is a correct weak consensus algorithm.
\end{proof}

We fix the following parameters for the rest of the proof:

\begin{table} [h]
    \begin{tabular}{|c|m{8.5cm}|}
    \hline
        $(A, B, C)$ & any partition of $\Pi$ such that (1) $|A| = n - \frac{t}{2}$, (2) $|B| = \frac{t}{4}$, and (3) $|C| = \frac{t}{4}$
         \\ \hline
        $\mathcal{E}_0$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, and (2) all processes are correct \\ \hline
        $\mathcal{E}_0^{B(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup C$ are correct, and (3) group $B$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A \cup B$ are correct, and (3) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_0^{B(k_1), C(k_2)}, k_1,k_2 \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k_1$, and (4) group $C$ is isolated from round $k_2$ \\ \hline
        %$\mathcal{E}_0^{B(k + 1), C(k)}, k \in \mathbb{N}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $0$, (2) processes from $A$ are correct, (3) group $B$ is isolated from round $k + 1$, and (4) group $C$ is isolated from round $k$ \\ \hline
        $\mathcal{E}_1^{C(1)}$ & the infinite execution of $\mathcal{A}$ in which (1) all processes propose $1$, (2) processes from  $A \cup B$ are correct, and (3) group $C$ is isolated from round $1$  \\ \hline
    \end{tabular}
    % \caption{Fixed parameters}
    \label{tab:fixed_parameters_am}
\end{table}

Below, we define \emph{inconsistent executions}.

\begin{definition} [Inconsistent execution] \label{definition:inconsistent_execution_am}
Consider any infinite execution $\mathcal{E}$ such that (1) processes from $A$ are correct, and (2) processes from $B \cup C$ are faulty.
Let $b_A \in \{0, 1\}$ denote the bit decided by processes all processes from group $A$ (to satisfy \emph{Termination} and \emph{Agreement}).
We say that $\mathcal{E}$ is \emph{inconsistent} if and only if:
\begin{compactitem}
    \item group $B$ is isolated from some round $k_B \in \mathbb{N}$ in $\mathcal{E}$; and

    \item group $C$ is isolated from some round $k_C \in \mathbb{N}$ in $\mathcal{E}$; and

    \item the following holds:
    \begin{compactitem}
        \item more than $\frac{|B|}{2}$ processes from group $B$ do not decide $b_A$ in $\mathcal{E}$, or

        \item more than $\frac{|C|}{2}$ processes from group $C$ do not decide $b_A$ in $\mathcal{E}$.
    \end{compactitem}
\end{compactitem}
\end{definition}

In summary, an infinite execution is inconsistent if (1) both groups $B$ and $C$ are isolated (potentially from different rounds), and (2) more than half of processes from group $B$ or $C$ do not decide the bit decided by correct processes from group $A$.
The following lemma proves that no inconsistent execution of $\mathcal{A}$ exists.

\begin{restatable}{lemma}{noexecutionam}\label{lemma:no_execution_main_am}
No inconsistent execution of $\mathcal{E}$ exists.
\end{restatable}
\begin{sketch}
We prove the lemma by contradiction.
Thus, let us assume that an (infinite) inconsistent execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ exists in which processes from group $A$ decide a bit $b_A$.
Given the partition $(A, B, C)$ (resp., $(A, C, B)$) of $\Pi$, \Cref{lemma:lower_bound_helper} proves that there exists a subset of $B$ (resp., $C$) with more than $\frac{|B|}{2}$ (resp., $\frac{|C|}{2}$) processes which decide $b_A$.
Therefore, $\mathcal{E}$ is not an inconsistent execution, which proves the lemma.
\end{sketch}

We define pairs of \emph{mergeable} executions.

\begin{definition}\label{definition:mergeable_executions_am}
    A pair of infinite executions of the form $(\mathcal{E}_{b_u}^{B(k_u)}, \mathcal{E}_{b_v}^{C(k_v)})$ with $b_u,b_v \in \{0,1\}$ and $k_u,k_v \in \mathbb{N}^{>0}$ are said \emph{mergeable} if either:
    \begin{compactenum}
        \item $k_u = k_v = 1$, or
        \item $|k_u-k_v| \leq 1$ and $b_u = b_v$
    \end{compactenum}
\end{definition}

We show that processes in $A$ agree on the same bit in two mergeable executions.

\begin{lemma}\label{lemma:mergeable_executions_am}
    Processes in $A$ agree on the same bit in two mergeable executions.
\end{lemma}

\begin{proof}
    Let 
    $(\mathcal{E}^{u}, \mathcal{E}^{v}) =(\mathcal{E}_{b_u}^{B(k_u)}, \mathcal{E}_{b_v}^{C(k_v)})$ be two mergeable (infinite) executions with $b_u,b_v \in \{0,1\}$ and $k_u,k_v \in \mathbb{N}^{>0}$.
    To satisfy \emph{Termination} and \emph{Agreement}, all processes from $A$ decide the same bit $\tilde{b}_u$ (resp., $\tilde{b}_v$) in $\mathcal{E}^u$ (resp., $\mathcal{E}^v$).
By contradiction, let $\tilde{b}_u \neq \tilde{b}_v$.
Given the partition $(A \cup C, B, \emptyset)$, there exists a set $B' \subseteq B$ of more than $\frac{|B|}{2}$ processes such that every process $p_{B'} \in B'$ decides $\tilde{b}_u$ in $\mathcal{E}^u$.
Similarly, given the partition $(A \cup B, C, \emptyset)$, there exists a set $C' \subseteq C$ of more than $\frac{|C|}{2}$ processes such that every process $p_{C'} \in C'$ decides $\tilde{b}_v \neq \tilde{b}_u$ in $\mathcal{E}^{v}$.

We now construct an infinite execution $\mathcal{E}^{*}$ of $\mathcal{A}$:
\begin{compactenum}
    \item Processes from group $A$ are correct (commit no omission faults), whereas processes from $B \cup C$ are faulty.
    
    \item All processes from $A \cup B$ propose $b_u$, whereas all processes from group $C$ propose $b_v$.

    \item Every process $p_B \in B$ (resp., $p_C \in C$) behaves in the same manner as in $\mathcal{E}^u$ (resp., $\mathcal{E}^v$).
    Note that this step of construction is valid in each case of the definition of mergeable executions:
    \begin{compactenum}
        \item Assume $k_u = k_v = 1$.
        From round $1$ onward, every process $p_B \in B$ (resp., $p_c \in C$) receives messages only from other processes in group $B$ (resp., $C$).
    Moreover, this step ensures that both groups $B$ and $C$ are isolated from round $1$ in $\mathcal{E}^{*}$.
    
        \item Alternatively, assume $|k_u-k_v| \leq 1$ and $b_u = b_v$.
        %%%%
        In this case, (1) processes' behaviors in $\mathcal{E}^{*}$ until (and excluding) round $\mathit{min}(k_u,k_v)$ are identical to processes' behaviors until (and excluding) round $\mathit{min}(k_u,k_v)$ in both $\mathcal{E}^u$ and $\mathcal{E}^v$. Moreover, (2) the same set of messages is sent in round $R$ of both $\mathcal{E}^{u}$ and $\mathcal{E}^v$, and (3) from round $k_u$ (resp., $k_v$) onward, every process $p_B \in B$ (resp., $p_c \in C$) receives messages only from processes in group $B$ (resp., $C$).
        %%%%
    \end{compactenum}
    
\end{compactenum}
In $\mathcal{E}^{*}$, there are $|B \cup C| < t$ faulty processes, which implies that $\mathcal{E}^{*}$ is indeed a valid infinite execution in $\mathcal{A}$.
%Moreover, in $\mathcal{E}^{*}$, groups $B$ and $C$ are isolated from round $1$.

%%%
Furthermore, group $B$ (resp., $C$) is isolated from round $k_u$ (resp., $k_v$) in $\mathcal{E}^{*}$.
    Lastly, as no process $p_B \in B$ (resp., $p_C \in C$) distinguishes $\mathcal{E}^{*}$ from $\mathcal{E}^u$ (resp., $\mathcal{E}^v$), more than $\frac{|B|}{2}$ (resp., $\frac{|C|}{2}$) processes from group $B$ (resp., $C$) decide $\tilde{b}_u$ (resp., $\tilde{b}_v$) in $\mathcal{E}$. 
    Thus, in both cases, $\mathcal{E}^{*}$ is an inconsistent execution, which contradicts \Cref{lemma:no_execution_main_am}.
As the statement of the lemma holds in both possible cases, the proof is concluded.

\end{proof}

\begin{figure}[ht]
    \centering
    % \begin{minipage}{.2\textwidth}
    %     \centering
    %     %\vspace{.4cm}
    %     \includegraphics[width=.85\linewidth]{figures/legend.pdf}
    %     %\vspace{.95cm}
    %     \caption{Legend}
    %     \label{figure:legend}
    % \end{minipage}%
    \begin{minipage}{1\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/last_lemma.pdf}
        \caption{Illustration of \Cref{lemma:final_am}.
        The arrows denoting (blocked) messages are not exhaustive.
        As in \Cref{figure:helper_isolation_illustration_am}, the colors represent the local behaviors of processes (including messages sent).
        The crucial observation is that, even though processes in non-isolated groups eventually behave differently in every execution, it happens too late to affect the behavior of the isolated groups.
        For example, group $C$ (potentially) sends different messages to group $B$ at round $R+1$, depending on if its execution $\mathcal{E}_0^{C(R)}$ or $\mathcal{E}_0^{B(R+1),C(R)}$.
        However, in either execution, group $B$ does not receive any messages from group $C$ from round $R+1$ onward and therefore cannot perceive the difference.}
        \label{figure:helper_final_lemma_illustration_am}
    \end{minipage}
\end{figure}

%%%
%%%
%%%
The next lemma proves that processes from group $A$ decide the same bit in both $\mathcal{E}_0^{B(k)}$ and $\mathcal{E}_1^{C(1)}$.

\begin{restatable}{lemma}{eitheram}
\label{lemma:either_or_am}
All processes from group $A$ decide the same bit in $\mathcal{E}_0^{B(1)}$ and $\mathcal{E}_1^{C(1)}$.
\end{restatable}
\begin{sketch}
By direct application of \Cref{lemma:mergeable_executions_am}
\end{sketch}

Without loss of generality, we assume that all processes from group $A$ decide $1$ in $\mathcal{E}_0^{B(1)}$.
The next lemma proves that there exists a round $R \in \mathbb{N}$ such that processes from group $A$ have different decisions in $\mathcal{E}_0^{B(R)}$ and $\mathcal{E}_0^{B(R + 1)}$.

\begin{restatable}{lemma}{criticalroundam} \label{lemma:R_am}
There exists a round $R \in \mathbb{N}$ such that (1) processes from group $A$ decide $1$ in $\mathcal{E}_0^{B(R)}$, and (2) processes from group $A$ decide $0$ in $\mathcal{E}_0^{B(R + 1)}$.
\end{restatable}
\begin{sketch}
Let $R_{\mathit{max}} \in \mathbb{N}$ denote the round before which every process decides $0$ in $\mathcal{E}_0$ (to satisfy \emph{Termination} and \emph{Weak Validity}).
By our assumptions, all processes from group $A$ decide $1$ in $\mathcal{E}_0^{B(1)}$.
Therefore, there exists a round $R \in [1, R_{\mathit{max}})$ which satisfies the statement of the lemma.
\end{sketch}

Finally, we prove an inconsistency, proving \Cref{lemma:lower_bound_omission_am}.

\lowerboundomissionam*

\begin{sketch}
According to \Cref{lemma:R_am}, there exists a round $R \in \mathbb{N}$ such that (1) all processes from group $A$ decide $1$ in $\mathcal{E}_0^{B(R)}$, and (2) all processes from group $A$ decide $0$ in $\mathcal{E}_0^{B(R + 1)}$.
Given the partition $(A \cup B, C, \emptyset)$, By correctness of algorithm $\mathcal{A}$, processes from group $A$ decide the same bit $b_C$ in $\mathcal{E}_0^{C(R)}$.
However, both the pair $(\mathcal{E}_0^{B(R + 1)},\mathcal{E}_0^{C(R)})$ and the pair $(\mathcal{E}_0^{B(R)},\mathcal{E}_0^{C(R)})$ are mergeable, implying both $b_C = 0$ and $b_C = 1$ by of \Cref{lemma:mergeable_executions_am}, leading to a contradiction and concluding the proof.


\begin{figure}[ht]
    \centering
    % \begin{minipage}{.2\textwidth}
    %     \centering
    %     %\vspace{.4cm}
    %     \includegraphics[width=.85\linewidth]{figures/legend.pdf}
    %     %\vspace{.95cm}
    %     \caption{Legend}
    %     \label{figure:legend}
    % \end{minipage}%
    \begin{minipage}{1\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/last_lemma.pdf}
        \caption{Illustration of \Cref{lemma:final_am}.
        The arrows denoting (blocked) messages are not exhaustive.
        As in \Cref{figure:helper_isolation_illustration_am}, the colors represent the local behaviors of processes (including messages sent).
        The crucial observation is that, even though processes in non-isolated groups eventually behave differently in every execution, it happens too late to affect the behavior of the isolated groups.
        For example, group $C$ (potentially) sends different messages to group $B$ at round $R+1$, depending on if its execution $\mathcal{E}_0^{C(R)}$ or $\mathcal{E}_0^{B(R+1),C(R)}$.
        However, in either execution, group $B$ does not receive any messages from group $C$ from round $R+1$ onward and therefore cannot perceive the difference.}
        \label{figure:helper_final_lemma_illustration_am}
    \end{minipage}
\end{figure}
\end{sketch}

==> sections/application.tex <==
\section{Our Results in the Wild}

In this section, we investigate some well-studied validity properties. 
Specifically, we study the consequences our findings yield when applied to specific validity properties.

\subsection{Our Results in the Context of Well-Studied Validity Properties}

\paragraph{Strong Validity}
Recall that \emph{Strong Validity}~\cite{CGL18,civit2022byzantine,Momose2021} states that, if all correct processes propose the same value, only that value can be decided.
Observe that \emph{Strong Validity} is a non-trivial validity property.
As such, due to \Cref{theorem:triviality_main}, \emph{Strong Validity} is unsolvable with $n \leq 3t$.

Moreover, Dolev-Reischuk bound states that \emph{Strong Validity} requires $\Omega(t^2)$ messages (and words) to be sent by correct processes.
When $O(t) = O(n)$, the bound is tight: Civit \emph{et al.}~\cite{civit2022byzantine} introduced \textsc{Squad}, a Byzantine consensus algorithm with \emph{Strong Validity}, which achieves $O(n^2)$ message and communication complexities.
In this paragraph, we show that the structure of \textsc{Squad} is similar to the structure of our general algorithm.

\textsc{Squad} is built on top of \textsc{Quad}.
The authors assume an existence of a $(n - 2t, n)$-threshold signature scheme~\cite{libert2014born}.
In a nutshell, these are the steps taken by a correct process $P_i$ in \textsc{Squad}:
\begin{compactenum}
    \item Process $P_i$ broadcasts its proposal $v \in \mathcal{V}_I$, which is share-signed by $P_i$ (with the threshold $n - 2t$).

    \item Once $P_i$ collects $n - t$ proposals, it checks whether there exists a proposal $v^*$ sent by (at least) $n - 2t$.
    
    \begin{compactenum}
        \item If there is, $P_i$ creates a constant-sized threshold signature $\sigma^*$ and proposes $(v^*, \sigma^*)$ to \textsc{Quad}.

        \item Otherwise:
        \begin{compactenum}
            \item $P_i$ broadcasts a predetermined string ``any value'', which is share-signed by $P_i$ (with the threshold $n - 2t$).

            \item $P_i$ waits to obtain either a ``positivity'' proof $\sigma_p$ for some value $v_p$ ($n - 2t$ identical proposals for $p$) or a ``negativity'' proof $\sigma_n$ ($n - 2t$ ``any value'' messages).
            Once this happens, $P_i$ either proposes (1) $(v_p, \sigma_p)$, or (2) $(\mathit{default\_value}, \sigma_n)$ to \textsc{Quad}.
        \end{compactenum}
    \end{compactenum}
\end{compactenum}
Importantly, the pre-processing phase of \textsc{Squad} exists solely for ensuring that the proofs forwarded to \textsc{Quad} are of constant size.
Hence, the structure of \textsc{Squad} is similar to the structure of our general algorithm.
Indeed, our Byzantine consensus algorithm with \emph{Interactive-Consistency Validity} could be modified (in the same way as the pre-processing phase of \textsc{Squad}) to allow constant-sized proofs in the case of \emph{Strong Validity}.

\paragraph{Weak Validity}
\emph{Weak Validity} says that, if all processes are correct and propose the same value, only that value can be decided.
As \emph{Weak Validity} is non-trivial, it cannot be solved with $n \leq 3t$ (by \Cref{theorem:triviality_main}).
Note that \textsc{Quad}~\cite{civit2022byzantine}, a Byzantine consensus algorithm with \emph{Weak Validity}, achieves $O(n^2)$ message and communication complexities.
However, until now, it was not known what the lower bound on message and communication complexities was for Byzantine consensus algorithm with \emph{Weak Validity}.
As we show, the lower bound are $\Omega(t^2)$, which further proves that \textsc{Quad} is indeed optimal (as $t = O(n)$ in \textsc{Quad}).

\paragraph{From-Correct Validity}
Thus far, we have not mentioned \emph{From-Correct Validity}.
\begin{compactitem}
    \item \emph{From-Correct Validity:} If a correct process decides a value $v$, then $v$ was proposed by a correct process.
\end{compactitem}
This validity property was used to define the \emph{strong consensus} problem~\cite{fitzi2003efficient}.

In their paper~\cite{fitzi2003efficient}, Fitzi and Garay show that Byzantine consensus algorithm with \emph{From-Correct Validity} is exists if and only if $n > (|\mathcal{D}| + 1)t$, where $\mathcal{D} = |\mathcal{V}_I|$.
We now show the same result using our formalism.

\begin{theorem} [new proof]
Solving the Byzantine consensus problem with \emph{From-Correct Validity} is possible if and only if $n > (d + 1)t$, where $d = |\mathcal{V}_I| = |\mathcal{V}_O|$.
\end{theorem}
\begin{proof}
First, we show that, if $n \leq (d + 1)t$, it is impossible to solve the Byzantine consensus problem with \emph{From-Correct Validity}.
By contradiction, suppose that it is possible to solve the Byzantine consensus problem with \emph{From-Correct Validity} with $n \leq (d + 1)t$.
Let $\mathit{base} \in \mathcal{I}$ be an input configuration such that (1) $|\mathit{base}| = n - t$, and (2) no proposal $v \in \mathcal{V}_I$ appears with more than $t$ processes in $\mathit{base}$; note that we can construct $\mathit{base}$ as $n - t \leq dt$.
For every value $v \in \mathcal{V}_I$, we construct an input configuration $c_v \in \mathcal{I}$ in the following way:
\begin{compactenum}
    \item Let $c_v \gets \mathit{base}$.

    \item We remove from $c_v$ all process-proposal pairs $\mathit{pp}$ with $\mathsf{proposal}(\mathit{pp}) = v$.

    \item For every process $P \notin \processes{\mathit{base}}$, we add $(P, v')$ to $c_v$, where $v' \neq v$.
\end{compactenum}
For every input configuration $c_v$, (1) $c_v \sim \mathit{base}$, and (2) $\text{\emph{From-Correct Validity}}(c_v) = \mathcal{V}_O \setminus{\{v\}}$.
Hence, \emph{From-Correct Validity} does not satisfy $\mathcal{C}_S$, which contradicts \Cref{theorem:similarity_condition_necessary}.
Thus, it is impossible that $n \leq (d + 1)t$.
\end{proof}

\subsection{On External Validity}


==> sections/byzantine.tex <==
   \section{Validity Properties in the Byzantine Failure Model}

In this section, we investigate the validity properties of the consensus problem in the Byzantine failure model.

\subsection{Preliminaries}

\paragraph{System model.}
We consider a static system $\Psi = \{P_1, ..., P_n\}$ of $n$ processes among which $f < n$ processes can be Byzantine.
If a process is Byzantine, the process is \emph{faulty}; otherwise, the process is \emph{correct}.

\paragraph{Byzantine consensus.}
Each process has its \emph{proposal}, and it should eventually \emph{decide}.
We denote by $\mathcal{V}$ the set of values a process can propose and decide.
The consensus problem in the Byzantine failure model requires the following three properties to hold:
\begin{compactitem}
    \item \emph{Agreement:} No two correct processes decide different values.
    
    \item \emph{Termination:} Every correct process eventually decides.
    
    \item \emph{Validity}
\end{compactitem}

\paragraph{Validity property.}
First, we define a \emph{process-proposal} pair as a pair $(P_x, \mathit{val}_x)$, where (1) $P_x \in \Psi$, and (2) $\mathit{val}_x \in \mathcal{V}$ is a value.
Intuitively, $(P, \mathit{val})$ denotes that a \emph{correct} process $P \in \Psi$ has proposed a value $\mathit{val} \in \mathcal{V}$.
We denote by $\mathit{pp}.\mathsf{process}$ the process associated with a process-proposal $\mathit{pp}$, whereas $\mathit{pp}.\mathsf{proposal}$ denotes the proposal associated with $\mathit{pp}$.

Next, an \emph{input configuration} is a tuple $\big[ \mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_x \big]$, where (1) $\mathit{pp}_i$ is a process-proposal, for every $i \in [1, x]$, (2) $x \geq n - f$, and (3) every process-proposal pair is associated with a distinct process.
We denote by $\mathcal{I}$ the set of all possible input configurations.
For every input configuration $\mathit{input} \in \mathcal{I}$ and every $i \in [1, n]$, we denote by $\mathit{input}[i]$ the process-proposal pair associated with process $P_i$; if such process-proposal does not exist, $\mathit{input}[i] = \bot$.
% Furthermore, $\mathit{correct}(\mathit{input} \in \mathcal{I}) = \{P \,|\, (P, *) \text{ belongs to } \mathit{input}\}$ denotes the set of correct processes as established by $\mathit{input}$.
% Lastly, we define $\mathit{identical\_proposals}: \mathcal{I} \times \mathcal{I} \to \{\mathit{false}, \mathit{true}\}$ such that $\mathit{identical\_proposals}(i_1 \in \mathcal{I}, i_2 \in \mathcal{I}) = \top$ if and only if every process is associated with the same proposal in both $i_1$ and $i_2$.

By slightly abusing the notation, for any two input configurations $i_1, i_2 \in \mathcal{I}$, we define $i_1 \subseteq i_2$ in the following manner:
\begin{equation*}
    i_1 \subseteq i_2 \iff \forall j \in [1, n]: i_1[j] \neq \bot \implies i_2[j] = i_1[j].
\end{equation*}
In other words, $i_1 \subseteq i_2$ if and only if, the set that corresponds to the input configuration $i_1$ is a subset of the set that corresponds to the input configuration $i_2$.

We define a \emph{validity property} $\mathit{val}$ as a function $\mathcal{I} \to 2^{\mathcal{V}}$ such that, for every $\mathit{input} \in \mathcal{I}$, $\mathit{val}(\mathit{input}) \neq \emptyset$.
Finally, we say that a Byzantine consensus algorithm $\mathcal{A}_B$ satisfies a validity property $\mathit{val}$ if and only if the following holds:
\begin{compactitem}
    \item \emph{Validity safety:} In every execution $e$ of $\mathcal{A}_B$, $\mathit{dec}_e \in \mathit{val}(\mathit{input})$, where (1) $\mathit{dec}_e$ is the decided value in $e$, and (2) $\mathit{input}$ is the input configuration that corresponds to $e$.
    
    \item \emph{Validity liveness:} For every input configuration $\mathit{input} \in \mathcal{I}$ and every value $v \in \mathit{val}(\mathit{input})$, there exists an execution $e$ of $\mathcal{A}_B$ such that (1) $e$ corresponds to $\mathit{input}$, and (2) the decided value in $e$ is $v$.
\end{compactitem}

\subsection{Synchronous Environments}

First, we investigate validity properties of Byzantine consensus in a synchronous setting.

\paragraph{Communication.}
In a synchronous environment, there exists an upper bound $\Delta$ on message delays between processes.
In other words, if a correct process sends a message to another correct process at time $t$, the message will be received by time $t + \Delta$; note that the message might be received at time $t^* \in [t, t + \Delta]$ (the actual message delay for each message is chosen by the adversary).

\paragraph{Necessary conditions.}
We start by introducing the \emph{Byzantine containment condition}.

\begin{definition} [Byzantine containment condition] \label{definition:Byzantine_containment}
Let $\mathit{val}$ be a validity property.
We say that $\mathit{val}$ satisfies the \emph{Byzantine containment condition} if and only if the following holds:
\begin{equation*}
    \forall i_1, i_2 \in \mathcal{I}: i_1 \subseteq i_2 \implies \mathit{val}(i_2) \subseteq \mathit{val}(i_1).
\end{equation*}
\end{definition}

We now show that the Byzantine containment condition (\Cref{definition:Byzantine_containment}) is necessary for a validity property to be satisfiable in a Byzantine environment.

\begin{lemma} [Byzantine containment condition is necessary] \label{lemma:byzantine_containment_necessary}
Let $\mathit{val}$ be a validity property that does not satisfy the Byzantine containment condition.
No algorithm (even if synchronous) solves the Byzantine consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the Byzantine containment condition, there exist two input configuration $i_1, i_2 \in \mathcal{I}$ such that (1) $i_1 \subseteq i_2$, and (2) $\mathit{val}(i_2) \not\subseteq \mathit{val}(i_1)$.
In other words, there exists a value $x \in \mathcal{V}$ such that $x \in \mathit{val}(i_2)$ and $x \notin \mathit{val}(i_1)$.

By contradiction, suppose that there exists a Byzantine algorithm $\mathcal{A}_B$ that satisfies $\mathit{val}$.
Without loss of generality, let $\mathcal{A}_B$ be a synchronous algorithm.

Since $\mathcal{A}_B$ satisfies $\mathit{val}$, there exists an execution $e$ of $\mathcal{A}_B$ that corresponds to the input configuration $i_2$ in which the decided value is $x$ (due to the validity liveness).
We now create an execution $e'$ such that (1) $e'$ corresponds to $i_1$, and (2) the decided value in $e'$ is $x \notin \mathit{val}(i_1)$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item After the first correct process decides in $e'$, we crash all processes which are correct according to $i_2$ and faulty according to $i_1$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $x \notin \mathit{val}(i_1)$, which means that $\mathcal{A}_B$ does not satisfy $\mathit{val}$ in $e'$.
This contradicts the fact that $\mathcal{A}_B$ satisfies $\mathit{val}$, which concludes the lemma.
\end{proof}

\paragraph{Sufficient conditions.}
We now show that the Byzantine containment condition is sufficient for a validity property to be satisfiable in a Byzantine setting.

\begin{theorem} [Byzantine containment condition is sufficient]
Let $\mathit{val}$ be a validity property that satisfies the Byzantine containment condition.
There exists an algorithm that solves the Byzantine consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a synchronous Byzantine-tolerant algorithm $\mathcal{A}_B$ that solves $\mathit{val}$.

Before devising $\mathcal{A}_B$, we are implementing a synchronous Byzantine-tolerant consensus algorithm $\mathcal{A}_{\mathit{correct}}$ in which processes agree on an input configuration.
Specifically, $\mathcal{A}_{\mathit{correct}}$ satisfies the following validity property:
\begin{compactitem}
    \item \emph{All-correct validity:} Let the decided value be $i = \big[ (P_{i_1}, v_{i_1}), (P_{i_2}, v_{i_2}), ..., (P_{i_x}, v_{i_x}) \big]$.
    Then, for every correct process $P_x$, $(P_x, v_x)$ belongs to $i$, where $v_x$ is the proposed value by $P_x$.
\end{compactitem}
Intuitively, $\mathcal{A}_{\mathit{correct}}$ allows correct processes to agree on the input configuration that contains \emph{all} process-proposals associated with correct processes.

\begin{algorithm}
\caption{Byzantine-tolerant algorithm $\mathcal{A}_{\mathit{correct}}$ that solves consensus with all-correct validity: Pseudocode for process $P_i$}
\label{algorithm:a_correct}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Synchronous Byzantine Reliable Broadcast, \textbf{instance} $\mathit{brb}$

\medskip
\State \textbf{At time $0$:}
\State \hskip2em \textbf{trigger} $\langle \mathit{brb}, \mathsf{broadcast}([\textsc{proposal}, \mathit{proposal}]) \rangle$

\medskip
\LineComment{$\mathit{brb}$ is implemented using synchronous HotStuff protocol accompanied by the certification phase given in the DISC submission}
\State \textbf{At time $8(f + 1)\Delta + 3\Delta$:} \label{line:decide_all_correct}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\text{the input configuration built out of all delivered \textsc{proposal} messages})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_{\mathit{correct}}$ (\Cref{algorithm:a_correct}) solves the Byzantine consensus problem with all-correct validity:
\begin{compactitem}
    \item Termination: Termination holds as every correct process decides at time $8(f + 1)\Delta + 3\Delta$ (line~\ref{line:decide_all_correct}).
    
    \item Agreement: Agreement follows from the agreement property of $\mathit{brb}$ and the fact that, if a correct process delivers a message from $\mathit{brb}$, it does so by time $8(f + 1)\Delta + 3\Delta$.
    
    \item All-correct validity: Follows from the validity property of $\mathit{brb}$ and the fact that a message $\mathit{brb}$-broadcast by a correct process is $\mathit{brb}$-delivered by time $8(f + 1)\Delta + 3\Delta$.
\end{compactitem}

Finally, we are ready to present $\mathcal{A}_B$.

\begin{algorithm}
\caption{Byzantine-tolerant algorithm $\mathcal{A}_B$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:synchronous_byzantine}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Synchronous Byzantine-Tolerant Consensus with All-Correct Validity, \textbf{instance} $\mathcal{A}_{\mathit{correct}}$
\State \hskip2em Synchronous Byzantine-Tolerant Consensu with External Validity, \textbf{instance} $c$

\medskip
\State \textbf{At time $0$:}
\State \hskip2em \textbf{trigger} $\langle \mathcal{A}_{\mathit{correct}}, \mathsf{propose}(\mathit{proposal}) \rangle$

\medskip
\State \textbf{upon} $\langle \mathcal{A}_{\mathit{correct}}, \mathsf{decide}(i) \rangle$:
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \text{a value from } \mathit{val}(i)$
\State \hskip2em \(\triangleright\) values which are valid for $c$ are all the values from $\mathit{val}(i)$
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$
\end{algorithmic}
\end{algorithm}

Termination of $\mathcal{A}_B$ follows from termination of $\mathcal{A}_{\mathit{correct}}$ and $c$.
Furthermore, agreement of $\mathcal{A}_B$ follows from agreement of $c$.
Hence, we need to prove the validity property of $\mathcal{A}_B$.

Fix an input configuration $\mathit{input}$.
Since all correct processes agree in $\mathcal{A}_{\mathit{correct}}$ on an input configuration $i$, all correct processes agree on the set of valid values in $c$.
Hence, the decided value $v \in \mathit{val}(i)$.
Moreover, we have that $\mathit{input} \subseteq i$ (due to the all-correct validity of $\mathcal{A}_{\mathit{correct}}$).
Thus, $v \in \mathit{val}(\mathit{input})$ (since $\mathit{val}$ satisfies the Byzantine containment condition), and the validity safety property is ensured.

As for the validity liveness, we can easily modify $\mathcal{A}_{\mathit{correct}}$ to take into account the exact time of decision.
Then, as done before, we can map the time into a specific value from $\mathit{val}(i)$.
Therefore, validity liveness is (i.e., can be) ensured by $\mathcal{A}_B$, which concludes the theorem.
\end{proof}

\subsection{Partially Synchronous Environments}

Next, we investigate validity properties of Byzantine consensus in a partially synchronous setting.

\paragraph{Communication.}
In a partially synchronous environment, there exists an unknown time Global Stabilization Time (GST) such that the system behaves asynchronously before GST, and behaves synchronously after GST.
Formally, there exist a known upper bound $\delta$ on message delays after GST.

\paragraph{Necessary conditions.}
First, note that the Byzantine containment condition is necessary for a validity property to be satisfied in a partially synchronous environment (as this condition is necessary in a synchronous setting).
We now define when an input configuration is ``Byzantine-correct-similar'' to another configuration.
Formally, for every input configuration $\mathit{input} \in \mathcal{I}$, we define $\mathit{ByzSim}(\mathit{input})$ in the following manner:
\begin{equation*}
    \mathit{ByzSim}(\mathit{input}) = \{i' \in \mathcal{I} \,|\, \forall j \in [1, n]: \mathit{input}[j] \neq \bot \land i'[j] \neq \bot \implies \mathit{input}[j] = i'[j]\}.
\end{equation*}
In other words, an input configuration $i' \in \mathcal{I}$ is \emph{Byzantine-correct-similar} to $\mathit{input}$ if all processes which belong to both $\mathit{input}$ and $i'$ propose the same values in both input configurations.

Next, we introduce the \emph{Byzantine-correct-similarity condition}.

\begin{definition} [Byzantine-correct-similarity condition] \label{definition:f+1_similarity}
Let $\mathit{val}$ be a validity property.
% Let $\mathit{input} \in \mathcal{I}$ be an input configuration.
% We define $\mathit{AlmostSim}(\mathit{input}) = \{\mathit{input}' \in \mathcal{I} \,|\, \text{proposed values of processes correct according to } i \text{ are identical}\}$.
We say that $\mathit{val}$ satisfies the \emph{Byzantine-correct-similarity condition} if and only if the following holds:
\begin{equation*}
    \forall \mathit{input} \in \mathcal{I}: \bigcap\limits_{i' \in \mathit{ByzSim}(\mathit{input})} \big(\mathit{val}(i')\big) \neq \emptyset.
\end{equation*}
\end{definition}

We now show that the Byzantine-correct-similarity condition is necessary in a partially synchronous setting.

\begin{lemma} [Byzantine-correct-similarity condition is necessary] \label{lemma:f+1_similarity_necessary}
Let $\mathit{val}$ be a validity property that does not satisfy the Byzantine-correct-similarity condition.
No partially synchronous algorithm solves the Byzantine consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the Byzantine-correct-similarity condition, there exists an input configuration $i \in \mathcal{I}$ such that $\bigcap\limits_{i' \in \mathit{ByzSim}(i)} \big( \mathit{val}(i') \big) = \emptyset$ (by \Cref{definition:f+1_similarity}).
By contradiction, suppose that there exists a partially synchronous Byzantine consensus algorithm $\mathcal{A}_B$ that satisfies $\mathit{val}$.

Consider an execution $e$ of $\mathcal{A}_B$ that corresponds to $i$ (i.e., all processes propose the values as established by $i$, and $i$ establishes which processes are correct and which are faulty) such that all faulty processes in $e$ crash immediately (without sending any message); observe that there might be no faulty processes in $e$ (according to $i$).
Let the decided value in $e$ be $\mathit{dec}_e$.
Importantly, there exists an input configuration $i' \in \mathit{ByzSim}(i)$ such that $\mathit{dec}_e \notin \mathit{val}(i')$ (otherwise, the Byzantine-correct-similarity condition would be satisfied for $i$).

Now, we create an execution $e'$ of $\mathcal{A}_B$ such that (1) $e'$ corresponds to $i'$, and (2) the decided value in $e'$ is $\mathit{dec}_e \notin \mathit{val}(i')$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item No process correct in both $e$ and $e'$ (there exist at least $f + 1$ such processes) hears from any process $P \in \Psi$ in $e'$ until a value is decided in $e'$, where $P$ is faulty in $e$ (i.e., according to $i$) and correct in $e'$ (i.e., correct according to $i'$).
    
    \item After a decision has been made in $e'$, we crash all processes which are faulty according to $i'$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $\mathit{dec}_e \notin \mathit{val}(i')$, which means that $\mathcal{A}_B$ does not satisfy the validity property in the execution $e'$ (as the validity safety property is not satisfied).
This contradicts the fact that $\mathcal{A}_B$ satisfies the validity property $\mathit{val}$, which concludes the lemma.
\end{proof}

\paragraph{Sufficient conditions.}
Finally, we are ready to show that Byzantine containment and Byzantine-correct-similarity conditions are sufficient for a validity property to be satisfiable in a partially synchronous setting.

\begin{theorem} [Byzantine containment and Byzantine-correct-similarity conditions are sufficient in partial synchrony]
Let $\mathit{val}$ be a validity property that satisfies Byzantine containment and Byzantine-correct-similarity conditions.
There exists a partially synchronous algorithm that solves the Byzantine consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a partially synchronous Byzantine consensus algorithm $\mathcal{A}_B$ (\Cref{algorithm:partially_synchronous_byzantine}) that solves consensus with $\mathit{val}$.

\begin{algorithm}
\caption{Partially synchronous Byzantine algorithm $\mathcal{A}_B$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:partially_synchronous_byzantine}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Partially Synchronous Byzantine Consensus with External Validity, \textbf{instance} $c$
\State \hskip2em Byzantine Consistent Broadcast, \textbf{instance} $\mathit{bcb}$

\medskip
\State \textbf{upon} $\mathsf{start}$:
\State \hskip2em \textbf{trigger} $\langle \mathit{bcb}, \mathsf{broadcast}\big([\textsc{proposal}, \mathit{proposal}]\big) \rangle$

\medskip
\State \textbf{upon} delivery of $n - f$ \textsc{proposal} messages:
\State \hskip2em \textbf{trigger} timer for $\Delta$ time \Comment{$\Delta$ is some predefined constant}

\medskip
\State \textbf{upon} timer elapsed:
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
\State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:partially_build_i_byzantine}
\State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
\State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
\State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
\State \hskip2em \textbf{else:} 
\State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{ByzSim}(i)$ \label{line:partially_set_to_propose}

\State \hskip2em \(\triangleright\) all values are associated with received \textsc{proposal} messages which proves the validity of the proposed values
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:partially_propose_c_byzantine}

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_B$ (\Cref{algorithm:partially_synchronous_byzantine}) solves the Byzantine consensus problem with $\mathit{val}$.
First, termination and agreement follow directly from termination and agreement of a used partially synchronous Byzantine consensus (instance $c$ in \Cref{algorithm:partially_synchronous_byzantine}).
Hence, it is left to show that $\mathcal{A}_B$ satisfies $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \mathcal{I}$.
We first show that $\mathcal{A}_B$ satisfies the validity safety.
Let $P$ be a process that proposes to $c$ (at line~\ref{line:partially_propose_c_byzantine}) and let $i$ be the input configuration that corresponds to messages $P$ accompanies its proposal by.
We have the following: $i \in \mathit{ByzSim}(\mathit{input})$.
% ; observe that, if $P$ does not receive \textsc{proposal} messages from all processes, $i$ is not, strictly speaking, an input configuration.
% We ``extend'' $i$ by adding process-proposals associated with processes from which $P$ has not heard, i.e., for every $P' \in \Psi$ from which $P$ has not received a \textsc{proposal} message, we add $(\bar{P}', \text{any value})$ to $i$.
% Importantly, $\mathit{input} \in \mathit{CorrectSim}(i)$.
Hence, the proposed value must belong to $\mathit{val}(\mathit{input})$.
% Hence, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$.
Therefore, for every value $v$ proposed to the black-box partially synchronous Byzantine consensus $c$, $v \in \mathit{val}(\mathit{input})$.
Given that $c$ decides only values accompanied with \textsc{proposal} messages, the decided value must belong to $\mathit{val}(\mathit{input})$.
Thus, the validity safety is satisfied by \Cref{algorithm:partially_synchronous_byzantine}.

It is left to show that the validity liveness is satisfied.
In order to solve the validity liveness, $\mathcal{A}_B$ relies on time.
We assume that the time maps to a value in the same way at all processes.

Again, let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
We need to show that, for every value $v \in \mathit{val}(\mathit{input})$, there exists an execution that corresponds to $\mathit{input}$ in which the decided value is $v$.
Hence, let us fix a value $v \in \mathit{val}(\mathit{input})$.
We construct an execution $e$ that corresponds to $\mathit{input}$ in which the decided value is $v$:
\begin{compactenum}
    \item All correct processes propose their values according to $\mathit{input}$.
    All Byzantine processes immediately announce themselves by broadcasting ``I am Byzantine'' to all processes.
    
    \item The first \textsc{proposal} message at each process is received at the \emph{exactly} the same time that maps to $v$.
    
    \item Every correct process receives messages from all correct processes before proposing to $c$.
\end{compactenum}
Hence, all correct processes build $\mathit{input}$ at line~\ref{line:partially_build_i_byzantine}.
Thus, all processes propose $v$ to $c$, which means $v$ is decided.
Let us underline that, in this case, the attack exploited in \Cref{lemma:f+1_similarity_necessary} cannot be used, which means that the execution preserves the safety violation (since $\mathit{val}$ satisfies the Byzantine containment property).
The theorem holds.
\end{proof}

==> sections/classification.tex <==
% \newpage
\section{Necessary solvability conditions}  \label{section:classification}

This section gives the necessary conditions for the solvability of validity properties. 
We start by focusing on the case of $n \leq 3t$: we prove that, if $n \leq 3t$, all solvable validity properties are trivial (\Cref{subsection:triviality_main}).
Then, we consider the case of $n > 3t$: we define the similarity condition, and prove its necessity for solvability (\Cref{subsection:necessary_condition}).

\subsection{Triviality of Solvable Validity Properties if $n \leq 3t$} \label{subsection:triviality_main}

%\manuel{It is doubtful whether we should include the next couple of sentences before the last.}
Some validity properties, such as \emph{Weak Validity} and \emph{Strong Validity}, are known to be unsolvable with $n \leq 3t$~\cite{DLS88,PeaseSL80}.
%\pierre{I would write Weak Validity (and maybe for Binary Consensus) to stress the fact that the result is known for quite weak validity properties, but we clarify the fact that there does not exists a super weak validity property that circumvents the $n/3$-bound}.
This seems to imply a split of validity properties depending on the resilience threshold.
We prove that such a split indeed exists for $n \leq 3t$, and, importantly, that it applies to \emph{all} solvable validity properties.
Implicitly, this means that there is no ``useful'' relaxation of the validity property that can tolerate $t \geq \lceil n / 3 \rceil$ failures.
Concretely, we prove the following theorem:

\begin{theorem} \label{theorem:triviality_main}
% Let $n$ denote the total number of processes, and $t$ the number of tolerated failures.
If a validity property is solvable with $n \leq 3t$, then the validity property is trivial, i.e., there exists a value $v' \in \mathcal{V}_O$ such that $v' \in \bigcap\limits_{c \in \mathcal{I}} \mathit{val}(c)$.
\end{theorem}

% Concretely, if $n \leq 3t$, all solvable validity properties are trivial (require no communication).
% % and can be solved without any communication.
% Let us start by formally defining the notion of a trivial validity property.

% \begin{definition} [Trivial validity property] \label{definition:trivial_validity}
% We say that a validity property $\mathit{val}$ is \emph{trivial} if and only if there exists a value $v' \in \mathcal{V}_O$ such that $v' \in \bigcap\limits_{c \in \mathcal{I}} \mathit{val}(c)$.
% \end{definition}

% Observe that the Byzantine consensus problem with a trivial validity property can be solved without any communication: processes decide the same always-admissible value.
% This subsection proves the following theorem:



Before presenting the proof of the theorem, we introduce the \emph{compatibility relation} between input configurations, which we use throughout this subsection.
% notion of \emph{compatible} input configurations.

\paragraph{Compatibility.}
We define the compatibility relation (``$\diamond$'') between input configurations:
\begin{equation*}
    \forall c_1, c_2 \in \allconfigurations: c_1 \diamond c_2 \iff \big(|\processes{c_1} \cap \processes{c_2}| \leq t\big) \land \big(\exists P \in \processes{c_1} \setminus{\processes{c_2}}\big) \land \big(\exists Q \in \processes{c_2} \setminus{\processes{c_1}}\big).
\end{equation*}

That is, $c_1$ is compatible with $c_2$ if and only if (1) there are at most $t$ processes in common, (2) there exists a process which belongs to $c_1$ and does not belong to $c_2$, and (3) there exists a process which belongs to $c_2$ and does not belong to $c_1$.
For example, when $n = 3$ and $t = 1$, $c = \big[ (P_1, 0), (P_2, 0) \big]$ is compatible with $\big[ (P_1, 1), (P_3, 1) \big]$, whereas $c$ is not compatible with $\big[ (P_1, 1), (P_2, 1), (P_3, 1) \big]$.
Observe that the compatibility relation is symmetric and irreflexive.
% Note that any trivial validity property satisfies $\mathcal{C}_S$: for every input configuration $c \in \mathcal{I}$, $\lambda(c)$ is defined as an always-admissible value.
% Moreover, the Byzantine consensus problem with a trivial validity property can be solved with no communication: processes immediately decide the same always-admissible value.

\paragraph{Proof of \Cref{theorem:triviality_main}.}
Throughout the rest of the subsection, we fix any validity property $\mathit{val}$ which is solvable with $n \leq 3t$; our aim is to prove the triviality of $\mathit{val}$.
Moreover:
\begin{compactitem}
    \item We assume that $n \leq 3t$.

    \item We fix any algorithm $\mathcal{A}$ which solves consensus with $\mathit{val}$.

    \item We fix any input configuration $\mathit{base} \in \mathcal{I}_{n - t}$ with exactly $n - t$ process-proposal pairs.

    \item We fix any infinite canonical execution $\mathcal{E}_{\mathit{base}} \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}_{\mathit{base}}) = \mathit{base}$.
    As $\mathcal{A}$ satisfies \emph{Termination} and $\mathit{val}$, and $\mathcal{E}_{\mathit{base}}$ is infinite, some value $v_{\mathit{base}} \in \mathit{val}(\mathit{base})$ is decided by a correct process in $\mathcal{E}_{\mathit{base}}$.
\end{compactitem}

%In our proof, we rely on a partitioning argument~\cite{LSP82}, as well as on canonical similarity (\Cref{subsection:intermediate_results}).

% Our proof works as follows:
% \begin{compactenum}
%     \item By applying the partitioning argument~\cite{LSP82}, we show that, in any canonical execution which corresponds to an input configuration compatible with $\mathit{base}$, $v_{\mathit{base}}$ must be decided.
    
%     \item We show that, for every input configuration with $n$ process-proposal pairs (i.e., every process is correct), there exists an execution in which $v_{\mathit{base}}$ is decided.
    
%     \item Finally, by ``removing'' process-proposal pairs from input configurations with $n$ process-proposal, we show that, for every input configuration $c$, $v_{\mathit{base}}$ is decided in (at least) one execution which corresponds to $c$.
% \end{compactenum}
% Recall that an input configuration $c_1 \in \mathcal{I}$ is compatible with an input configuration $c_2 \in \mathcal{I}$ (we write ``$c_1 \diamond c_2$'') if and only if (1) there are at most $t$ processes in common, (2) there exists a process which belongs to $c_1$ and does not belong to $c_2$, and (3) there exists a process which belongs to $c_2$ and does not belong to $c_1$.

First, we show that only $v_{\mathit{base}}$ can be decided in any canonical execution which corresponds to any input configuration compatible with $\mathit{base}$.
If a value different from $v_{\mathit{base}}$ is decided, we can apply the classical partitioning argument~\cite{LSP82}: the adversary causes a disagreement by partitioning processes into two disagreeing groups.

\begin{lemma} \label{lemma:triviality_compatible}
Let $c \in \mathcal{I}$ be any input configuration such that $c \diamond \mathit{base}$.
Let $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ be any (potentially infinite) canonical execution such that $\mathsf{input\_conf}(\mathcal{E}_c) = c$.
If a value $v_c \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_c$, then $v_c = v_{\mathit{base}}$.
\end{lemma}
\begin{proof}
By contradiction, suppose that some value $v_c \neq v_{\mathit{base}}$ is decided by a correct process in $\mathcal{E}_c$.
Since $c \diamond \mathit{base}$, there exists a process $Q \in \processes{c}\setminus{\processes{\mathit{base}}}$.
If $\mathcal{E}_c$ is infinite, let $\mathcal{E}_c^Q \gets \mathcal{E}_c$.
Otherwise, let $\mathcal{E}_c^Q$ be an infinite canonical continuation of $\mathcal{E}_c$.
The following holds for process $Q$: (1) $Q$ decides $v_c$ in $\mathcal{E}_c^Q$ (as $\mathcal{A}$ satisfies \emph{Agreement} and \emph{Termination}), and (2) $Q$ is silent in $\mathcal{E}_{\mathit{base}}$.
Let $t_Q$ denote the time at which $Q$ decides in $\mathcal{E}_c^Q$.
Similarly, there exists a process $P \in \processes{\mathit{base}} \setminus{\processes{c}}$; note that (1) $P$ decides $v_{\mathit{base}}$ in $\mathcal{E}_{\mathit{base}}$, and (2) $P$ is silent in $\mathcal{E}_c^Q$.
Let $t_P$ denote the time at which $P$ decides in $\mathcal{E}_{\mathit{base}}$.

In the next step, we construct an execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ by ``merging'' $\mathcal{E}_{\mathit{base}}$ and $\mathcal{E}_c^Q$:
\begin{compactenum}
    \item We separate processes into 4 groups: (1) group $A = \pi(\mathit{base}) \setminus{\pi(c)}$, (2) group $B = \pi(\mathit{base}) \cap \pi(c)$, (3) group $C = \pi(c) \setminus{\pi(\mathit{base})}$, and (4) group $D = \Pi \setminus{(A \cup B \cup C)}$.

    \item Processes in $B$ behave towards processes in $A$ as in $\mathcal{E}_{\mathit{base}}$, and towards processes in $C$ as in $\mathcal{E}_c^Q$.

    \item Communication between groups $A$ and $C$ is delayed until after time $\max(t_P, t_Q)$.

    \item Processes in group $D$ ``wake up'' at time $T_D > \max(t_P,t_Q)$ (with any proposals), and behave correctly throughout the entire execution.
    % $P$ has decided $v_{\mathit{base}}$ and $Q$ has decided $v_c$. 
    
    \item We set GST to after $T_D$.
\end{compactenum}
The following holds for $\mathcal{E}$:
\begin{compactitem}
    \item Processes in $\Pi \setminus{B}$ are correct in $\mathcal{E}$.
    In other words, only processes in $B$ are faulty in $\mathcal{E}$.
    Recall that $|B| \leq t$ as $\mathit{base} \diamond c$.

    \item Process $Q$, which is correct in $\mathcal{E}$, cannot distinguish $\mathcal{E}$ from $\mathcal{E}_c^Q$ until after time $\max(t_P, t_Q)$.
    % in which it decides $v_c$.
    Hence, process $Q$ decides $v_c$ in $\mathcal{E}$.

    \item Process $P$, which is correct in $\mathcal{E}$, cannot distinguish $\mathcal{E}$ from $\mathcal{E}_{\mathit{base}}$ until after time $\max(t_P, t_Q)$.
    % in which it decides $v_{\mathit{base}}$.
    Hence, process $P$ decides $v_{\mathit{base}} \neq v_c$ in $\mathcal{E}$.
\end{compactitem}
Therefore, we reach a contradiction with the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Thus, $v_c = v_{\mathit{base}}$.
\end{proof}


\iffalse
\begin{sketch}
By contradiction, suppose that some value $v_c \neq v_{\mathit{base}}$ is decided by a correct process in $\mathcal{E}_c$.
Since $c \diamond \mathit{base}$, there exists a correct process $Q \in \processes{c}\setminus{\processes{\mathit{base}}}$; note that (1) process $Q$ decides $v_c$ in $\mathcal{E}_c$ (as $\mathcal{A}$ satisfies \emph{Termination} and \emph{Agreement}), and (2) process $Q$ is silent in $\mathcal{E}_{\mathit{base}}$.
Similarly, there exists a process $P \in \processes{\mathit{base}} \setminus{\processes{c}}$; observe that (1) process $P$ decides $v_{\mathit{base}}$ in $\mathcal{E}_{\mathit{base}}$, and (2) process $P$ is silent in $\mathcal{E}_c$.

In order to prove the lemma, we construct an execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ by ``merging'' $\mathcal{E}_{\mathit{base}}$ and $\mathcal{E}_c$:
\begin{compactenum}
    \item Processes in $\processes{c} \cap \processes{\mathit{base}}$ behave (1) towards processes in $\processes{\mathit{base}} \setminus{\processes{c}}$ as in $\mathcal{E}_{\mathit{base}}$, and (2) towards processes in $\processes{c} \setminus{\processes{\mathit{base}}}$ as in $\mathcal{E}_c$.

    \item Communication between (1) processes in $\processes{\mathit{base}} \setminus{\processes{c}}$ and (2) processes in $\processes{c} \setminus{\processes{\mathit{base}}}$ is delayed.
\end{compactenum}
The following holds for $\mathcal{E}$:
\begin{compactitem}
    \item Processes in $\processes{\mathit{base}} \ominus \processes{c}$ (symmetric difference) are correct in $\mathcal{E}$.

    \item Only processes in $\processes{\mathit{base}} \cap \processes{c}$ are faulty in $\mathcal{E}$.
    Recall that $|\processes{\mathit{base}} \cap \processes{c}| \leq t$ as $\mathit{base} \diamond c$.

    \item Process $Q$, which is correct in $\mathcal{E}$, cannot distinguish $\mathcal{E}$ from $\mathcal{E}_c$.
    Hence, process $Q$ decides $v_c$ in $\mathcal{E}$.

    \item Process $P$, which is correct in $\mathcal{E}$, cannot distinguish $\mathcal{E}$ from $\mathcal{E}_{\mathit{base}}$.
    Hence, process $P$ decides $v_{\mathit{base}} \neq v_c$ in $\mathcal{E}$.
\end{compactitem}
Therefore, \emph{Agreement} is violated in $\mathcal{E}$, which contradicts the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Thus, $v_c = v_{\mathit{base}}$.
\end{sketch}
\fi

Observe that the proposals of an input configuration compatible with $\mathit{base}$ do not influence the decision: given an input configuration $c \in \mathcal{I}$, $c \diamond \mathit{base}$, only $v_{\mathit{base}}$ can be decided in any canonical execution which corresponds to $c$, \emph{irrespectively} of the proposals.

Next, we prove a direct consequence of \Cref{lemma:triviality_compatible}: for every input configuration $c_n \in \mathcal{I}_n$, there exists an infinite execution $\mathcal{E}_{n}$ such that (1) $\mathcal{E}_{n}$ corresponds to $c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_{n}$.
% Below, we give a proof sketch of the claim; the formal proof can be found in \Cref{section:triviality_appendix}.

% The results follows directly from \Cref{lemma:triviality_compatible}.

\begin{lemma} \label{lemma:triviality_complete}
For any input configuration $c_n \in \mathcal{I}_n$, there exists an infinite execution $\mathcal{E}_{n} \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_{n}) = c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_{n}$.
\end{lemma}
\begin{proof}
Fix any input configuration $c_n \in \mathcal{I}_n$.
We construct an input configuration $c_{n - t} \in \mathcal{I}_{n - t}$:
\begin{compactenum}
    \item For every process $P_i \notin \processes{\mathit{base}}$, we include a process-proposal pair $(P_i, v)$ in $c_{n - t}$ such that $v = \mathsf{proposal}(c_n[i])$.
    Note that there are $t$ such processes as $|\processes{\mathit{base}}| = n - t$.

    \item We include any $n - 2t$ process-proposal pairs $(P_i, v)$ in $c_{n - t}$ such that (1) $P_i \in \processes{\mathit{base}}$, and (2) $v = \mathsf{proposal}(c_n[i])$.
    That is, we ``complete'' $c_{n - t}$ (constructed in the step 1) with $n - 2t$ process-proposal pairs such that the process is ``borrowed'' from $\mathit{base}$, and its proposal is ``borrowed'' from $c_n$.
\end{compactenum}
Observe that $c_{n - t} \diamond \mathit{base}$ as (1) $|\processes{c_{n - t}} \cap \processes{\mathit{base}}| \leq t$ ($n - 2t \leq t$ when $n \leq 3t$), (2) there exists a process $P \in \processes{\mathit{base}} \setminus \processes{c_{n - t}}$ (while constructing $c_{n - t}$, we excluded $t > 0$ processes from $\mathit{base}$; step 2), and (3) there exists a process $Q \in \processes{c_{n - t}} \setminus{\processes{\mathit{base}}}$ (we included $t > 0$ processes in $\mathit{c_{n - t}}$ which are not in $\mathit{base}$; step 1).

Let $\mathcal{E}_{n - t} \in \mathit{execs}(\mathcal{A})$ denote any infinite canonical execution such that $\mathsf{input\_conf}(\mathcal{E}_{n - t}) = c_{n - t}$.
As $\mathcal{A}$ satisfies \emph{Termination}, some value is decided by correct processes in $\mathcal{E}_{n - t}$; due to \Cref{lemma:triviality_compatible}, that value is $v_{\mathit{base}}$.
Finally, we are able to construct an infinite execution $\mathcal{E}_n \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_n) = c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_n$:
\begin{compactenum}
    \item All processes are correct in $\mathcal{E}_n$.

    \item Until some correct process $P \in \processes{c_{n - t}}$ decides $v_{\mathit{base}}$, $\mathcal{E}_n$ is identical to $\mathcal{E}_{n - t}$.
    Let $\mathcal{S}$ denote the set of all processes which take a computational step in $\mathcal{E}_{n - t}$ until $P$ decides $v_{\mathit{base}}$; note that $\mathcal{S} \subseteq \processes{c_{n - t}}$ and $P \in \mathcal{S}$.

    \item Afterwards, every process $Q \notin \mathcal{S}$ ``wakes up'' with the proposal specified in $c_n$.
    
    \item GST is set to after all processes have taken a computational step.
\end{compactenum}
Therefore, $v_{\mathit{base}}$ is indeed decided in $\mathcal{E}_n$ and $\mathsf{input\_conf}(\mathcal{E}_n) = c_n$, which concludes the proof.
\end{proof}

\iffalse
*********
\begin{sketch}
Fix any input configuration $c_n \in \mathcal{I}_n$.
There exists an input configuration $c_{n - t} \in \mathcal{I}_{n - t}$ such that (1) for every process $P \in \processes{c_n} \cap \processes{c_{n - t}}$, proposals of $P$ in $c_n$ and $c_{n - t}$ are identical, and (2) $c_{n - t} \diamond \mathit{base}$.
Hence, $v_{\mathit{base}}$ is decided in any infinite canonical execution $\mathcal{E}_{n - t}$ which corresponds to $c_{n - t}$ (by \Cref{lemma:triviality_compatible}).
Thus, by ``waking up'' processes in $\processes{c_n} \setminus{\processes{c_{n - t}}}$ after $v_{\mathit{base}}$ is decided in $\mathcal{E}_{n - t}$, we build an execution $\mathcal{E}_n$ such that (1) $\mathcal{E}_n$ corresponds to $c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_n$.
\end{sketch}
**********
\fi


\iffalse
\begin{sketch}
Fix any input configuration $c \in \mathcal{I}_n$.
We construct another input configuration $c^* \in \mathcal{I}$:
\begin{compactenum}
    \item For every process $Q \notin \processes{\mathit{base}}$, we include a process-proposal pair $(Q, v)$ in $c^*$, for any value $v \in \mathcal{V}_I$.
    Note that there are $t$ such processes $Q$ as $|\processes{\mathit{base}}| = n - t$.

    \item We include $n - 2t$ process-proposal pairs $(P_i, v)$ in $c^*$ such that (1) $P_i \in \processes{\mathit{base}}$, and (2) $v = \mathsf{proposal}(c[i])$.
    That is, we ``complete'' $c^*$ (constructed in the step 1) with $n - 2t$ process-proposal pairs such that the process is ``borrowed'' from $\mathit{base}$ and its proposal is ``borrowed'' from $c$.
\end{compactenum}
Observe that $c^* \diamond \mathit{base}$ as (1) $|\processes{c^*} \cap \mathit{base}| \leq t$ (because $n - 2t \leq t$ when $n \leq 3t$), (2) there exists a process $P \in \processes{\mathit{base}} \setminus \processes{c^*}$ (because we excluded $t > 0$ processes from $\mathit{base}$ when constructing $c^*$; step 1), and (3) there exists a process $Q \in \processes{c^*} \setminus{\processes{\mathit{base}}}$ (because we included $t > 0$ processes in $\mathit{c^*}$ which are not in $\processes{\mathit{base}}$; step 1).

Let $\mathcal{E}_{c^*} \in \mathit{execs}(\mathcal{A})$ denote any infinite canonical execution such that $\mathsf{corresponds}(\mathcal{E}_{c^*}) = c^*$.
As $\mathcal{A}$ satisfies \emph{Termination}, some value is decided by correct processes in $\mathcal{E}_{c^*}$; due to \Cref{lemma:triviality_compatible}, that value is $v_{\mathit{base}}$.
Finally, we are able to construct an infinite execution $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{corresponds}(\mathcal{E}_c) = c$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_c$:
\begin{compactenum}
    \item All processes are correct in $\mathcal{E}_c$.

    \item Until some correct process $P \in \processes{c^*}$ decides $v_{\mathit{base}}$, $\mathcal{E}_c$ is identical to $\mathcal{E}_{c^*}$.

    \item Afterwards, every process $Q \notin \processes{c^*}$ ``wakes up'' with the proposal specified in $c$.
\end{compactenum}
Due to the construction, 
$v_{\mathit{base}}$ is indeed decided in $\mathcal{E}_c$ and $\mathsf{corresponds}(\mathcal{E}_c) = c$, which concludes the proof.
\end{sketch}
\fi

We are now ready to prove that $\mathit{val}$ is trivial.
We do so by showing that, for any input configuration $c \in \mathcal{I}$, $v_{\mathit{base}} \in \mathit{val}(c)$.

\begin{lemma}
\label{lemma:triviality_main_2} 
Validity property $\mathit{val}$ is trivial.
\end{lemma}
\begin{proof}
We fix any input configuration $c \in \mathcal{I}$.
Let us distinguish two possible scenarios:
\begin{compactitem}
    \item Let $c \in \mathcal{I}_n$.
    There exists an infinite execution $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_c) = c$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_c$ (by \Cref{lemma:triviality_complete}).
    As $\mathcal{A}$ satisfies $\mathit{val}$, $v_{\mathit{base}} \in \mathit{val}(c)$.

    \item Let $c \notin \mathcal{I}_n$.
    We construct an input configuration $c_n \in \mathcal{I}_n$ in the following way:
    \begin{compactenum}
        \item Let $c_n \gets c$.

        \item For every process $P \notin \processes{c}$, $(P, \text{any proposal})$ is included in $c_n$.
        % , where $v \in \mathcal{V}_I$ is any proposal.
    \end{compactenum}
    Due to the construction of $c_n$, $c_n \sim c$.
    By \Cref{lemma:triviality_complete}, there exists an infinite execution $\mathcal{E}_{n} \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_n) = c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_{n}$; $\mathcal{E}_n$ is a canonical execution.
    Therefore, canonical similarity ensures that $v_{\mathit{base}} \in \mathit{val}(c)$ (\Cref{lemma:helper_main}).
\end{compactitem}
In both possible cases, $v_{\mathit{base}} \in \mathit{val}(c)$.
Thus, the theorem.
\end{proof}

% Given that $\mathit{val}$ is any solvable validity property with $n \leq 3t$ and it is shown that $\mathit{val}$ is trivial (\Cref{theorem:triviality_main}), every solvable validity property with $n \leq 3t$ is trivial.
\Cref{lemma:triviality_main_2} concludes the proof of \Cref{theorem:triviality_main}, as \Cref{lemma:triviality_main_2} proves that $\mathit{val}$, any solvable validity property with $n \leq 3t$, is trivial.
\Cref{fig:triviality} depicts the proof of \Cref{theorem:triviality_main}.
% Consensus with a trivial validity property can be solved without any communication: processes decide on the same always-admissible value.
Since this subsection shows that consensus cannot be useful when $n \leq 3t$, the rest of the paper focuses on the case of $n > 3t$.
% in the rest of the paper.
% Throughout the rest of the paper, we focus on the case of $n > 3t$.
% Throughout the rest of the paper, we focus on the case of $n > 3t$.

\begin{figure}[ht]
    \centering
    \includegraphics[scale = 0.44]{figures/export-13-crop.pdf}
    \caption{\Cref{theorem:triviality_main}: Overview of the proof in the case of $n = 6$, $t = 2$, and $\mathit{base} = \big[ (P_1, 0), (P_2, 0), (P_3, 0), (P_4, 0) \big]$.}
    \label{fig:triviality}
\end{figure}

% \newpage
\subsection{Similarity Condition: Necessary Solvability Condition} \label{subsection:necessary_condition}

This subsection defines the similarity condition, and proves its necessity for solvable validity properties.

\begin{definition} [Similarity condition] \label{definition:similarity_condition}
A validity property $\mathit{val}$ satisfies the \emph{similarity condition} ($\mathcal{C}_S$, in short) if and only if there exists a Turing-computable function $\Lambda: \mathcal{I}_{n - t} \to \mathcal{V}_O$ such that:
\begin{equation*}
 \forall c \in \mathcal{I}_{n - t}: \Lambda(c) \in \bigcap\limits_{c' \in \mathit{sim}(c)} \mathit{val}(c').
\end{equation*}
\end{definition}

$\mathcal{C}_S$ states that, for every input configuration $c \in \mathcal{I}_{n - t}$, there exists a Turing-computable function $\Lambda(c)$ which retrieves a common admissible decision among all input configurations similar to $c$.\footnote{A function is Turing-computable if there exists a finite procedure to compute the function.}
The necessity of $\mathcal{C}_S$ follows from the canonical similarity result: in any infinite canonical execution, a common admissible value must be decided (\Cref{lemma:helper_main}).

\begin{theorem} \label{theorem:similarity_condition_necessary}
Any solvable validity property satisfies $\mathcal{C}_S$.
\end{theorem}
\begin{proof}
By the means of contradiction, let there exist a validity property $\mathit{val}$ such that (1) $\mathit{val}$ does not satisfy $\mathcal{C}_S$, and (2) $\mathit{val}$ is solvable.
Let $\mathcal{A}$ be any algorithm which solves the Byzantine consensus problem with $\mathit{val}$.
As $\mathit{val}$ does not satisfy $\mathcal{C}_S$, there does not exist a Turing-computable function $\Lambda: \mathcal{I}_{n - t} \to \mathcal{V}_O$ such that, for every input configuration $c \in \mathcal{I}_{n - t}$, $\Lambda(c) \in \bigcap\limits_{c' \in \mathit{sim}(c)} \mathit{val}(c')$.
% (by \Cref{definition:similarity_condition}).

Fix any input configuration $c \in \mathcal{I}_{n - t}$ for which $\Lambda(c)$ is not defined or not Turing-computable.
% ; such an input configuration exists as $\mathit{val}$ does not satisfy $\mathcal{C}_S$.
Let $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ be an infinite canonical execution such that (1) $\mathsf{input\_conf}(\mathcal{E}_c) = c$, (2) the system is synchronous from the very beginning ($\text{GST} = 0$), and (3) the message delays are exactly $\delta$.
In other words, $\mathcal{E}_c$ unfolds in a ``lock-step'' manner.
As $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_c$ is an infinite execution, some value $v_c \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_c$; observe that the prefix of $\mathcal{E}_c$ in which $v_c$ is decided is finite as processes take only finitely many steps in finite time.
By canonical similarity (\Cref{lemma:helper_main}), $v_c \in \bigcap\limits_{c' \in \similar{c}} \mathit{val}(c')$.
Hence, $\Lambda(c)$ is defined ($\Lambda(c) = v_c$) and Turing-computable ($\mathcal{A}$ computes it).
Thus, we reach a contradiction with the fact that $\Lambda(c)$ is not defined or not Turing-computable.
% , which concludes the proof.
% , which concludes the proof.
\end{proof}

Notice that, for proving the necessity of $\mathcal{C}_S$ (\Cref{theorem:similarity_condition_necessary}), we do not rely on the $n > 3t$ assumption.
% that $n > 3t$.
Hence, $\mathcal{C}_S$ is necessary for \emph{all} solvable validity properties (irrespectively of the resilience threshold).
However, as proven in \Cref{subsection:triviality_main}, $\mathcal{C}_S$ is not sufficient when $n \leq 3t$: e.g., \emph{Weak Validity} satisfies $\mathcal{C}_S$, but it is unsolvable with $n \leq 3t$~\cite{DLS88,PeaseSL80}.
(Observe that any trivial validity property satisfies $\mathcal{C}_S$.)

% \jovan{I believe we will need to cut the part below. No space.}
\paragraph{Similarity condition (example).}
Consider \emph{Correct-Proposal Validity}, a validity property which states that any decided value must have been proposed by a correct process.
Consensus with \emph{Correct-Proposal Validity} is also known as \emph{strong}  consensus~\cite{fitzi2003efficient,siu1998reaching}.
Strong  consensus assumes $\mathcal{V}_I = \mathcal{V}_O$.
It was shown that, in partial synchrony,  strong consensus  cannot be solved if $n \leq (|\mathcal{V}_I| + 1)t$~\cite{fitzi2003efficient}.
We now present an alternative proof.
Namely, we show that \emph{Correct-Proposal Validity} does not satisfy $\mathcal{C}_S$ if $n \leq (|\mathcal{V}_I| + 1)t$, which makes it unsolvable by \Cref{theorem:similarity_condition_necessary}.

\begin{theorem}
Strong consensus is unsolvable unless $n > (|\mathcal{V}_I| + 1)t$.
\end{theorem}
\begin{proof}
We prove the theorem by contradiction.
Let $|\mathcal{V}_I| = |\mathcal{V}_O| = m$.
Without loss of generality, let $n = (m + 1)t$.
We define an input configuration $\mathit{base} \in \mathcal{I}_{n - t}$ such that (1) $|\processes{\mathit{base}}| = n - t = mt$, and (2) every value $v \in \mathcal{V}_I$ is the proposal of exactly $t$ processes in $\mathit{base}$.
Therefore, all values are admissible for $\mathit{base}$ ($\mathit{val}(\mathit{base}) = \mathcal{V}_O$).
Next, for each value $v \in \mathcal{V}_I$, we design an input configuration $c_{\notni v}$ such that (1) $v$ is not admissible for $c_{\notni v}$, and (2) $c_{\notni v} \sim \mathit{base}$:
\begin{compactenum}
    \item Let $c_{\notni v} \gets \mathit{base}$.
    
    \item We remove from $c_{\notni v}$ all process-proposal pairs $\mathit{pp}$ with $\mathsf{proposal}(\mathit{pp}) = v$.

    \item For every process $P \notin \processes{\mathit{base}}$, we add $(P, v')$ to $c_{\notni v}$, for any value $v' \neq v$.
\end{compactenum}
Hence, \emph{Correct-Proposal Validity} does not satisfy $\mathcal{C}_S$ when $n \leq (m + 1)t$ as, for every $v \in \mathcal{V}_O$, there exists an input configuration $c_{\not\ni v} \sim \mathit{base}$ for which $v$ is not admissible.
% there does not exist a common admissible decision among input configurations similar to $\mathit{base}$.
Thus, \emph{Correct-Proposal Validity} is unsolvable if $n \leq (m + 1)t$ (by \Cref{theorem:similarity_condition_necessary}).
\end{proof}


% \medskip
% In this subsection, we introduced $\mathcal{C}_S$, and showed its necessity for solvable validity properties.
% % that any solvable validity property satisfies $\mathcal{C}_S$.
% In \Cref{subsection:general_algorithm}, we prove that, if a validity property satisfies $\mathcal{C}_S$ and $n > 3t$, the property is solvable.
% Therefore, $\mathcal{C}_S$ represents a necessary and sufficient condition for solvable validity properties when $n > 3t$.

% As $\mathit{val}$ is  shown to be trivial (by \Cref{theorem:triviality_main}), the corollary bellow directly follows.

% \begin{corollary} \label{corollary:triviality}
% If a validity property is solvable with $n \leq 3t$, the validity property is trivial.    
% \end{corollary}

% \subsection{Lower Bound on Message Complexity for Non Trivial and Solvable Validity Properties}
% \label{subsection:lower_bound}

% This subsection proves that any Byzantine consensus algorithm with a non-trivial and solvable validity property incurs $\Omega(t^2)$ message complexity.
% This result generalizes the seminal Dolev-Reischuk bound~\cite{dolev1985bounds}, which says that any Byzantine consensus algorithm with \emph{Strong Validity} exchanges (at least) $\Omega(t^2)$ messages.
% Our proof is by the means of contradiction and it consists of two steps: 
% \begin{compactenum}
%     \item If the message complexity of a Byzantine consensus algorithm is less than quadratic, we identify a process $Q$ which can decide some value $v \in \mathcal{V}_O$ without having received any message (from any other process).
%     The first step of our proof is identical to the first step of the original Dolev-Reischuk proof~\cite{dolev1985bounds,DBLP:conf/podc/AbrahamCDNP0S19}.
    
%     \item We show that there exists an execution such that (1) $Q$ is faulty and silent, and (2) other processes decide a value $v' \neq v$.
%     We can then ``merge'' this execution with a valid behavior of $Q$ in which $Q$ decides $v$ without having received any message, thus constructing an execution in which \emph{Agreement} is violated.
    
%     The original proof of the Dolev-Reischuk bound follows the same idea.
%     However, given that the original bound concerns only \emph{Strong Validity}, the second step in the original proof is straightforward.
%     Conversely, as our bound considers \emph{all} validity properties, completing the second step proved more challenging.
% \end{compactenum}
% In this subsection, we give an informal proof of our lower bound; the formal treatment is delegated to \Cref{section:lower_bound_appendix}.

% Throughout the entire subsection, we fix any non-trivial and solvable validity property $\mathit{val}$.
% Moreover, we fix $\mathcal{A}$, any Byzantine consensus algorithm with $\mathit{val}$.
% Finally, $n > 3t$ as $\mathit{val}$ is non-trivial (see \Cref{theorem:triviality_main}).

% \paragraph{Execution $\mathcal{E}_{\mathit{base}}$ of $\mathcal{A}$.}
% We start by defining a specific infinite execution $\mathcal{E}_{\mathit{base}} \in \mathit{execs}(\mathcal{A})$ in the following manner:
% \begin{compactenum}
%      \item $\text{GST}_{\mathit{base}} = 0$.
%      That is, the system is synchronous throughout the entire execution.
     
%      \item All processes are separated into two groups: (1) group $A$, with $|A| = n - \frac{t}{2}$, and (2) group $B$, with $|B| = \frac{t}{2}$.
     
%      \item All processes in the group $A$ are correct, whereas all processes in the group $B$ are faulty.
     
%      \item We fix any value $v^* \in \mathcal{V}_I$.
%      For every correct process $P \in A$, the proposal of $P$ in $\mathcal{E}_{\mathit{base}}$ is $v^*$.
     
%      \item For every faulty process $Q \in B$, $Q$ behaves correctly in $\mathcal{E}_{\mathit{base}}$ with its proposal being $v^*$, except that (1) $Q$ ignores the first $\frac{t}{2}$ messages received from other processes, and (2) $Q$ omits sending messages to other processes in $B$. 
% \end{compactenum}

% \medskip
% If correct processes send $(\frac{t}{2})^2$ (or more) messages in $\mathcal{E}_{\mathit{base}}$, the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
% Hence, in the rest of the subsection, we assume that correct processes send less than $(\frac{t}{2})^2$ messages in $\mathcal{E}_{\mathit{base}}$.

% The first step of our proof shows that, if correct processes indeed send less than $(\frac{t}{2})^2$ messages in $\mathcal{E}_{\mathit{base}}$, there must exist a process $Q \in B$ such that $Q$ can correctly decide some value $v \in \mathcal{V}_O$ without having received \emph{any} message from any other process.
% We prove this claim using the pigeonhole principle.

% \begin{lemma} \label{lemma:behavior_without_receptions}
% There exist a value $v \in \mathcal{V}_O$ and a process $Q \in B$ such that $Q$ can correctly decide $v$ without having received any message from any other process.
% \end{lemma}
% \begin{sketch}
% Recall that, by assumption, correct processes (i.e., processes in the group $A$) send less than $(\frac{t}{2})^2$ messages in $\mathcal{E}_{\mathit{base}}$.
% Therefore, due to the pigeonhole principle, there exists a process $Q \in B$ which receives less than $\frac{t}{2}$ messages in $\mathcal{E}_{\mathit{base}}$.
% Recall that $Q$ behaves correctly in $\mathcal{E}_{\mathit{base}}$ with its proposal being $v^*$, except that (1) $Q$ ignores the first $\frac{t}{2}$ messages received from other processes, and (2) $Q$ does not send any messages to other processes in the group $B$.
% We denote by $S_Q$ the set of processes, not including $Q$, which send messages to $Q$ in $\mathcal{E}_{\mathit{base}}$; note that $|S_Q| \leq \frac{t}{2}$.

% Next, we construct an infinite execution $\mathcal{E}_{\mathit{base}}'$ in the following manner:
% \begin{compactenum}
%     % \item $\text{GST}_{\mathit{core}}' = 0$, i.e., the system is synchronous from the beginning.
    
%     \item Processes in $(A \cup \{Q\}) \setminus{S_Q}$ are correct; other processes are faulty.
%     That is, we make $Q$ correct in $\mathcal{E}'_{\mathit{base}}$, and we make all processes in $S_Q$ faulty in $\mathcal{E}'_{\mathit{base}}$.
    
%     \item Processes in $B \setminus{\{Q\}}$ behave exactly as in $\mathcal{E}_{\mathit{base}}$.
%     Moreover, processes in $S_Q$ behave exactly as in $\mathcal{E}_{\mathit{base}}$, except that they \emph{do not} send any message to $Q$.
% \end{compactenum}
% Importantly, there exists a process $P \in A \setminus{S_Q}$ (as $n > t$) such that $P$ cannot distinguish $\mathcal{E}_{\mathit{base}}'$ from $\mathcal{E}_{\mathit{base}}$.
% Hence, as $P$ decides some value $v \in \mathcal{V}_O$ in $\mathcal{E}_{\mathit{base}}$ (as $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{\mathit{base}}$ is infinite), $P$ decides the same value $v$ in $\mathcal{E}_{\mathit{base}}'$.
% Moreover, due to the construction of $\mathcal{E}_{\mathit{base}}'$, process $Q$ does not receive any message (from any other process) in $\mathcal{E}_{\mathit{base}}'$.
% Due to the fact that $Q$ is correct in $\mathcal{E}_{\mathit{base}}'$ and $\mathcal{A}$ satisfies \emph{Termination} and \emph{Agreement}, $Q$ decides $v$ in $\mathcal{E}_{\mathit{base}}'$.
% Thus, $Q$ can indeed correctly decide $v \in \mathcal{V}_O$ without having received any message from any other process. 
% \end{sketch}
% % \jovan{Is this proof ok? Please, try to attack is much as possible. Can there be any problems with timers or I don't know what.
% % I am not seeing any problems. Just want us to be very careful!}

% In the second step, we show that there exists an execution $\mathcal{E}$ of $\mathcal{A}$ such that (1) $Q$ is faulty and silent, and (2) other processes decide a value $v' \neq v$.
% As $\mathit{val}$ is a non-trivial validity property, there exists an input configuration $c \in \mathcal{I}$ such that $v \notin \mathit{val}(c)$; recall that $v$ is the value that $Q$ can correctly decide without having received any message from any other process (by \Cref{lemma:behavior_without_receptions}).
% The following lemma shows that $Q \in \processes{c}$; otherwise, we could construct an execution in which $\mathcal{A}$ violates \emph{Agreement}.

% \begin{lemma} \label{lemma:q_in_c}
% $Q \in \processes{c}$.
% \end{lemma}
% \begin{sketch}
% By contradiction, let $Q \notin \processes{c}$.
% We fix any infinite canonical execution $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{corresponds}(\mathcal{E}_c) = c$.
% Observe that $Q$ takes no computational steps in $\mathcal{E}_c$ as $Q \notin \processes{c}$.
% As $v \notin \mathit{val}(c)$, $\mathcal{E}_c$ is infinite and $\mathcal{A}$ satisfies \emph{Termination} and $\mathit{val}$, some value $v' \neq v$ is decided by a correct process in $\mathcal{E}_c$.

% Next, we can construct another execution $\mathcal{E}'$ such that $\mathcal{E}' \in \mathit{execs}(\mathcal{A})$ is identical to $\mathcal{E}$, except that:
% \begin{compactenum}
%     \item Process $Q$ is correct in $\mathcal{E}'$.
    
%     \item All messages sent by and to $Q$ are delayed.
    
%     \item Process $Q$ exhibits the behavior in which (1) it receives no messages by other processes (until some time as in-flight messages must eventually be received by $Q$), and (2) $Q$ decides $v$.
%     Such a behavior of the process $Q$ exists due to \Cref{lemma:behavior_without_receptions}.
% \end{compactenum}
% As messages from $Q$ are delayed in $\mathcal{E}'$, all other correct processes cannot distinguish $\mathcal{E}'$ from $\mathcal{E}_c$ (until some time); hence, all other correct processes decide $v' \neq v$ in $\mathcal{E}'$.
% Therefore, there is a disagreement in $\mathcal{E}'$, which contradicts the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
% Thus, $Q \in \processes{c}$.
% \end{sketch}

% The previous lemma shows that $Q \in \processes{c}$.
% Now, we construct an input configuration $c' \in \mathcal{I}$ such that $Q \notin \processes{c'}$:
% \begin{compactenum}
%     \item Let $c' \gets c$.

%     \item We remove $(Q, \cdot)$ from $c'$.

%     \item If $|\processes{c}| = n - t$, we add $(Z, \cdot)$ to $c'$, where $Z$ is any process such that $Z \notin \processes{c}$; note that such a process $Z$ exists as $t > 0$ and $Z \neq Q$ as $Q \in \processes{c}$ (by \Cref{lemma:q_in_c}).
% \end{compactenum}
% Due to the construction of $c'$, $c' \sim c$.
% Indeed, (1) $\processes{c'} \cap \processes{c} \neq \emptyset$ (as $n - t - 1 > 0$ when $n > 3t$ and $t > 0$), and (2) for every process $P \in \processes{c'} \cap \processes{c}$, the proposal of $P$ is identical in $c'$ and $c$ (by the step 1 of the construction).

% The lemma below shows that there exists a canonical execution $\mathcal{E}_{c'}$ such that (1) $\mathcal{E}_{c'}$ corresponds to $c'$, and (2) some value $v' \neq v$ is decided in $\mathcal{E}_{c'}$.

% \begin{lemma} \label{lemma:another execution}
% There exists a canonical execution $\mathcal{E}_{c'} \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_{c'}) = c'$, and (2) a value $v' \neq v$ is decided by a correct process in $\mathcal{E}_{c'}$.
% \end{lemma}
% \begin{proof}
% We fix any infinite canonical execution $\mathcal{E}_{c'} \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}_{c'}) = c'$.
% As $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{c'}$ is infinite, some value $v' \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_{c'}$.
% As $c' \sim c$, $v' \in \mathit{val}(c)$ (by \Cref{lemma:helper_main}).
% Finally, $v' \neq v$ as (1) $v' \in \mathit{val}(c)$, and (2) $v \notin \mathit{val}(c)$, which concludes the proof.
% % Thus, xthe lemma.
% \end{proof}

% At last, we can ``merge'' the execution $\mathcal{E}_{c'}$ (from \Cref{lemma:another execution}) with the valid behavior of $Q$ in which $Q$ decides $v$ without having received any message (from \Cref{lemma:behavior_without_receptions}).
% Hence, we can construct an execution in which $\mathcal{A}$ violates \emph{Agreement}, which represents a contradiction with the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
% Therefore, correct processes send $\geq (\frac{t}{2})^2$ messages in $\mathcal{E}_{\mathit{base}}$, which means that the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.

% \begin{theorem} [Lower bound on message complexity] \label{theorem:lower_bound_main}
% The message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
% \end{theorem}

% Observe that, as each message contains (at least) a single word, \Cref{theorem:lower_bound_main} implies the $\Omega(t^2)$ lower bound on the communication complexity, as well.

% \subsection{Similarity \& Knowledge Conditions are Sufficient if $n > 3t$: General Algorithm \textsc{Complete}} \label{subsection:general_algorithm}

% In this subsection, we prove that $\mathcal{C}_S$ and $\mathcal{C}_K$ are sufficient conditions for a validity property to be solvable if $n > 3t$.\footnote{Recall that, when $n \leq 3t$, all solvable properties are trivial (\Cref{subsection:triviality_main}).}
% Namely, we present \textsc{Complete}, a Byzantine consensus algorithm with \emph{any} validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$.
% Importantly, \textsc{Complete} achieves $O(n^2)$ message complexity, which makes it optimal (when $t \in \Omega(n)$); the communication complexity of \textsc{Complete} is $O(n^3)$.

% First, we formally define \emph{Interactive-Consistency Validity} \pierre{I guess interactive consistency is highly connoted with the desire to agree on the inputs of all correct processes, which is obviously possible iff the network is synchronous.}, and present a Byzantine consensus algorithm \textsc{Icon} with \emph{Interactive-Consistency Validity} (\Cref{subsubsection:interactive_consistency}).
% Then, we utilize \textsc{Icon} to obtain \textsc{Complete} (\Cref{subsubsection:Complete}).
% Throughout the entire subsection, $n > 3t$.

% % \newpage
% \subsubsection{\textsc{Icon}: Byzantine consensus with Interactive-Consistency Validity.} \label{subsubsection:interactive_consistency}
% In \textsc{Icon}, processes propose values, and agree on sets of $n - t$ process-proposal pairs.
% That is, processes agree on input configurations: $\mathcal{V}_O = \mathcal{I}_{n - t}$.

% Let us start by formally defining the \emph{Interactive-Consistency Validity} property:
% \begin{compactitem}
%      \item \emph{Interactive-Consistency Validity:} Let a correct process decide $\mathit{vector} \in \mathcal{I}_{n - t}$ such that (1) $(P, v)$ belongs to $\mathit{vector}$, for some value $v \in \mathcal{V}_I$, and (2) $P$ is a correct process.
%      Then, $v$ is $P$'s proposal.
% \end{compactitem}
% Intuitively, \emph{Interactive-Consistency Validity} states that, if a correct process decides that a value $v$ was proposed by a correct process $P$, then $P$'s proposal was indeed $v$.
% Observe that the Byzantine consensus problem with \emph{Interactive-Consistency Validity} is identical to the well-known interactive-consistency problem~\cite{ben2003resilient,thambidurai1988interactive,diamantopoulos2015interactive,fischer1982lower}, except that it does not require agreement on the proposals of \emph{all} processes: processes need to agree on the proposals of $n - t$ processes.

% The pseudocode of \textsc{Icon} is presented in \Cref{algorithm:interactive_consistency}.
% \textsc{Icon} achieves $O(n^2)$ message complexity and $O(n^3)$ communication complexity.
% We construct \textsc{Icon} by relying on \textsc{Quad}, a partially synchronous Byzantine consensus algorithm introduced by Civit \emph{et al.}~\cite{civit2022byzantine}; we give a brief description of \textsc{Quad} below.


% \paragraph{\textsc{Quad}.}
% Formally, \textsc{Quad} is concerned with two sets: (1) $\mathcal{V}_{\textsc{Quad}}$, a set of values, and (2) $\mathcal{P}_{\textsc{Quad}}$, a set of proofs.
% In \textsc{Quad}, processes propose and decide value-proof pairs.
% Moreover, there exists a function $\mathsf{valid}: \mathcal{V}_{\textsc{Quad}} \times \mathcal{P}_{\textsc{Quad}} \to \{ \mathit{true}, \mathit{false} \}$.
% As for the validity property, $\textsc{Quad}$ satisfies \emph{External Validity}: If a correct process decides a pair $(v, \Sigma)$, then $\mathsf{valid}(v, \Sigma) = \mathit{true}$.\footnote{We underline that our formalism in its current form is not expressive enough to describe \emph{External Validity}. However, we extend our formalism to accommodate for \emph{External Validity} in \Cref{subsection:external_validity}.}
% Importantly, \textsc{Quad} achieves $O(n^2)$ message complexity, which allows the message complexity of \textsc{Icon} to be $O(n^2)$.
% As for the communication complexity of \textsc{Quad}, it is $O(n^2 \cdot x)$, where $x$ denotes the maximum size of a proof.
% For completeness, we provide a detailed explanation of \textsc{Quad} in \Cref{section:quad_appendix}; 

% In our implementation of \textsc{Icon}
% (\Cref{algorithm:interactive_consistency}), we rely on a specific instance of \textsc{Quad} where (1) $\mathcal{V}_{\textsc{Quad}} = \mathcal{I}_{n - t}$ (i.e., processes propose input configurations), and (2) $\mathcal{P}_{\textsc{Quad}}$ is a set of $n - t$ \textsc{proposal} messages.
% Moreover, given an input configuration $c \in \mathcal{V}_{\textsc{Quad}}$ and a set of messages $\Sigma \in \mathcal{P}_{\textsc{Quad}}$, $\mathsf{valid}(c, \Sigma) = \mathit{true}$ if and only if, for every process-proposal pair $(P_j, v_j)$ which belongs to $c$, $\langle \textsc{proposal}, v_j \rangle_{\sigma_j} \in \Sigma$ (i.e., every process-proposal pair is accompanied by a properly signed \textsc{proposal} message).

% \paragraph{Description of \textsc{Icon}.}
% When a correct process $P_i$ proposes a value $v \in \mathcal{V}_I$ to \textsc{Icon} (line~\ref{line:propose}), the process broadcasts a signed \textsc{proposal} message (line~\ref{line:broadcast_proposal}).
% Once $P_i$ receives $n - t$ \textsc{proposal} messages (line~\ref{line:received_n_t_proposals}), $P_i$ constructs an input configuration $\mathit{vector}$ (line~\ref{line:construct_input_configuration}) and a proof 
% $\Sigma$ (line~\ref{line:construct_proof}) from the received \textsc{proposal} messages.
% Moreover, $P_i$ proposes $(\mathit{vector}, \Sigma)$ to \textsc{Quad} (line~\ref{line:propose_quad}).
% Finally, when $P_i$ decides a pair $(\mathit{vector}', \Sigma')$ from \textsc{Quad} (line~\ref{line:decide_quad}), $P_i$ decides $\mathit{vector}'$ 
%  from \textsc{Icon} (line~\ref{line:decide}).

% \begin{algorithm}
% \caption{\textsc{Icon}: Pseudocode for process $P_i$}
% \label{algorithm:interactive_consistency}
% \begin{algorithmic} [1]
% \State \textbf{Uses:}
% \State \hskip2em Best-Effort Broadcast, \textbf{instance} $\mathit{beb}$
% \State \hskip2em \textsc{Quad}, \textbf{instance} $\mathit{quad}$

% \medskip
% \State \textbf{upon} $\mathsf{init}$:
% \State \hskip2em $\mathsf{Integer}$ $\mathit{received\_proposals}_i \gets 0$ \Comment{the number of received proposals}
% \State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathcal{V}_I)$ $\mathit{proposals}_i \gets \text{empty}$ \Comment{received proposals}
% \State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathsf{Message})$ $\mathit{messages}_i \gets \text{empty}$ \Comment{received \textsc{proposal} messages}

% \medskip
% \State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$: \label{line:propose}
% \State \hskip2em \textbf{trigger} $\mathit{beb}.\mathsf{broadcast}\big( \langle \textsc{proposal}, v \rangle_{\sigma_i} \big)$ \Comment{broadcast a signed proposal} \label{line:broadcast_proposal}

% \medskip
% \State \textbf{upon} reception of $\mathsf{Message}$ $m = \langle \textsc{proposal}, v_j \rangle_{\sigma_j}$ from process $P_j$ and $\mathit{received\_proposals} < n - t$:
% \State \hskip2em $\mathit{received\_proposals}_i \gets \mathit{received\_proposals}_i + 1$
% \State \hskip2em $\mathit{proposals}_i[P_j] \gets v_j$
% \State \hskip2em $\mathit{messages}_i[P_j] \gets m$

% \State \hskip2em \textbf{if} $\mathit{received\_proposals}_i = n - t$: \label{line:received_n_t_proposals}
% \State \hskip4em $\mathsf{Input\_Configuration}$ $\mathit{vector} \gets $ input configuration containing all process-proposal pairs from $\mathit{proposals}_i$ \label{line:construct_input_configuration}
% \State \hskip4em $\mathsf{Proof}$ $\Sigma \gets $ set of messages containing all \textsc{proposal} messages from $\mathit{messages}_i$ \label{line:construct_proof}
% \State \hskip4em $\mathit{quad}.\mathsf{propose}\big( (\mathit{vector}, \Sigma) \big)$ \label{line:propose_quad}

% \medskip
% \State \textbf{upon} $\mathit{quad}.\mathsf{decide}\big( (\mathsf{Input\_Configuration} \text{ } \mathit{vector}', \mathsf{Proof} \text{ } \Sigma') \big)$: \label{line:decide_quad}
% \State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{vector}')$ \label{line:decide}

% \end{algorithmic}
% \end{algorithm}

% \medskip
% For the lack of space, we delegate the proof of the correctness and complexity of \textsc{Icon} to \Cref{subsection:icon_appendix}
% \begin{theorem} [\textsc{Icon} is correct] \label{theorem:icon}
% \textsc{Icon} (\Cref{algorithm:interactive_consistency}) is a Byzantine consensus algorithm with Interactive-Consistency Validity.
% The message complexity of \textsc{Icon} is $O(n^2)$, whereas its communication complexity is $O(n^3)$.
% \end{theorem}
% % \begin{proof}
% % \emph{Agreement} follows directly from \emph{Agreement} of \textsc{Quad}.
% % Moreover, as there are (at least) $n - t$ correct processes, every correct process eventually proposes to \textsc{Quad} (line~\ref{line:propose_quad}).
% % Due to \emph{Termination} of \textsc{Quad}, every correct process eventually decides.
% % Therefore, \Cref{algorithm:interactive_consistency} satisfies \emph{Termination}.

% % It is left to prove that \textsc{Icon} satisfies \emph{Interactive-Consistency Validity}.
% % Let $\mathit{vector}' \in \mathcal{I}_{n - t}$ be an input configuration decided by a correct process.
% % Due to \emph{External Validity} of \textsc{Quad}, if a process-proposal pair $(P_j, v_j)$ belongs to $\mathit{vector}'$, for some value $v_j \in \mathcal{V}_I$, $P_j$ has sent a properly signed \textsc{proposal} message for $v_j$.
% % If $P_j$ is correct, $v_j$ is its proposal as correct processes send \textsc{proposal} messages only for their proposals (line~\ref{line:broadcast_proposal}).
% % Thus, \Cref{algorithm:interactive_consistency} satisfies \emph{Interactive-Consistency Validity}.

% % The $O(n^2)$ message complexity of \textsc{Icon} follows from the following two facts: (1) correct processes only broadcast \textsc{proposal} messages (line~\ref{line:broadcast_proposal}) before proposing to \textsc{Quad}, and (2) the message complexity of \textsc{Quad} is $O(n^2)$.
% % As for the communication complexity of \textsc{Icon}, it is indeed $O(n^3)$ as (1) correct processes only broadcast $O(n^2)$ words (via the \textsc{proposal} messages; line~\ref{line:broadcast_proposal}) before proposing to \textsc{Quad}, and (2) the communication complexity of \textsc{Quad} is $O(n^3)$ (because the maximum size of a proof is $O(n)$ words).
% % Thus, the theorem.
% % \end{proof}

% Observe that \textsc{Icon} (\Cref{algorithm:interactive_consistency}) utilizes cryptographic signatures (\textsc{proposal} messages are signed).
% We underline that a Byzantine consensus algorithm with \emph{Interactive-Consistency Validity} can be obtained even in a \emph{non-authenticated} setting; we provide such an algorithm in \Cref{section:appendix_non_authenticated}.

% \subsubsection{\textsc{Complete}: Byzantine consensus with any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$.} \label{subsubsection:Complete}
% The pseudocode of \textsc{Complete} is given in \Cref{algorithm:general}.
% \textsc{Complete} is directly obtained from \textsc{Icon}.
% When a correct process $P_i$ proposes (line~\ref{line:propose_general}) to \textsc{Complete}, the proposal is forwarded to \textsc{Icon} (line~\ref{line:propose_ic}).
% Once $P_i$ decides an input configuration $c \in \mathcal{I}_{n - t}$ from \textsc{Icon} (line~\ref{line:decide_ic}), $P_i$ decides the common value $\Lambda(c)$ from \textsc{Complete} (line~\ref{line:decide_general}).

% \begin{algorithm}
% \caption{\textsc{Complete}: Pseudocode for process $P_i$}
% \label{algorithm:general}
% \begin{algorithmic} [1]
% \State \textbf{Uses:}
% \State \hskip2em \textsc{Icon}, \textbf{instance} $\mathit{icon}$

% \medskip
% \State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$: \label{line:propose_general}
% \State \hskip2em \textbf{trigger} $\mathit{icon}.\mathsf{propose}(v)$ \label{line:propose_ic}

% \medskip
% \State \textbf{upon} $\mathit{icon}.\mathsf{decide}(\mathsf{Input\_Configuration} \text{ } c)$: \label{line:decide_ic}
% \State \hskip2em \textbf{trigger} $\mathsf{decide}\big( \Lambda(c) \big)$ \label{line:decide_general}
% \end{algorithmic}
% \end{algorithm}

% \begin{theorem} [\textsc{Complete} is correct] \label{theorem:general_algorithm}
% Let $\mathit{val}$ be any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$.
% \textsc{Complete} (\Cref{algorithm:general}) is a Byzantine consensus algorithm with $\mathit{val}$.
% The message complexity of \textsc{Complete} is $O(n^2)$, whereas its communication complexity is $O(n^3)$.
% \end{theorem}
% \begin{proof}
% \emph{Termination} and \emph{Agreement} of \textsc{Complete} follow from \emph{Termination} and \emph{Agreement} of \textsc{Icon}, respectively.
% Moreover, the message (resp., communication) complexity of \textsc{Complete} follows from the message (resp., communication) complexity of \textsc{Icon}.

% Finally, we prove that \textsc{Complete} satisfies $\mathit{val}$.
% Consider any execution $\mathcal{E}$ of $\textsc{Complete}$ such that $\mathsf{input\_conf}(\mathcal{E}) = c^*$, for some input configuration $c^* \in \mathcal{I}$.
% Let $c \in \mathcal{I}_{n - t}$ be the input configuration correct processes decide from \textsc{Icon} in $\mathcal{E}$ (line~\ref{line:decide_ic}).
% As \textsc{Icon} satisfies \emph{Interactive-Consistency Validity}, we have that, for every process $P \in \processes{c^*} \cap \processes{c}$, $P$'s proposals in $c^*$ and $c$ are identical.
% Hence, $c \sim c^*$.
% Therefore, $\Lambda(c) \in \mathit{val}(c^*)$ (by the definition of the $\Lambda$ function).
% Thus, $\mathit{val}$ is satisfied by \textsc{Complete}, which concludes the proof.
% \end{proof}

% As \textsc{Complete} (\Cref{algorithm:general}) is a Byzantine consensus algorithm with any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$ (\Cref{theorem:general_algorithm}), $\mathcal{C}_S$ and $\mathcal{C}_K$ are sufficient conditions for solvable validity properties when $n > 3t$.
% We underline that any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$ can be solved even in a non-authenticated setting: we simply use a non-authenticated version of \textsc{Icon} (see \Cref{section:non_auth}) in \Cref{algorithm:general}.

% Lastly, as \textsc{Complete} relies on \textsc{Icon}, we conclude that \emph{Interactive-Consistency Validity} is a \emph{strongest} validity property.
% That is, a Byzantine consensus algorithm with any solvable validity property (i.e., with any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$) can be obtained from a Byzantine consensus algorithm with \emph{Interactive-Consistency Validity}.

\iffalse
\paragraph{\emph{$\textsc{IC}_{\mathit{non-auth}}$}: Solution in a non-authenticated setting.}
In order to implement $\textsc{IC}_{\mathit{non-auth}}$, we rely on the binary DBFT~\cite{CGL18} consensus algorithm.
DBFT is a partially synchronous Byzantine consensus algorithm, which (1) satisfies \emph{Strong Validity}, and (2) does not require digital signatures.

\begin{algorithm}
\caption{$\textsc{IC}_{\mathit{non-auth}}$: Pseudocode for process $P_i$}
\label{algorithm:interactive_consistency}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Byzantine Reliable Broadcast, \textbf{instance} $\mathit{brb}$
\State \hskip2em Binary DBFT, \textbf{instances} $\mathit{dbft}[1], ..., \mathit{dbft}[n]$

\medskip
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\mathsf{Integer}$ $\mathit{decided}_0 \gets 0$
\State \hskip2em $\mathsf{Integer}$ $\mathit{decided}_1 \gets 0$
\State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathcal{V}_I)$ $\mathit{proposals} \gets \text{empty}$
\State \hskip2em $\mathsf{Set}(\mathsf{Integer})$ $\mathit{proposed\_to} \gets \emptyset$

\medskip
\State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$:
\State \hskip2em \textbf{trigger} $\mathit{brb}.\mathsf{broadcast}\big( \langle \textsc{proposal}, v \rangle \big)$

\medskip
\State \textbf{upon} $\mathit{brb}.\mathsf{deliver}\big( \langle \textsc{proposal}, v_j \rangle \big)$ from process $P_j$:
\State \hskip2em $\mathit{proposals}[P_j] \gets v_j$
\State \hskip2em $\mathit{proposed\_to} \gets \mathit{proposed\_to} \cup \{j\}$
\State \hskip2em \textbf{trigger} $\mathit{dbft}[j].\mathsf{propose}(1)$

\medskip
\State \textbf{upon} $\mathit{dbft}[j].\mathsf{decide}(x)$:
\State \hskip2em $\mathit{decided}_x \gets \mathit{decided}_x + 1$

\medskip
\State \textbf{upon} $\mathit{decided}_1 \geq n - t$ for the first time:
\State \hskip2em \textbf{for every} $j \in [1, n] \setminus{\mathit{proposed\_to}}$:
\State \hskip4em \textbf{trigger} $\mathit{dbft}[j].\mathsf{propose}(0)$

\medskip
\State \textbf{upon} $\mathit{decided}_0 + \mathit{decided}_1 = n$ and, for the first $n - t$ processes $P_j$ with $\mathit{dbft}[j].\mathsf{decide}(1)$, $\mathit{proposals}[j] \neq \bot$:
\State \hskip2em $\mathit{vector} \gets \text{input configuration constructed of the first } n - t \text{ process-proposal pairs}$
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{vector})$

\end{algorithmic}
\end{algorithm}

\subsection{similarity and knowledge condition}

Let $\mathcal{A}$ be an algorithm with consensus interface and ensuring termination. Let $c\in \mathcal{I}$ be a an input configuration. The \emph{canonical execution w.r.t. $\mathcal{A}$ and $c$}, noted $\mathit{can}(\mathcal{A},c)$, is the infinite execution $e$ of $\mathcal{A}$ s.t. (1) $\mathit{GST}_e = 0$, (2) $\forall P_j \notin \pi(c)$, $P_j$ crashes immediately without any computational step, (3) $\forall P_i \in \pi(c)$, $P_i$ proposes the value $c[i]$, (4) All the messages are received in time $\delta$ exactly.
Let $c' \in \mathcal{I}$, s.t. $c' \sim c$. The \emph{dual execution w.r.t. $\mathcal{A}$, $c$ and $c'$}, noted $\mathit{dual}(\mathcal{A},c,c')$ is the infinite execution $e'$ s.t. (1) We note $e = \mathit{can}(\mathcal{A},c)$ and $T$ the minimum time s.t. all processes in $\pi(c)$ have decided in $e$, (2) the longest prefix of $e$ that does not exceed time $T$ is equal to the longest prefix of $e'$ that does not exceed time $T$ (3) $GST_{e'} = T$, (4) The processes in $\pi(c') \setminus \pi(c)$ start at time $T$, (5) The processes in $\pi(c) \setminus \pi(c')$ crash at time $T$.

Let $\mathit{val}$ be a validity property.
If $\mathcal{A}$ is a consensus algorithm ensuring $\mathit{val}$, then $\mathit{val}$ verifies similarity condition.

Indeed, otherwise we note $c$ s.t. $\bigcap_{c' \in \mathit{sim}(c)} \mathit{val}(c') = \emptyset$, $e = \mathit{can}(\mathcal{A},c)$, $\mathit{dec}$ the decision decided in $e$, $c'$ an input configuration in $\mathit{sim}(c)$ s.t. $dec \notin \mathit{val}(c')$ and $e' = \mathit{dual}(\mathcal{A},c,c')$.
By construction, there exists $P_j \in \pi(c) \cap \pi(c')$ with the same behavior in both $e$ and $e'$ until time $T$.
Thus $P_j$ decides $dec$ in $e'$, which contradicts the fact that $\mathcal{A}$ ensures $\mathit{val}$ since $\mathit{dec} \notin \mathit{val}(c')$.

Finally, we can note $\Lambda_{\mathcal{A},\mathit{val}} : c \in \mathcal{I} \mapsto \mathit{decision}(\mathit{can}(\mathcal{A},c))$.


\pierre{end of the discussion about knowledge condition about}
\jovan{I do not really understand the difference between what you wrote and what was already written before. What am I missing?}

\pierre{Ideally, I would like to stress that authencation is not required for computability. Here are some thoughts}
\jovan{I completely agree!}

\paragraph*{Brief Description of Vector Consensus Without Authentication}

Every correct process Reliable-Bcast its proposal (without Authentication). Upon, RB-delivery of message from $P_i$, propose $1$ to a binary-DBFT instance implementing a Binary Consensus with Strong Validity (without authentication). Eventually $n-t$ instances will be decided and their value will be $1$ because of strong validity. Then propose $0$ to the remaining instances. Decide the associated vector with at least $n-t$ components.

\jovan{Yes, definitely. Good point!}

\paragraph*{Sufficiency of similarity condition}

\begin{lemma}
Let $\mathit{val}$ be a validity property verifying similarity condition (with $t<n/3$), then there exists a $t$-resilient partially synchronous algorithm among $n$ processes that solves Byzantine consensus with validity $\mathit{val}$.
\end{lemma}

\begin{proof}
(Sketch)

We use a vector consensus that will allow the processes to agree on a vector of $n-t$ proposals associated with an id. We note $k$ the associated input configuration of size $|\pi(k)| \geq n-t$. Let us note that $P_j \in \pi(k)$ does not imply that $P_j$ is correct.
Then, every correct process decides $\Lambda(k)$.
Since $\mathit{val}$ verifies similarity condition, $\Lambda(k) \in \bigcap_{c \in \mathit{sim}(k)} \mathit{val}(c)$. Moreover, every input configuration $c$ matched by the execution $e$ that led to the pre-decision of vector $k$ is in $\mathit{sim}(k)$. Indeed, if a process $P_j$ in $\pi(k)$ is Byzantine, then its $P_j \notin \pi(c)$, while if a process $P_i \in \pi(c) \cap \pi(k)$, it is correct in $e$ and this is its input $c[i]$ that appears in $k[i]$ by property of Reliable-Broadcast.
\end{proof}

\paragraph*{A few comments}

\begin{itemize}
    \item The vector validity $\mathit{val}_{\mathit{vect}}$ (the decided value is a vector of $n-t$ values whose $n-2t$ among them correspond to the correct proposal of correct processes only) is the strongest achievable validity property in the sense that if you have an algorithm $\mathcal{A}_{\mathit{vect}}$ that achieves vector validity, then for every every satisfiable validity property $\mathit{val}$, it is possible to trivially design an algorithm $\mathcal{A}$ that returns $\Lambda_{\mathcal{A}}(\overset{\rightarrow}{v})$, where $\overset{\rightarrow}{v}$ is the value returned by $\mathcal{A}_{\mathit{vect}})$ as a black-box.
    Let us note that this transformation uses only one instance of $\mathcal{A}_{\mathit{vect}})$ and no additional communication nor latency.
    
    \item The impossibility results for validity properties that do not ensure similarity conditions only needs asynchrony and crash failures (we do not need to invocate Byzantine failures for this proof).
    
    \item If $\Theta(t^2)$ is a tight bound for partially synchronous Byzantine Agreement with strong validity or weak validity under threshold setup (Quad, SQuad and new lower bound for weak validity), here are some open problems:
    \begin{itemize}
        \item  bound for vector validity for any setup
        \item  bound for any validity for any setup except threshold setup
    \end{itemize}
\end{itemize}




\pierre{end of the discussion about sufficiency without authentication}
\jovan{I like it very much. All very good points! }

\subsection{The Similarity and Knowledge Conditions are Sufficient}

In this subsection, we prove that both the similarity and knowledge conditions together are sufficient for a validity property to be satisfiable.
We divide the subsection into two parts: (1) we consider the case of $n > 3t$, and (2) we consider the case of $n \leq 3t$.

\subsubsection{$n > 3t$}

We now prove the following theorem.

\begin{theorem} [The similarity and knowledge conditions are sufficient] \label{theorem:similarity_sufficient}
If a validity property satisfies the similarity and knowledge conditions, the validity property is satisfiable.
\end{theorem}

%In order to prove \ref{theorem:similarity_sufficient}, we will be constructing a general algorithm that solves consensus given any validity property that satisfies [GONE FOR LUNCH, WORK IN PROGRESS]


\begin{proof}
Let $\mathit{val}$ be any validity property that satisfies the similarity condition and the knowledge condition.
In order to conclude the theorem, we present an algorithm that solves the Byzantine consensus problem with $\mathit{val}$.

First, we assume an existence of a black-box Byzantine consensus protocol in which every value is proposed along with a matching proof. 
and where the protocol satisfies the following properties:
\begin{compactitem}
   \item Termination: Every correct process eventually decides.
   
   \item Agreement: No two correct processes decide different values.
   
   \item Validity-by-proof: If a correct process decides a value $v$, then $v$ is accompanied by a matching proof.
\end{compactitem}
The protocol is provided with the function $\mathit{matches}$ such that $\mathit{matches}(v, \mathit{proof}) = \mathit{true}$ if $\mathit{proof}$ matches $v$.
For example, by adding proofs to values and providing the $\mathit{matches}$ function, one can modify the HotStuff~\cite{yin2019hotstuff} or \textsc{quad}~\cite{civit2022byzantine} protocol to solve the aforementioned consensus problem with $n > 3t$. A more detailed explanation of the construction of this type of black-box can also be found in \textsc{quad}~\cite{civit2022byzantine}.

\begin{algorithm}
\caption{Partially synchronous Byzantine algorithm $\mathcal{A}_B$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:partially_synchronous_byzantine}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Partially Synchronous Byzantine Consensus with Validity-By-Proof, \textbf{instance} $c$
\State \hskip2em Byzantine Consistent Broadcast, \textbf{instance} $\mathit{bcb}$

\medskip
\State \textbf{upon} $\mathsf{start}$:
\State \hskip2em \textbf{trigger} $\mathit{bcb}.\mathsf{broadcast}\big( [\textsc{proposal}, \mathit{proposal}] \big)$

\medskip
\State \textbf{upon} delivery of $n - t$ \textsc{proposal} messages:
\State \hskip2em $\mathsf{Input\_Configuration}$ $\mathit{input} \gets$ the input configuration built out of the received $n - t$ \textsc{proposal} messages
\State \hskip2em $\mathsf{Value}$ $\mathit{to\_propose} \gets $ find a common value among all input configurations that belong to $\mathit{sim}(\mathit{input})$
\State \hskip2em \(\triangleright\) $\mathit{to\_propose}$ is accompanied by the received \textsc{proposal} messages which act as a proof of $\mathit{to\_propose}$
\State \hskip2em \textbf{trigger} $c.\mathsf{propose}(\mathit{to\_propose}, \text{all received \textsc{proposal} messages})$ \label{line:partially_propose_c_byzantine}

% \medskip
% \State \textbf{upon} timer elapsed:
% \State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
% \State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:partially_build_i_byzantine}
% \State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
% \State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
% \State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
% \State \hskip2em \textbf{else:} 
% \State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{ByzSim}(i)$ \label{line:partially_set_to_propose}

% \State \hskip2em \(\triangleright\) all values are associated with received \textsc{proposal} messages which proves the validity of the proposed values
% \State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:partially_propose_c_byzantine}

\medskip
\State \textbf{upon} $c.\mathsf{decide}(\mathit{dec})$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

First, \Cref{algorithm:partially_synchronous_byzantine} ensures termination as (1) every correct process eventually receives $n - t$ \textsc{proposal} messages, and (2) $c$ ensures termination.
Furthermore, \Cref{algorithm:partially_synchronous_byzantine} ensures agreement as $c$ ensures agreement.
Hence, it is left to prove that \Cref{algorithm:partially_synchronous_byzantine} ensures $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \allconfigurations$.
Let $P$ be a (faulty or correct) process that obtains a value $v$ with its proof; the proof of value $v$ is an input configuration $i$ which consists of $n - t$ process-proposal pairs such that $v \in \bigcap\limits_{i' \in \mathit{sim}(i)} \mathit{val}(i')$.
If there exist process-proposal pairs $\mathit{pp}$ and $\mathit{pp}'$ such that (1) $\mathit{pp}$ belongs to $\mathit{input}$, (2) $\mathit{pp}'$ belongs to $i$, and (3) $\mathit{pp}$ and $\mathit{pp}'$ are associated with the same process, then $\mathit{pp} = \mathit{pp}'$ as correct processes truthfully report their proposal via the \textsc{proposal} message.
Hence, $\mathit{i} \sim \mathit{input}$, which means that $v \in \mathit{val}(\mathit{input})$.
Thus, for any value $v^*$ for which a proof is obtained, $v^* \in \mathit{val}(\mathit{input})$.
Due to the validity-by-proof property of $c$, the decided value must belong to $\mathit{val}(\mathit{input})$, which means that \Cref{algorithm:partially_synchronous_byzantine} satisfies $\mathit{val}$.
Finally, $\mathit{val}$ is satisfiable, which concludes the proof of the theorem.
\end{proof}

\subsubsection{$n \leq 3t$}

If $n \leq 3t$, we prove that each satisfiable validity property is trivial, i.e., correct processes can decide with \emph{no communication}.
We fix a satisfiable validity property $\mathit{val}$ such that (1) $n \leq 3t$, and (2) a partially synchronous distributed protocol $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$.

We start by defining compatibility of executions.

\begin{definition} [Compatible executions] \label{definition:compatible_executions}
Let $e$ be an infinite execution of $\mathcal{A}$ such that all faulty processes (if any) crash immediately (i.e., without taking any computational step).
Let $e'$ be an infinite execution of $\mathcal{A}$ such that all faulty processes (if any) crash immediately (i.e., without taking any computational step).
Let $x = |\mathit{Corr}_{\mathcal{A}}(e) \cap \mathit{Corr}_{\mathcal{A}}(e')|$.
We say that executions $e$ and $e'$ are \emph{compatible} if (1) $x \leq t$, (2) $x < |\mathit{Corr}_{\mathcal{A}}(e)|$, and (3) $x < |\mathit{Corr}_{\mathcal{A}}(e')|$.
\end{definition}

Let $e$ be an infinite execution of $\mathcal{A}$ such that all faulty processes (if any) crash immediately (i.e., without sending any message).
We denote by $\mathit{compatible}(e)$ the set of all infinite executions compatible with $e$, i.e., $\mathit{compatible}(e) = \{e' \,|\, e \text{ and } e' \text{ are compatible} \}$.

% Consider an infinite execution $e_1$ of $\mathcal{A}$ such that all faulty processes immediately crash (i.e., without sending any message).
% Let $c_1$ denote the number of correct processes in $e_1$; $c_1 \geq n - t$.
% Consider another infinite execution $e_2$ of $\mathcal{A}$ such that all faulty processes immediately crash (i.e., without sending any message).
% Let $c_2$ denote the number of correct processes in $e_2$; $c_2 \geq n -t$.
% We say that $e_2$ is \emph{compatible} with $e_1$ if the number of processes correct in both $e_1$ and $e_2$ is $x$ such that (1) $x \leq t$, (2) $x < c_1$, and (3) $x < c_2$.
% Finally, we denote by $\mathit{compatible}(e_1)$ the set of all infinite executions compatible with $e_1$, i.e., $\mathit{compatible}(e_1) = \{e \,|\, e \text{ is compatible with } e_1\}$.

\begin{lemma} \label{lemma:first_step}
Let $e$ be an infinite execution of $\mathcal{A}$ such that all faulty processes (if any) crash immediately (i.e., without taking any computational step).
Let $\mathit{dec}$ be the value decided in $e$.
For every execution $e' \in \mathit{compatible}(e)$, $\mathit{dec}$ is decided in $e'$.
\end{lemma}
\begin{proof}
By contradiction, let there exist an infinite execution $e' \in \mathit{compatible}(e)$ such that $\mathit{dec}$ is not decided in $e'$.
Let $x = |\mathit{Corr}_{\mathcal{A}}(e) \cap \mathit{Corr}_{\mathcal{A}}(e')|$.
As $e$ and $e'$ are compatible, we have: (1) $x \leq t$, (2) $x < |\mathit{Corr}_{\mathcal{A}}(e)|$, and (3) $x < |\mathit{Corr}_{\mathcal{A}}(e')|$ (by \Cref{definition:compatible_executions}).
Hence, there exists a process $P$ such that (1) $P$ is correct in $e$, and (2) $P$ is not correct in $e'$ (as $x < |\mathit{Corr}_{\mathcal{A}}(e)|$).
Similarly, there exists another process $Q \neq P$ such that (1) $Q$ is correct in $e'$, and (2) $Q$ is not correct in $e$ (as $x < |\mathit{Corr}_{\mathcal{A}}(e')|$).
Thus, we can merge executions $e$ and $e'$ into an execution with $x \leq t$ faulty processes in which $P$ and $Q$ disagree.
Therefore, we reach a contradiction with the fact that $\mathcal{A}$ satisfies agreement while tolerating up to $t$ faulty processes, which concludes the proof of the lemma.
% The number of correct processes in $e$ is $c$, whereas the number of correct processes in $e'$ is $c'$.
% The number of correct processes in $e'$ is $\geq n - t$.
% Moreover, the number of processes which are correct in both $e_1$ and $e_2$ is $x$ such that (1) $x \leq t$, (2) $x < c$, and (3) $x < c'$.
% $< n - t$ and $\leq t$.
% Hence, there exists one process $P$ such that (1) $P$ is correct in $e$, and (2) $P$ is not correct in $e'$.
% Moreover, there exists another process $Q \neq P$ such that (1) $Q$ is correct in $e'$, and (2) $Q$ is not correct in $e$.
% Thus, we can merge executions $e$ and $e'$ into an execution with $x \leq t$ faulty processes in which $P$ and $Q$ disagree.
% The lemma holds.
\end{proof}  

We fix an input configuration with exactly $n - t$ process-proposal pairs; we denote this input configuration by $\mathit{base}$.
Let $E_{\mathit{base}}$ be an infinite execution of $\mathcal{A}$ such that (1) $E_{\mathit{base}}$ corresponds to $\mathit{base}$, and (2) all faulty processes ($t$ of them) crash immediately (i.e., without sending any message).
Let $\mathit{dec}$ be the value decided in $E_{\mathit{base}}$. 

\begin{lemma} \label{lemma:second_step}
$\mathit{compatible}(E_{\mathit{base}}) \neq \emptyset$.
\end{lemma}
\begin{proof}
Let us take a set $B$ of processes such that (1) $|B| = n - t$, and (2) $B$ contains all $t$ processes that do not belong to $\mathit{base}.\mathsf{processes}$.
Hence, $B \cap \mathit{base}.\mathsf{processes } = n - 2t$.
Moreover, $n - 2t \leq t$ as $n \leq 3t$.
Lastly, there exists a process $P \in B \setminus{\mathit{base}.\mathsf{processes}}$ (as $t > 0$ and $B$ contains $t$ processes which do not belong to $\mathit{base}.\mathsf{processes}$).
% Any two groups of $n - t$ processes intersect at at most $t$ processes as $n \leq 3t$.
% Indeed, $n - t + n - t - n \leq t$, which implies that $n - 2t \leq t$, which is always true as $n \leq 3t$.
% Furthermore, there exists a process $P$ which is faulty in $E_{\mathit{base}}$ as $t > 0$.
Hence, there exists an infinite execution $e$ such that (1) exactly $n - t$ processes are correct in $e$ (processes from the group $B$), (2) $P \in B$ is correct in $e$, and (3) all faulty processes ($t$ of them) crash immediately.
Moreover, $e$ and $E_{\mathit{base}}$ are compatible (by \Cref{definition:compatible_executions}).
Thus, the lemma.
\end{proof}


% By \Cref{lemma:first_step}, $\mathit{dec}$ must be decided in every execution of $\mathit{compatible}(e)$.
% Furthermore, $\mathit{dec} \in \mathit{val}(i)$, for every input configuration $i \in \allconfigurations$ that corresponds to an execution which belongs to $\mathit{compatible}(e)$.
% We now show that $\mathit{dec} \in \mathit{val}(i')$, for every $i' \in \allconfigurations$.

\begin{theorem} 
For every input configuration $i \in \allconfigurations$, $\mathit{dec} \in \mathit{val}(i)$.
\end{theorem}
\begin{proof}
By \Cref{lemma:second_step}, $\mathit{compatible}(E_{\mathit{base}}) \neq \emptyset$.
By \Cref{lemma:first_step}, $\mathit{dec}$ is decided in every execution compatible with $E_{\mathit{base}}$.
We fix one such execution; let this execution be denoted by $E_{i'} \in \mathit{compatible}(E_{\mathit{base}})$.
Let $x = |\mathit{Corr}_{\mathcal{A}}(E_{\mathit{base}}) \cap \mathit{Corr}_{\mathcal{A}}(E_{i'})|$.
As $e \in \mathit{compatible}(E_{\mathit{base}})$, we have: (1) $x \leq t$, (2) $x < |\mathit{Corr}_{\mathcal{A}}(E_{\mathit{base}})|$, and (3) $x < |\mathit{Corr}_{\mathcal{A}}(E_{i'})|$. 
Let $i'$ be an input configuration which corresponds to $E_{i'}$.
Recall that $\mathit{dec}$ is decided in $E_{i'}$.
% As $\mathit{dec}$ is decided in $e$, $\mathit{dec} \in \mathit{val}(i')$.

Let $i \in \allconfigurations$ be any input configuration.
Let $y = |i.\mathsf{processes} \cap i'.\mathsf{processes}|$.
We consider two possible cases:
\begin{compactitem}
   \item Let (1) $y \leq t$, (2) $y < |i.\mathsf{processes}|$, and (3) $y < |i'.\mathsf{processes}|$.
   Let $E_i$ be an infinite execution of $\mathcal{A}$ such that (1) $E_i$ corresponds to $i$, and (2) all faulty processes (if any) crash immediately.
   Hence, $E_i$ and $E_{i'}$ are compatible (by \Cref{definition:compatible_executions}).
   As $\mathit{dec}$ is decided in $E_{i'}$, $\mathit{dec}$ is decided in $E_i$ (by \Cref{lemma:first_step}).
   Therefore, $\mathit{dec} \in \mathit{val}(i)$, which concludes this case.
   
   \item Let (1) $y > t$, or (2) $y \geq |i.\mathsf{processes}|$, or (3) $y \geq |i'.\mathsf{processes}|$.
   We further distinguish three cases:
   \begin{compactitem}
        \item Let $y > t$.
        We build an input configuration $i^* \in \allconfigurations$ in the following manner:
        \begin{compactenum}
            \item For every process $P_j \in \Psi$:
            \begin{compactenum}
                \item If $P_j \in i.\mathsf{processes} \cap i'.\mathsf{processes}$, then (1) $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i$, and (2) go to step 1.
                
                \item If $P_j \in i'.\mathsf{processes}$, then $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i'$.
            \end{compactenum}
        \end{compactenum}
        Let $E^*$ be an infinite execution of $\mathcal{A}$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (if any) crash immediately.
        We have that $i^*.\mathsf{processes} = i'.\mathsf{processes}$ (by construction of $i^*$).
        Therefore, $E^*$ and $E_{\mathit{base}}$ are compatible (as $E_{i'}$ and $E_{\mathit{base}}$ are compatible).
        Hence, $\mathit{dec}$ is decided in $E^*$ (by \Cref{lemma:first_step}).
        
        Lastly, for every process $P$ such that (1) $P$ is correct in $E^*$, and (2) $P \in i.\mathsf{processes}$, $P$'s proposal in $E^*$ is identical to its proposal as specified by $i$ (follows from the construction of $i^*$).
        Hence, we can create an execution $E_i$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process $P \in i.\mathsf{processes}$ that decides in $E^*_{\mathit{prefix}}$.
            Such a prefix of $E^*$ exists as $y > t > 0$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, all processes that belong to $i.\mathsf{processes}$ are correct and live and have the proposals as specified by $i$.
            All other processes crash (if not have crashed before).
        \end{compactenum}
        Therefore, the following holds for $E_i$: (1) $E_i$ corresponds to $i$, and (2) $\mathit{dec}$ is decided in $E_i$.
        Thus, $\mathit{dec} \in \mathit{val}(i)$, which confirms the statement of the lemma in this case.
        
        \item Let $y \geq |i.\mathsf{processes}|$.
        Hence, $y = |i.\mathsf{processes}|$, which means that, for every process $P \in i.\mathsf{processes}$, $P \in i'.\mathsf{processes}$.
        We build an input configuration $i^* \in \allconfigurations$ in the following manner:
        \begin{compactenum}
            \item For every process $P_j \in \Psi$:
            \begin{compactenum}
                \item If $P_j \in i.\mathsf{processes} \cap i'.\mathsf{processes}$, then (1) $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i$, and (2) go to step 1.
                
                \item If $P_j \in i'.\mathsf{processes}$, then $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i'$.
            \end{compactenum}
        \end{compactenum}
        Let $E^*$ be an infinite execution of $\mathcal{A}$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (if any) crash immediately.
        We have that $i^*.\mathsf{processes} = i'.\mathsf{processes}$ (by the construction of $i^*$).
        Therefore, $E^*$ and $E_{\mathit{base}}$ are compatible (because $E_{i'}$ and $E_{\mathit{base}}$ are compatible).
        Thus, $\mathit{dec}$ is decided in $E^*$ (by \Cref{lemma:first_step}).
        
        For every process $P$ such that (1) $P$ is correct in $E^*$, and (2) $P \in i.\mathsf{processes}$, $P$'s proposal in $E^*$ is identical to its proposal as specified by $i$ (follows from the construction of $i^*$).
        Hence, we can create an execution $E_i$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process $P \in i.\mathsf{processes}$ that decides in $E^*_{\mathit{prefix}}$.
            Such a process exists as every process that belongs to $i.\mathsf{processes}$ also belongs to $\mathit{Corr}_{\mathcal{A}}(E^*)$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, all processes that belong to $i.\mathsf{processes}$ are correct and live and have the proposals as specified by $i$.
            All other processes crash (if not have crashed before).
        \end{compactenum}
        Therefore, (1) $E_i$ corresponds to $i$, and (2) $\mathit{dec}$ is decided in $E_i$.
        Thus, $\mathit{dec} \in \mathit{val}(i)$.
        
        \item Let $y \geq |i'.\mathsf{processes}|$.
        Hence, $y = |i'.\mathsf{processes}|$, which means that, for every process $P \in i'.\mathsf{processes}$, $P \in i.\mathsf{processes}$.
        We build an input configuration $i^* \in \allconfigurations$ in the following manner:
        \begin{compactenum}
            \item For every process $P_j \in \Psi$:
            \begin{compactenum}
                \item If $P_j \in i.\mathsf{processes} \cap i'.\mathsf{processes}$, then $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i$.
            \end{compactenum}
        \end{compactenum}
        Let $E^*$ be an infinite execution of $\mathcal{A}$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (if any) crash immediately.
        We have that $i^*.\mathsf{processes} = i'.\mathsf{processes}$ (by the construction of $i^*$).
        Therefore, $E^*$ and $E_{\mathit{base}}$ are compatible (because $E_{i'}$ and $E_{\mathit{base}}$ are compatible).
        Thus, $\mathit{dec}$ is decided in $E^*$ (by \Cref{lemma:first_step}).
        
        For every process $P$ such that (1) $P$ is correct in $E^*$, and (2) $P \in i.\mathsf{processes}$, $P$'s proposal in $E^*$ is identical to its proposal as specified by $i$ (follows from the construction of $i^*$).
        Hence, we can create an execution $E_i$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process $P \in i.\mathsf{processes}$ that decides in $E^*_{\mathit{prefix}}$.
            Such a process exists as every process that belongs to $\mathit{Corr}_{\mathcal{A}}(E^*)$ also belongs to $i.\mathsf{processes}$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, all processes that belong to $i.\mathsf{processes}$ are correct and live and have the proposals as specified by $i$.
            All other processes crash (if not have crashed before).
        \end{compactenum}
        Therefore, (1) $E_i$ corresponds to $i$, and (2) $\mathit{dec}$ is decided in $E_i$.
        Thus, $\mathit{dec} \in \mathit{val}(i)$.
   \end{compactitem}
\end{compactitem}
We have shown that, for every input configuration $i \in \allconfigurations$, $\mathit{dec} \in \mathit{val}(i)$.
Thus, the theorem.
\end{proof}

\begin{corollary} \label{corollary:trivial_validity}
Let $\mathit{val}$ be any satisfiable validity property.
Let $n \leq 3t$.
Then, $\mathit{val}$ is a trivial validity property, i.e., there exists a value $v \in \mathcal{V}$ such that, for every input configuration $i \in \allconfigurations$, $v \in \mathit{val}(i)$.
\end{corollary}


\iffalse
Let $\Pi \subseteq \Psi$ be any set of processes.
Moreover, let $x < |\Pi|$ be an integer.
We denote by $\mathit{execs}_{\mathcal{A}}(\Pi, x)$ a set of infinite executions of $\mathcal{A}$ such that (1) at most $x$ members of $\Pi$ does not crash immediately (i.e., without sending any message), and (2)  in every execution of $\mathit{execs}_{\mathcal{A}}(\Pi, x)$.
 




\paragraph{Let $n \leq 2t$.}
Let $\Pi \subseteq \Psi$ be any set of processes.
We denote by $\mathit{execs}_{\mathcal{A}}(\Pi)$ a set of infinite executions of $\mathcal{A}$ such that all processes from $\Pi$ crash immediately (i.e., without sending any message) in every execution of $\mathit{execs}_{\mathcal{A}}(\Pi)$.

We fix an input configuration $\mathit{input} \in \allconfigurations$ such that $\mathit{input}$ consists of exactly $n - t$ process-proposal pairs.
Let $\Pi$ denote the set of processes that belong to $\mathit{input}$; recall that $|\Pi| = n - t$.
We show that there exists a value $x \in \mathcal{V}$ such that (1) $x \in \mathit{val}(\mathit{input})$, and (2) $x$ is decided in every execution that belongs to $\mathit{execs}_{\mathcal{A}}(\Pi)$.

\begin{lemma}
Let $\mathit{input} \in \allconfigurations$ be any input configuration such that $|\mathit{input}| = n - t$.
Let $\Pi$ denote the set of processes associated with $\mathit{input}$; $|\Pi| = n - t$.
There exists a value $x \in \mathit{val}(\mathit{input})$ such that $x$ is decided in every execution $e$ that belongs to $\mathit{execs}_{\mathcal{A}}(\Pi)$.\footnote{Recall that $\mathit{execs}_{\mathcal{A}}(\Pi) \neq \emptyset$ as $n \leq 2t$.}
\end{lemma}
\begin{proof}
First, we show that, in every execution that belongs to $\mathit{execs}_{\mathcal{A}}(\Pi)$, the decided value belongs to $\mathit{val}(\mathit{input})$.
By contradiction, let there exist an infinite $e \in \mathit{execs}_{\mathcal{A}}(\Pi)$ such that the decided value is $v \notin \mathit{val}(\mathit{input})$.
Let $\mathit{input}' \in \allconfigurations$ be an input configuration that corresponds to $e$.
We denote by $e^*$ the prefix of $e$ in which a process $P$ decides $v \notin \mathit{val}(\mathit{input})$.

Now, consider any execution $E$ that corresponds to $\mathit{input}$ in which all faulty processes (per $\mathit{input}$) crash immediately (i.e., without sending any messages).
As $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$, processes decide a value $v' \in \mathit{val}(\mathit{input})$ in $E$.
Hence, we can merge executions $e^*$ and $E$ to construct another execution in which two correct processes disagree (as one decides $v$ and another $v'$ such that $v \neq v'$). 
Thus, in every execution that belongs to $\mathit{execs}_{\mathcal{A}}(\Pi)$, the decided value belongs to $\mathit{val}(\mathit{input})$.

Finally, by contradiction, let there exist executions $e_1, e_2 \in \mathit{execs}_{\mathcal{A}}(\Pi)$ such that (1) the decided value in $e_1$ is $v_1 \in \mathit{val}(\mathit{input})$, (2) the decided value in $e_2$ is $v_2 \in \mathit{val}(\mathit{input})$, and (3) $v_1 \neq v_2$.
Let us take one execution $E$ that corresponds to $\mathit{input}$ in which all faulty processes (per $\mathit{input}$) crash without sending any message.
Hence, the value decided in $E$ is different from $v_1$ or different from $v_2$.
If it is different from $v_1$, we can merge executions $E$ and $e_1$ to reach disagreement.
Otherwise, we can merge executions $E$ and $e_2$ to reach disagreement.
Therefore, the lemma holds.
\end{proof}
\fi
\fi

==> sections/crash-stop.tex <==
\section{Validity Properties In The Crash-Stop Failure Model}

In this section, we take a closer look at the validity properties of the consensus problem in the crash-stop failure model.

\subsection{Preliminaries}

\paragraph{System model.}
We consider a static system $\Psi = \{P_1, ..., P_n\}$ of $n$ processes among which $f < n$ processes can fail by \emph{crashing}.
If a process crashes, the process is \emph{faulty}; otherwise, the process is \emph{correct}.
This failure model is known as the \emph{crash-stop} failure model.

\paragraph{Crash-stop consensus.}
Each process has its \emph{proposal}, and it should eventually \emph{decide}.
We denote by $\mathcal{V}$ the set of values a process can propose and decide.
The consensus problem in the crash-stop failure model requires the following three properties to hold:
\begin{compactitem}
    \item \emph{Agreement:} No two processes decide different values.
    
    \item \emph{Termination:} Every correct process eventually decides.
    
    \item \emph{Validity}
\end{compactitem}

\paragraph{Validity property.}
First, we define a \emph{process-proposal} pair as a pair $(P_x, \mathit{val}_x)$, where (1) $P_x$ is either $P \in \Psi$ or $\bar{P}$, with $P \in \Psi$, and (2) $\mathit{val}_x \in \mathcal{V}$ is a value.
Intuitively, $(P, \mathit{val})$ denotes that a \emph{correct} process $P \in \Psi$ has proposed a value $\mathit{val} \in \mathcal{V}$; on the other hand, $(\bar{P}, \mathit{val}')$ denotes that a \emph{faulty} process $P \in \Psi$ has proposed a value $\mathit{val}' \in \mathcal{V}$.
We denote by $\mathit{pp}.\mathsf{process}$ the process associated with a process-proposal $\mathit{pp}$, whereas $\mathit{pp}.\mathsf{proposal}$ denotes the proposal associated with $\mathit{pp}$.
Finally, $\mathit{pp}.\mathsf{correct}$ returns $\top$ if and only if $\mathit{pp}$ is associated with a correct processes; $\mathit{pp}.\mathsf{correct}$ returns $\bot$ otherwise.

Next, an \emph{input configuration} is a tuple $\big[ \mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_n \big]$, where (1) $\mathit{pp}_i$ is a process-proposal, for every $i \in [1, n]$, (2) every process-proposal pair is associated with a distinct process, and (3) at most $f$ process-proposals refer to faulty processes (i.e., there can exist at most $f$ process-proposals of the format $(\bar{P}, v)$, where $P \in \Psi$ and $v \in \mathcal{V}$).
We denote by $\mathcal{I}$ the set of all possible input configurations.
For every input configuration $\mathit{input} \in \mathcal{I}$ and every $i \in [1, n]$, we denote by $\mathit{input}[i]$ the process-proposal pair associated with process $P_i$.

Furthermore, $\mathit{correct}(\mathit{input} \in \mathcal{I}) = \{P \in \Psi \,|\, \mathit{pp} \text{ belongs to } \mathit{input} \land \mathit{pp}.\mathsf{process} = P \land \mathit{pp}.\mathsf{correct} = \top\}$ denotes the set of correct processes as established by $\mathit{input}$.
We define $\mathit{identical\_proposals}: \mathcal{I} \times \mathcal{I} \to \{\top, \bot\}$ in the following manner:
\begin{equation*}
    \mathit{identical\_proposals}(i_1, i_2) = \top \iff \forall j \in [1, n]: i_1[j].\mathsf{proposal} = i_2[j].\mathsf{proposal}.
\end{equation*}

We define a \emph{validity property} $\mathit{val}$ as a function $\mathcal{I} \to 2^{\mathcal{V}}$ such that, for every $\mathit{input} \in \mathcal{I}$, $\mathit{val}(\mathit{input}) \neq \emptyset$.
Finally, we say that a crash-stop consensus algorithm $\mathcal{A}_C$ satisfies a validity property $\mathit{val}$ if and only if the following holds:
\begin{compactitem}
    \item \emph{Validity safety:} In every execution $e$ of $\mathcal{A}_C$, $\mathit{dec}_e \in \mathit{val}(\mathit{input})$, where (1) $\mathit{dec}_e$ is the decided value in $e$, and (2) $\mathit{input}$ is the input configuration that corresponds to $e$.
    
    \item \emph{Validity liveness:} For every input configuration $\mathit{input} \in \mathcal{I}$ and every value $v \in \mathit{val}(\mathit{input})$, there exists an execution $e$ of $\mathcal{A}_C$ such that (1) $e$ corresponds to $\mathit{input}$, and (2) the decided value in $e$ is $v$.
\end{compactitem}


% Finally, we say that a crash-stop consensus algorithm $\mathcal{A}_C$ satisfies a validity property $\mathit{val}$ if and only if, in every execution $e$ of $\mathcal{A}_C$, $\mathit{dec}_e \in \mathit{val}(\mathit{input})$, where (1) $\mathit{dec}_e$ is the decided value in $e$, and (2) $\mathit{input}$ is the input configuration that corresponds to $e$.

% \paragraph{Core valid values.}
% Consider a crash-stop consensus algorithm $\mathcal{A}_C$ that satisfies a validity property $\mathit{val}$.
% Let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
% We say that a value $v \in \mathit{val}(\mathit{input})$ is a \emph{core valid value} of $\mathit{input}$ in $\mathcal{A}_C$ if and only if there exists an execution $e$ of $\mathcal{A}_C$ such that (1) $e$ corresponds to $\mathit{input}$, and (2) the decided value in $e$ is $v$.
% We denote by $\mathit{core}(\mathcal{A}_C, \mathit{input})$ the set of core valid values of $\mathit{input}$ in $\mathcal{A}_C$; note that $\mathit{core}(\mathcal{A}_C, \mathit{input}) \subseteq \mathit{val}(\mathit{input})$.

% Why do we define core valid values?
% Consider an input configuration $\mathit{input} \in \mathcal{I}$.
% Since $\mathcal{A}_C$ satisfies $\mathit{val}$, $\mathcal{A}_C$ satisfies $\mathit{val}'$, which is a validity property identical to $\mathit{val}$, except that $\mathit{val}'(\mathit{input}) = \mathit{val}(\mathit{input}) \cup \{v^*\}$, where $v^* \notin \mathit{val}(\mathit{input})$.
% Indeed, $\mathcal{A}_C$ satisfies $\mathit{val}'$; however, $\mathcal{A}_C$ never decides $v^*$ in an execution that corresponds to $\mathit{input}$.
% Therefore, $v^*$ is not ``important'' to $\mathcal{A}_C$; we say that $v^*$ is \emph{not} a core valid value of $\mathit{input}$ in $\mathcal{A}_C$.
% In the rest of the section, we will usually talk about validity properties from the lenses of their core valid values.
 
\subsection{Synchronous Environments}

First, we investigate validity properties of crash-stop consensus in a synchronous setting.

\paragraph{Communication.}
In a synchronous environment, there exists an upper bound $\Delta$ on message delays between processes.
In other words, if a correct process sends a message to another correct process at time $t$, the message will be received by time $t + \Delta$; note that the message might be received at time $t^* \in [t, t + \Delta]$ (the actual message delay for each message is chosen by the adversary).

\paragraph{Necessary conditions.}
First, we define when two input configurations are similar.
Specifically, for every input configuration $\mathit{input} \in \mathcal{I}$, we define $\mathit{Sim}(\mathit{input})$ in the following manner:
\begin{equation*}
    \mathit{Sim}(\mathit{input}) = \{i' \in \mathcal{I} \,|\, \forall j \in [1, n]: \mathit{input}[j].\mathsf{correct} = \top \lor \mathit{i'}[j].\mathsf{correct} = \top \implies \mathit{input}[j] = \mathit{i'}[j]\}.
\end{equation*}
In other words, $i' \in \mathit{Sim}(\mathit{input})$ if and only if both input configurations have the identical ``set'' of process-proposals concerned with correct processes.
Note that $\mathit{Sim}(\mathit{input}) = \{\mathit{input}\}$ if, for every $j \in [1, n]$, $\mathit{input}[j].\mathsf{correct} = \top$.
Next, we introduce the \emph{similarity condition}.

\begin{definition} [Similarity condition] \label{definition:similarity_crash}
Let $\mathit{val}$ be a validity property.
% Let $\mathit{input} \in \mathcal{I}$ be an input configuration.
% We define $\mathit{Sim}(\mathit{input}) = \{\mathit{input'} \in \mathcal{I} \,|\, \text{all process-proposals concerned with correct processes are identical in } \mathit{input} \text{ and } \mathit{input}'\}$.
We say that $\mathit{val}$ satisfies the \emph{similarity condition} if and only if the following holds:
\begin{equation*}
    \forall \mathit{input} \in \mathcal{I}: \bigcap\limits_{i' \in \mathit{Sim}(\mathit{input})} \big(\mathit{val}(i')\big) \neq \emptyset.
\end{equation*}
\end{definition}

Now, we show that crash-stop consensus with a validity property that does not satisfy the similarity condition (\Cref{definition:similarity_crash}) cannot be satisfied by any algorithm.

\begin{lemma} [Similarity condition is necessary] \label{lemma:similarity_necessary_crash}
Let $\mathit{val}$ be a validity property that does not satisfy the similarity condition.
No algorithm (even if synchronous) solves the crash-stop consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the similarity condition, there exists an input configuration $i \in \mathcal{I}$ such that $\bigcap\limits_{i' \in \mathit{Sim}(i)} \big( \mathit{val}(i') \big) = \emptyset$ (by \Cref{definition:similarity_crash}).
Note that $i$ does not contain only process-proposals concerned with correct processes; otherwise, $\bigcap\limits_{i' \in \mathit{Sim}(i)} \neq \emptyset$ as $\mathit{Sim}(i) = \{i\}$.
By contradiction, suppose that there exists a crash-stop consensus algorithm $\mathcal{A}_C$ that satisfies $\mathit{val}$.
Without loss of generality, let $\mathcal{A}_C$ be a synchronous algorithm.

Consider an execution $e$ of $\mathcal{A}_C$ that corresponds to $i$ (i.e., all processes propose the values as established by $i$, and $i$ establishes which processes are correct and which are faulty) such that all faulty processes in $e$ crash immediately (without sending any message); recall that there are faulty processes in $e$ as $i$ does not contain only process-proposals concerned with correct processes.
Let the decided value in $e$ be $\mathit{dec}_e$.
Importantly, there exists an input configuration $i' \in \mathit{Sim}(i)$ such that $\mathit{dec}_e \notin \mathit{val}(i')$ (otherwise, the similarity condition would be satisfied for $i$).
Again, note that there exist some faulty processes according to $i'$ (since there exist faulty processes according to $i$).

Now, we create an execution $e'$ of $\mathcal{A}_C$ such that (1) $e'$ corresponds to $i'$, and (2) the decided value in $e'$ is $\mathit{dec}_e \notin \mathit{val}(i')$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item For each process who is faulty according to $e'$ (and $e$), we set its proposed value according to $e'$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $\mathit{dec}_e \notin \mathit{val}(i')$, which means that $\mathcal{A}_C$ does not satisfy the validity property in the execution $e'$ (as the validity safety property is not satisfied).
This contradicts the fact that $\mathcal{A}_C$ satisfies the validity property $\mathit{val}$, which concludes the lemma.
\end{proof}

Next, we define the \emph{containment condition}.

\begin{definition} [Containment condition] \label{definition:containment_crash}
Let $\mathit{val}$ be a validity property.
% and let $\mathcal{A}_C$ be an algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
We say that $\mathit{val}$ satisfies the \emph{containment condition} if and only if the following holds:
\begin{equation*}
    \forall i_1, i_2 \in \mathcal{I}: \big(\mathit{identical\_proposals}(i_1, i_2) = \top \land \mathit{correct}(i_1) \subseteq \mathit{correct}(i_2)\big) \implies \mathit{val}(i_2) \subseteq \mathit{val}(i_1).
\end{equation*}
% \begin{equation*}
%     \forall i_1, i_2 \in \mathcal{I}: \big(\mathit{identical\_proposals}(i_1, i_2) = \top \land \mathit{correct}(i_1) \subseteq \mathit{correct}(i_2)\big) \implies \mathit{core}(\mathcal{A}_C, i_2) \subseteq \mathit{val}(i_1).
% \end{equation*}
\end{definition}

Next, we show that the containment condition is necessary for a validity property to be ``satisfiable''.

\begin{lemma} [Containment condition is necessary] \label{lemma:containment_necessary_crash}
Let $\mathit{val}$ be a validity property that does not satisfy the containment condition.
No algorithm (even if synchronous) solves the crash-stop consensus problem with $\mathit{val}$.
% Let $\mathit{val}$ be a validity property and let $\mathcal{A}_C$ be an algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
% Then, $\mathit{val}$ satisfies the containment condition with respect to $\mathcal{A}_C$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the containment condition, there exist two input configurations $i_1, i_2 \in \mathcal{I}$ such that (1) $\mathit{identical\_proposals}(i_1, i_2) = \top$, (2) $\mathit{correct}(i_1) \subseteq \mathit{correct}(i_2)$, and (3) $\mathit{val}(i_2) \not\subseteq \mathit{val}(i_1)$.
In other words, there exists a value $x \in \mathcal{V}$ such that $x \in \mathit{val}(i_2)$ and $x \notin \mathit{val}(i_1)$.

By contradiction, suppose that there exists a crash-stop algorithm $\mathcal{A}_C$ that satisfies $\mathit{val}$.
Without loss of generality, let $\mathcal{A}_C$ be a synchronous algorithm.

Since $\mathcal{A}_C$ satisfies $\mathit{val}$, there exists an execution $e$ of $\mathcal{A}_C$ that corresponds to the input configuration $i_2$ in which the decided value is $x$ (due to the validity liveness).
We now create an execution $e'$ such that (1) $e'$ corresponds to $i_1$, and (2) the decided value in $e'$ is $x \notin \mathit{val}(i_1)$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item After the first process decides in $e'$, we crash all processes which are correct according to $i_2$ and faulty according to $i_1$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $x \notin \mathit{val}(i_1)$, which means that $\mathcal{A}_C$ does not satisfy $\mathit{val}$ in $e'$.
This contradicts the fact that $\mathcal{A}_C$ satisfies $\mathit{val}$, which concludes the lemma.
\end{proof}

% Hence, the similarity and containment conditions are necessary for a validity property to be ``satisfiable''.

% \begin{corollary}
% Let $\mathit{val}$ be a validity property for which there exists an algorithm $\mathcal{A}_C$ which solves the crash-stop consensus problem with $\mathit{val}$.
% Then, $\mathit{val}$ satisfies both similarity and containment conditions.
% % Then, $\mathit{val}$ satisfies both (1) the similarity condition, and (2) the containment condition with respect to $\mathcal{A}_C$.
% \end{corollary}

\paragraph{Sufficient conditions.}
We now show that the similarity and containment conditions are sufficient for a validity property to be satisfiable.

\begin{theorem} [Similarity and containment conditions are sufficient]
Let $\mathit{val}$ be a validity property that satisfies the similarity and the containment conditions.
There exists an algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a synchronous crash-stop consensus algorithm $\mathcal{A}_C$ (\Cref{algorithm:synchronous_crash_stop}) that solves consensus with $\mathit{val}$.

\begin{algorithm}
\caption{Crash-stop algorithm $\mathcal{A}_C$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:synchronous_crash_stop}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Synchronous Crash-Stop Consensus, \textbf{instance} $c$

\medskip
\State \textbf{At time $0$:}
\State \hskip2em \textbf{broadcast} $[\textsc{proposal}, \mathit{proposal}]$

\medskip
\State \textbf{At time $\Delta$:}
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
\State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:build_i}
\State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
\State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
\State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
\State \hskip2em \textbf{else:} 
\State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{Sim}(i)$ \label{line:set_to_propose}
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:propose_c}

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_C$ (\Cref{algorithm:synchronous_crash_stop}) solves the consensus problem with $\mathit{val}$.
First, termination and agreement follow directly from termination and agreement of a black-box synchronous crash-stop consensus (instance $c$ in \Cref{algorithm:synchronous_crash_stop}).
Hence, it is left to show that $\mathcal{A}_C$ satisfies $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \mathcal{I}$.
We first show that $\mathcal{A}_C$ satisfies the validity safety.
Let $P \in \Psi$ be a process that proposes to $c$ (at line~\ref{line:propose_c}) and let $i$ be the ``input configuration'' $P$ constructs at line~\ref{line:build_i} (if $P$ does not hear from all processes, $i$ is not, technically speaking, an input configuration as it does not contain $n$ process-proposals).
We separate two cases:
\begin{compactitem}
    \item $P$ receives \textsc{proposal} messages from all processes:
    In this case, we have that $\mathit{identical\_proposals}(i, \mathit{input}) = \top$.
    Moreover, $\mathit{correct}(\mathit{input}) \subseteq \mathit{correct}(i)$.
    Since $\mathit{to\_propose} \in \mathit{val}(i)$, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$ (as $\mathit{val}$ satisfies the containment property). 
    Hence, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$ in this case.
    
    \item $P$ does not receive \textsc{proposal} messages from all processes:
    In this case, $i$ does not contain proposals from all $n$ processes (i.e., $i$ is not, strictly speaking, an input configuration).
    Let $i^*$ be an input configuration identical to $i$, except that, for all processes whose proposal is missing in $i$, we add the process-proposal established by $\mathit{input}$; observe that all processes whose proposal is missing in $i$ are faulty according to $\mathit{input}$.
    
    Now, we ``extend'' $i$ by adding process-proposals associated with processes from which $P$ has not heard, i.e., for every $P' \in \Psi$ from which $P$ has not heard, we add $(\bar{P'}, \text{any value})$ to $i$.
    Observe that $i^* \in \mathit{Sim}(i)$.
    
    Let $\mathit{to\_propose} = v$ (set at line~\ref{line:set_to_propose}).
    Hence, $v \in \mathit{val}(i^*)$ (as $i^* \in \mathit{Sim}(i)$).
    
    Furthermore, we have that $\mathit{identical\_proposals}(i^*, \mathit{input}) = \top$ and $\mathit{correct}(\mathit{input}) \subseteq \mathit{correct}(i^*)$.
    According to the containment condition, $v \in \mathit{val}(\mathit{input})$.
\end{compactitem}
In both possible cases, we have that $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$.
Hence, for every value $v$ proposed to the black-box synchronous consensus $c$, $v \in \mathit{val}(\mathit{input})$.
Given that $c$ decides only proposed values, the decided value must belong to $\mathit{val}(\mathit{input})$.
Thus, the validity safety is satisfied by \Cref{algorithm:synchronous_crash_stop}.

It is left to show that the validity liveness is satisfied.
In order to solve the validity liveness, $\mathcal{A}_C$ relies on time (importantly, $\mathcal{A}_C$ can avoid relying on time if $|\mathit{val}(\mathit{input})| < \infty$, for every $\mathit{input} \in \mathcal{I}$; we leave this modification for the future work).
We assume that the function mapping time to values is the same at all processes.

Again, let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
We need to show that, for every value $v \in \mathit{val}(\mathit{input})$, there exists an execution that corresponds to $\mathit{input}$ in which the decided value is $v$.
Hence, let us fix a value $v \in \mathit{val}(\mathit{input})$.
We construct an execution $e$ that corresponds to $\mathit{input}$ in which the decided value is $v$:
\begin{compactenum}
    \item All processes propose their values according to $\mathit{input}$.
    
    \item The first \textsc{proposal} message at each process is received at the \emph{exactly} the same time that maps to $v$.
    
    \item Once all processes have decided from $c$, all processes faulty according to $\mathit{input}$ crash.
\end{compactenum}
Since all processes receive the first \textsc{proposal} message at the same time (which maps to $v$), all processes propose $v$ to $c$.
Hence, the decided value must be $v$ (due to the validity property of $c$).
The validity liveness property is satisfied, which concludes the theorem.
\end{proof}

\subsection{Partially Synchronous Environments}

Next, we investigate validity properties of crash-stop consensus in a partially synchronous setting.

\paragraph{Communication.}
In a partially synchronous environment, there exists an unknown time Global Stabilization Time (GST) such that the system behaves asynchronously before GST, and behaves synchronously after GST.
Formally, there exist a known upper bound $\delta$ on message delays after GST.

\paragraph{Necessary conditions.}
First, note that the similarity and containment conditions are necessary for a validity property to be satisfied in a partially synchronous environment (as these conditions are necessary in a synchronous setting).
We now define when an input configuration is ``correct-similar'' to another configuration.
Formally, for every input configuration $\mathit{input} \in \mathcal{I}$, we define $\mathit{CorrectSim}(\mathit{input})$ in the following manner:
\begin{equation*}
    \mathit{CorrectSim}(\mathit{input}) = \{i' \in \mathcal{I} \,|\, \forall j \in [1, n]: \mathit{input}[j].\mathsf{correct} = \top \implies \mathit{input}[j].\mathsf{proposal} = i'[j].\mathsf{proposal}\}.
\end{equation*}
In other words, an input configuration $i' \in \mathcal{I}$ is \emph{correct-similar} to $\mathit{input}$ if proposed values of processes correct according to $\mathit{input}$ are identical in $i'$ and $\mathit{input}$.

Observe that $i_1 \in \mathit{CorrectSim}(i_2)$ does not imply $i_2 \in \mathit{CorrectSim}(i_1)$.
For example, let $i_1 = \big[(P_1, v_1), (P_2, v_2), (\bar{P}_3, v_3)\big]$ and $i_2 = \big[(\bar{P}_1, v_1), (P_2, v_2), (P_3, v_3')\big]$.
We have that $i_2 \in \mathit{CorrectSim}(i_1)$, but $i_1 \notin \mathit{CorrectSim}(i_2)$.
Next, we introduce the \emph{correct-similarity condition}.

\begin{definition} [Correct-similarity condition] \label{definition:correct_similarity}
Let $\mathit{val}$ be a validity property.
% Let $\mathit{input} \in \mathcal{I}$ be an input configuration.
% We define $\mathit{AlmostSim}(\mathit{input}) = \{\mathit{input}' \in \mathcal{I} \,|\, \text{proposed values of processes correct according to } i \text{ are identical}\}$.
We say that $\mathit{val}$ satisfies the \emph{correct-similarity condition} if and only if the following holds:
\begin{equation*}
    \forall \mathit{input} \in \mathcal{I}: \bigcap\limits_{i' \in \mathit{CorrectSim}(\mathit{input})} \big(\mathit{val}(i')\big) \neq \emptyset.
\end{equation*}
\end{definition}

% Note that, if all processes are correct according to $i \in \mathcal{I}$, $\mathit{AlmostSim}(i)$ contains input configurations $i' \in \mathcal{I}$ such that $\mathit{identical\_proposals}(i, i') = \top$ and $\mathit{correct}(i') \subseteq \mathit{correct}(i)$.
We now show that the correct-similarity condition is necessary in a partially synchronous setting.

\begin{lemma} [Correct-similarity condition is necessary] \label{lemma:correct_similarity_necessary_crash}
Let $\mathit{val}$ be a validity property that does not satisfy the correct-similarity condition.
No partially synchronous algorithm solves the crash-stop consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the correct-similarity condition, there exists an input configuration $i \in \mathcal{I}$ such that $\bigcap\limits_{i' \in \mathit{CorrectSim}(i)} \big( \mathit{val}(i') \big) = \emptyset$ (by \Cref{definition:correct_similarity}).
By contradiction, suppose that there exists a partially synchronous crash-stop consensus algorithm $\mathcal{A}_C$ that satisfies $\mathit{val}$.

Consider an execution $e$ of $\mathcal{A}_C$ that corresponds to $i$ (i.e., all processes propose the values as established by $i$, and $i$ establishes which processes are correct and which are faulty) such that all faulty processes in $e$ crash immediately (without sending any message); observe that there might be no faulty processes in $e$ (according to $i$).
Let the decided value in $e$ be $\mathit{dec}_e$.
Importantly, there exists an input configuration $i' \in \mathit{CorrectSim}(i)$ such that $\mathit{dec}_e \notin \mathit{val}(i')$ (otherwise, the correct-similarity condition would be satisfied for $i$).

Now, we create an execution $e'$ of $\mathcal{A}_C$ such that (1) $e'$ corresponds to $i'$, and (2) the decided value in $e'$ is $\mathit{dec}_e \notin \mathit{val}(i')$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    We adjust the proposals according to $i'$.
    
    \item No process correct in $e$ hears from any process $P \in \Psi$ in $e'$ until a value is decided in $e'$, where $P$ is faulty in $e$ (i.e., according to $i$) and correct in $e'$ (i.e., correct according to $i'$).
    
    \item After a decision has been made in $e'$, we crash all processes which are faulty according to $i'$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $\mathit{dec}_e \notin \mathit{val}(i')$, which means that $\mathcal{A}_C$ does not satisfy the validity property in the execution $e'$ (as the validity safety property is not satisfied).
This contradicts the fact that $\mathcal{A}_C$ satisfies the validity property $\mathit{val}$, which concludes the lemma.
\end{proof}

\paragraph{Sufficient conditions.}
Finally, we are ready to show that similarity, containment and correct-similarity conditions are sufficient for a validity property to be satisfiable in a partially synchronous setting.

\begin{theorem} [Similarity, containment and correct-similarity conditions are sufficient in partial synchrony]
Let $\mathit{val}$ be a validity property that satisfies similarity, containment and correct-similarity conditions.
There exists a partially synchronous algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a partially synchronous crash-stop consensus algorithm $\mathcal{A}_C$ (\Cref{algorithm:partially_synchronous_crash_stop}) that solves consensus with $\mathit{val}$.

\begin{algorithm}
\caption{Partially synchronous crash-stop algorithm $\mathcal{A}_C$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:partially_synchronous_crash_stop}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Partially Synchronous Crash-Stop Consensus, \textbf{instance} $c$

\medskip
\State \textbf{upon} $\mathsf{start}$:
\State \hskip2em \textbf{broadcast} $[\textsc{proposal}, \mathit{proposal}]$

\medskip
\State \textbf{upon} reception of $n - f$ \textsc{proposal} messages:
\State \hskip2em \textbf{trigger} timer for $\Delta$ time \Comment{$\Delta$ is some predefined constant}

\medskip
\State \textbf{upon} timer elapsed:
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
\State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:partially_build_i}
\State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
\State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
\State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
\State \hskip2em \textbf{else:} 
\State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{CorrectSim}(i)$ \label{line:partially_set_to_propose}
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:partially_propose_c}

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_C$ (\Cref{algorithm:partially_synchronous_crash_stop}) solves the consensus problem with $\mathit{val}$.
First, termination and agreement follow directly from termination and agreement of a used partially synchronous crash-stop consensus (instance $c$ in \Cref{algorithm:partially_synchronous_crash_stop}).
Hence, it is left to show that $\mathcal{A}_C$ satisfies $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \mathcal{I}$.
We first show that $\mathcal{A}_C$ satisfies the validity safety.
Let $P$ be a process that proposes to $c$ (at line~\ref{line:partially_propose_c}) and let $i$ be the input configuration $P$ constructs at line~\ref{line:partially_build_i}; observe that, if $P$ does not receive \textsc{proposal} messages from all processes, $i$ is not, strictly speaking, an input configuration.
We ``extend'' $i$ by adding process-proposals associated with processes from which $P$ has not heard, i.e., for every $P' \in \Psi$ from which $P$ has not received a \textsc{proposal} message, we add $(\bar{P}', \text{any value})$ to $i$.
Importantly, $\mathit{input} \in \mathit{CorrectSim}(i)$.
Hence, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$.
Therefore, for every value $v$ proposed to the black-box partially synchronous consensus $c$, $v \in \mathit{val}(\mathit{input})$.
Given that $c$ decides only proposed values, the decided value must belong to $\mathit{val}(\mathit{input})$.
Thus, the validity safety is satisfied by \Cref{algorithm:partially_synchronous_crash_stop}.

It is left to show that the validity liveness is satisfied.
In order to solve the validity liveness, $\mathcal{A}_C$ relies on time (importantly, $\mathcal{A}_C$ can avoid relying on time if $|\mathit{val}(\mathit{input})| < \infty$, for every $\mathit{input} \in \mathcal{I}$).
We assume that the time maps to a value in the same way at all processes.

Again, let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
We need to show that, for every value $v \in \mathit{val}(\mathit{input})$, there exists an execution that corresponds to $\mathit{input}$ in which the decided value is $v$.
Hence, let us fix a value $v \in \mathit{val}(\mathit{input})$.
We construct an execution $e$ that corresponds to $\mathit{input}$ in which the decided value is $v$:
\begin{compactenum}
    \item All processes propose their values according to $\mathit{input}$.
    
    \item The first \textsc{proposal} message at each process is received at the \emph{exactly} the same time that maps to $v$.
    
    \item Once all processes have decided from $c$, all faulty processes crash.
\end{compactenum}
Since all processes receive the first \textsc{proposal} message at the same time (which maps to $v$), all processes propose $v$ to $c$.
Hence, the decided value must be $v$ (due to the validity property of $c$).
The theorem holds. 
\end{proof}

==> sections/crash.tex <==
\section{Validity Properties of the Crash-Stop Consensus}

In this section, we deal with the satisfiability of the validity properties of the crash-stop consensus problem.
First, we formally define a validity property of the crash-stop consensus (\Cref{subsection:crash_stop_definition}).
Then, we define necessary and sufficient conditions for satisfiability of a validity property in synchronous, and partially synchronous environments.

\subsection{Validity of the Crash-Stop Consensus: Formal Definition} \label{subsection:crash_stop_definition}

Let us fix the $f$-resilient crash-stop consensus problem $\mathcal{P}_C$.

We start by defining a \emph{process-proposal} pair as a pair $(P_x, \mathit{val}_x)$, where (1) $P_x$ is either $P \in \Psi$ or $\bar{P}$, with $P \in \Psi$, and (2) $\mathit{val}_x \in \mathcal{V}$.
Intuitively, $(P, \mathit{val})$ denotes that a \emph{correct} process $P \in \Psi$ has proposed a value $\mathit{val} \in \mathcal{V}$; on the other hand, $(\bar{P}, \mathit{val}')$ denotes that a \emph{faulty} process $P \in \Psi$ has proposed a value $\mathit{val}' \in \mathcal{V}$.
We denote by $\mathit{pp}.\mathsf{process}$ the process associated with a process-proposal $\mathit{pp}$, whereas $\mathit{pp}.\mathsf{proposal}$ denotes the proposal associated with $\mathit{pp}$.
Finally, $\mathit{pp}.\mathsf{correct}$ returns $\mathit{true}$ if and only if $\mathit{pp}$ is associated with a correct process; otherwise, $\mathit{pp}.\mathsf{correct}$ returns $\mathit{false}$.

An \emph{input configuration} is a tuple $\big[\mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_n \big]$ such that (1) $\mathit{pp}_i$ is a process-proposal pair, for every $i \in [1, n]$, (2) every process-proposal pair is associated with a distinct process which belongs to $\Psi$, and (3) at most $f$ process-proposal pairs refer to faulty processes (i.e., there can exist at most $f$ process-proposal pairs of the format $(\bar{P}, \cdot)$, where $P \in \Psi$).
We denote    by $\mathcal{I}$ the set of all possible input configurations.
For every input configuration $\mathit{input} \in \mathcal{I}$ and every $i \in [1, n]$, we denote by $\mathit{input}[i]$ the process-proposal pair associated with process $P_i$.

==> sections/difficulties_jovan.tex <==
\paragraph{Why is achieving a synchronous lower bound for WBC hard?}

Let us fix any synchronous algorithm $\mathcal{A}$ which solves WBC.
Moreover, let us define two infinite executions of $\mathcal{A}$:
\begin{compactitem}
    \item $\mathcal{E}_0$: All processes are correct and they all propose $0$; and

    \item $\mathcal{E}_1$: All processes are correct and they all propose $1$.
\end{compactitem}
Note that, in order to satisfy \emph{Weak Validity}, all processes decide $0$ (resp., $1$) in $\mathcal{E}_0$ (resp., $\mathcal{E}_1$).
Crucially, in any other execution $\mathcal{E}$ ($\mathcal{E} \neq \mathcal{E}_0$ and $\mathcal{E} \neq \mathcal{E}_1$) any predetermined value (say, $\bot$) can be decided.

==> sections/extensions.tex <==
\section{Beyond our Formalism}

\subsection{Extension to External Validity} \label{subsection:external_validity}

\subsection{Extension to Crash-Stop Validity}

==> sections/external_main.tex <==
\section{Extended Formalism: A Brief Introduction} \label{section:extended_formalism_main}

In this section, we briefly introduce an extended version of our formalism to accommodate for blockchain-specific validity properties.
Namely, we make our formalism more expressive by (1) allowing the input ($\mathcal{V}_I$) and output ($\mathcal{V}_O$) spaces to be unknown to processes, and (2) taking into account the ``proposals'' of faulty processes.
The full extended formalism can be found in \Cref{section:extended_formalim_appendix}. \Cref{section:classification_extended,section:blockchain_validity_appendix} are devoted to reestablishing, in the extended formalism, our previous results.

\paragraph{Intuition.}
In the original formalism, processes know the entire input ($\mathcal{V}_I$) and output ($\mathcal{V}_O$) space.
That is, processes are able to ``produce'' any value which belongs to $\mathcal{V}_I$ or $\mathcal{V}_O$.
However, this assumption limits the expressiveness of the formalism as it is impossible to describe a Byzantine consensus problem in which input or output spaces are unknown.
Let us give an example.

Imagine a committee-based blockchain which establishes two roles:
\begin{compactitem}
    \item \emph{Clients} are the users of the blockchain.
    They issue \emph{signed} transactions to the blockchain.
    
    \item \emph{Servers} are the operating nodes of the blockchain.
    Servers receive signed transactions issued by the clients, and solve the Byzantine consensus problem to agree on the exact order the transactions are processed.
\end{compactitem}
The Byzantine consensus problem at the heart of our blockchain satisfies \emph{External Validity}: if a transaction is processed, then it satisfies a predetermined $\mathsf{valid}$ predicate.
Notice that, for example, \emph{Strong Validity} is not suitable in this case, as, if not all correct processes propose the same transaction, \emph{any} transaction (even a ``useless'' one, such as $\bot$) can be decided.
Since servers rarely propose the same transactions, \emph{Strong Validity} would render our system useless a majority of the time.

As servers propose transactions \emph{signed by the clients} and servers do not have access to the private keys of the clients, servers do not know the input space $\mathcal{V}_I$ nor the output space $\mathcal{V}_O$.
% of the Byzantine consensus problem.
Hence, our original formalism is insufficient to describe the Byzantine consensus problem in the core of the aforementioned blockchain.
To address such scenarios, we introduce the extended formalism.

\paragraph{Extended vs. original formalism.}
As highlighted above, the main difference between the two formalisms is that the extended one allows us to specify the ``knowledge level'' of the input and output spaces.
In the extended formalism, a process is able to ``learn'' output values by observing input values.
That is, we define a \emph{discovery function} that specifies which output values are learned given observed input values.
In the committee-based blockchain example, once a server observes signed transactions $\mathit{tx}_1$ and $\mathit{tx}_2$, it learns the following output values: (1) $\mathit{tx}_1$, (2) $\mathit{tx}_2$, (3) $\mathit{tx}_1 || \mathit{tx}_2$, and (4) $\mathit{tx}_2 || \mathit{tx}_1$; we denote by ``$||$'' the concatenation.
% \footnote{We denote by ``$||$'' the concatenation operation.} 

The second difference between the original and the extended formalism is that the extended formalism takes into account the ``proposals'' of Byzantine processes.
Indeed, the original formalism does not allow us to define which values are admissible given the adversary's knowledge of the input space.
Think of the aforementioned example with a blockchain system.
If no process (correct or faulty) obtains a transaction $\mathit{tx}$ from the clients, $\mathit{tx}$ cannot be decided.
However, if \emph{only} a faulty process obtains a transaction $\mathit{tx}$, $\mathit{tx}$ is an admissible decision.
This scenario \emph{can} be expressed by the extended formalism (and not by the original one).



==> sections/formal_proof.tex <==
\section{Lower Bound on Message Complexity for Non-Uniform Consensus with Weak Validity in the Omission Failure Model}

\subsection{Preliminaries}

\subsubsection{Messages.}
Each message $m$ encodes the following information:
\begin{compactitem}
    \item the sender of $m$ (denoted by $m.\mathsf{sender} \in \Pi$); and

    \item the receiver of $m$ (denoted by $m.\mathsf{receiver} \in \Pi$); and

    \item the round in which $m$ is sent (denoted by $m.\mathsf{round} \in [1, \infty)$).
\end{compactitem}
As the aforementioned information is encoded in any message $m$, $\mathcal{A}$ does not instruct $m.\mathsf{sender}$ to send $m$ more than once.
Indeed, $m$ can only be sent in round $m.\mathsf{round}$ and only to $m.\mathsf{receiver}$.
As $\mathcal{A}$ instructs $m.\mathsf{sender}$ to send at most one message to $m.\mathsf{receiver}$ in any round, $m$ cannot be sent more than once.


\subsubsection{States.}
% We start by introducing \emph{states} that processes can take at the start of each round.
Let $\mathcal{S}$ denote the set of all states processes can take.
Each state $s$ encodes the following information:
\begin{compactitem}
    \item the process associated with $s$ (denoted by $s.\mathsf{process} \in \Pi$);

    \item the round associated with $s$ (denoted by $s.\mathsf{round} \in [1, \infty)$);

    \item the proposal-bit associated with $s$ (denoted by $s.\mathsf{proposal} \in \{0, 1\}$);

    \item the decision-bit associated with $s$ (denoted by $s.\mathsf{decision} \in \{\bot, 0, 1 \}$).
\end{compactitem} 
% A state $s$ such that $s.\mathsf{process} = P_i$ and $s.\mathsf{round} = k$ is denoted by $\pstate{i}{k}$.
Intuitively, a state $s \in \mathcal{S}$, where (1) $s.\mathsf{process} = P_i$, (2) $s.\mathsf{round} = k$, (3) $s.\mathsf{proposal} = b$, and (4) $s.\mathsf{decision} = b'$, denotes the state of process $P_i$ at the start of round $k$ with $P_i$'s proposal being $b$ and $P_i$'s decision being $b'$ (if $b' = \bot$, $P_i$ has not yet decided by the start of round $k$).

For each process $P_i$, there are two \emph{initial states} $\pstatezero{i} \in \mathcal{S}$ and $\pstateone{i} \in \mathcal{S}$ associated with $P_i$ such that (1) $\pstatezero{i}.\mathsf{process} = \pstateone{i}.\mathsf{process} = P_i$, (2) $\pstatezero{i}.\mathsf{proposal} = 0$, and (3) $\pstateone{i}.\mathsf{proposal} = 1$.
Each process $P_i$ starts round $1$ in either $\pstatezero{i}$ or $\pstateone{i}$.


\subsubsection{Algorithm $\mathcal{A}$ as a state-transition function.}
Algorithm $\mathcal{A}$ maps (1) a state of a process at the start of a round, and (2) messages the process received in the round into (1) a new state of the process at the start of the next round, and (2) messages the process sends in the next round.
Formally, given (1) a state $s$, and (2) a set of messages $M^R$ such that, for every message $m \in M^R$, $m.\mathsf{receiver} = s.\mathsf{process}$ and $m.\mathsf{round} = s.\mathsf{round}$, $\mathcal{A}(s, M^R) = (s', M^S)$, where 
\begin{compactitem}
    \item $s'$ is a state such that:
    \begin{compactitem}
        \item $s'.\mathsf{process} = s.\mathsf{process}$, 

        \item $s'.\mathsf{round} = s.\mathsf{round} + 1$, 

        \item $s'.\mathsf{proposal} = s.\mathsf{proposal}$,

        \item if $s.\mathsf{decision} \neq \bot$, $s'.\mathsf{decision} = s.\mathsf{decision}$, and
    \end{compactitem}

    \item $M^S$ is a set of messages such that, for every message $m \in M^S$, the following holds:
    \begin{compactitem}
        \item $m.\mathsf{sender} = s'.\mathsf{process} = s.\mathsf{process}$,

        \item $m.\mathsf{round} = s'.\mathsf{round} = s.\mathsf{round} + 1$,

        \item $m.\mathsf{receiver} \neq m.\mathsf{sender}$, and

        \item there is no message $m' \in M^S$ such that (1) $m' \neq m$, and (2) $m.\mathsf{receiver} = m'.\mathsf{receiver}$.
    \end{compactitem}
\end{compactitem}
The messages each process $P_i$ sends in the first round depend solely on $P_i$'s initial state:
\begin{compactitem}
    \item If $P_i$'s state at the start of the first round is $\pstatezero{i}$, then $\mathcal{M}_i^0$ denotes the messages $P_i$ sends in the first round.
    For every message $m \in \mathcal{M}_i^0$, the following holds: (1) $m.\mathsf{sender} = P_i$, (2) $m.\mathsf{round} = 1$, (3) $m.\mathsf{receiver} \neq P_i$, and (4) there is no message $m' \in \mathcal{M}_i^0$ such that (1) $m' \neq m$, and (2) $m'.\mathsf{receiver} = m.\mathsf{receiver}$.

    \item If $P_i$'s state at the start of the first round is $\pstateone{i}$, then $\mathcal{M}_i^1$ denotes the messages $P_i$ sends in the first round. 
    For every message $m \in \mathcal{M}_i^1$, the following holds: (1) $m.\mathsf{sender} = P_i$, (2) $m.\mathsf{round} = 1$, (3) $m.\mathsf{receiver} \neq P_i$, and (4) there is no message $m' \in \mathcal{M}_i^1$ such that (1) $m' \neq m$, and (2) $m'.\mathsf{receiver} = m.\mathsf{receiver}$.
\end{compactitem}

% \subsubsection{Internal fragments.}
% A tuple $\mathit{IF} = (s, M^S, M^R)$, where $s \in \mathcal{S}$ is a state, $M^S$ is a set of messages and $M^R$ is a set of messages, is a \emph{$k$-round internal fragment}, for some $k \geq 1$, of a process $P_i$ if and only if:
% \begin{compactitem}
%     \item $s.\mathsf{process} = P_i$; and

%     \item $s.\mathsf{round} = k$; and

%     \item for every message $m \in M^S$, $m.\mathsf{sender} = P_i$; and

%     \item for every message $m \in M^R$, $m.\mathsf{receiver} = P_i$; and

%     \item there is no message $m \in M^S \cup M^R$ such that $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

%     \item there are no two messages $m, m' \in M^S$ such that $m.\mathsf{receiver} = m'.\mathsf{receiver}$; and

%     \item there are no two messages $m, m' \in M^R$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
% \end{compactitem}
% Intuitively, a $k$-round internal fragment of a process describes the what happens from the perspective of the process in the $k$-th round.

% A $k$-round internal fragment of process $P_i$ is denoted by $\mathit{IF^k_i} = (s^k_i, M^{S(k)}_i, M^{R(k)}_i)$

% \subsubsection{Internal behaviors.}
% A tuple $\mathit{IB} = \big[ \mathit{IF}^1 = (s^1, M^{S(1)}, M^{R(1)}), \mathit{IF}^2 = (s^2, M^{S(2)}, M^{R(2)}), ..., \mathit{IF}^k = (s^k, M^{S(k)}, M^{R(k)}) \big]$ is a \emph{$k$-round internal behavior}, for some $k \geq 1$, of a process $P_i$ if and only if:
% \begin{compactitem}
%     \item for every $j \in [1, k]$, $\mathit{IF}^j$ is a $j$-round internal fragment of $P_i$; and

%     \item $s^1 = \pstatezero{i}$ or $s^1 = \pstateone{i}$; and

%     \item $s^1.\mathsf{proposal} = s^2.\mathsf{proposal} = ... = s^k.\mathsf{proposal}$; and

%     \item if there exists $j \in [1, k]$ such that $s^j.\mathsf{decision} \neq \bot$, then there exists $j^* \in [1, j]$ such that (1) for every $j' \in [1, j^* - 1]$, $s^{j'}.\mathsf{decision} = \bot$, and (2) $s^{j^*}.\mathsf{decision} = s^{j^* + 1}.\mathsf{decision} = ... = s^k.\mathsf{decision}$; and
    
%     \item for every $j \in [1, k - 1]$, $\mathcal{A}(s^j, M^{R(j)}) = (s^{j + 1}, M^{S(j + 1)})$.
% \end{compactitem}
% The following functions are defined on the aforementioned internal behavior $\mathit{IB}$ of $P_i$:
% \begin{compactitem}
%     \item For every $j \in [1, k]$, $\pstate{i}{j}(\mathit{IB}) = s^j$.

%     \item For every $j \in [1, k]$, $\msgs{i}{j}(\mathit{IB}) = M^{S(j)}$ and $\msgr{i}{j}(\mathit{IB}) = M^{R(j)}$.

%     \item $S(\mathit{IB}) = \bigcup\limits_{j \in [1, k]} \msgs{i}{j}(\mathit{IB})$.

%     \item For every $j \in [1, k]$, $S(\mathit{IB}, j) = \bigcup\limits_{j' \in [j, k]} \msgs{i}{j'}(\mathit{IB})$.

%     \item $R(\mathit{IB}) = \bigcup\limits_{j \in [1, k]} \msgr{i}{j}(\mathit{IB})$.

%     \item For every $j \in [1, k]$, $R(\mathit{IB}, j) = \bigcup\limits_{j' \in [j, k]} \msgr{i}{j'}(\mathit{IB})$.
% \end{compactitem}

\subsubsection{Fragments.}
A tuple $\mathcal{F} = \Bigl( s, M^{S}, M^{\mathit{SO}}, M^R, M^{\mathit{RO}} \Bigl)$, where $s$ is a state and $M^S$, $M^{\mathit{SO}}$, $M^R$ and $M^{\mathit{RO}}$ are sets of messages, is a \emph{$k$-round fragment}, for some $k \in \mathbb{N}^+ \cup \{+ \infty\}$, of a process $P_i$ if and only if:
\begin{compactenum}
    \item $s.\mathsf{process} = P_i$; and

    \item $s.\mathsf{round} = k$; and

    \item for every $m \in M^S \cup M^{\mathit{SO}} \cup M^R \cup M^{\mathit{RO}}$, $m.\mathsf{round} = k$; and

    \item $M^S \cap M^{\mathit{SO}} = \emptyset$; and

    \item $M^R \cap M^{\mathit{RO}} = \emptyset$; and

    \item for every message $m \in M^S \cup M^{\mathit{SO}}$, $m.\mathsf{sender} = P_i$; and

    \item for every message $m \in M^R \cup M^{\mathit{RO}}$, $m.\mathsf{receiver} = P_i$; and

    \item there is no message $m \in M^S \cup M^{\mathit{SO}} \cup M^R \cup M^{\mathit{RO}}$ such that $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

    \item there are no two messages $m, m' \in M^S \cup M^{\mathit{SO}}$ such that $m.\mathsf{receiver} = m'.\mathsf{receiver}$; and

    \item there are no two messages $m, m' \in M^R \cup M^{\mathit{RO}}$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
\end{compactenum}
Intuitively, a $k$-round fragment of a process describes what happens at a process from the perspective of an omniscient external observer in the $k$-th round.
We now present a few simple results about fragments.

\begin{lemma} \label{lemma:fragment_receive_omitted}
Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) fragment $\mathcal{F} = \Bigl( s, M^{S}, M^{\mathit{SO}}, M^R, M^{\mathit{RO}} \Bigl)$ of any process $P_i$, and any tuple $\mathcal{F}' = \Bigl( s, M^{S}, M^{\mathit{SO}}, M^R, X\Bigl)$ such that $X$ is a set of messages where:
\begin{compactenum}[(i)]
    \item for every $m \in X$, $m.\mathsf{round} = k$; and 
    
    \item $M^{R} \cap  X = \emptyset$; and

    \item for every $m \in X$, $m.\mathsf{receiver} = P_i$; and

    \item there is no message $m \in X$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

    \item there are no two messages $m, m' \in M^{R} \cup X$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
\end{compactenum}
Then, $\mathcal{F}'$ is a $k$-round fragment of $P_i$.
\end{lemma}
\begin{proof}
To prove that $\mathcal{F}'$ is a $k$-round fragment of $P_i$, we prove that all ten conditions hold for $\mathcal{F}'$.
Due to the statement of the lemma, $\mathcal{F}$ is a $k$-round fragment of $P_i$.
Conditions (1), (2), (4), (6), and (9) hold directly for $\mathcal{F}'$ as the first four elements of the tuple $\mathcal{F}'$ are identical to the first four elements of $\mathcal{F}$.
Conditions (3), (5), (7), (8), and (10) hold due to conditions (i), (ii), (iii), (iv), and (v), respectively.
\end{proof}

\begin{lemma} \label{lemma:fragment_send_transfer}
Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) fragment $\mathcal{F} = \Bigl( s, M^{S}, M^{\mathit{SO}}, M^R, M^{\mathit{RO}} \Bigl)$ of any process $P_i$ and any tuple $\mathcal{F}' = \Bigl( s, X, Y, M^R, M^{\mathit{RO}}\Bigl)$ such that $X$ and $Y$ are sets of messages where:
\begin{compactenum}[(i)]
    \item for every $m \in X \cup Y$, $m.\mathsf{round} = k$; and 
    
    \item $X \cap  Y = \emptyset$; and

    \item for every $m \in X \cup Y$, $m.\mathsf{sender} = P_i$; and

    \item there is no message $m \in X \cup Y$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

    \item there are no two messages $m, m' \in X \cup Y$ such that $m.\mathsf{receiver} = m'.\mathsf{receiver}$.
\end{compactenum}
Then, $\mathcal{F}'$ is a $k$-round fragment of $P_i$.
\end{lemma}
\begin{proof}
Due to the statement of the lemma, $\mathcal{F}$ is a $k$-round fragment of $P_i$. 
Therefore, conditions (1), (2), (5), (7), and (10) hold directly for $\mathcal{F}'$ as the first, fourth, and fifth elements of $\mathcal{F}'$ are identical to the first, fourth and fifth elements of $\mathcal{F}$.
Conditions (3), (4), (6), (8), and (9) hold due to conditions (i), (ii), (iii), (iv), and (v), respectively.
\end{proof}

\subsubsection{Behaviors.}
A tuple $\mathcal{B} = \Bigl \langle \mathcal{F}^1 = \Bigl( s^1, M^{S(1)}, M^{\mathit{SO}(1)}, M^{\mathit{R}(1)}, M^{\mathit{RO}(1)} \Bigl), ..., \mathcal{F}^k = \Bigl( s^k, M^{S(k)}, M^{\mathit{SO}(k)}, M^{\mathit{R}(k)}, M^{\mathit{RO}(k)} \Bigl) \Bigl \rangle$ is a \emph{$k$-round behavior}, for some $k \in \mathbb{N}^+ \cup \{+ \infty\}$, of a process $P_i$ if and only if:
\begin{compactenum}
    \item for every $j \in [1, k]$, $\mathcal{F}^j$ is a $j$-round fragment of $P_i$; and

    \item $s^1 = \pstatezero{i}$ or $s^1 = \pstateone{i}$; and

    \item if $s^1 = \pstatezero{i}$, then $M^{S(1)} \cup M^{\mathit{SO}(1)} = \mathcal{M}_i^0$; and

    \item if $s^1 = \pstateone{i}$, then $M^{S(1)} \cup M^{\mathit{SO}(1)} = \mathcal{M}_i^1$; and

    \item $s^1.\mathsf{proposal} = s^2.\mathsf{proposal} = ... = s^k.\mathsf{proposal}$; and

    \item if there exists $j \in [1, k]$ such that $s^j.\mathsf{decision} \neq \bot$, then there exists $j^* \in [1, j]$ such that (1) for every $j' \in [1, j^* - 1]$, $s^{j'}.\mathsf{decision} = \bot$, and (2) $s^{j^*}.\mathsf{decision} = s^{j^* + 1}.\mathsf{decision} = ... = s^k.\mathsf{decision}$; and
    
    \item for every $j \in [1, k - 1]$, $\mathcal{A}(s^j, M^{R(j)}) = (s^{j + 1}, M^{S(j+1)} \cup M^{\mathit{SO}(j+1)})$.
\end{compactenum}
If $k = +\infty$, we say that $\mathcal{B}$ is an \emph{infinite behavior} of $P_i$.
Next, we introduce some functions defined on the aforementioned behavior $\mathcal{B}$:

\begin{algorithm}
\floatname{algorithm}{Listing}
\caption{Functions defined on behavior $\mathcal{B}$}
\label{algorithm:behavior_functions}
\begin{algorithmic} [1]
\State \textbf{function} $\fstate{\mathcal{B}}{j \in [1, k]}$:
\State \hskip2em \textbf{return} $s^j$ \BlueComment{return the state at the start of round $j$}

\medskip
\State \textbf{function} $\fmsgs{\mathcal{B}}{j \in [1, k])}$:
\State \hskip2em \textbf{return} $M^{S(j)}$ \BlueComment{return the messages sent in round $j$}

\medskip
\State \textbf{function} $\fmsgso{\mathcal{B}}{j \in [1, k])}$:
\State \hskip2em \textbf{return} $M^{\mathit{SO}(j)}$ \BlueComment{return the messages send-omitted in round $j$}

\medskip
\State \textbf{function} $\fmsgr{\mathcal{B}}{j \in [1, k])}$:
\State \hskip2em \textbf{return} $M^{R(j)}$ \BlueComment{return the messages received in round $j$}

\medskip
\State \textbf{function} $\fmsgro{\mathcal{B}}{j \in [1, k])}$:
\State \hskip2em \textbf{return} $M^{\mathit{RO}(j)}$ \BlueComment{return the messages receive-omitted in round $j$}
\end{algorithmic}
\end{algorithm}

For any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B}_i$ of any process $P_i$, the following holds:
\begin{compactitem}
    \item $P_i$ \emph{decides} a bit $b \in \{0, 1\}$ in $\mathcal{B}_i$ if and only if there exists $j \in [1, k]$ such that $\fstate{\mathcal{B}_i}{j}.\mathsf{decision} = b \neq \bot$.

    \item $P_i$ \emph{does not decide} in $\mathcal{B}_i$ if and only if, for every $j \in [1, k]$, $\fstate{\mathcal{B}_i}{j}.\mathsf{decision} = \bot$.

    \item $P_i$ commits a \emph{send-omission} (resp., \emph{receive-omission}) fault in round $j \in [1, k]$ of $\mathcal{B}_i$ if and only if $\fmsgso{\mathcal{B}_i}{j} \neq \emptyset$ (resp., $\fmsgro{\mathcal{B}_i}{j} \neq \emptyset$).

    % \item $P_i$ commits an \emph{omission fault} in $\mathcal{B}_i$ if and only if $P_i$ commits a send-omission or receive-omission fault in $\mathcal{B}_i$. 
\end{compactitem}

\begin{lemma} \label{lemma:behavior_receive_omitted}
Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k \Bigl \rangle$ of any process $P_i$, and any tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
Moreover, for every $j \in [1, k]$, $\mathcal{FR}^{j} = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{R(j)}, X^j \Bigl)$, such that $X^j$ is a set of messages where:
\begin{compactitem}
    \item for every $m \in X^j$, $m.\mathsf{round} = j$; and 

    \item $M^{R(j)} \cap  X^j = \emptyset$; and

    \item for every $m \in X^j$, $m.\mathsf{receiver} = P_i$; and

    \item there is no message $m \in X^j$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

    \item there are no two messages $m, m' \in M^{R(j)} \cup X^j$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
\end{compactitem}
Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
\end{lemma}

\begin{proof}
    Since $\mathcal{B}$ is a behavior of $P_i$, $\mathcal{F}^1, \cdots, \mathcal{F}^k$ are fragments of $P_i$.
    Thus, for every $j \in [1, k]$, $\mathcal{FR}^j$ is a $j$-round fragment of $P_i$ due to conditions (i) to (v) and \Cref{lemma:fragment_receive_omitted}, which implies that condition (1) holds for $\mathcal{B}'$.
    Conditions (3) and (4) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the second and third elements of $\mathcal{FR}^j$ are identical to the second and third elements of $\mathcal{F}^j$.
    Similarly, conditions (2), (5) and (6) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the first element of $\mathcal{FR}^j$ is identical to the state from $\mathcal{F}^j$.
    Finally, condition (7) holds for $\mathcal{B}'$: first, for every $j \in [1, k]$, the first four elements of $\mathcal{FR}^j$ are identical to the first four elements of $\mathcal{F}^j$; second, condition (7) holds for $\mathcal{B}'$.
\end{proof}

% A consequence of \Cref{lemma:behavior_receive_omitted} is \Cref{corollary:behavior_receive_omitted_contained}.

% \begin{corollary}
% \label{corollary:behavior_receive_omitted_contained}
%     Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k\Bigl \rangle$  of any process $P_i$ and a tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
%     For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
%     Moreover, for every $j \in [1, k]$, $\mathcal{FR}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, X^j\Bigl)$ such that $X^j$ is a set of messages and $X^j \subseteq M^{\mathit{RO}(j)}$.
%     Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
% \end{corollary}

% \begin{lemma} \label{lemma:behavior_receive_omitted}
% Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k\Bigl \rangle$  of any process $P_i$ and a tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
% For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
% Moreover, for every $j \in [1, k]$, $\mathcal{FR}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, X^j\Bigl)$ such that $X^j$ is a set of messages and $X^j \subseteq M^{\mathit{RO}(j)}$.
% Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
% \end{lemma}
% \begin{proof}
% In order to prove that $\mathcal{B}'$ is a $k$-round behavior of $P_i$, we show that all seven conditions are satisfied by $\mathcal{B}'$.
% As $\mathcal{B}$ is a behavior of $P_i$, $\mathcal{F}^1, \cdots \mathcal{F}^k$ are fragments of $P_i$.
% Thus, for every $j \in [1, k]$, $\mathcal{FR}^j$ is a $j$-round fragment of $P_i$ due to \Cref{lemma:fragment_receive_omitted}, which implies that condition (1) holds for $\mathcal{B}'$.
% Conditions (3) and (4) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the second and third elements of $\mathcal{FR}^j$ are identical to the second and third elements of $\mathcal{F}^j$.
% Similarly, conditions (2), (5) and (6) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the first element of $\mathcal{FR}^j$ is identical to the state from $\mathcal{F}^j$.
% Finally, condition (7) holds for $\mathcal{B}'$: first, for every $j \in [1, k]$, the first four elements of $\mathcal{FR}^j$ are identical to the first four elements of $\mathcal{F}^j$; second, condition (7) holds for $\mathcal{B}'$.
% % Since $\mathcal{B}$ is a behavior, $\mathcal{F}^1, \mathcal{F}^2, \cdots, \mathcal{F}^k$ are fragments, thus, condition (1) holds by \Cref{lemma:fragment_receive_omitted}.
% % Conditions (2), (3) and (4) hold since $\forall j, \fstate{\mathcal{B}'}{j} = \fstate{\mathcal{B}}{j}$ and $\mathcal{B}$ satisfies these conditions.
% % Finally, condition (5) holds since $\mathcal{A}(\fstate{\mathcal{B}'}{j}, \fmsgr{\mathcal{B}'}{j}) = \mathcal{A}(s^j, M^{R(j)}) = (s^{j + 1}, M^{S(j+1)} \cup M^{\mathit{SO}(j+1)}) = (\fstate{\mathcal{B}}{j + 1}, \fmsgs{\mathcal{B}}{j + 1} \cup \fmsgso{\mathcal{B}}{j + 1})$, where the second equality comes from the fact that condition (5) holds for $\mathcal{B}$.
% \end{proof}

\begin{lemma} \label{lemma:behavior_send_transfer}
Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k \Bigl \rangle$ of any process $P_i$ and a tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
Moreover, for every $j \in [1, k]$, $\mathcal{FR}^{j} = \Bigl( s^j, X^j, Y^j, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$ such that (1) $X^j$ and $Y^j$ are sets of messages, (2) $X^j \cup Y^j = M^{S(j)} \cup M^{\mathit{SO}(j)}$, and (3) $X^j \cap Y^j = \emptyset$. 
Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
\end{lemma}
\begin{proof}
Since $\mathcal{B}$ is a behavior of $P_i$, $\mathcal{F}^1, \cdots, \mathcal{F}^k$ are fragments of $P_i$.
Thus, for every $j \in [1, k]$, $\mathcal{FR}^j$ is a $j$-round fragment of $P_i$ due to \Cref{lemma:fragment_send_transfer}, which implies that condition (1) holds for $\mathcal{B}'$.
Conditions (3) and (4) hold for $\mathcal{B}'$ as (1) both conditions hold for $\mathcal{B}'$, and (2) for every $j \in [1, k]$, $X^j \cup Y^j = M^{S(j)} \cup M^{\mathit{SO}(j)}$.
Similarly, conditions (2), (5) and (6) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the first element of $\mathcal{FR}^j$ is identical to the state from $\mathcal{F}^j$.
Finally, condition (7) holds for $\mathcal{B}'$: first, for every $j \in [1, k]$, $X^j \cup Y^j = M^{S(j)} \cup M^{\mathit{SO}(j)}$ and the first and the fourth elements of $\mathcal{FR}^j$ are identical to the first and the fourth elements of $\mathcal{F}^j$; second, condition (7) holds for $\mathcal{B}'$.
\end{proof}

% The following functions are defined on the aforementioned external behavior $\mathit{EB}$ of $P_i$:
% \begin{compactitem}
%     \item For every $j \in [1, k]$, $\pstate{i}{j}(\mathit{EB}) = s^j$.

%     \item For every $j \in [1, k]$, (1) $\msgs{i}{j}(\mathit{EB}) = M^{S(j)}$, (2) $\msgso{i}{j}(\mathit{EB}) = M^{\mathit{SO}(j)}$, (3) $\msgr{i}{j}(\mathit{EB}) = M^{R(j)}$, and (3) $\msgro{i}{j}(\mathit{EB}) = M^{\mathit{RO}(j)}$.

%     \item $S(\mathit{EB}) = \bigcup\limits_{j \in [1, k]} \msgs{i}{j}(\mathit{EB})$ and $\mathit{SO}(\mathit{EB}) = \bigcup\limits_{j \in [1, k]} \msgso{i}{j}(\mathit{EB})$.

%     \item For every $j \in [1, k]$, $S(\mathit{EB}, j) = \bigcup\limits_{j' \in [j, k]} \msgs{i}{j'}(\mathit{EB})$ and $\mathit{SO}(\mathit{EB}, j) = \bigcup\limits_{j' \in [j, k]} \msgso{i}{j'}(\mathit{EB})$.

%     \item $R(\mathit{EB}) = \bigcup\limits_{j \in [1, k]} \msgr{i}{j}(\mathit{EB})$ and $\mathit{RO}(\mathit{EB}) = \bigcup\limits_{j \in [1, k]} \msgro{i}{j}(\mathit{EB})$.

%     \item For every $j \in [1, k]$, $R(\mathit{EB}, j) = \bigcup\limits_{j' \in [j, k]} \msgr{i}{j'}(\mathit{EB})$ and $\mathit{RO}(\mathit{EB}, j) = \bigcup\limits_{j' \in [j, k]} \msgro{i}{j'}(\mathit{EB})$.
% \end{compactitem}

% Consider any $k$-round external behavior $\mathit{EB}_i$ of a process $P_i$:
% \begin{compactitem}
%     \item We say that $P_i$ proposes a bit $b \in \{0, 1\}$ if and only if $\pstate{i}{1}(\mathit{EB}_i).\mathsf{proposal} = b$.

%     \item We say that $P_i$ decides a bit $b' \in \{0, 1\}$ if and only if $\pstate{i}{k}(\mathit{EB}_i).\mathsf{decision} = b'$.

%     \item We say that $P_i$ sends (resp., send-omits) a message $m$ in a round $j \in [1, k]$ of $\mathit{EB}_i$ if and only if $m \in \msgs{i}{j}(\mathit{EB}_i)$ (resp., $m \in \msgso{i}{j}(\mathit{EB}_i)$).

%     \item We say that $P_i$ receives (resp., receive-omits) a message $m$ in a round $j \in [1, k]$ of $\mathit{EB}_i$ if and only if $m \in \msgr{i}{j}(\mathit{EB}_i)$ (resp., $m \in \msgro{i}{j}(\mathit{EB}_i)$).

%     \item We say that $P_i$ commits a send-omission fault in $\mathit{EB}_i$ if and only if there exists $j \in [1, k]$ such that $\msgso{i}{j}(\mathit{EB}_i) \neq \emptyset$.

%     \item We say that $P_i$ commits a receive-omission fault in $\mathit{EB}_i$ if and only if there exists $j \in [1, k]$ such that $\msgro{i}{j}(\mathit{EB}_i) \neq \emptyset$.

%     \item We say that $P_i$ commits an omission fault in $\mathit{EB}_i$ if and only if (1) $P_i$ commits a send-omission fault in $\mathit{EB}_i$, or (2) $P_i$ commits a receive-omission fault in $\mathit{EB}_i$.
% \end{compactitem}

% A $k$-round $(k \geq 1)$ external behavior $\mathit{EB}_i = \big[ \mathit{EF}_1 = (s_1, M_1^S, M_1^{\mathit{SO}}, M_1^R, M_1^{\mathit{RO}}), \mathit{EF}_2 = (s_2, M_2^S, M_2^{\mathit{SO}}, M_2^R, M_2^{\mathit{RO}}), ..., \mathit{EF}_k = (s_k, M_k^S, M_k^{\mathit{SO}}, M_k^R, M_k^{\mathit{RO}}) \big]$ of a process $P_i$ \emph{reduces} to a $k$-round internal behavior $\mathit{IB}_i = \big[ \mathit{IF}_1 = (\bar{s}_1, \bar{M}_1^S, \bar{M}_1^R), \mathit{IF}_2 = (\bar{s}_2, \bar{M}_2^S, \bar{M}_2^R), ..., \mathit{IF}_k = (\bar{s}_k, \bar{M}_k^S, \bar{M}_k^R) \big]$ if $P_i$ if and only if:
% \begin{compactitem}
%     \item for every $j \in [1, k]$, $s_j = \bar{s}_j$; and

%     \item for every $j \in [1, k]$, $\bar{M}_j^S = M_j^S \cup M_j^{\mathit{SO}}$; and

%     \item for every $j \in [1, k]$, $\bar{M}_j^R = M_j^R$.
% \end{compactitem}

\subsubsection{Executions of $\mathcal{A}$.}
A \emph{$k$-round execution} $\mathcal{E}$, for some $k \in \mathbb{N}^+ \cup \{+ \infty\}$, is a tuple $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1,  ..., \mathcal{B}_n]$ such that the following guarantees hold:
\begin{compactitem}
    \item \emph{Faulty processes:} $\mathcal{F}$ is a set of $|\mathcal{F}| \leq t$ processes.
    
    \item \emph{Composition:} For every $j \in [1, n]$, $\mathcal{B}_j$ is a $k$-round behavior of process $P_j$.

    \item \emph{Send-validity:} If there exists a message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \mathsf{sent}(\mathcal{B}_s, j)$, then (1) $m \in \mathsf{received}(\mathcal{B}_r, j)$, or (2) $m \in \mathsf{receive\_omitted}(\mathcal{B}_r, j)$.
    That is, if a message is sent, the message is either received or receive-omitted in the same round.

    \item \emph{Receive-validity:} If there exists a message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \mathsf{received}(\mathcal{B}_r, j) \cup \fmsgro{\mathcal{B}_r}{j}$, then $m \in \mathsf{sent}(\mathcal{B}_s, j)$.
    That is, if a message is received or receive-omitted, the message is sent in the same round.

    \item \emph{Omission-validity:} If there exists a process $P_i$ and $j \in [1, k]$ such that (1) $\mathsf{send\_omitted}(\mathcal{B}_i, j) \neq \emptyset$, or (2) $\mathsf{receive\_omitted}(\mathcal{B}_i, j) \neq \emptyset$, then $P_i \in \mathcal{F}$.
    That is, if a process commits an omission fault, the process is in $\mathcal{F}$.
\end{compactitem}
If $k = +\infty$, we say that $\mathcal{E}$ is an \emph{infinite execution}.

For any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, .., \mathcal{B}_n]$, the following holds:
\begin{compactitem}
    \item A process $P_i$ is \emph{faulty} in $\mathcal{E}$ if and only if $P_i \in \mathcal{F}$; otherwise, $P_i$ is \emph{correct} in $\mathcal{E}$.

    \item A process $P_i$ \emph{decides} a bit $b \in \{0, 1\}$ in $\mathcal{E}$ if and only if $P_i$ decides $b$ in $\mathcal{B}_i$.

    \item A process $P_i$ \emph{does not decide} in $\mathcal{E}$ if and only if $P_i$ does not decide in $\mathcal{B}_i$.

    \item A process $P_i$ commits a \emph{send-omission} (resp., \emph{receive-omission}) fault in round $j \in [1, k]$ of $\mathcal{E}$ if and only if $P_i$ commits a send-omission (resp., receive-omission) fault in round $j$ of $\mathcal{B}_i$.

    % \item A process $P_i$ commits an \emph{omission fault} in $\mathcal{E}$ if and only if $P_i$ commits an omission fault in $\mathcal{B}_i$.
\end{compactitem}

% \begin{lemma} \label{lemma:behavior_from_execution}
% Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{ +\infty \}$) execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ and any process $P_i$.
% Let $\mathcal{B}_i = \Bigl \langle \mathcal{F}_i^1, ..., \mathcal{F}_i^k \Bigl \rangle$ and, for every $j \in [1, k]$, let $\mathcal{F}_i^1 = \Bigl( s_i^j, M_i^{S(j)}, M_i^{\mathit{SO}(j)}, M_i^{R(j)}, M_i^{\mathit{RO}(j)} \Bigl)$.
% Consider any tuple $\mathcal{B}_i' = \Bigl \langle \mathcal{FR}_i^1, ..., \mathcal{FR}_i^k \Bigl \rangle$ such that, for every $j \in [1, k]$, $\mathcal{FR}_i^1 = \Bigl( s_i^j, M_i^{S(j)}, M_i^{\mathit{SO}(j)}, M_i^{R(j)}, X_i^j \Bigl)$, where the following holds for $X_i^j$:
% \begin{compactitem}
%     \item for every $m \in X_i^j$, $m.\mathsf{round} = j$; and 

%     \item $M_i^{R(j)} \cap  X_i^j = \emptyset$; and

%     \item for every $m \in X_i^j$, $m.\mathsf{receiver} = P_i$; and

%     \item there is no message $m \in X_i^j$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

%     \item there are no two messages $m, m' \in M_i^{R(j)} \cup X_i^j$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
% \end{compactitem}
% Then, $\mathcal{B}_i'$ is a $k$-round behavior of $P_i$.
% \end{lemma}

% \begin{lemma} \label{lemma:behavior_from_execution}
% Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k \Bigl \rangle$ of any process $P_i$, and any tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
% For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
% Moreover, for every $j \in [1, k]$, $\mathcal{FR}^{j} = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{R(j)}, X^j \Bigl)$, such that $X^j$ is a set of messages where:
% \begin{compactitem}
%     \item for every $m \in X^j$, $m.\mathsf{round} = j$; and 

%     \item $M^{R(j)} \cap  X^j = \emptyset$; and

%     \item for every $m \in X^j$, $m.\mathsf{receiver} = P_i$; and

%     \item there is no message $m \in X^j$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

%     \item there are no two messages $m, m' \in M^{R(j)} \cup X^j$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
% \end{compactitem}
% Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
% \end{lemma}

% \begin{proof}
%     Since $\mathcal{B}$ is a behavior of $P_i$, $\mathcal{F}^1, \cdots, \mathcal{F}^k$ are fragments of $P_i$.
%     Thus, for every $j \in [1, k]$, $\mathcal{FR}^j$ is a $j$-round fragment of $P_i$ due to \Cref{lemma:fragment_receive_omitted}, which implies that condition (1) holds for $\mathcal{B}'$.
%     Conditions (3) and (4) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the second and third elements of $\mathcal{FR}^j$ are identical to the second and third elements of $\mathcal{F}^j$.
%     Similarly, conditions (2), (5) and (6) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the first element of $\mathcal{FR}^j$ is identical to the state from $\mathcal{F}^j$.
%     Finally, condition (7) holds for $\mathcal{B}'$: first, for every $j \in [1, k]$, the first four elements of $\mathcal{FR}^j$ are identical to the first four elements of $\mathcal{F}^j$; second, condition (7) holds for $\mathcal{B}'$.
% \end{proof}

% \begin{lemma} \label{lemma:behavior_from_execution_A}
% Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{ +\infty \}$) execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ and any process $P_i$.
% Let $\mathcal{B}_i = \Bigl \langle \mathcal{F}_i^1, ..., \mathcal{F}_i^k \Bigl \rangle$ and, for every $j \in [1, k]$, let $\mathcal{F}_i^1 = \Bigl( s_i^j, M_i^{S(j)}, M_i^{\mathit{SO}(j)}, M_i^{R(j)}, M_i^{\mathit{RO}(j)} \Bigl)$.
% Consider any tuple $\mathcal{B}_i' = \Bigl \langle \mathcal{FR}_i^1, ..., \mathcal{FR}_i^k \Bigl \rangle$ such that, for every $j \in [1, k]$, $\mathcal{FR}_i^1 = \Bigl( s_i^j, M_i^{S(j)}, M_i^{\mathit{SO}(j)}, M_i^{R(j)}, X_i^j \Bigl)$, where the following holds for $X_i^j$:
% \begin{compactitem}
%     \item for every $m \in X_i^j$, $m.\mathsf{round} = j$; and 

%     \item $M_i^{R(j)} \cap  X_i^j = \emptyset$; and

%     \item for every $m \in X_i^j$, $m.\mathsf{receiver} = P_i$; and

%     \item there is no message $m \in X_i^j$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

%     \item there are no two messages $m, m' \in M_i^{R(j)} \cup X_i^j$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
% \end{compactitem}
% Then, $\mathcal{B}_i'$ is a $k$-round behavior of $P_i$.
% \end{lemma}

\subsection{Proof}

\begin{definition} [Receive-isolation] \label{definition:isolation}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) execution.
We say that a group $G$ of $|G| \leq t$ processes is \emph{receive-isolated from a round $k' \in \mathbb{N}^+$} ($k' \leq k$) in $\mathcal{E}$ if and only if, for every process $P_g \in G$, the following holds:
\begin{compactitem}
    \item $P_g \in \mathcal{F}$; and

    \item for every $j \in [1, k' - 1]$, $\mathsf{receive\_omitted}(\mathcal{B}_g, j) = \emptyset$; and

    \item for every $j \in [1, k]$, $\mathsf{send\_omitted}(\mathcal{B}_g, j) = \emptyset$; and

    \item for every $j \in [k', k]$, if there exists a message $m$ such that $m \in \mathsf{received}(\mathcal{B}_g, j)$, then $m.\mathsf{sender} \in G$.
\end{compactitem}
\end{definition}
Intuitively, a group $G$ is receive-isolated from some round $k'$ in an execution if and only if the following holds for every process $P_g \in G$: (1) $g$ is faulty, (2) $g$ does not commit any receive-omission failures in any round before $k'$, (3) $g$ does not commit any send-omission failures throughout the entire execution, and (4) from round $k'$ onward, $g$ receives messages only from processes in $G$.
This can be understood as a simultaneous unidirectional partition of $G$: messages from $G$ to other processes are always \emph{sent} successfully while no message from $\overline{G}$ to $G$ is \emph{received} from round $k'$ onward.
% JOVAN: I really like this last sentence.

\manuel{The next lemma is an auxiliary Lemma for future refactoring, currently unused/not ready}
\begin{lemma}
\label{lemma:similar_decision}
    Consider any two infinite executions $\mathcal{E}, \mathcal{E'}$ and any group of processes $X$ such that (1) in both $\mathcal{E}$ and $\mathcal{E}'$, $X$ is receive-isolated from some round $k \in \mathbb{N}^+$, (2) the behaviors of processes in $X$ in execution $\mathcal{E}'$ are identical to $\mathcal{E}$ up to round $k-1$, and (3) no message $m$ between any two processes $i,j \in X$ is send-omitted or receive-omitted in $\mathcal{E}$ or $\mathcal{E'}$.
    Then, for any process $i\in X$ and any $j \geq 1$, $s^j_i(\mathcal{E}).\mathsf{decision} = s^j_i(\mathcal{E'}).\mathsf{decision}$.
\end{lemma}
\begin{proof}
    Suppose by contradiction that the lemma is not true.
    Then there is a process $i\in X$ and a round $j \geq 1$ such that $s^j_i(\mathcal{E}) \neq s^j_i(\mathcal{E'})$.
    Consider the smallest round $j$ such that there is a process $P_i \in X$ where $s^j_i(\mathcal{E}) \neq s^j_i(\mathcal{E'})$.
    This implies $M^{j-1}_i(\mathcal{E}) \neq M^{j-1}_i(\mathcal{E'})$, since $s^{j-1}_i(\mathcal{E}) = s^{j-1}_i(\mathcal{E}')$ and $\mathcal{A}(s^{j-1}_i(\mathcal{E}), M^{j-1}_i(\mathcal{E})) \neq \mathcal{A}(s^{j-1}_i(\mathcal{E}'), M^{j-1}_i(\mathcal{E})')$.
    Now consider the smallest round $j$ such that there is a process $P_i \in X$ where $M^{R(j)}_i(\mathcal{E}) \neq M^{R(j)}_i(\mathcal{E'})$.
    Note that $j \geq k$ since the behaviors of $P_i$ in $\mathcal{E}$ and $\mathcal{E}'$ are identical up to $k-1$.
    This means that $\forall p \in X$, both $s^{j-1}_p(\mathcal{E})$ and $M^{R(j-1)}_p$ are identical in $\mathcal{E}$ and $\mathcal{E}'$ which implies (by $\mathcal{A}$) that the union $M^{S(j)}_p \cup M^{SO(j)}_p$ is also identical in $\mathcal{E}$ and $\mathcal{E}'$.
    If $M^{R(j)}_i(\mathcal{E}) \neq M^{R(j)}_i(\mathcal{E'})$, then there must be some message $m$ such that $m \in M^{R(j)}_i(\mathcal{E})$ and $m \notin M^{R(j)}_i(\mathcal{E}')$, or vice-versa.
    Without loss of generality, assume that there is $m$ such that $m \in M^{R(j)}_i(\mathcal{E})$ and $m \notin M^{R(j)}_i(\mathcal{E}')$.
    There are two possibilities:
    \begin{compactitem}
        \item $m.\mathsf{sender} \in \overline{X}$. However, this would contradict the fact that, for $j \geq k$, all messages from processes in $\overline{X}$ are receive-omitted from round $k$ onward.
        \item $m.\mathsf{sender} \in X$.
        Let $P_l$ be that sender.
        Due to the receive-validity of $\mathcal{E}$, $m \in M^{R(j)}_i(\mathcal{E}) \implies m \in M^{S(j)}_l(\mathcal{E}) \implies m \in M^{S(j)}_l(\mathcal{E}') \cup M^{SO(j)}_l(\mathcal{E}')$. 
        Due to (3), we know that $m \notin M^{SO(j)}_l(\mathcal{E}')$, so $m \in M^{S(j)}_l(\mathcal{E}')$.
        % Since $\mathcal{E}'$ is also an execution, this then means that $m \in M^{SO(j)}_i(\mathcal{E})$
        Due to the send-validity of $\mathcal{E}'$, $m \in M^{S(j)}_i(\mathcal{E}) \implies m \in M^{S(j)}_i(\mathcal{E}) \cup M^{SO(j)}_i(\mathcal{E})$. 
        Due to (3), we also know that $m \notin M^{RO(j)}_i(\mathcal{E}')$. 
        Therefore, $m \in M^{R(j)}_i(\mathcal{E}')$, which contradicts the assumption.
    \end{compactitem}
    Hence, the lemma holds.
    
    
    
    
\end{proof}

\begin{figure}[ht]
    \centering
    \begin{minipage}{.3\textwidth}
        \centering
        %\vspace{.4cm}
        \includegraphics[width=.85\linewidth]{figures/legend.pdf}
        %\vspace{.95cm}
        \caption{Legend}
        \label{figure:legend}
    \end{minipage}%
    \begin{minipage}{.7\textwidth}
        \centering
        \includegraphics[width=.75\linewidth]{figures/forced_termination.pdf}
        \caption{Proof sketch of Lemma \ref{lemma:forced_termination}. $S_i$ denotes the senders of $P_i$ in $\overline{X}$. 
        Messages that $P_i$ receive-omits in $\mathcal{E}$ are instead send-omitted in $\mathcal{E'}$.
        Thus, $P_i$'s behavior is identical and executions $\mathcal{E}$ and $\mathcal{E'}$ are indistinguishable.}
        \label{figure:forced_termination}
    \end{minipage}
\end{figure}

\begin{lemma} \label{lemma:forced_termination_formal}
Consider any infinite execution $\mathcal{E}$ such that (1) some group $X$ of $|X| = \frac{t}{4}$ processes is receive-isolated from some round $k \in \mathbb{N}^+$, and (2) all processes in $\Bar{X}$ are correct.
At least $\frac{|X|}{2}$ processes from $X$ decide in $\mathcal{E}$.
\end{lemma}
\begin{proof}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Due to the statement of the lemma, $\mathcal{F} = X$.
Moreover, no process commits any send-omission failure in $\mathcal{E}$: for every process $P_i$ and every round $j \in \mathbb{N}^+ \cup \{+\infty\}$, $\mathsf{send\_omitted}(\mathcal{B}_i, j) = \emptyset$.

We prove the lemma by contradiction.
Therefore, assume that there exists a subset $X' \subseteq X$ of $|X'| > \frac{|X|}{2} = \frac{t}{8}$ processes which do not decide in $\mathcal{E}$.
Let $M_{\bar{X}} = \bigcup\limits_{P_i \in \bar{X}} \big( \fmsgs{\mathcal{B}_i}{k} \cup \fmsgs{\mathcal{B}_i}{k + 1} \cup ... \big)$ denote the set of messages sent by processes in $\bar{X}$ from (and including) round $k$ onward in $\mathcal{E}$.
For every process $P_i \in X'$, we define $M_{\bar{X} \to P_i}$ as the set containing all messages sent to $P_i$ by processes in $\bar{X}$ from (and including) round $k$ onward of $\mathcal{E}$:
\begin{equation*}
    M_{\bar{X} \to P_i} = \{ m \,|\, m \in M_{\bar{X}} \land m.\mathsf{receiver} = P_i \}.
\end{equation*}
Note that, for every $P_i \in X'$, each message $m \in M_{\bar{X} \to P_i}$ is receive-omitted in $\mathcal{B}_i$.

Let $M_{\bar{X} \to X'} = \bigcup\limits_{P_i \in X'} M_{\bar{X} \to P_i}$.
As $\mathcal{A}$ sends less than $\frac{t^2}{32}$ in any execution, less than $\frac{t^2}{32}$ messages are sent in $\mathcal{E}$ by correct processes (i.e., processes in $\bar{X}$), which implies $|M_{\bar{X} \to X'}| < \frac{t^2}{32}$.
Hence, there exists a process $P_i \in X'$ such that $|M_{\bar{X} \to P_i}| < \frac{t}{4}$.
Recall that $P_i$ does not decide in $\mathcal{E}$.

Let $S_i$ denote the set of processes whose messages $P_i$ receive-omits from (and including) round $k$ onward in $\mathcal{B}_i$:
\begin{equation*}
    S_i = \{ P_j \in \Pi \,|\, \exists j \in [k, \infty], \exists m \in \fmsgro{\mathcal{B}_i}{j}: m.\mathsf{sender} = P_j \}.
\end{equation*}
Note that $P_i \notin S_i$ (as no process ever sends messages to itself).
Moreover, as $|M_{\bar{X} \to P_i}| < \frac{t}{4}$, $|S_i \cap \bar{X}| < \frac{t}{4}$.
We now create another execution $\mathcal{E}' = [\mathcal{F}', \mathcal{B}_1', ..., \mathcal{B}_n']$:
\begin{compactenum}
    \item $\mathcal{F}' \gets S_i \cup (X \setminus{ \{P_i\}})$.

    %\item For every process $P_j \in \bar{X} \setminus{S_i}$, let $\mathcal{B}_j' \gets \mathcal{B}_j$, i.e., $P_j$'s behavior in $\mathcal{E}'$ is identical to $P_j$'s behavior in $\mathcal{E}$.

    \item For every process $P_j \in \Pi \setminus{ (S_i \cup \{P_i\}) }$, let $\mathcal{B}_j' \gets \mathcal{B}_j$, i.e., $P_j$'s behavior in $\mathcal{E}'$ is identical to $P_j$'s behavior in $\mathcal{E}$.

    \item For the process $P_i$, we build $\mathcal{B}_i'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_i' \gets \mathcal{B}_i$.

        \item For every round $k' \in [k, \infty]$ such that $\fmsgro{\mathcal{B}_i}{k'} \neq \emptyset$, we remove all messages from $\fmsgro{\mathcal{B}'_i}{k'}$: $\fmsgro{\mathcal{B}'_i}{k'} \gets \emptyset$.
        Note that all messages removed from $\fmsgro{\mathcal{B}'_i}{k'}$ are sent by processes in $S_i$.
    \end{compactenum}
    Note that $P_i$ does not commit any omission faults in $\mathcal{B}_i'$: (1) it does not commit any send-omission faults due to the statement of the lemma, and (2) it does not commit any receive-omission faults due to the step (3)(b).

    \item For every process $P_j \in S_i$, we build $\mathcal{B}_j'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_j' \gets \mathcal{B}_j$.

        \item For every message $m$ such that there exists a round $k' \geq [k, \infty]$ with (1) $m \in \fmsgs{\mathcal{B}_j}{k'}$, and (2) $m \in \fmsgro{\mathcal{B}_i}{k'}$, we perform the following steps:
        \begin{compactenum}
            \item We remove $m$ from sent messages: $\fmsgs{\mathcal{B}_j'}{k'} \gets \fmsgs{\mathcal{B}_j'}{k'} \setminus{\{m\}}$.

            \item We add $m$ to send-omitted messages:
            $\fmsgso{\mathcal{B}_j'}{k'} \gets \fmsgso{\mathcal{B}_j'}{k'} \cup \{m\}$.
        \end{compactenum}
    \end{compactenum}
    % Note that resulting $\mathcal{B}_j'$ satisfies the definition of a behavior.
\end{compactenum}

Let us prove that $\mathcal{E}'$ is indeed an execution:
\begin{compactitem}
    \item Faulty processes: As $\mathcal{F}' = S_i \cup X \setminus{\{ P_i \}}$ and $|S_i \cap \bar{X}| < \frac{t}{4}$, $|\mathcal{F}'| < t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore:
    \begin{compactitem}
        \item For any process $P_j \in \Pi \setminus{ (S_i \cup \{P_i\}) }$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ since $\mathcal{B}_j' = \mathcal{B}_j$. 
        \item For process $P_i$, $\mathcal{B}_i'$ is an infinite behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
        \item For any process $P_j \in S_i$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ due to \Cref{lemma:behavior_send_transfer}.
    \end{compactitem}
    

    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$).
    We consider two possibilities:
    \begin{compactitem}
        \item If $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (3)(b), then $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ as $m$ is included in step (3)(a).

        \item Otherwise, $m$ is excluded by step (3)(b).
        This implies that $j \geq k$, $P_r = P_i$, $P_s \in S_i$, $m \in \fmsgro{\mathcal{B}_r}{j}$ and $m \in \fmsgs{\mathcal{B}_s}{j}$.
        Then, by step (4)(b)(i), $m \notin \fmsgs{\mathcal{B}_s'}{j}$ making this case impossible.
    \end{compactitem}
    Send-validity is satisfied in $\mathcal{E}'$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $j \geq k$ and $P_r = P_i$ and $m \in \fmsgro{\mathcal{B}_r}{j}$.
        However, this case is impossible as $m \notin \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ due to the step (3)(b).

        \item Otherwise, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
        Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (4)(b)(i) while constructing $\mathcal{B}_s'$.
    \end{compactitem}
    Receive-validity is satisfied in $\mathcal{E}'$.

    \item Omission-validity:
    Consider a process $P_j$ which commits an omission-fault in $\mathcal{B}_j'$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $P_j$ commit a send-omission fault in $\mathcal{B}_j'$.
        As no process $P_z$ commits a send-omission fault in $\mathcal{B}_z$, $P_j \in S_i$ given that we only add send-omitted messages to processes in $S_i$.
        \sout{As $P_i \notin S_i$, $S_i \subset \mathcal{F}'$.}
        In this case, omission-validity is satisfied.

        \item Let $P_j$ commit a receive-omission fault in $\mathcal{B}_j'$.
        Note that no process $P_z \in \bar{X}$ commits a receive-omission fault in $\mathcal{B}_z$, which implies that no process $P_z \in \bar{X}$ commits a receive-omission fault in $\mathcal{B}_z'$ (as our construction does not add receive-omitted messages to any process).
        
        Moreover, $P_i$ does not commit a receive-omission fault in $\mathcal{B}_i'$ as (1) it does not commit any receive-omission faults in any round $k' \in [1, k - 1]$ in $\mathcal{B}_i$ (due to \Cref{definition:isolation}), and (2) all receive-omitted messages in any round $k' \in [k, \infty]$ are removed by the step (3)(b).
        Therefore, $P_j \in X \setminus{\{P_i\}}$, which means that omission-validity holds in this case as well.
    \end{compactitem}
    Omission-validity is satisfied in $\mathcal{E}'$.
\end{compactitem}
Thus, $\mathcal{E}'$ is indeed an execution of $\mathcal{A}$.

Observe that $P_i$ is correct in $\mathcal{E}'$, and $P_i$ does not decide in $\mathcal{E}'$ as (1) $P_i$'s states in $\mathcal{B}_i'$ and $\mathcal{B}_i$ are identical, and (2) $P_i$ does not decide in $\mathcal{B}_i$.
Therefore, \emph{Termination} is violated in $\mathcal{E}'$, which represents a contradiction with the fact that $\mathcal{A}$ solves non-uniform consensus.
Hence, the lemma holds.
\end{proof}

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\textwidth]{figures/disagreement_quadratic.pdf}
\caption{Proof sketch of Lemma \ref{lemma:disagreement_quadratic_messages}}
\label{figure:disagreement_quadratic}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.7\textwidth]{figures/kplus1_picture1.pdf}
\caption{Proof sketch of Lemma \ref{lemma:disagreement_quadratic_messages} (LAST LEMMA)}
\label{figure:disagreement_quadratic}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\textwidth]{figures/kplus1_picture2.pdf}
\caption{Proof sketch of Lemma \ref{lemma:disagreement_quadratic_messages} (LAST LEMMA)}
\label{figure:disagreement_quadratic}
\end{figure}


% \newpage
\begin{lemma} \label{lemma:disagreement_quadratic_messages_formal}
Let there exist an infinite execution $\mathcal{E}$ such that:
\begin{compactitem}
    \item Group $B$ is receive-isolated from some round $k_B \in \mathbb{N}^+$.

    \item Group $C$ is receive-isolated from some round $k_C \in \mathbb{N}^+$.

    \item Processes from group $A$ are correct.

    \item At least $\frac{|B|}{4}$ processes from $B$ decide the same bit $b$.

    \item At least $\frac{|C|}{4}$ processes from $C$ decide the same bit $b'$ such that $b' \neq b$.
\end{compactitem}
Then, at least $\frac{t^2}{32}$ messages are sent by correct processes (i.e., processes in $A$) in $\mathcal{E}$.
\end{lemma}
\begin{proof}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Due to the statement of the lemma, $\mathcal{F} = B \cup C$.
Moreover, no process commits any send-omission failure: for every process $P_i$ and every round $j \in \mathbb{N}^+ \cup \{+\infty\}$, $\fmsgso{\mathcal{B}_i}{j} = \emptyset$.

Let $B' \subseteq B$ denote the set of all processes from $B$ which decide $b$ in $\mathcal{E}$; $|B'| \geq \frac{t}{16}$.
Similarly, let $C' \subseteq C$ denote the set of all processes from $C$ which decide $b' \neq b$ in $\mathcal{E}$; $|C'| \geq \frac{t}{16}$.
Without loss of generality, assume that (1) processes in $A$ decide $0$ in $\mathcal{E}$ (to ensure \emph{Termination} and \emph{Agreement}), (2) processes in $B'$ decide $0$ (i.e., $b = 0$), and (3) processes in $C'$ decide $1$ (i.e., $b' = 1$).
Let $M_{A} = \bigcup\limits_{P_i \in A} \big( \fmsgs{\mathcal{B}_i}{k_C} \cup \fmsgs{\mathcal{B}_i}{k_C + 1} \cup ... \big)$ denote the set of messages sent by processes in $A$ from (and including) round $k_C$ onward in $\mathcal{E}$.
For every process $P_i \in C'$, we define $M_{A \to P_i}$ as the set containing all messages sent to $P_i$ by processes in $A$ from (and including) round $k_C$ onward:
\begin{equation*}
    M_{A \to P_i} = \{ m \,|\, m \in M_A \land m.\mathsf{receiver} = P_i \}.
\end{equation*}
Similarly, let $M_{B} = \bigcup\limits_{P_i \in B} \big( \fmsgs{\mathcal{B}_i}{k_C} \cup \fmsgs{\mathcal{B}_i}{k_C + 1} \cup ... \big)$ denote the set of messages sent by processes in $B$ from (and including) round $k_C$ onward in $\mathcal{E}$.
For every process $P_i \in C'$, we define $M_{B \to P_i}$ as the set containing all messages sent to $P_i$ by processes in $B$ from (and including) round $k_C$ onward:
\begin{equation*}
    M_{B \to P_i} = \{ m \,|\, m \in M_B \land m.\mathsf{receiver} = P_i \}.
\end{equation*}
Note that, for every $P_i \in C'$, each message $m \in M_{A \to P_i} \cup M_{B \to P_i}$ is receive-omitted in $\mathcal{B}_i$.

Let $M_{A \to C'} = \bigcup\limits_{P_i \in C'} M_{A \to P_i}$ and $M_{B \to C'} = \bigcup\limits_{P_i \in C'} M_{B \to P_i}$.
Assume that $|M_{A \to C'}| < \frac{t^2}{32}$ (otherwise, the lemma holds).
As $|M_{A \to C'}| < \frac{t^2}{32}$, there exists a process $P_i \in C'$ such that $|M_{A \to P_i}| < \frac{t}{2}$.
Recall that $P_i$ decides $1$ in $\mathcal{B}_i$.

Let $S_i$ denote the set of processes whose messages $P_i$ receive-omits from (and including) round $k_C$ onward:
\begin{equation*}
    S_i = \{ P_j \in \Pi \,|\, \exists j \in [k_C, \infty], \exists m \in \fmsgro{\mathcal{B}_i}{j}: m.\mathsf{sender} = P_j \}.
\end{equation*}
Note that $P_i \notin S_i$.
As $|M_{A \to P_i}| < \frac{t}{2}$, $|S_i \cap A| < \frac{t}{2}$.
We now construct another execution $\mathcal{E}' = [\mathcal{F}', \mathcal{B}_1', ..., \mathcal{B}_n']$:
\begin{compactenum}
    \item $\mathcal{F}' \gets S_i \cup B \cup (C \setminus{\{P_i\}})$.

    \item For every process $P_j \in \Pi \setminus{ (S_i \cup \{P_i\}) }$, let $\mathcal{B}_j' \gets \mathcal{B}_j$, i.e., $P_j$'s behavior in $\mathcal{E}'$ is identical to $P_j$'s behavior in $\mathcal{E}$.

    \item For the process $P_i$, we build $\mathcal{B}_i'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_i' \gets \mathcal{B}_i$.

        \item For every round $k' \geq k_C$ such that $\fmsgro{\mathcal{B}_i}{k'} \neq \emptyset$, we remove all messages from $\fmsgro{\mathcal{B}'_i}{k'}$: $\fmsgro{\mathcal{B}'_i}{k'} \gets \emptyset$.
        Note that all messages removed from $\fmsgro{\mathcal{B}'_i}{k'}$ are sent by processes in $S_i$.
    \end{compactenum}

    \item For every process $P_j \in S_i$, we construct $\mathcal{B}_j'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_j' \gets \mathcal{B}_j$.

        \item For every message $m$ such that there exists a round $k' \geq k_C$ with (1) $m \in \fmsgs{\mathcal{B}_j}{k'}$, and (2) $m \in \fmsgro{\mathcal{B}_i}{k'}$, we perform the following steps:
        \begin{compactenum}
            \item We remove $m$ from sent messages: $\fmsgs{\mathcal{B}_j'}{k'} \gets \fmsgs{\mathcal{B}_j'}{k} \setminus{ \{m\} }$.

            \item We add $m$ to send-omitted messages: $\fmsgso{\mathcal{B}_j'}{k'} \gets \fmsgso{\mathcal{B}_j'}{k'} \cup \{m\}$.
        \end{compactenum}
    \end{compactenum}
\end{compactenum}
Let us prove that $\mathcal{E}'$ is an execution:
\begin{compactitem}
    \item Faulty processes: As $\mathcal{F}' = S_i \cup B \cup (C \setminus{ \{P_i\} })$ and $|S_i \cap A| < \frac{t}{2}$, $|\mathcal{F}'| < t$.

    \item Composition: As $\mathcal{E}$ is an execution, $\mathcal{B}_j$ is an infinite behavior of $P_j$, for every process $P_j$.
    Therefore, the following holds:
    \begin{compactitem}
        \item For any process $P_j \in \Pi \setminus{ S_i \cup \{P_i\} }$, $\mathcal{B}_j'$ is an infinite behavior of $P_i$ as $\mathcal{B}_j' = \mathcal{B}_j$.

        \item For the process $P_i$, $\mathcal{B}_i'$ is an infinite behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.

        \item For any process $P_j \in S_i$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ due to \Cref{lemma:behavior_send_transfer}.
    \end{compactitem}

    \item Send-validity: Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$).
    We consider two possibilities:
    \begin{compactitem}
        \item Let $j \geq k$ and $P_r = P_i$ and $m \in \fmsgro{\mathcal{B}_r}{j}$.
        Hence, $P_s \in S_i$.
        However, this case is impossible as $m$ is not sent in $\mathcal{B}_s'$ due to step (4)(b)(i).

        \item Otherwise, $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ as no received or receive-omitted message is removed from $\mathcal{B}_r$.
    \end{compactitem}
    Send-validity is satisfied in $\mathcal{E}'$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $j \geq k$ and $P_r = P_i$ and $m \in \fmsgro{\mathcal{B}_r}{j}$.
        However, this case is impossible as $m \notin \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ due to the step (3)(b).

        \item Otherwise, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
        Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed while constructing $\mathcal{B}_s'$.
    \end{compactitem}
    Receive-validity is satisfied in $\mathcal{E}'$.

    \item Omission-validity: Consider any process $P_j$ which commits an omission-fault in $\mathcal{B}_j'$.
    We focus on two possibilities:
    \begin{compactitem}
        \item Let $P_j$ commit a send-omission fault in $\mathcal{B}_j'$.
        As no process $P_z$ commits a send-omission fault in $\mathcal{B}_z$, $P_j \in S_i$ given that we only add send-omitted messages to processes in $S_i$.
        As $P_i \notin S_i$, $S_i \subset \mathcal{F}'$.
        In this case, omission-validity is satisfied.

        \item Let $P_j$ commit a receive-omission fault in $\mathcal{B}_j'$.
        Note that no process $P_z \in A$ commits a receive-omission fault in $\mathcal{B}_z$, which implies that no process $P_z \in A$ commits a receive-omission fault in $\mathcal{B}_z'$ (as our construction does not add receive-omitted messages to any process).

        Moreover, $P_i$ does not commit a receive-omission fault in $\mathcal{B}_i'$ as (1) it does not commit any receive-omission faults in any round $k' \in [1, k_C - 1]$ in $\mathcal{B}_i$ (due to \Cref{definition:isolation}), and (2) all receive-omitted messages in any round $k' \in [k_C, \infty]$ are removed by the step (3)(b).
        Therefore, $P_j \in B \cup (C \setminus{\{P_i\}})$, which means that omission-validity holds in this case as well.
    \end{compactitem}
    Omission-validity holds in $\mathcal{E}'$.
\end{compactitem}
Thus, $\mathcal{E}'$ is indeed an execution.

Observe that $P_i$ is correct in $\mathcal{E}'$, and $P_i$ decides $1$ in $\mathcal{E}'$ as (1) $P_i$'s states in $\mathcal{B}_i'$ and $\mathcal{B}_i$ are identical, and (2) $P_i$ decides $1$ in $\mathcal{B}_i$.
Moreover, there exists a process $P_j \in A \setminus{S_i}$ such that (1) $P_j$ is correct in $\mathcal{E}'$ (as $|S_i \cap A| < \frac{t}{2}$ and $|A| = \frac{t}{2}$), and (2) $P_j$ decides $0$ in $\mathcal{E}'$ (as $P_j$ decides $0$ in $\mathcal{B}_j$ and $\mathcal{B}_j = \mathcal{B}_j'$).
Therefore, \emph{Agreement} is violated in $\mathcal{E}'$, which represents a contradiction with the fact that $\mathcal{A}$ solves non-uniform consensus.
Hence, the lemma holds.
\end{proof}

In the rest of the proof, we rely on the following two infinite executions:
\begin{compactitem}
    \item $\mathcal{E}_0$: All processes propose $0$. Group $B$ is receive-isolated from round $1$, whereas all other processes are correct.

    \item $\mathcal{E}_1$: All processes propose $1$. Group $C$ is receive-isolated from round $1$, whereas all other processes are correct.
\end{compactitem}

\begin{lemma} \label{lemma:either}
At least $\frac{|B|}{4}$ processes from $B$ decide $1$ in $\mathcal{E}_0$ or at least $\frac{|C|}{4}$ processes from $C$ decide $0$ in $\mathcal{E}_1$.
\end{lemma}
\manuel{The next proof is an attempt at an alternative proof of the previous Lemma.}
\begin{proof}
    Suppose also that (1) in $\mathcal{E}_0$, no message $m$ between any two processes $i,j \in B$ is send-omitted or receive-omitted, and (2) in $\mathcal{E}_1$, no message $m$ between any two processes $i,j \in C$ is send-omitted or receive-omitted. \manuel{Honestly, we should just make this part of the definition of receive-isolation. Either way,  \Cref{lemma:forced_termination_formal} holds.}
    
    By \Cref{lemma:forced_termination_formal}, at least $\frac{|B|}{2}$ processes from $B$ decide in $\mathcal{E}_0$.
    As the only possible decisions are $0$ and $1$, at least $\frac{|B|}{4}$ processes from $B$ (denoted by $B' \subseteq B$) decide the same bit $b$ in $\mathcal{E}_0$.

    Similarly, let $\mathcal{E}_1 = [\mathcal{F}^1, \mathcal{B}_1^1, ..., \mathcal{B}_n^0]$.
    We have that (1) $\mathcal{F}^1 = C$, and (2) no process $P_i$ commits a send-omission fault in $\mathcal{B}_i^1$.
    By \Cref{lemma:forced_termination_formal}, at least $\frac{|C|}{2}$ processes from $C$ decide in $\mathcal{E}_1$.
    As the only possible decisions are $0$ and $1$, at least $\frac{|C|}{4}$ processes from $C$ (denoted by $C' \subseteq C$) decide the same bit $b'$ in $\mathcal{E}_1$.

    We prove the lemma by contradiction.
    Assume that (1) all processes from $B'$ decide $0$ in $\mathcal{E}_0$ (i.e., $b = 0$), and (2) all processes from $C'$ decide $1$ in $\mathcal{E}_1$ (i.e., $b' = 1$).

    Now consider the infinite execution $\mathcal{E}_2$ with the same set of processes as $\mathcal{E}_0$ (and $\mathcal{E}_1$).
    \begin{compactitem}
        \item $\mathcal{E}_2$: Processes in $C$ propose $1$; all other processes propose 0. 
        Group $B$ is receive-isolated from round 1.
        No message $m$ between any two processes $i,j \in B$ is send-omitted or receive-omitted.
        Group $C$ is receive-isolated from round 1.
        No message $m$ between any two processes $i,j \in C$ is send-omitted or receive-omitted.
        All other processes (i.e., those in $A$) are correct.
    \end{compactitem}
Note that $|\mathcal{F}(\mathcal{E}_2)| = |\mathcal{F}(\mathcal{E}_0)| + |\mathcal{F}(\mathcal{E}_1)| \leq \frac{t}{2} \leq t$, so such an execution exists.

Consider the pair of executions $\mathcal{E}_0$ and $\mathcal{E}_2$.
\Cref{lemma:similar_decision} applies, which means that all processes in $B'$ must decide $0$ in $\mathcal{E}_2$, as they do in $\mathcal{E}_0$.
Similarly, consider the pair of executions $\mathcal{E}_1$ and $\mathcal{E}_2$.
\Cref{lemma:similar_decision} also applies, which means that all processes in $C'$ must decide $1$ in $\mathcal{E}_2$, as they do in $\mathcal{E}_1$.
However, by \Cref{lemma:disagreement_quadratic_messages_formal}, that means that correct processes send at least $\frac{t^2}{32}$ messages in $\mathcal{E}_2$, which is impossible as $\mathcal{A}$ sends less than $\frac{t^2}{32}$ messages in any execution.
\end{proof}

\begin{proof}
Let $\mathcal{E}_0 = [\mathcal{F}^0, \mathcal{B}_1^0, ..., \mathcal{B}_n^0]$.
Note that $\mathcal{F}^0 = B$.
Moreover, no process $P_i$ commits a send-omission fault in $\mathcal{B}_i^0$.
By \Cref{lemma:forced_termination}, at least $\frac{|B|}{2}$ processes from $B$ decide in $\mathcal{E}_0$.
As the only possible decisions are $0$ and $1$, at least $\frac{|B|}{4}$ processes from $B$ (denoted by $B' \subseteq B$) decide the same bit $b$ in $\mathcal{E}_0$.

Similarly, let $\mathcal{E}_1 = [\mathcal{F}^1, \mathcal{B}_1^1, ..., \mathcal{B}_n^0]$.
We have that (1) $\mathcal{F}^1 = C$, and (2) no process $P_i$ commits a send-omission fault in $\mathcal{B}_i^1$.
By \Cref{lemma:forced_termination}, at least $\frac{|C|}{2}$ processes from $C$ decide in $\mathcal{E}_1$.
As the only possible decisions are $0$ and $1$, at least $\frac{|C|}{4}$ processes from $C$ (denoted by $C' \subseteq C$) decide the same bit $b'$ in $\mathcal{E}_1$.

We prove the lemma by contradiction.
Assume that (1) all processes from $B'$ decide $0$ in $\mathcal{E}_0$ (i.e., $b = 0$), and (2) all processes from $C'$ decide $1$ in $\mathcal{E}_1$ (i.e., $b' = 1$).
We now construct an infinite execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$: 
\begin{compactenum}
    \item $\mathcal{F} = B \cup C$.

    \item For every process $P_i$, $\mathcal{B}_i \gets \text{empty behavior}$.

    \item For every round $k \in \mathbb{N}^+ \cup \{ +\infty \}$, we consider $k$-round fragments of each process:
    \begin{compactenum}
            \item For every process $P_i \in A$, we define $s_i(k)$ and $M_i^S(k)$ in the following way:
            \begin{compactitem}
                \item If $k = 1$, then $s_i(k) \gets \pstatezero{i}$ and $M_i^S(k) \gets \mathcal{M}_i^0$.
                Note that, for every message $m \in M_i^S(k)$, $m.\mathsf{sender} = P_i$, $m.\mathsf{round} = 1$, $m.\mathsf{receiver} \neq P_i$ and there is no other message $m' \in M_i^S(k)$ with $m'.\mathsf{receiver} = m.\mathsf{receiver}$.

                \item Otherwise, $\mathcal{A}(\fstate{\mathcal{B}_i}{k - 1}, \fmsgr{\mathcal{B}_i}{k - 1}) = (s_i(k), M_i^S(k))$.
                Note that the following holds: (1) $s_i(k).\mathsf{process} = P_i$, (2) $s_i(k).\mathsf{round} = k$, (3) $s_i(k).\mathsf{proposal} = \fstate{\mathcal{B}_i}{k - 1}.\mathsf{proposal}$, (4) if $\fstate{\mathcal{B}_i}{k - 1}.\mathsf{decision} = b \neq \bot$, then $s_i(k).\mathsf{decision} = b$, and (5) for every message $m \in M_i^S(k)$, $m.\mathsf{sender} = P_i$, $m.\mathsf{round} = k$, $m.\mathsf{receiver} \neq P_i$ and there is no other message $m' \in M_i^S(k)$ with $m'.\mathsf{receiver} = m.\mathsf{receiver}$.
            \end{compactitem}  

            \item Let $M^S(k) = \bigcup\limits_{P_i \in A} M_i^S(k) \cup \bigcup\limits_{P_i \in B} \fmsgs{\mathcal{B}_i^{0}}{k} \cup \bigcup\limits_{P_i \in C} \fmsgs{\mathcal{B}_i^1}{k}$.

            \item For every process $P_i$, $M^R_i(k) = \{ m \,|\, m \in M^S(k) \land m.\mathsf{receiver} = P_i\}$.
            The following holds for $M_i^R(k)$:
            \begin{compactitem}
                \item For every message $m \in M_i^R(k)$, $m.\mathsf{round} = k$.
                This claim follows directly from the fact that, for every $m' \in M^S(k)$, $m'.\mathsf{round} = k$.

                \item For every message $m \in M_i^R(k)$, $m.\mathsf{receiver} = P_i$.
                This follows from the definition of $M_i^R(k)$.

                \item There is no message $m \in M_i^R(k)$ such that $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$.
                This claim follows directly from the fact that, for every $m' \in M^S(k)$, $m'.\mathsf{sender} \neq m'.\mathsf{receiver}$.

                \item If $P_i \in B$, then there are no two messages $m, m' \in \fmsgr{\mathcal{B}_i^0}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$, for some process $P_j$.
                We prove this claim by contradiction.
                Hence, let there be two messages $m, m' \in \fmsgr{\mathcal{B}_i^0}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$.
                Let us consider all possibilities:
                \begin{compactitem}
                    \item $m, m' \in \fmsgr{\mathcal{B}_i^0}{k}$.
                    In this case, $P_j \in B$ (as $B$ is receive-isolated from round $1$ in $\mathcal{E}_0$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^0$.

                    \item $m, m' \in M_i^R(k)$.
                    This case is impossible as, for any two messages $m_1, m_2 \in M^S(k)$ with $m_1.\mathsf{receiver} = m_2.\mathsf{receiver} = P_i$, $m_1.\mathsf{sender} \neq m_2.\mathsf{sender}$.

                    \item Without loss of generality, let $m \in \fmsgr{\mathcal{B}_i^0}{k}$ and $m' \in M_i^R(k)$.
                    Hence, $P_j \in B$ (as $B$ is receive-isolated from round $1$ in $\mathcal{E}_0$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^0$.
                \end{compactitem}

                \item If $P_i \in C$, then there are no two messages $m, m' \in \fmsgr{\mathcal{B}_i^1}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$, for some process $P_j$.
                We prove this claim by contradiction.
                Hence, let there be two messages $m, m' \in \fmsgr{\mathcal{B}_i^1}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$.
                Let us consider all possibilities:
                \begin{compactitem}
                    \item $m, m' \in \fmsgr{\mathcal{B}_i^1}{k}$.
                    In this case, $P_j \in C$ (as $C$ is receive-isolated from round $1$ in $\mathcal{E}_1$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^1$.

                    \item $m, m' \in M_i^R(k)$.
                    This case is impossible as, for any two messages $m_1, m_2 \in M^S(k)$ with $m_1.\mathsf{receiver} = m_2.\mathsf{receiver} = P_i$, $m_1.\mathsf{sender} \neq m_2.\mathsf{sender}$.

                    \item Without loss of generality, let $m \in \fmsgr{\mathcal{B}_i^1}{k}$ and $m' \in M_i^R(k)$.
                    Hence, $P_j \in C$ (as $C$ is receive-isolated from round $1$ in $\mathcal{E}_1$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^1$.
                \end{compactitem}
            \end{compactitem}

            \item For every process $P_i \in A$, let $\mathcal{F}^k_i = \Bigl( s_i(k), M_i^S(k), \emptyset, M_i^R(k), \emptyset \Bigl)$.
            We concatenate $\mathcal{F}^k_i$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k$-round behavior of $P_i$. \manuel{needs aux lemma}
            % Note that $\mathcal{F}^k_i$ is a $k$-round fragment of $P_i$ and $\mathcal{B}_i$ is a $k$-round behavior of $P_i$.

            \item For every process $P_i \in B$, let $\mathcal{F}^k_i = \Bigl( \fstate{\mathcal{B}_i^0}{k}, \fmsgs{\mathcal{B}_i^{0}}{k}, \emptyset = \fmsgso{\mathcal{B}_i^{0}}{k}, \fmsgr{\mathcal{B}_i^{0}}{k}, M_i^R(k) \setminus{\fmsgr{\mathcal{B}_i^{0}}{k}} \Bigl)$.
            We concatenate $\mathcal{F}_i^k$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k$-round behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
            % Note that $\mathcal{F}_i^k$ is a $k$-round fragment of $P_i$ and $\mathcal{B}_i$ is a $k$-round behavior of $P_i$.

            \item For every process $P_i \in C$, let $\mathcal{F}^k_i = \Bigl( \fstate{\mathcal{B}_i^1}{k}, \fmsgs{\mathcal{B}_i^1}{k}, \emptyset = \fmsgso{\mathcal{B}_i^1}{k}, \fmsgr{\mathcal{B}_i^1}{k}, M_i^R(k) \setminus{\fmsgr{\mathcal{B}_i^1}{k}} \Bigl)$.
            We concatenate $\mathcal{F}^k_i$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k$-round behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
            % Note that $\mathcal{F}^k_i$ is a $k$-round fragment of $P_i$ and $\mathcal{B}_i$ is a $k$-round behavior of $P_i$. 
        \end{compactenum}
\end{compactenum}
Let us prove that $\mathcal{E}$ is an execution:
\begin{compactitem}
    \item Faulty processes: As $\mathcal{F} = B \cup C$, $|\mathcal{F}| \leq t$.

    \item Composition: Proven during the construction.
    
    % Holds as, for every process $P_i$, $\mathcal{B}_i$ is an infinite behavior of $P_i$.

    \item Send-validity: Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s}{j}$.
    Note that $m \in M^S(j)$, which implies that $m \in M_r^R(j)$.
    We consider three possible cases:
    \begin{compactitem}
        \item Let $P_r \in A$.
        In this case, $m$ is received by $P_r$ due to the step (3)(d).

        \item Let $P_r \in B$.
        In this case, $m$ is received or receive-omitted by $P_r$ due to the step (3)(e).

        \item Let $P_r \in C$.
        In this case, $m$ is received or receive-omitted by $P_r$ due to the step (3)(f).
    \end{compactitem}

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
    We prove that $m \in M_r^R(j)$:
    \begin{compactitem}
        \item If $P_r \in A$, the statement is true due to the step (3)(d).

        \item If $P_r \in B$, we further consider two scenarios:
        \begin{compactitem}
            \item If $m \in \fmsgr{\mathcal{B}_r}{j}$, then $m \in \fmsgr{\mathcal{B}_r^0}{j}$ due to the step (3)(e).
            Hence, $P_s \in B$, which implies $m \in \fmsgs{\mathcal{B}_s^0}{j}$ (as $\mathcal{E}_0$ satisfies receive-validity).
            Therefore, $m \in M^S(j)$, which implies that $m \in M_r^R(j)$.

            \item If $m \in \fmsgro{\mathcal{B}_r}{j}$, then $m \in M_r^R(j)$ due to the step (3)(e).
        \end{compactitem}

        \item If $P_r \in C$, we further consider two scenarios:
        \begin{compactitem}
            \item If $m \in \fmsgr{\mathcal{B}_r}{j}$, then $m \in \fmsgr{\mathcal{B}_r^1}{j}$ due to the step (3)(f).
            Hence, $P_s \in C$, which implies $m \in \fmsgs{\mathcal{B}_s^1}{j}$ (as $\mathcal{E}_1$ satisfies receive-validity).
            Therefore, $m \in M^S(j)$, which implies that $m \in M_r^R(j)$.

            \item If $m \in \fmsgro{\mathcal{B}_r}{j}$, then $m \in M_r^R(j)$ due to the step (3)(f).
        \end{compactitem}
    \end{compactitem}
    Indeed, $m \in M_r^R(j)$, which implies that $m \in M^S(j)$.
    Therefore, $m$ is indeed sent in $\mathcal{B}_s$.

    \item Omission-validity: No process $P_i \in A$ commits any omission fault in $\mathcal{B}_i$.
\end{compactitem}
Thus, $\mathcal{E}$ is indeed an execution of $\mathcal{A}$.
Moreover, (1) $B$ is receive-isolated from round $1$ in $\mathcal{E}$, (2) $C$ is receive-isolated from round $1$ in $\mathcal{E}$, (3) processes from group $A$ are correct in $\mathcal{E}$, (4) at least $\frac{|B|}{4}$ processes from $B$ (i.e., $B'$) decide $0$ in $\mathcal{E}$, and (5) at least $\frac{|C|}{4}$ processes from $C$ (i.e., $C'$) decide $1$ in $\mathcal{E}$.
However, by \Cref{lemma:disagreement_quadratic_messages_formal}, correct processes send at least $\frac{t^2}{32}$ messages in $\mathcal{E}$, which is impossible as $\mathcal{A}$ sends less than $\frac{t^2}{32}$ messages in any execution.
\end{proof}

Without loss of generality, the rest of the proof assumes that at least $\frac{|B|}{4}$ processes from $B$ decide $1$ in $\mathcal{E}_0$.
% ; we denote this set of processes by $B_1$.
Next, let $\mathcal{E}^*_0$ denote the fully-correct infinite execution in which all processes propose $0$.
Note that, in order to satisfy \emph{Weak Validity}, all processes decide $0$ in $\mathcal{E}_0^*$.
Let $k_0^* \in \mathbb{N}^+$ denote the first round in which (at least) $\frac{|B|}{4}$ processes from $B$ decide the same bit in $\mathcal{E}_0^*$.

For every round $k \in [1, k_0^*]$, we perform the following actions:
\begin{compactenum}
    \item We consider the infinite execution $\mathcal{E}^k$ such that (1) every process proposes $0$, (2) every process behaves correctly until (and including) round $k - 1$ (i.e., no omission faults occur), (3) group $B$ is receive-isolated from round $k$, and (4) processes in $A \cup C$ are correct.

    \item By \Cref{lemma:forced_termination}, at least $\frac{|B|}{2}$ processes from $B$ decide in $\mathcal{E}^k$.
    As there are only two decision-bits, at least $\frac{|B|}{4}$ processes from $B$ decide the same bit $b_k$ in $\mathcal{E}^k$.
\end{compactenum}
Importantly, $b_1 = 1$ (due to the assumption) and $b_{k_0^*} = 0$ (due to the execution $\mathcal{E}_0^*$).
Hence, there exists a round $k^* \geq 1$ such that $b_{k^*} = 1$ and $b_{k^* + 1} = 0$.

Now, consider an infinite execution $\mathcal{E}_C$ such that (1) every process proposes $0$, (2) every process behaves correctly until (and including) round $k^* - 1$, (3) group $C$ is receive-isolated from round $k^*$, and (4) processes in $A \cup B$ are correct.
By \Cref{lemma:forced_termination} and the fact that only two decision-bits exist, at least $\frac{|C|}{4}$ processes from $C$ decide the same bit $b_C$.
Finally, we are ready to prove that there exists an execution of $\mathcal{A}$ with (at least) $\frac{t^2}{32}$ messages sent by correct processes.

Let $\mathcal{E}^{k^*} = [\mathcal{F}^{k^*} = B, \mathcal{B}^{k^*}_1, ..., \mathcal{B}^{k^*}_n]$, let $\mathcal{E}^{k^* + 1} = [\mathcal{F}^{k^* + 1} = B, \mathcal{B}^{k^* + 1}_1, ..., \mathcal{B}^{k^* + 1}_n]$ and let $\mathcal{E}^C = [\mathcal{F}^C = C, \mathcal{B}_1^C, ..., \mathcal{B}_n^C]$.
The following holds:
\begin{compactitem}
    \item At least $\frac{|B|}{4}$ processes from $B$ decide the $1$ in $\mathcal{E}^{k^*}$.

    \item At least $\frac{|B|}{4}$ processes from $B$ decide the $0$ in $\mathcal{E}^{k^* + 1}$.
    
    \item At least $\frac{|C|}{4}$ processes from $C$ decide the same bit $b_C$ in $\mathcal{E}^C$.

    \item Until (and including) round $k^* - 1$, $\mathcal{B}_i^{k^*} = \mathcal{B}_i^{k^* + 1} = \mathcal{B}_i^C$, for every process $P_i$.
\end{compactitem}

\begin{lemma} \label{lemma:final_formal}
There exists an infinite execution of $\mathcal{A}$ in which correct processes send (at least) $\frac{t^2}{32}$ messages.
\end{lemma}

\manuel{The next proof is an attempt at an alternative proof of the previous Lemma. Work in Progress...}

\begin{proof}
    Suppose also that (1) in $\mathcal{E}^{k^*}$ or $\mathcal{E}^{k}$, no message $m$ between any two processes $i,j \in B$ is send-omitted or receive-omitted, and (2) in $\mathcal{E}^C$, no message $m$ between any two processes $i,j \in C$ is send-omitted or receive-omitted. \manuel{Again, we can just make this part of the definition of receive-isolation.}

    Now consider the two infinite execution $\mathcal{E}^{Ck^*}$ and $\mathcal{E}^{Ck^*+1}$.
    \begin{compactitem}
        \item $\mathcal{E}^{Ck^*}$: All processes propose 0. 
        Group $B$ is receive-isolated from round $k^{*}$.
        No message $m$ between any two processes $i,j \in B$ is send-omitted or receive-omitted.
        Group $C$ is receive-isolated from round $k^*$.
        No message $m$ between any two processes $i,j \in C$ is send-omitted or receive-omitted.
        All other processes (i.e., those in $A$) are correct.
        
        \item $\mathcal{E}^{Ck^*+1}$: All processes propose 0. 
        Group $B$ is receive-isolated from round $k^*+1$.
        No message $m$ between any two processes $i,j \in B$ is send-omitted or receive-omitted.
        Group $C$ is receive-isolated from round $k^*$.
        No message $m$ between any two processes $i,j \in C$ is send-omitted or receive-omitted.
        All other processes (i.e., those in $A$) are correct.
    \end{compactitem}

    Applying \Cref{lemma:similar_decision} to both ($\mathcal{E}^{Ck^*}$, $\mathcal{E}^{C}$) and ($\mathcal{E}^{Ck^*+1}$, $\mathcal{E}^{C}$), we get that in both executions at least $\frac{|C|}{4}$ processes from $C$ decide the same bit $b_C$.
    Applying \Cref{lemma:similar_decision} to ($\mathcal{E}^{Ck^*}$, $\mathcal{E}^{k^*}$), we get that in $\mathcal{E}^{Ck^*}$ at least $\frac{|B|}{4}$ processes from $B$ decide the same bit $0$.
    Applying \Cref{lemma:similar_decision} to ($\mathcal{E}^{Ck^*+1}$, $\mathcal{E}^{k^*+1}$), we get that in $\mathcal{E}^{Ck^*+1}$ at least $\frac{|B|}{4}$ processes from $B$ decide the same bit $1$.
    Thus, no matter the value of $b_C$, in either $\mathcal{E}^{Ck^*+1}$ or $\mathcal{E}^{Ck^*}$, at least $\frac{|B|}{4}$ processes decide the same bit $b$ and at least $\frac{|C|}{4}$ decide the same bit $b'$ such that $b \neq b'$.
    But, by \Cref{lemma:disagreement_quadratic_messages_formal}, correct processes send at least $\frac{t^2}{32}$ messages in that execution, which proves the lemma.
\end{proof}

\begin{proof}
We construct an execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Let us consider two possible cases:
\begin{compactitem}
    \item Let $b_C = 0$.
    We construct $\mathcal{E}$ in the following manner:
    \begin{compactenum}
        \item $\mathcal{F} = B \cup C$.

        \item For every process $P_i$, $\mathcal{B}_i \gets \mathsf{prefix}(\mathcal{B}_i^{k^*}, k^* - 1)$.
        In other words, $\mathcal{B}_i$ is identical to $\mathcal{B}_i^{k^*} = \mathcal{B}_i^C$ until (and including) round $k^* - 1$, which implies that, at this point, $\mathcal{B}_i$ is a $(k^* - 1)$-round behavior of $P_i$.

        \item Next, we consider $k$-round fragments of each process, for every $k \in [k^*, \infty]$:
        \begin{compactenum}
            \item For every process $P_i \in A$, we define $s_i(k)$ and $M_i^S(k)$ in the following way:
            \begin{compactitem}
                \item If $k^* = 1$, then $s_i(k) \gets \pstatezero{i}$ and $M_i^S(k) \gets \mathsf{send\_init}(0)$.
                Note that, for every message $m \in M_i^S(k)$, $m.\mathsf{sender} = P_i$, $m.\mathsf{round} = 1$, $m.\mathsf{receiver} \neq P_i$ and there is no other message $m' \in M_i^S(k)$ with $m'.\mathsf{receiver} = m.\mathsf{receiver}$.

                \item Otherwise, $\mathcal{A}(\fstate{\mathcal{B}_i}{k - 1}, \fmsgr{\mathcal{B}_i}{k - 1}) = (s_i(k), M_i^S(k))$.
                Note that the following holds: (1) $s_i(k).\mathsf{process} = P_i$, (2) $s_i(k).\mathsf{round} = k$, (3) $s_i(k).\mathsf{proposal} = \fstate{\mathcal{B}_i}{k - 1}.\mathsf{proposal}$, (4) if $\fstate{\mathcal{B}_i}{k - 1}.\mathsf{decision} = b \neq \bot$, then $s_i(k).\mathsf{decision} = b$, and (5) for every message $m \in M_i^S(k)$, $m.\mathsf{sender} = P_i$, $m.\mathsf{round} = k$, $m.\mathsf{receiver} \neq P_i$ and there is no other message $m' \in M_i^S(k)$ with $m'.\mathsf{receiver} = m.\mathsf{receiver}$.
            \end{compactitem}  

            \item Let $M^S(k) = \bigcup\limits_{P_i \in A} M_i^S(k) \cup \bigcup\limits_{P_i \in B} \fmsgs{\mathcal{B}_i^{k^*}}{k} \cup \bigcup\limits_{P_i \in C} \fmsgs{\mathcal{B}_i^C}{k}$.

            \item For every process $P_i$, $M^R_i(k) = \{ m \,|\, m \in M^S(k) \land m.\mathsf{receiver} = P_i\}$.
            The following holds for $M_i^R(k)$:
            \begin{compactitem}
                \item For every message $m \in M_i^R(k)$, $m.\mathsf{round} = k$.
                This claim follows directly from the fact that, for every $m' \in M^S(k)$, $m'.\mathsf{round} = k$.

                \item For every message $m \in M_i^R(k)$, $m.\mathsf{receiver} = P_i$.
                This follows from the definition of $M_i^R(k)$.

                \item There is no message $m \in M_i^R(k)$ such that $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$.
                This claim follows directly from the fact that, for every $m' \in M^S(k)$, $m'.\mathsf{sender} \neq m'.\mathsf{receiver}$.

                \item If $P_i \in B$, then there are no two messages $m, m' \in \fmsgr{\mathcal{B}_i^{k^*}}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$, for some process $P_j$.
                We prove this claim by contradiction.
                Hence, let there be two messages $m, m' \in \fmsgr{\mathcal{B}_i^{k^*}}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$.
                Let us consider all possibilities:
                \begin{compactitem}
                    \item $m, m' \in \fmsgr{\mathcal{B}_i^{k^*}}{k}$.
                    In this case, $P_j \in B$ (as $B$ is receive-isolated from round $k^*$ in $\mathcal{E}^{k^*}$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^{k^*}$.

                    \item $m, m' \in M_i^R(k)$.
                    This case is impossible as, for any two messages $m_1, m_2 \in M^S(k)$ with $m_1.\mathsf{receiver} = m_2.\mathsf{receiver} = P_i$, $m_1.\mathsf{sender} \neq m_2.\mathsf{sender}$.

                    \item Without loss of generality, let $m \in \fmsgr{\mathcal{B}_i^{k^*}}{k}$ and $m' \in M_i^R(k)$.
                    Hence, $P_j \in B$ (as $B$ is receive-isolated from round $k^*$ in $\mathcal{E}^{k^*}$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^{k^*}$.
                \end{compactitem}

                \item If $P_i \in C$, then there are no two messages $m, m' \in \fmsgr{\mathcal{B}_i^C}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$, for some process $P_j$.
                We prove this claim by contradiction.
                Hence, let there be two messages $m, m' \in \fmsgr{\mathcal{B}_i^C}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$.
                Let us consider all possibilities:
                \begin{compactitem}
                    \item $m, m' \in \fmsgr{\mathcal{B}_i^C}{k}$.
                    In this case, $P_j \in C$ (as $C$ is receive-isolated from round $k^*$ in $\mathcal{E}^C$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^C$.

                    \item $m, m' \in M_i^R(k)$.
                    This case is impossible as, for any two messages $m_1, m_2 \in M^S(k)$ with $m_1.\mathsf{receiver} = m_2.\mathsf{receiver} = P_i$, $m_1.\mathsf{sender} \neq m_2.\mathsf{sender}$.

                    \item Without loss of generality, let $m \in \fmsgr{\mathcal{B}_i^C}{k}$ and $m' \in M_i^R(k)$.
                    Hence, $P_j \in C$ (as $C$ is receive-isolated from round $k^*$ in $\mathcal{E}^C$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^C$.
                \end{compactitem}
            \end{compactitem}

            \item For every process $P_i \in A$, let $\mathcal{F}^k_i = \Bigl( s_i(k), M_i^S(k), \emptyset, M_i^R(k), \emptyset \Bigl)$.
            We concatenate $\mathcal{F}^k_i$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k$-round behavior of $P_i$. \manuel{needs aux lemma}
            
            \item For every process $P_i \in B$, let $\mathcal{F}^k_i = \Bigl( \fstate{\mathcal{B}_i^{k^*}}{k}, \fmsgs{\mathcal{B}_i^{k^*}}{k}, \emptyset = \fmsgso{\mathcal{B}_i^{k^*}}{k}, \fmsgr{\mathcal{B}_i^{k^*}}{k}, M_i^R(k) \setminus{\fmsgr{\mathcal{B}_i^{k^*}}{k}} \Bigl)$.
            We concatenate $\mathcal{F}_i^k$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k$-round behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.

            \item For every process $P_i \in C$, let $\mathcal{F}^k_i = \Bigl( \fstate{\mathcal{B}_i^C}{k}, \fmsgs{\mathcal{B}_i^C}{k}, \emptyset = \fmsgso{\mathcal{B}_i^C}{k}, \fmsgr{\mathcal{B}_i^C}{k}, M_i^R(k) \setminus{\fmsgr{\mathcal{B}_i^C}{k}} \Bigl)$.
            We concatenate $\mathcal{F}^k_i$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k$-round behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
            \end{compactenum}
    \end{compactenum}
    Let us prove that $\mathcal{E}$ is an execution:
    \begin{compactitem}
        \item Faulty processes: As $\mathcal{F} = B \cup C$, $|\mathcal{F}| \leq t$.

        \item Composition: Proven during the construction.

        \item Send-validity: Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s}{j}$.
        Note that $m \in M^S(j)$, which implies that $m \in M_r^R(j)$.
        We consider three possible cases:
        \begin{compactitem}
            \item Let $P_r \in A$.
            In this case, $m$ is received by $P_r$ due to the step (3)(d).

            \item Let $P_r \in B$.
            In this case, $m$ is received or receive-omitted by $P_r$ due to the step (3)(e).

            \item Let $P_r \in C$.
            In this case, $m$ is received or receive-omitted by $P_r$ due to the step (3)(f).
        \end{compactitem}

        \item Receive-validity:
        Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
        We prove that $m \in M_r^R(j)$:
    \begin{compactitem}
        \item If $P_r \in A$, the statement is true due to the step (3)(d).

        \item If $P_r \in B$, we further consider two scenarios:
        \begin{compactitem}
            \item If $m \in \fmsgr{\mathcal{B}_r}{j}$, then $m \in \fmsgr{\mathcal{B}_r^{k^*}}{j}$ due to the step (3)(e).
            Hence, $P_s \in B$, which implies $m \in \fmsgs{\mathcal{B}_s^{k^*}}{j}$ (as $\mathcal{E}^{k^*}$ satisfies receive-validity).
            Therefore, $m \in M^S(j)$, which implies that $m \in M_r^R(j)$.

            \item If $m \in \fmsgro{\mathcal{B}_r}{j}$, then $m \in M_r^R(j)$ due to the step (3)(e).
        \end{compactitem}

        \item If $P_r \in C$, we further consider two scenarios:
        \begin{compactitem}
            \item If $m \in \fmsgr{\mathcal{B}_r}{j}$, then $m \in \fmsgr{\mathcal{B}_r^C}{j}$ due to the step (3)(f).
            Hence, $P_s \in C$, which implies $m \in \fmsgs{\mathcal{B}_s^C}{j}$ (as $\mathcal{E}^C$ satisfies receive-validity).
            Therefore, $m \in M^S(j)$, which implies that $m \in M_r^R(j)$.

            \item If $m \in \fmsgro{\mathcal{B}_r}{j}$, then $m \in M_r^R(j)$ due to the step (3)(f).
        \end{compactitem}
    \end{compactitem}
    Indeed, $m \in M_r^R(j)$, which implies that $m \in M^S(j)$.
    Therefore, $m$ is indeed sent in $\mathcal{B}_s$.
        
        \item Omission-validity: No process $P_i \in A$ commits any omission fault in $\mathcal{B}_i$.
    \end{compactitem}
    Thus, $\mathcal{E}$ is indeed an infinite execution of $\mathcal{A}$.
    Moreover, (1) $B$ is receive-isolated from round $k^*$ in $\mathcal{E}$, (2) $C$ is receive-isolated from round $k^*$ in $\mathcal{E}$, (3) processes from group $A$ are correct in $\mathcal{E}$, (4) at least $\frac{|B|}{4}$ processes from $B$ decide $1$ in $\mathcal{E}$, and (5) at least $\frac{|C|}{4}$ processes from $C$ decide $0$ in $\mathcal{E}$.
    By \Cref{lemma:disagreement_quadratic_messages_formal}, correct processes send at least $\frac{t^2}{32}$ messages in $\mathcal{E}$, which proves the lemma in this case.


    \item Let $b_C = 1$. We construct $\mathcal{E}$ in the following steps:
    \begin{compactenum}
        \item $\mathcal{F} = B \cup C$.

        \item For every process $P_i$, $\mathcal{B}_i \gets \mathsf{prefix}(\mathcal{B}_i^{k^*}, k^* - 1)$.
        In other words, $\mathcal{B}_i$ is identical to $\mathcal{B}_i^{k^*} = \mathcal{B}_i^{k^* + 1} = \mathcal{B}_i^C$ until (and including) round $k^* - 1$, which implies that, at this point, $\mathcal{B}_i$ is a $(k^* - 1)$-round behavior of $P_i$.

        \item Next, we consider $k^*$-fragments of each process:
        \begin{compactenum}
            \item Let $M^S(k^*) = \bigcup\limits_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{k^*}}{k^*}$.

            \item For every process $P_i$, $M^R_i(k^*) = \{ m \,|\, m \in M^S(k^*) \land m.\mathsf{receiver} = P_i\}$.
            The following holds for $M_i^R(k^*)$:
            \begin{compactitem}
                \item For every message $m \in M_i^R(k^*)$, $m.\mathsf{round} = k^*$.
                This claim follows directly from the fact that, for every $m' \in M^S(k^*)$, $m'.\mathsf{round} = k^*$.

                \item For every message $m \in M_i^R(k^*)$, $m.\mathsf{receiver} = P_i$.
                This follows from the definition of $M_i^R(k^*)$.

                \item There is no message $m \in M_i^R(k^*)$ such that $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$.
                This claim follows directly from the fact that, for every $m' \in M^S(k^*)$, $m'.\mathsf{sender} \neq m'.\mathsf{receiver}$.

                \item If $P_i \in B$, then there are no two messages $m, m' \in \fmsgr{\mathcal{B}_i^{k^* + 1}}{k^*} \cup M_i^R(k^*)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$, for some process $P_j$.
                We prove this claim by contradiction.
                Hence, let there be two messages $m, m' \in \fmsgr{\mathcal{B}_i^{k^* + 1}}{k^*} \cup M_i^R(k^*)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$.
                Let us consider all possibilities:
                \begin{compactitem}
                    \item $m, m' \in \fmsgr{\mathcal{B}_i^{k^* + 1}}{k^*}$.
                    Thus, $m, m' \in \fmsgs{\mathcal{B}_j^{k^* + 1}}{k^*}$ (as $\mathcal{E}^{k^*}$ satisfies receive-validity).
                    Hence, this case is impossible.

                    \item $m, m' \in M_i^R(k^*)$.
                    This case is impossible as, for any two messages $m_1, m_2 \in M^S(k^*)$ with $m_1.\mathsf{receiver} = m_2.\mathsf{receiver} = P_i$, $m_1.\mathsf{sender} \neq m_2.\mathsf{sender}$.

                    \item Without loss of generality, let $m \in \fmsgr{\mathcal{B}_i^{k^* + 1}}{k^*}$ and $m' \in M_i^R(k^*)$.
                    As $m' \in M_i^R(k^*)$, $m' \in M^S(k^*)$.
                    As $m \in \fmsgr{\mathcal{B}_i^{k^* + 1}}{k^*}$, $m \in \fmsgs{\mathcal{B}_j^{k^* + 1}}{k^*}$ (as $\mathcal{E}^{k^* + 1}$ satisfies receive-validity).
                    Moreover, since $\fmsgs{\mathcal{B}^{k^* + 1}_j}{k^*} = \fmsgs{\mathcal{B}^{k^*}_j}{k^*}$, $m \in M^S(k^*)$.
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^{k^*}$.
                \end{compactitem}

                \item If $P_i \in C$, then there are no two messages $m, m' \in \fmsgr{\mathcal{B}_i^C}{k^*} \cup M_i^R(k^*)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$, for some process $P_j$.
                We prove this claim by contradiction.
                Hence, let there be two messages $m, m' \in \fmsgr{\mathcal{B}_i^C}{k^*} \cup M_i^R(k^*)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$.
                Let us consider all possibilities:
                \begin{compactitem}
                    \item $m, m' \in \fmsgr{\mathcal{B}_i^C}{k^*}$.
                    In this case, $P_j \in C$ (as $C$ is receive-isolated from round $k^*$ in $\mathcal{E}^C$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^C$.

                    \item $m, m' \in M_i^R(k^*)$.
                    This case is impossible as, for any two messages $m_1, m_2 \in M^S(k)$ with $m_1.\mathsf{receiver} = m_2.\mathsf{receiver} = P_i$, $m_1.\mathsf{sender} \neq m_2.\mathsf{sender}$.

                    \item Without loss of generality, let $m \in \fmsgr{\mathcal{B}_i^C}{k^*}$ and $m' \in M_i^R(k^*)$.
                    Hence, $P_j \in C$ (as $C$ is receive-isolated from round $k^*$ in $\mathcal{E}^C$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^C$.
                \end{compactitem}
            \end{compactitem}

            \item For every process $P_i \in A$, let $\mathcal{F}^{k^*}_i = \Bigl( \fstate{\mathcal{B}_i^{k^*}}{k^*}, \fmsgs{\mathcal{B}_i^{k^*}}{k^*}, \emptyset, M_i^R(k^*), \emptyset \Bigl)$.
            We concatenate $\mathcal{F}^{k^*}_i$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k^*$-round behavior of $P_i$. \manuel{not done yet}

            \item For every process $P_i \in B$, let $\mathcal{F}^{k^*}_i = \Bigl( \fstate{\mathcal{B}_i^{k^*}}{k^*}, \fmsgs{\mathcal{B}_i^{k^*}}{k^*}, \emptyset = \fmsgso{\mathcal{B}_i^{k^*}}{k^*}, \fmsgr{\mathcal{B}_i^{k^*}}{k^*}, M_i^R(k^*) \setminus{\fmsgr{\mathcal{B}_i^{k^*}}{k^*}} = \emptyset \Bigl)$.
            We concatenate $\mathcal{F}_i^{k^*}$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k^*$-round behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.

            \item For every process $P_i \in C$, let $\mathcal{F}^{k^*}_i = \Bigl( \fstate{\mathcal{B}_i^C}{k^*}, \fmsgs{\mathcal{B}_i^C}{k^*}, \emptyset = \fmsgso{\mathcal{B}_i^C}{k^*}, \fmsgr{\mathcal{B}_i^C}{k^*}, M_i^R(k^*) \setminus{\fmsgr{\mathcal{B}_i^C}{k^*}} \Bigl)$.
            We concatenate $\mathcal{F}^{k^*}_i$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k^*$-round behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
        \end{compactenum}

        \item Next, we consider $k$-round fragments of each process, for every $k \in [k^* + 1, \infty]$:
        \begin{compactenum}
            \item For every process $P_i \in A$, let $\mathcal{A}(\fstate{\mathcal{B}_i}{k - 1}, \fmsgr{\mathcal{B}_i}{k - 1}) = (s_i(k), M_i^S(k))$.
                Note that the following holds: (1) $s_i(k).\mathsf{process} = P_i$, (2) $s_i(k).\mathsf{round} = k$, (3) $s_i(k).\mathsf{proposal} = \fstate{\mathcal{B}_i}{k - 1}.\mathsf{proposal}$, (4) if $\fstate{\mathcal{B}_i}{k - 1}.\mathsf{decision} = b \neq \bot$, then $s_i(k).\mathsf{decision} = b$, and (5) for every message $m \in M_i^S(k)$, $m.\mathsf{sender} = P_i$, $m.\mathsf{round} = k$, $m.\mathsf{receiver} \neq P_i$ and there is no other message $m' \in M_i^S(k)$ with $m'.\mathsf{receiver} = m.\mathsf{receiver}$.

            \item Let $M^S(k) = \bigcup\limits_{P_i \in A} M_i^S(k) \cup \bigcup\limits_{P_i \in B} \fmsgs{\mathcal{B}_i^{k^* + 1}}{k} \cup \bigcup\limits_{P_i \in C} \fmsgs{\mathcal{B}_i^C}{k}$.

            \item For every process $P_i$, $M^R_i(k) = \{ m \,|\, m \in M^S(k) \land m.\mathsf{receiver} = P_i\}$.
            The following holds for $M_i^R(k)$:
            \begin{compactitem}
                \item For every message $m \in M_i^R(k)$, $m.\mathsf{round} = k$.
                This claim follows directly from the fact that, for every $m' \in M^S(k)$, $m'.\mathsf{round} = k$.

                \item For every message $m \in M_i^R(k)$, $m.\mathsf{receiver} = P_i$.
                This follows from the definition of $M_i^R(k)$.

                \item There is no message $m \in M_i^R(k)$ such that $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$.
                This claim follows directly from the fact that, for every $m' \in M^S(k)$, $m'.\mathsf{sender} \neq m'.\mathsf{receiver}$.

                \item If $P_i \in B$, then there are no two messages $m, m' \in \fmsgr{\mathcal{B}_i^{k^* + 1}}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$, for some process $P_j$.
                We prove this claim by contradiction.
                Hence, let there be two messages $m, m' \in \fmsgr{\mathcal{B}_i^{k^* + 1}}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$.
                Let us consider all possibilities:
                \begin{compactitem}
                    \item $m, m' \in \fmsgr{\mathcal{B}_i^{k^*+ 1}}{k}$.
                    In this case, $P_j \in B$ (as $B$ is receive-isolated from round $k^*+ 1$ in $\mathcal{E}^{k^*+ 1}$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^{k^*+ 1}$.

                    \item $m, m' \in M_i^R(k)$.
                    This case is impossible as, for any two messages $m_1, m_2 \in M^S(k)$ with $m_1.\mathsf{receiver} = m_2.\mathsf{receiver} = P_i$, $m_1.\mathsf{sender} \neq m_2.\mathsf{sender}$.

                    \item Without loss of generality, let $m \in \fmsgr{\mathcal{B}_i^{k^*+ 1}}{k}$ and $m' \in M_i^R(k)$.
                    Hence, $P_j \in B$ (as $B$ is receive-isolated from round $k^*+ 1$ in $\mathcal{E}^{k^*+ 1}$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^{k^*}$.
                \end{compactitem}

                \item If $P_i \in C$, then there are no two messages $m, m' \in \fmsgr{\mathcal{B}_i^C}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$, for some process $P_j$.
                We prove this claim by contradiction.
                Hence, let there be two messages $m, m' \in \fmsgr{\mathcal{B}_i^C}{k} \cup M_i^R(k)$ such that $m.\mathsf{sender} = m'.\mathsf{sender} = P_j$.
                Let us consider all possibilities:
                \begin{compactitem}
                    \item $m, m' \in \fmsgr{\mathcal{B}_i^C}{k}$.
                    In this case, $P_j \in C$ (as $C$ is receive-isolated from round $k^*$ in $\mathcal{E}^C$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^C$.

                    \item $m, m' \in M_i^R(k)$.
                    This case is impossible as, for any two messages $m_1, m_2 \in M^S(k)$ with $m_1.\mathsf{receiver} = m_2.\mathsf{receiver} = P_i$, $m_1.\mathsf{sender} \neq m_2.\mathsf{sender}$.

                    \item Without loss of generality, let $m \in \fmsgr{\mathcal{B}_i^C}{k}$ and $m' \in M_i^R(k)$.
                    Hence, $P_j \in C$ (as $C$ is receive-isolated from round $k^*$ in $\mathcal{E}^C$).
                    This case is impossible as $P_j$ does not send $m$ and $m'$ in $\mathcal{B}_j^C$.
                \end{compactitem}
            \end{compactitem}

            \item For every process $P_i \in A$, let $\mathcal{F}^k_i = \Bigl( s_i(k), M_i^S(k), \emptyset, M_i^R(k), \emptyset \Bigl)$.
            We concatenate $\mathcal{F}^k_i$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k^*$-round behavior of $P_i$ due to the composition of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}. \manuel{not done yet}

            \item For every process $P_i \in B$, let $\mathcal{F}^k_i = \Bigl( \fstate{\mathcal{B}_i^{k^*+1}}{k}, \fmsgs{\mathcal{B}_i^{k^*+1}}{k}, \emptyset = \fmsgso{\mathcal{B}_i^{k^*+1}}{k}, \fmsgr{\mathcal{B}_i^{k^*+1}}{k}, M_i^R(k) \setminus{\fmsgr{\mathcal{B}_i^{k^*+1}}{k}} \Bigl)$.
            We concatenate $\mathcal{F}_i^k$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k^*$-round behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}. \manuel{not done yet}

            \item For every process $P_i \in C$, let $\mathcal{F}^k_i = \Bigl( \fstate{\mathcal{B}_i^C}{k}, \fmsgs{\mathcal{B}_i^C}{k}, \emptyset = \fmsgso{\mathcal{B}_i^C}{k}, \fmsgr{\mathcal{B}_i^C}{k}, M_i^R(k) \setminus{\fmsgr{\mathcal{B}_i^C}{k}} \Bigl)$.
            We concatenate $\mathcal{F}^k_i$ to $\mathcal{B}_i$.
            Resulting $\mathcal{B}_i$ is a $k^*$-round behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}. \manuel{not done yet}
            \end{compactenum}
    \end{compactenum}
    Let us prove that $\mathcal{E}$ is an execution:
    \begin{compactitem}
        \item Faulty processes: As $\mathcal{F} = B \cup C$, $|\mathcal{F}| \leq t$.

        \item Composition: Proven during the construction.

        \item Send-validity: Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s}{j}$.
        Note that $m \in M^S(j)$, which implies that $m \in M_r^R(j)$.
        We consider three possible cases:
        \begin{compactitem}
            \item Let $P_r \in A$.
            In this case, $m$ is received by $P_r$ due to the step (3)(c) or (4)(d).

            \item Let $P_r \in B$.
            In this case, $m$ is received or receive-omitted by $P_r$ due to the step (3)(d) or (4)(e).

            \item Let $P_r \in C$.
            In this case, $m$ is received or receive-omitted by $P_r$ due to the step (3)(e) or (4)(f).
        \end{compactitem}

        \item Receive-validity:
        Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
        We prove that $m \in M_r^R(j)$:
    \begin{compactitem}
        \item If $P_r \in A$, the statement is true due to the steps (3)(c) and (4)(e).

        \item If $P_r \in B$, we further consider two scenarios:
        \begin{compactitem}
            \item If $m \in \fmsgr{\mathcal{B}_r}{j}$, then $m \in \fmsgr{\mathcal{B}_r^{k^* + 1}}{j}$ due to the step (3)(d) and (4)(e).
            If $j = k^*$, then $m \in M^S(j)$.
            If $j > k^*$, then $P_s \in B$, which implies $m \in \fmsgs{\mathcal{B}_s^{k^* + 1}}{j}$ (as $\mathcal{E}^{k^* + 1}$ satisfies receive-validity).
            Therefore, $m \in M^S(j)$, which implies that $m \in M_r^R(j)$.

            \item If $m \in \fmsgro{\mathcal{B}_r}{j}$, then $m \in M_r^R(j)$ due to the steps (3)(c) and (4)(e).
        \end{compactitem}

        \item If $P_r \in C$, we further consider two scenarios:
        \begin{compactitem}
            \item If $m \in \fmsgr{\mathcal{B}_r}{j}$, then $m \in \fmsgr{\mathcal{B}_r^C}{j}$ due to the steps (3)(e) and (4)(f).
            Hence, $P_s \in C$, which implies $m \in \fmsgs{\mathcal{B}_s^C}{j}$ (as $\mathcal{E}^C$ satisfies receive-validity).
            Therefore, $m \in M^S(j)$, which implies that $m \in M_r^R(j)$.

            \item If $m \in \fmsgro{\mathcal{B}_r}{j}$, then $m \in M_r^R(j)$ due to the step (3)(e) and (4)(f).
        \end{compactitem}
    \end{compactitem}
    Indeed, $m \in M_r^R(j)$, which implies that $m \in M^S(j)$.
    Therefore, $m$ is indeed sent in $\mathcal{B}_s$.
        
    \item Omission-validity: No process $P_i \in A$ commits any omission fault in $\mathcal{B}_i$.
    \end{compactitem}
    Thus, $\mathcal{E}$ is indeed an infinite execution of $\mathcal{A}$.
    Moreover, (1) $B$ is receive-isolated from round $k^* + 1$ in $\mathcal{E}$, (2) $C$ is receive-isolated from round $k^*$ in $\mathcal{E}$, (3) processes from group $A$ are correct in $\mathcal{E}$, (4) at least $\frac{|B|}{4}$ processes from $B$ decide $0$ in $\mathcal{E}$, and (5) at least $\frac{|C|}{4}$ processes from $C$ decide $1$ in $\mathcal{E}$.
    By \Cref{lemma:disagreement_quadratic_messages_formal}, correct processes send at least $\frac{t^2}{32}$ messages in $\mathcal{E}$, which proves the lemma in this case.
\end{compactitem}
As the statement of the lemma holds in both possible cases, the proof is concluded.
\end{proof}

==> sections/formal_proof_lower_bound_old_version.tex <==
\section{Lower Bound on Message Complexity for Non-Uniform Consensus with Weak Validity in the Omission Failure Model} \label{section:lower_bound_formal}

\pierre{I have simply merged the file formal\_proof.tex (until definition of receive isolation) and the file suggestions\_4.tex}

\subsection{Preliminaries}

\subsubsection{Messages.}
Each message $m$ encodes the following information:
\begin{compactitem}
    \item the sender of $m$ (denoted by $m.\mathsf{sender} \in \Pi$); and

    \item the receiver of $m$ (denoted by $m.\mathsf{receiver} \in \Pi$); and

    \item the round in which $m$ is sent (denoted by $m.\mathsf{round} \in [1, \infty)$).
\end{compactitem}
As the aforementioned information is encoded in any message $m$, $\mathcal{A}$ does not instruct $m.\mathsf{sender}$ to send $m$ more than once.
Indeed, $m$ can only be sent in round $m.\mathsf{round}$ and only to $m.\mathsf{receiver}$.
As $\mathcal{A}$ instructs $m.\mathsf{sender}$ to send at most one message to $m.\mathsf{receiver}$ in any round, $m$ cannot be sent more than once.


\subsubsection{States.}
% We start by introducing \emph{states} that processes can take at the start of each round.
Let $\mathcal{S}$ denote the set of all states processes can take.
Each state $s$ encodes the following information:
\begin{compactitem}
    \item the process associated with $s$ (denoted by $s.\mathsf{process} \in \Pi$);

    \item the round associated with $s$ (denoted by $s.\mathsf{round} \in [1, \infty)$);

    \item the proposal-bit associated with $s$ (denoted by $s.\mathsf{proposal} \in \{0, 1\}$);

    \item the decision-bit associated with $s$ (denoted by $s.\mathsf{decision} \in \{\bot, 0, 1 \}$).
\end{compactitem} 
% A state $s$ such that $s.\mathsf{process} = P_i$ and $s.\mathsf{round} = k$ is denoted by $\pstate{i}{k}$.
Intuitively, a state $s \in \mathcal{S}$, where (1) $s.\mathsf{process} = P_i$, (2) $s.\mathsf{round} = k$, (3) $s.\mathsf{proposal} = b$, and (4) $s.\mathsf{decision} = b'$, denotes the state of process $P_i$ at the start of round $k$ with $P_i$'s proposal being $b$ and $P_i$'s decision being $b'$ (if $b' = \bot$, $P_i$ has not yet decided by the start of round $k$).

For each process $P_i$, there are two \emph{initial states} $\pstatezero{i} \in \mathcal{S}$ and $\pstateone{i} \in \mathcal{S}$ associated with $P_i$ such that (1) $\pstatezero{i}.\mathsf{process} = \pstateone{i}.\mathsf{process} = P_i$, (2) $\pstatezero{i}.\mathsf{proposal} = 0$, and (3) $\pstateone{i}.\mathsf{proposal} = 1$.
Each process $P_i$ starts round $1$ in either $\pstatezero{i}$ or $\pstateone{i}$.


\subsubsection{Algorithm $\mathcal{A}$ as a state-transition function.}
Algorithm $\mathcal{A}$ maps (1) a state of a process at the start of a round, and (2) messages the process received in the round into (1) a new state of the process at the start of the next round, and (2) messages the process sends in the next round.
Formally, given (1) a state $s$, and (2) a set of messages $M^R$ such that, for every message $m \in M^R$, $m.\mathsf{receiver} = s.\mathsf{process}$ and $m.\mathsf{round} = s.\mathsf{round}$, $\mathcal{A}(s, M^R) = (s', M^S)$, where 
\begin{compactitem}
    \item $s'$ is a state such that:
    \begin{compactitem}
        \item $s'.\mathsf{process} = s.\mathsf{process}$, 

        \item $s'.\mathsf{round} = s.\mathsf{round} + 1$, 

        \item $s'.\mathsf{proposal} = s.\mathsf{proposal}$,

        \item if $s.\mathsf{decision} \neq \bot$, $s'.\mathsf{decision} = s.\mathsf{decision}$, and
    \end{compactitem}

    \item $M^S$ is a set of messages such that, for every message $m \in M^S$, the following holds:
    \begin{compactitem}
        \item $m.\mathsf{sender} = s'.\mathsf{process} = s.\mathsf{process}$,

        \item $m.\mathsf{round} = s'.\mathsf{round} = s.\mathsf{round} + 1$,

        \item $m.\mathsf{receiver} \neq m.\mathsf{sender}$, and

        \item there is no message $m' \in M^S$ such that (1) $m' \neq m$, and (2) $m.\mathsf{receiver} = m'.\mathsf{receiver}$.
    \end{compactitem}
\end{compactitem}
The messages each process $P_i$ sends in the first round depend solely on $P_i$'s initial state:
\begin{compactitem}
    \item If $P_i$'s state at the start of the first round is $\pstatezero{i}$, then $\mathcal{M}_i^0$ denotes the messages $P_i$ sends in the first round.
    For every message $m \in \mathcal{M}_i^0$, the following holds: (1) $m.\mathsf{sender} = P_i$, (2) $m.\mathsf{round} = 1$, (3) $m.\mathsf{receiver} \neq P_i$, and (4) there is no message $m' \in \mathcal{M}_i^0$ such that (1) $m' \neq m$, and (2) $m'.\mathsf{receiver} = m.\mathsf{receiver}$.

    \item If $P_i$'s state at the start of the first round is $\pstateone{i}$, then $\mathcal{M}_i^1$ denotes the messages $P_i$ sends in the first round. 
    For every message $m \in \mathcal{M}_i^1$, the following holds: (1) $m.\mathsf{sender} = P_i$, (2) $m.\mathsf{round} = 1$, (3) $m.\mathsf{receiver} \neq P_i$, and (4) there is no message $m' \in \mathcal{M}_i^1$ such that (1) $m' \neq m$, and (2) $m'.\mathsf{receiver} = m.\mathsf{receiver}$.
\end{compactitem}

% \subsubsection{Internal fragments.}
% A tuple $\mathit{IF} = (s, M^S, M^R)$, where $s \in \mathcal{S}$ is a state, $M^S$ is a set of messages and $M^R$ is a set of messages, is a \emph{$k$-round internal fragment}, for some $k \geq 1$, of a process $P_i$ if and only if:
% \begin{compactitem}
%     \item $s.\mathsf{process} = P_i$; and

%     \item $s.\mathsf{round} = k$; and

%     \item for every message $m \in M^S$, $m.\mathsf{sender} = P_i$; and

%     \item for every message $m \in M^R$, $m.\mathsf{receiver} = P_i$; and

%     \item there is no message $m \in M^S \cup M^R$ such that $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

%     \item there are no two messages $m, m' \in M^S$ such that $m.\mathsf{receiver} = m'.\mathsf{receiver}$; and

%     \item there are no two messages $m, m' \in M^R$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
% \end{compactitem}
% Intuitively, a $k$-round internal fragment of a process describes the what happens from the perspective of the process in the $k$-th round.

% A $k$-round internal fragment of process $P_i$ is denoted by $\mathit{IF^k_i} = (s^k_i, M^{S(k)}_i, M^{R(k)}_i)$

% \subsubsection{Internal behaviors.}
% A tuple $\mathit{IB} = \big[ \mathit{IF}^1 = (s^1, M^{S(1)}, M^{R(1)}), \mathit{IF}^2 = (s^2, M^{S(2)}, M^{R(2)}), ..., \mathit{IF}^k = (s^k, M^{S(k)}, M^{R(k)}) \big]$ is a \emph{$k$-round internal behavior}, for some $k \geq 1$, of a process $P_i$ if and only if:
% \begin{compactitem}
%     \item for every $j \in [1, k]$, $\mathit{IF}^j$ is a $j$-round internal fragment of $P_i$; and

%     \item $s^1 = \pstatezero{i}$ or $s^1 = \pstateone{i}$; and

%     \item $s^1.\mathsf{proposal} = s^2.\mathsf{proposal} = ... = s^k.\mathsf{proposal}$; and

%     \item if there exists $j \in [1, k]$ such that $s^j.\mathsf{decision} \neq \bot$, then there exists $j^* \in [1, j]$ such that (1) for every $j' \in [1, j^* - 1]$, $s^{j'}.\mathsf{decision} = \bot$, and (2) $s^{j^*}.\mathsf{decision} = s^{j^* + 1}.\mathsf{decision} = ... = s^k.\mathsf{decision}$; and
    
%     \item for every $j \in [1, k - 1]$, $\mathcal{A}(s^j, M^{R(j)}) = (s^{j + 1}, M^{S(j + 1)})$.
% \end{compactitem}
% The following functions are defined on the aforementioned internal behavior $\mathit{IB}$ of $P_i$:
% \begin{compactitem}
%     \item For every $j \in [1, k]$, $\pstate{i}{j}(\mathit{IB}) = s^j$.

%     \item For every $j \in [1, k]$, $\msgs{i}{j}(\mathit{IB}) = M^{S(j)}$ and $\msgr{i}{j}(\mathit{IB}) = M^{R(j)}$.

%     \item $S(\mathit{IB}) = \bigcup\limits_{j \in [1, k]} \msgs{i}{j}(\mathit{IB})$.

%     \item For every $j \in [1, k]$, $S(\mathit{IB}, j) = \bigcup\limits_{j' \in [j, k]} \msgs{i}{j'}(\mathit{IB})$.

%     \item $R(\mathit{IB}) = \bigcup\limits_{j \in [1, k]} \msgr{i}{j}(\mathit{IB})$.

%     \item For every $j \in [1, k]$, $R(\mathit{IB}, j) = \bigcup\limits_{j' \in [j, k]} \msgr{i}{j'}(\mathit{IB})$.
% \end{compactitem}

\subsubsection{Fragments.}
A tuple $\mathcal{F} = \Bigl( s, M^{S}, M^{\mathit{SO}}, M^R, M^{\mathit{RO}} \Bigl)$, where $s$ is a state and $M^S$, $M^{\mathit{SO}}$, $M^R$ and $M^{\mathit{RO}}$ are sets of messages, is a \emph{$k$-round fragment}, for some $k \in \mathbb{N}^+ \cup \{+ \infty\}$, of a process $P_i$ if and only if:
\begin{compactenum}
    \item $s.\mathsf{process} = P_i$; and

    \item $s.\mathsf{round} = k$; and

    \item for every $m \in M^S \cup M^{\mathit{SO}} \cup M^R \cup M^{\mathit{RO}}$, $m.\mathsf{round} = k$; and

    \item $M^S \cap M^{\mathit{SO}} = \emptyset$; and

    \item $M^R \cap M^{\mathit{RO}} = \emptyset$; and

    \item for every message $m \in M^S \cup M^{\mathit{SO}}$, $m.\mathsf{sender} = P_i$; and

    \item for every message $m \in M^R \cup M^{\mathit{RO}}$, $m.\mathsf{receiver} = P_i$; and

    \item there is no message $m \in M^S \cup M^{\mathit{SO}} \cup M^R \cup M^{\mathit{RO}}$ such that $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

    \item there are no two messages $m, m' \in M^S \cup M^{\mathit{SO}}$ such that $m.\mathsf{receiver} = m'.\mathsf{receiver}$; and

    \item there are no two messages $m, m' \in M^R \cup M^{\mathit{RO}}$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
\end{compactenum}
Intuitively, a $k$-round fragment of a process describes what happens at a process from the perspective of an omniscient external observer in the $k$-th round.
We now present a few simple results about fragments.

\begin{lemma} \label{lemma:fragment_receive_omitted}
Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) fragment $\mathcal{F} = \Bigl( s, M^{S}, M^{\mathit{SO}}, M^R, M^{\mathit{RO}} \Bigl)$ of any process $P_i$, and any tuple $\mathcal{F}' = \Bigl( s, M^{S}, M^{\mathit{SO}}, M^R, X\Bigl)$ such that $X$ is a set of messages where:
\begin{compactenum}[(i)]
    \item for every $m \in X$, $m.\mathsf{round} = k$; and 
    
    \item $M^{R} \cap  X = \emptyset$; and

    \item for every $m \in X$, $m.\mathsf{receiver} = P_i$; and

    \item there is no message $m \in X$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

    \item there are no two messages $m, m' \in M^{R} \cup X$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
\end{compactenum}
Then, $\mathcal{F}'$ is a $k$-round fragment of $P_i$.
\end{lemma}
\begin{proof}
To prove that $\mathcal{F}'$ is a $k$-round fragment of $P_i$, we prove that all ten conditions hold for $\mathcal{F}'$.
Due to the statement of the lemma, $\mathcal{F}$ is a $k$-round fragment of $P_i$.
Conditions (1), (2), (4), (6), and (9) hold directly for $\mathcal{F}'$ as the first four elements of the tuple $\mathcal{F}'$ are identical to the first four elements of $\mathcal{F}$.
Conditions (3), (5), (7), (8), and (10) hold due to conditions (i), (ii), (iii), (iv), and (v), respectively.
\end{proof}

\begin{lemma} \label{lemma:fragment_send_transfer}
Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) fragment $\mathcal{F} = \Bigl( s, M^{S}, M^{\mathit{SO}}, M^R, M^{\mathit{RO}} \Bigl)$ of any process $P_i$ and any tuple $\mathcal{F}' = \Bigl( s, X, Y, M^R, M^{\mathit{RO}}\Bigl)$ such that $X$ and $Y$ are sets of messages where:
\begin{compactenum}[(i)]
    \item for every $m \in X \cup Y$, $m.\mathsf{round} = k$; and 
    
    \item $X \cap  Y = \emptyset$; and

    \item for every $m \in X \cup Y$, $m.\mathsf{sender} = P_i$; and

    \item there is no message $m \in X \cup Y$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

    \item there are no two messages $m, m' \in X \cup Y$ such that $m.\mathsf{receiver} = m'.\mathsf{receiver}$.
\end{compactenum}
Then, $\mathcal{F}'$ is a $k$-round fragment of $P_i$.
\end{lemma}
\begin{proof}
Due to the statement of the lemma, $\mathcal{F}$ is a $k$-round fragment of $P_i$. 
Therefore, conditions (1), (2), (5), (7), and (10) hold directly for $\mathcal{F}'$ as the first, fourth, and fifth elements of $\mathcal{F}'$ are identical to the first, fourth and fifth elements of $\mathcal{F}$.
Conditions (3), (4), (6), (8), and (9) hold due to conditions (i), (ii), (iii), (iv), and (v), respectively.
\end{proof}

\subsubsection{Behaviors.}
A tuple $\mathcal{B} = \Bigl \langle \mathcal{F}^1 = \Bigl( s^1, M^{S(1)}, M^{\mathit{SO}(1)}, M^{\mathit{R}(1)}, M^{\mathit{RO}(1)} \Bigl), ..., \mathcal{F}^k = \Bigl( s^k, M^{S(k)}, M^{\mathit{SO}(k)}, M^{\mathit{R}(k)}, M^{\mathit{RO}(k)} \Bigl) \Bigl \rangle$ is a \emph{$k$-round behavior}, for some $k \in \mathbb{N}^+ \cup \{+ \infty\}$, of a process $P_i$ if and only if:
\begin{compactenum}
    \item for every $j \in [1, k]$, $\mathcal{F}^j$ is a $j$-round fragment of $P_i$; and

    \item $s^1 = \pstatezero{i}$ or $s^1 = \pstateone{i}$; and

    \item if $s^1 = \pstatezero{i}$, then $M^{S(1)} \cup M^{\mathit{SO}(1)} = \mathcal{M}_i^0$; and

    \item if $s^1 = \pstateone{i}$, then $M^{S(1)} \cup M^{\mathit{SO}(1)} = \mathcal{M}_i^1$; and

    \item $s^1.\mathsf{proposal} = s^2.\mathsf{proposal} = ... = s^k.\mathsf{proposal}$; and

    \item if there exists $j \in [1, k]$ such that $s^j.\mathsf{decision} \neq \bot$, then there exists $j^* \in [1, j]$ such that (1) for every $j' \in [1, j^* - 1]$, $s^{j'}.\mathsf{decision} = \bot$, and (2) $s^{j^*}.\mathsf{decision} = s^{j^* + 1}.\mathsf{decision} = ... = s^k.\mathsf{decision}$; and
    
    \item for every $j \in [1, k - 1]$, $\mathcal{A}(s^j, M^{R(j)}) = (s^{j + 1}, M^{S(j+1)} \cup M^{\mathit{SO}(j+1)})$. \label{item:deterministic_transition}
\end{compactenum}
If $k = +\infty$, we say that $\mathcal{B}$ is an \emph{infinite behavior} of $P_i$.
Next, we introduce some functions defined on the aforementioned behavior $\mathcal{B}$:

\begin{algorithm}
\floatname{algorithm}{Listing}
\caption{Functions defined on behavior $\mathcal{B}$}
\label{algorithm:behavior_functions}
\begin{algorithmic} [1]
\State \textbf{function} $\fstate{\mathcal{B}}{j \in [1, k]}$:
\State \hskip2em \textbf{return} $s^j$ \BlueComment{return the state at the start of round $j$}

\medskip
\State \textbf{function} $\fmsgs{\mathcal{B}}{j \in [1, k])}$:
\State \hskip2em \textbf{return} $M^{S(j)}$ \BlueComment{return the messages sent in round $j$}

\medskip
\State \textbf{function} $\fmsgso{\mathcal{B}}{j \in [1, k])}$:
\State \hskip2em \textbf{return} $M^{\mathit{SO}(j)}$ \BlueComment{return the messages send-omitted in round $j$}

\medskip
\State \textbf{function} $\fmsgr{\mathcal{B}}{j \in [1, k])}$:
\State \hskip2em \textbf{return} $M^{R(j)}$ \BlueComment{return the messages received in round $j$}

\medskip
\State \textbf{function} $\fmsgro{\mathcal{B}}{j \in [1, k])}$:
\State \hskip2em \textbf{return} $M^{\mathit{RO}(j)}$ \BlueComment{return the messages receive-omitted in round $j$}
\end{algorithmic}
\end{algorithm}

For any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B}_i$ of any process $P_i$, the following holds:
\begin{compactitem}
    \item $P_i$ \emph{decides} a bit $b \in \{0, 1\}$ in $\mathcal{B}_i$ if and only if there exists $j \in [1, k]$ such that $\fstate{\mathcal{B}_i}{j}.\mathsf{decision} = b \neq \bot$.

    \item $P_i$ \emph{does not decide} in $\mathcal{B}_i$ if and only if, for every $j \in [1, k]$, $\fstate{\mathcal{B}_i}{j}.\mathsf{decision} = \bot$.

    \item $P_i$ commits a \emph{send-omission} (resp., \emph{receive-omission}) fault in round $j \in [1, k]$ of $\mathcal{B}_i$ if and only if $\fmsgso{\mathcal{B}_i}{j} \neq \emptyset$ (resp., $\fmsgro{\mathcal{B}_i}{j} \neq \emptyset$).

    % \item $P_i$ commits an \emph{omission fault} in $\mathcal{B}_i$ if and only if $P_i$ commits a send-omission or receive-omission fault in $\mathcal{B}_i$. 
\end{compactitem}

\begin{lemma} \label{lemma:behavior_receive_omitted}
Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k \Bigl \rangle$ of any process $P_i$, and any tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
Moreover, for every $j \in [1, k]$, $\mathcal{FR}^{j} = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{R(j)}, X^j \Bigl)$, such that $X^j$ is a set of messages where:
\begin{compactitem}
    \item for every $m \in X^j$, $m.\mathsf{round} = j$; and 

    \item $M^{R(j)} \cap  X^j = \emptyset$; and

    \item for every $m \in X^j$, $m.\mathsf{receiver} = P_i$; and

    \item there is no message $m \in X^j$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

    \item there are no two messages $m, m' \in M^{R(j)} \cup X^j$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
\end{compactitem}
Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
\end{lemma}

\begin{proof}
    Since $\mathcal{B}$ is a behavior of $P_i$, $\mathcal{F}^1, \cdots, \mathcal{F}^k$ are fragments of $P_i$.
    Thus, for every $j \in [1, k]$, $\mathcal{FR}^j$ is a $j$-round fragment of $P_i$ due to conditions (i) to (v) and \Cref{lemma:fragment_receive_omitted}, which implies that condition (1) holds for $\mathcal{B}'$.
    Conditions (3) and (4) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the second and third elements of $\mathcal{FR}^j$ are identical to the second and third elements of $\mathcal{F}^j$.
    Similarly, conditions (2), (5) and (6) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the first element of $\mathcal{FR}^j$ is identical to the state from $\mathcal{F}^j$.
    Finally, condition (7) holds for $\mathcal{B}'$: first, for every $j \in [1, k]$, the first four elements of $\mathcal{FR}^j$ are identical to the first four elements of $\mathcal{F}^j$; second, condition (7) holds for $\mathcal{B}'$.
\end{proof}

% A consequence of \Cref{lemma:behavior_receive_omitted} is \Cref{corollary:behavior_receive_omitted_contained}.

% \begin{corollary}
% \label{corollary:behavior_receive_omitted_contained}
%     Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k\Bigl \rangle$  of any process $P_i$ and a tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
%     For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
%     Moreover, for every $j \in [1, k]$, $\mathcal{FR}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, X^j\Bigl)$ such that $X^j$ is a set of messages and $X^j \subseteq M^{\mathit{RO}(j)}$.
%     Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
% \end{corollary}

% \begin{lemma} \label{lemma:behavior_receive_omitted}
% Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k\Bigl \rangle$  of any process $P_i$ and a tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
% For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
% Moreover, for every $j \in [1, k]$, $\mathcal{FR}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, X^j\Bigl)$ such that $X^j$ is a set of messages and $X^j \subseteq M^{\mathit{RO}(j)}$.
% Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
% \end{lemma}
% \begin{proof}
% In order to prove that $\mathcal{B}'$ is a $k$-round behavior of $P_i$, we show that all seven conditions are satisfied by $\mathcal{B}'$.
% As $\mathcal{B}$ is a behavior of $P_i$, $\mathcal{F}^1, \cdots \mathcal{F}^k$ are fragments of $P_i$.
% Thus, for every $j \in [1, k]$, $\mathcal{FR}^j$ is a $j$-round fragment of $P_i$ due to \Cref{lemma:fragment_receive_omitted}, which implies that condition (1) holds for $\mathcal{B}'$.
% Conditions (3) and (4) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the second and third elements of $\mathcal{FR}^j$ are identical to the second and third elements of $\mathcal{F}^j$.
% Similarly, conditions (2), (5) and (6) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the first element of $\mathcal{FR}^j$ is identical to the state from $\mathcal{F}^j$.
% Finally, condition (7) holds for $\mathcal{B}'$: first, for every $j \in [1, k]$, the first four elements of $\mathcal{FR}^j$ are identical to the first four elements of $\mathcal{F}^j$; second, condition (7) holds for $\mathcal{B}'$.
% % Since $\mathcal{B}$ is a behavior, $\mathcal{F}^1, \mathcal{F}^2, \cdots, \mathcal{F}^k$ are fragments, thus, condition (1) holds by \Cref{lemma:fragment_receive_omitted}.
% % Conditions (2), (3) and (4) hold since $\forall j, \fstate{\mathcal{B}'}{j} = \fstate{\mathcal{B}}{j}$ and $\mathcal{B}$ satisfies these conditions.
% % Finally, condition (5) holds since $\mathcal{A}(\fstate{\mathcal{B}'}{j}, \fmsgr{\mathcal{B}'}{j}) = \mathcal{A}(s^j, M^{R(j)}) = (s^{j + 1}, M^{S(j+1)} \cup M^{\mathit{SO}(j+1)}) = (\fstate{\mathcal{B}}{j + 1}, \fmsgs{\mathcal{B}}{j + 1} \cup \fmsgso{\mathcal{B}}{j + 1})$, where the second equality comes from the fact that condition (5) holds for $\mathcal{B}$.
% \end{proof}

\begin{lemma} \label{lemma:behavior_send_transfer}
Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k \Bigl \rangle$ of any process $P_i$ and a tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
Moreover, for every $j \in [1, k]$, $\mathcal{FR}^{j} = \Bigl( s^j, X^j, Y^j, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$ such that (1) $X^j$ and $Y^j$ are sets of messages, (2) $X^j \cup Y^j = M^{S(j)} \cup M^{\mathit{SO}(j)}$, and (3) $X^j \cap Y^j = \emptyset$. 
Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
\end{lemma}
\begin{proof}
Since $\mathcal{B}$ is a behavior of $P_i$, $\mathcal{F}^1, \cdots, \mathcal{F}^k$ are fragments of $P_i$.
Thus, for every $j \in [1, k]$, $\mathcal{FR}^j$ is a $j$-round fragment of $P_i$ due to \Cref{lemma:fragment_send_transfer}, which implies that condition (1) holds for $\mathcal{B}'$.
Conditions (3) and (4) hold for $\mathcal{B}'$ as (1) both conditions hold for $\mathcal{B}'$, and (2) for every $j \in [1, k]$, $X^j \cup Y^j = M^{S(j)} \cup M^{\mathit{SO}(j)}$.
Similarly, conditions (2), (5) and (6) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the first element of $\mathcal{FR}^j$ is identical to the state from $\mathcal{F}^j$.
Finally, condition (7) holds for $\mathcal{B}'$: first, for every $j \in [1, k]$, $X^j \cup Y^j = M^{S(j)} \cup M^{\mathit{SO}(j)}$ and the first and the fourth elements of $\mathcal{FR}^j$ are identical to the first and the fourth elements of $\mathcal{F}^j$; second, condition (7) holds for $\mathcal{B}'$.
\end{proof}

% The following functions are defined on the aforementioned external behavior $\mathit{EB}$ of $P_i$:
% \begin{compactitem}
%     \item For every $j \in [1, k]$, $\pstate{i}{j}(\mathit{EB}) = s^j$.

%     \item For every $j \in [1, k]$, (1) $\msgs{i}{j}(\mathit{EB}) = M^{S(j)}$, (2) $\msgso{i}{j}(\mathit{EB}) = M^{\mathit{SO}(j)}$, (3) $\msgr{i}{j}(\mathit{EB}) = M^{R(j)}$, and (3) $\msgro{i}{j}(\mathit{EB}) = M^{\mathit{RO}(j)}$.

%     \item $S(\mathit{EB}) = \bigcup\limits_{j \in [1, k]} \msgs{i}{j}(\mathit{EB})$ and $\mathit{SO}(\mathit{EB}) = \bigcup\limits_{j \in [1, k]} \msgso{i}{j}(\mathit{EB})$.

%     \item For every $j \in [1, k]$, $S(\mathit{EB}, j) = \bigcup\limits_{j' \in [j, k]} \msgs{i}{j'}(\mathit{EB})$ and $\mathit{SO}(\mathit{EB}, j) = \bigcup\limits_{j' \in [j, k]} \msgso{i}{j'}(\mathit{EB})$.

%     \item $R(\mathit{EB}) = \bigcup\limits_{j \in [1, k]} \msgr{i}{j}(\mathit{EB})$ and $\mathit{RO}(\mathit{EB}) = \bigcup\limits_{j \in [1, k]} \msgro{i}{j}(\mathit{EB})$.

%     \item For every $j \in [1, k]$, $R(\mathit{EB}, j) = \bigcup\limits_{j' \in [j, k]} \msgr{i}{j'}(\mathit{EB})$ and $\mathit{RO}(\mathit{EB}, j) = \bigcup\limits_{j' \in [j, k]} \msgro{i}{j'}(\mathit{EB})$.
% \end{compactitem}

% Consider any $k$-round external behavior $\mathit{EB}_i$ of a process $P_i$:
% \begin{compactitem}
%     \item We say that $P_i$ proposes a bit $b \in \{0, 1\}$ if and only if $\pstate{i}{1}(\mathit{EB}_i).\mathsf{proposal} = b$.

%     \item We say that $P_i$ decides a bit $b' \in \{0, 1\}$ if and only if $\pstate{i}{k}(\mathit{EB}_i).\mathsf{decision} = b'$.

%     \item We say that $P_i$ sends (resp., send-omits) a message $m$ in a round $j \in [1, k]$ of $\mathit{EB}_i$ if and only if $m \in \msgs{i}{j}(\mathit{EB}_i)$ (resp., $m \in \msgso{i}{j}(\mathit{EB}_i)$).

%     \item We say that $P_i$ receives (resp., receive-omits) a message $m$ in a round $j \in [1, k]$ of $\mathit{EB}_i$ if and only if $m \in \msgr{i}{j}(\mathit{EB}_i)$ (resp., $m \in \msgro{i}{j}(\mathit{EB}_i)$).

%     \item We say that $P_i$ commits a send-omission fault in $\mathit{EB}_i$ if and only if there exists $j \in [1, k]$ such that $\msgso{i}{j}(\mathit{EB}_i) \neq \emptyset$.

%     \item We say that $P_i$ commits a receive-omission fault in $\mathit{EB}_i$ if and only if there exists $j \in [1, k]$ such that $\msgro{i}{j}(\mathit{EB}_i) \neq \emptyset$.

%     \item We say that $P_i$ commits an omission fault in $\mathit{EB}_i$ if and only if (1) $P_i$ commits a send-omission fault in $\mathit{EB}_i$, or (2) $P_i$ commits a receive-omission fault in $\mathit{EB}_i$.
% \end{compactitem}

% A $k$-round $(k \geq 1)$ external behavior $\mathit{EB}_i = \big[ \mathit{EF}_1 = (s_1, M_1^S, M_1^{\mathit{SO}}, M_1^R, M_1^{\mathit{RO}}), \mathit{EF}_2 = (s_2, M_2^S, M_2^{\mathit{SO}}, M_2^R, M_2^{\mathit{RO}}), ..., \mathit{EF}_k = (s_k, M_k^S, M_k^{\mathit{SO}}, M_k^R, M_k^{\mathit{RO}}) \big]$ of a process $P_i$ \emph{reduces} to a $k$-round internal behavior $\mathit{IB}_i = \big[ \mathit{IF}_1 = (\bar{s}_1, \bar{M}_1^S, \bar{M}_1^R), \mathit{IF}_2 = (\bar{s}_2, \bar{M}_2^S, \bar{M}_2^R), ..., \mathit{IF}_k = (\bar{s}_k, \bar{M}_k^S, \bar{M}_k^R) \big]$ if $P_i$ if and only if:
% \begin{compactitem}
%     \item for every $j \in [1, k]$, $s_j = \bar{s}_j$; and

%     \item for every $j \in [1, k]$, $\bar{M}_j^S = M_j^S \cup M_j^{\mathit{SO}}$; and

%     \item for every $j \in [1, k]$, $\bar{M}_j^R = M_j^R$.
% \end{compactitem}

\subsubsection{Executions of $\mathcal{A}$.}
A \emph{$k$-round execution} $\mathcal{E}$, for some $k \in \mathbb{N}^+ \cup \{+ \infty\}$, is a tuple $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1,  ..., \mathcal{B}_n]$ such that the following guarantees hold:
\begin{compactitem}
    \item \emph{Faulty processes:} $\mathcal{F}$ is a set of $|\mathcal{F}| \leq t$ processes.
    
    \item \emph{Composition:} For every $j \in [1, n]$, $\mathcal{B}_j$ is a $k$-round behavior of process $P_j$.

    \item \emph{Send-validity:} If there exists a message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \mathsf{sent}(\mathcal{B}_s, j)$, then (1) $m \in \mathsf{received}(\mathcal{B}_r, j)$, or (2) $m \in \mathsf{receive\_omitted}(\mathcal{B}_r, j)$.
    That is, if a message is sent, the message is either received or receive-omitted in the same round.

    \item \emph{Receive-validity:} If there exists a message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \mathsf{received}(\mathcal{B}_r, j) \cup \fmsgro{\mathcal{B}_r}{j}$, then $m \in \mathsf{sent}(\mathcal{B}_s, j)$.
    That is, if a message is received or receive-omitted, the message is sent in the same round.

    \item \emph{Omission-validity:} If there exists a process $P_i$ and $j \in [1, k]$ such that (1) $\mathsf{send\_omitted}(\mathcal{B}_i, j) \neq \emptyset$, or (2) $\mathsf{receive\_omitted}(\mathcal{B}_i, j) \neq \emptyset$, then $P_i \in \mathcal{F}$.
    That is, if a process commits an omission fault, the process is in $\mathcal{F}$.
\end{compactitem}
If $k = +\infty$, we say that $\mathcal{E}$ is an \emph{infinite execution}.

For any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, .., \mathcal{B}_n]$, the following holds:
\begin{compactitem}
    \item A process $P_i$ is \emph{faulty} in $\mathcal{E}$ if and only if $P_i \in \mathcal{F}$; otherwise, $P_i$ is \emph{correct} in $\mathcal{E}$.

    \item A process $P_i$ \emph{decides} a bit $b \in \{0, 1\}$ in $\mathcal{E}$ if and only if $P_i$ decides $b$ in $\mathcal{B}_i$.

    \item A process $P_i$ \emph{does not decide} in $\mathcal{E}$ if and only if $P_i$ does not decide in $\mathcal{B}_i$.

    \item A process $P_i$ commits a \emph{send-omission} (resp., \emph{receive-omission}) fault in round $j \in [1, k]$ of $\mathcal{E}$ if and only if $P_i$ commits a send-omission (resp., receive-omission) fault in round $j$ of $\mathcal{B}_i$.

    % \item A process $P_i$ commits an \emph{omission fault} in $\mathcal{E}$ if and only if $P_i$ commits an omission fault in $\mathcal{B}_i$.
\end{compactitem}

% \begin{lemma} \label{lemma:behavior_from_execution}
% Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{ +\infty \}$) execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ and any process $P_i$.
% Let $\mathcal{B}_i = \Bigl \langle \mathcal{F}_i^1, ..., \mathcal{F}_i^k \Bigl \rangle$ and, for every $j \in [1, k]$, let $\mathcal{F}_i^1 = \Bigl( s_i^j, M_i^{S(j)}, M_i^{\mathit{SO}(j)}, M_i^{R(j)}, M_i^{\mathit{RO}(j)} \Bigl)$.
% Consider any tuple $\mathcal{B}_i' = \Bigl \langle \mathcal{FR}_i^1, ..., \mathcal{FR}_i^k \Bigl \rangle$ such that, for every $j \in [1, k]$, $\mathcal{FR}_i^1 = \Bigl( s_i^j, M_i^{S(j)}, M_i^{\mathit{SO}(j)}, M_i^{R(j)}, X_i^j \Bigl)$, where the following holds for $X_i^j$:
% \begin{compactitem}
%     \item for every $m \in X_i^j$, $m.\mathsf{round} = j$; and 

%     \item $M_i^{R(j)} \cap  X_i^j = \emptyset$; and

%     \item for every $m \in X_i^j$, $m.\mathsf{receiver} = P_i$; and

%     \item there is no message $m \in X_i^j$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

%     \item there are no two messages $m, m' \in M_i^{R(j)} \cup X_i^j$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
% \end{compactitem}
% Then, $\mathcal{B}_i'$ is a $k$-round behavior of $P_i$.
% \end{lemma}

% \begin{lemma} \label{lemma:behavior_from_execution}
% Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) behavior $\mathcal{B} = \Bigl \langle \mathcal{F}^1, \cdots, \mathcal{F}^k \Bigl \rangle$ of any process $P_i$, and any tuple $\mathcal{B}' = \Bigl \langle \mathcal{FR}^{1}, \cdots, \mathcal{FR}^{k}\Bigl \rangle$.
% For every $j \in [1, k]$, $\mathcal{F}^j = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{\mathit{R}(j)}, M^{\mathit{RO}(j)} \Bigl)$.
% Moreover, for every $j \in [1, k]$, $\mathcal{FR}^{j} = \Bigl( s^j, M^{S(j)}, M^{\mathit{SO}(j)}, M^{R(j)}, X^j \Bigl)$, such that $X^j$ is a set of messages where:
% \begin{compactitem}
%     \item for every $m \in X^j$, $m.\mathsf{round} = j$; and 

%     \item $M^{R(j)} \cap  X^j = \emptyset$; and

%     \item for every $m \in X^j$, $m.\mathsf{receiver} = P_i$; and

%     \item there is no message $m \in X^j$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

%     \item there are no two messages $m, m' \in M^{R(j)} \cup X^j$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
% \end{compactitem}
% Then, $\mathcal{B}'$ is a $k$-round behavior of $P_i$.
% \end{lemma}

% \begin{proof}
%     Since $\mathcal{B}$ is a behavior of $P_i$, $\mathcal{F}^1, \cdots, \mathcal{F}^k$ are fragments of $P_i$.
%     Thus, for every $j \in [1, k]$, $\mathcal{FR}^j$ is a $j$-round fragment of $P_i$ due to \Cref{lemma:fragment_receive_omitted}, which implies that condition (1) holds for $\mathcal{B}'$.
%     Conditions (3) and (4) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the second and third elements of $\mathcal{FR}^j$ are identical to the second and third elements of $\mathcal{F}^j$.
%     Similarly, conditions (2), (5) and (6) hold for $\mathcal{B}'$ as, for every $j \in [1, k]$, the first element of $\mathcal{FR}^j$ is identical to the state from $\mathcal{F}^j$.
%     Finally, condition (7) holds for $\mathcal{B}'$: first, for every $j \in [1, k]$, the first four elements of $\mathcal{FR}^j$ are identical to the first four elements of $\mathcal{F}^j$; second, condition (7) holds for $\mathcal{B}'$.
% \end{proof}

% \begin{lemma} \label{lemma:behavior_from_execution_A}
% Consider any $k$-round ($k \in \mathbb{N}^+ \cup \{ +\infty \}$) execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ and any process $P_i$.
% Let $\mathcal{B}_i = \Bigl \langle \mathcal{F}_i^1, ..., \mathcal{F}_i^k \Bigl \rangle$ and, for every $j \in [1, k]$, let $\mathcal{F}_i^1 = \Bigl( s_i^j, M_i^{S(j)}, M_i^{\mathit{SO}(j)}, M_i^{R(j)}, M_i^{\mathit{RO}(j)} \Bigl)$.
% Consider any tuple $\mathcal{B}_i' = \Bigl \langle \mathcal{FR}_i^1, ..., \mathcal{FR}_i^k \Bigl \rangle$ such that, for every $j \in [1, k]$, $\mathcal{FR}_i^1 = \Bigl( s_i^j, M_i^{S(j)}, M_i^{\mathit{SO}(j)}, M_i^{R(j)}, X_i^j \Bigl)$, where the following holds for $X_i^j$:
% \begin{compactitem}
%     \item for every $m \in X_i^j$, $m.\mathsf{round} = j$; and 

%     \item $M_i^{R(j)} \cap  X_i^j = \emptyset$; and

%     \item for every $m \in X_i^j$, $m.\mathsf{receiver} = P_i$; and

%     \item there is no message $m \in X_i^j$, $m.\mathsf{sender} = m.\mathsf{receiver} = P_i$; and

%     \item there are no two messages $m, m' \in M_i^{R(j)} \cup X_i^j$ such that $m.\mathsf{sender} = m'.\mathsf{sender}$.
% \end{compactitem}
% Then, $\mathcal{B}_i'$ is a $k$-round behavior of $P_i$.
% \end{lemma}

\subsection{Proof}

\begin{definition} [Receive-isolation] \label{definition:isolation}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be any $k$-round ($k \in \mathbb{N}^+ \cup \{+ \infty\}$) execution.
We say that a group $G$ of $|G| \leq t$ processes is \emph{receive-isolated from a round $k' \in \mathbb{N}^+$} ($k' \leq k$) in $\mathcal{E}$ if and only if, for every process $P_g \in G$, the following holds:
\begin{compactitem}
    \item $P_g \in \mathcal{F}$; and

    \item for every $j \in [1, k' - 1]$, $\mathsf{receive\_omitted}(\mathcal{B}_g, j) = \emptyset$; and

    \item for every $j \in [1, k]$, $\mathsf{send\_omitted}(\mathcal{B}_g, j) = \emptyset$; and

    \item for every $j \in [k', k]$, if there exists a message $m$ such that $m \in \mathsf{received}(\mathcal{B}_g, j)$, then $m.\mathsf{sender} \in G$.
\end{compactitem}
\end{definition}
Intuitively, a group $G$ is receive-isolated from some round $k'$ in an execution if and only if the following holds for every process $P_g \in G$: (1) $g$ is faulty, (2) $g$ does not commit any receive-omission failures in any round before $k'$, (3) $g$ does not commit any send-omission failures throughout the entire execution, and (4) from round $k'$ onward, $g$ receives messages only from processes in $G$.
This can be understood as a simultaneous unidirectional partition of $G$: messages from $G$ to other processes are always \emph{sent} successfully while no message from $\overline{G}$ to $G$ is \emph{received} from round $k'$ onward.

%%%%%%%%%%%%%%%%%%%
%% cut and merge %%
%%%%%%%%%%%%%%%%%%%

Now we are ready to provide a formal proof of the quadratic lower bound for the worst case complexity of weak agreement (see figure \ref{figure:lemma_map}). 

\begin{figure}[!t]
\centering
\includegraphics[width=6cm]{figures/lemma_map.eps}
\caption{Lemma Map (A draft to show what I would expect). The "lemma 21" in the figure corresponds to \Cref{lemma:0bis}, while "lemma 22" in the figure corresponds to \Cref{lemma:combining_receive_isolation}.}
\label{figure:lemma_map}
\end{figure}

First, we define a function that takes an execution and replace some receive-omitted messages by send-omitted messages.

\begin{definition}\label{definition:permutation_receive_omission_to_send_omission}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
We denote by $\mathcal{E}^{M \rightleftarrows} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$ the execution such that, for every process $P_i \in \Pi$:
\begin{compactenum}
    \item $\mathcal{B}'_i \gets \mathcal{B}_i$
    
    \item $\forall j \in [1:k]$, $\fmsgro{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgro{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_receive_omission}
    
    \item $\forall j \in [1:k]$, $\fmsgso{\mathcal{B}'_i}{j}$ $ \gets \fmsgso{\mathcal{B}'_i}{j} $ $\cup \{m \in M | m.\mathit{round} = j \wedge m.\mathit{sender} = P_i\}$ \label{item:add_send_omission}

    \item $\forall j \in [1:k]$, $\fmsgs{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgs{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_send}
    
    \item $\mathcal{F}' = \{P_i \in \Pi \; | \bigcup\limits_{k' \in [1:k]} ( \fmsgso{\mathcal{B}_i}{k'} \cup \fmsgro{\mathcal{B}_i}{k'} ) \neq \emptyset\}$ \label{item:faulty_processes}
\end{compactenum}
\end{definition}

Intuitively, $\mathcal{E}^{M \rightleftarrows}$ corresponds to the execution $\mathcal{E}$, where every receive-omitted message is send-omitted instead.

\begin{lemma}\label{lemma:switch_omission}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
Let $\fswitcho{\mathcal{E}}{M} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$. 
If $|\mathcal{F}'| \leq t$, then $\mathcal{E}^{M \rightleftarrows}$ is a valid execution.
\end{lemma}

\begin{proof}
$\;$
\begin{compactitem}
 \item Faulty processes: $|\mathcal{F}'| \leq t$ is a precondition of the lemma.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$). Necessarily $m \notin M$ by step (\ref{item:remove_send}). Thus, $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and so $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ by Send-Validity of $\mathcal{E}$.
    
    Send-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$. Necessarily, $m \notin M$. Indeed, if $m \in M$, $m \in \fmsgro{\mathcal{B}_r}{j} \setminus \fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and $m \notin \in \fmsgr{\mathcal{B}'_r}{j}$, since $\fmsgr{\mathcal{B}'_r}{j} = \fmsgr{\mathcal{B}_r}{j}$ by construction and $\fmsgr{\mathcal{B}_r}{j} \cap \fmsgro{\mathcal{B}_r}{j} = \emptyset$, since $\mathcal{B}_r$ is a behavior of process $P_r$.

    Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (\ref{item:remove_send}) while constructing $\mathcal{B}_s'$.
    
    Receive-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.
    
    \item Omission-validity is obviously satisfied in $\fswitcho{\mathcal{E}}{M}$. by step (\ref{item:faulty_processes}).
\end{compactitem}
Thus, $\fswitcho{\mathcal{E}}{M}$. is indeed an execution of $\mathcal{A}$. 
\end{proof}



\begin{lemma}[Some isolated processes must agree]\label{lemma:0}
Let's fix
\begin{itemize}
    \item $(P,Q,R)$ is a partition of the processes
    \item $t_S, t_Q \in \mathbb{N}, t_S + t_Q \leq t + 1$
    \item $|P|> t_S $
    \item $|Q| \geq t_Q$
    \item $|R|\leq t-t_S-t_Q+1$
    
    \item $\mathcal{A}$ is a synchronous protocol that solves non-uniform weak agreement in the omission model
\end{itemize}

Let $\mathcal{E}$ be an execution of $\mathcal{A}$ such that:
\begin{itemize}
    \item Every process in $P$ is correct and eventually decides $b_P$.
    \item Every process in $Q$ is receive-isolated after some round $k$.
    \item Every process in $R$ is faulty.
\end{itemize}

If there exists $t_{Q'} \in \mathbb{N}$, such that the communication complexity of $\mathcal{A}$ is less than $(t_Q -t_{Q'}) \cdot t_S$, then $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{lemma}

\begin{proof}[proof sketch] (see figure \ref{figure:lemma_0})
First, we can remark that (*) $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$. By contradiction, assume the opposite. There exists a set $Q''$ of $|Q''|= |Q|-t_{Q'}+1 > t_Q -t_{Q'}$ processes that would receive more than $t_S$ messages. Thus, the communication complexity of $\mathcal{A}$ would be strictly greater than $(t_Q -t_{Q'}) \cdot t_S$.

Let $q_i \in Q'$.
Let $S_i$ be the set of processes in $P$ that have sent at least 1 message after round $k$ (including) to process $q_i$ in execution $\mathcal{E}$.
By (*), $|S_i| \leq t_S$.
We can construct an execution $\mathcal{E}_i$ s.t. behaviour of every process except the ones in $R \cup S_i \cup \{q_i\}$ are unchanged. Every message receive-omitted by process $q_i$ in execution $\mathcal{E}$ is now send-omitted by $R \cup S_i$. the rest remains unchanged. By agreement, termination, and correctness, $q_i$ must decide in $\mathcal{E}_i$ the same value than $P \setminus S_i \neq \emptyset$, that is $b_P$.
Since, the behaviours of $q_i$ in $\mathcal{E}$ and $\mathcal{E}_i$ are equivalent, $q_i$ must decide $b_P$ in $\mathcal{E}$.

Hence, every process $q_j \in Q'$ decides $b_P$ in $\mathcal{E}$.
\end{proof}


\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_0_vector.eps}
\caption{Lemma \ref{lemma:0}}
\label{figure:lemma_0}
\end{figure}

%%%%%%%%%%%%%%%%%%
%% formal proof %%
%%%%%%%%%%%%%%%%%%
\begin{proof}[formal proof]
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Due to the statement of the lemma, $\mathcal{F} = Q \uplus R$.
Moreover, no process in $P \uplus Q$ commits any send-omission failure in $\mathcal{E}$: for every process $P_i \in P \uplus Q$ and every round $j \in \mathbb{N}^+ \cup \{+\infty\}$, $\mathsf{send\_omitted}(\mathcal{B}_i, j) = \emptyset$.

For every set of processes $U$, we note $M_{U} = \bigcup\limits_{P_i \in U} \big( \bigcup\limits_{k' \geq k}  \fmsgs{\mathcal{B}_i}{k'} \big)$ to denote the set of messages sent by processes in $U$ from (and including) round $k$ onward in $\mathcal{E}$.

For every pair of sets of processes $(U, V)$, we define $M_{U \to V}$ as the set containing all messages sent to a process in $V$ by processes in $U$ from (and including) round $k$ onward of $\mathcal{E}$:
\begin{equation*}
    M_{U \to V} = \{ m \,|\, m \in M_{U} \land m.\mathsf{receiver} \in V \}.
\end{equation*}
Note that, for every $P_i \in Q$, each message $m \in M_{(P \uplus R) \to \{P_i\}}$ is receive-omitted in $\mathcal{B}_i$.

First, we will prove by contradiction that $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ receives less than $t_S$ messages in $\mathcal{E}$ from processes in $P$. Therefore, assume that there exists a subset $Q'' \subseteq Q$ of $|Q''| > |Q|-t_{Q'} \geq t_Q-t_{Q'}$ processes which receive more than $t_S$ messages in $\mathcal{E}$ from processes in $P$.
As $\mathcal{A}$ sends less than $(t_Q-t_{Q'})\cdot t_S$ messages in execution $\mathcal{E}$, less than $(t_Q-t_{Q'})\cdot t_S$ messages are sent in $\mathcal{E}$ by correct processes (i.e., processes in $P$), which implies $|M_{P \to \tilde{Q}'}| < (t_Q-t_{Q'})\cdot t_S$, thus we reach a contradiction. Hence, $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$ from processes in $P$, i.e. $\forall P_i \in Q', |M_{P \to \{P_i\}}| \leq t_S$.

Let $P_i \in Q'$.
Let $S_i$ denote the set of processes in $P$ whose messages $P_i$ receive-omits from (and including) round $k$ onward in $\mathcal{B}_i$:
\begin{equation*}
    S_i = \{ P_j \in P \,|\, \exists j \in [k, \infty], \exists m \in \fmsgro{\mathcal{B}_i}{j}: m.\mathsf{sender} = P_j \}.
\end{equation*}
Note that $P_i \notin S_i$ (as no process ever sends messages to itself).
Moreover, as $|M_{P \to \{P_i\}}| \leq t_S$, $|S_i| \leq t_S$.
We now create another execution $\mathcal{E}'_i = [\mathcal{F}', \mathcal{B}_1', ..., \mathcal{B}_n'] = \fswitcho{\mathcal{E}}{\tilde{M}_i}$ where $\tilde{M}_i = M_{(P \uplus R) \to \{P_i\}}$.
We can observe that $P_i$ is correct in $\mathcal{E}'_i$.
Hence, $\mathcal{F}' \subseteq S_i \uplus R \uplus (Q \setminus{\{ P_i \}})$ and $|R| \leq t-t_S-t_Q+1$, thus $|\mathcal{F}'| \leq t$. 
Let us note that some processes in $R$ might be now correct.
By lemma \ref{lemma:switch_omission}, $\mathcal{E}'_i$ is an execution of $\mathcal{A}$.
\iffalse
:
\begin{compactenum}
    \item $\mathcal{F}' \gets S_i \uplus R \uplus (Q \setminus{ \{P_i\}})$.

    \item For every process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, let $\mathcal{B}_j' \gets \mathcal{B}_j$, i.e., $P_j$'s behavior in $\mathcal{E}'$ is identical to $P_j$'s behavior in $\mathcal{E}_i$.

    \item For the process $P_i$, we build $\mathcal{B}_i'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_i' \gets \mathcal{B}_i$.

        \item For every round $k' \in [k, \infty]$ such that $\fmsgro{\mathcal{B}_i}{k'} \neq \emptyset$, we remove all messages from $\fmsgro{\mathcal{B}'_i}{k'}$: $\fmsgro{\mathcal{B}'_i}{k'} \gets \emptyset$.
        Note that all messages removed from $\fmsgro{\mathcal{B}'_i}{k'}$ are sent by processes in $S_i \uplus R$.
    \end{compactenum}
    Note that $P_i$ does not commit any omission faults in $\mathcal{B}_i'$: (1) it does not commit any send-omission faults due to the statement of the lemma, and (2) it does not commit any receive-omission faults due to the step (3)(b). 

    \item For every process $P_j \in S_i \uplus R$, we build $\mathcal{B}_j'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_j' \gets \mathcal{B}_j$.

        \item For every message $m$ such that there exists a round $k' \geq [k, \infty]$ with (1) $m \in \fmsgs{\mathcal{B}_j}{k'}$, and (2) $m \in \fmsgro{\mathcal{B}_i}{k'}$, we perform the following steps:
        \begin{compactenum}
            \item We remove $m$ from sent messages: $\fmsgs{\mathcal{B}_j'}{k'} \gets \fmsgs{\mathcal{B}_j'}{k'} \setminus{\{m\}}$.

            \item We add $m$ to send-omitted messages:
            $\fmsgso{\mathcal{B}_j'}{k'} \gets \fmsgso{\mathcal{B}_j'}{k'} \cup \{m\}$.
        \end{compactenum}
    \end{compactenum}
\end{compactenum}

Let us prove that $\mathcal{E}_i'$ is indeed an execution:
\begin{compactitem}
    \item Faulty processes: As $\mathcal{F}' \subseteq S_i \uplus R \uplus (Q \setminus{\{ P_i \}})$ and $|R| \leq t-t_S-t_Q+1$, thus $|\mathcal{F}'| \leq t$. Potentially, some processes in $R$ are now correct.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore:
    \begin{compactitem}
        \item For any process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ since $\mathcal{B}_j' = \mathcal{B}_j$. 
        \item For process $P_i$, $\mathcal{B}_i'$ is an infinite behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
        \item For any process $P_j \in R \uplus S_i$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ due to \Cref{lemma:behavior_send_transfer}. 
    \end{compactitem}
    

    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$).
    We consider two possibilities:
    \begin{compactitem}
        \item If $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (3)(b), then $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ as $m$ is included in step (3)(a).

        \item Otherwise, $m$ is excluded by step (3)(b).
        This implies that $j \geq k$, $P_r = P_i$, $P_s \in S_i \uplus R$, $m \in \fmsgro{\mathcal{B}_r}{j}$ and $m \in \fmsgs{\mathcal{B}_s}{j}$.
        Then, by step (4)(b)(i), $m \notin \fmsgs{\mathcal{B}_s'}{j}$ making this case impossible.
    \end{compactitem}
    Send-validity is satisfied in $\mathcal{E}'_i$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $j \geq k$ and $P_r = P_i$ and $m \in \fmsgro{\mathcal{B}_r}{j}$.
        However, this case is impossible as $m \notin \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ due to the step (3)(b).

        \item Otherwise, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
        Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (4)(b)(i) while constructing $\mathcal{B}_s'$.
    \end{compactitem}
    Receive-validity is satisfied in $\mathcal{E}'_i$.

    \item Omission-validity:
    Consider a process $P_j$ which commits an omission-fault in $\mathcal{B}_j'$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $P_j$ commit a send-omission fault in $\mathcal{B}_j'$.
        As no process $P_z \in \Pi \setminus R$ commits a send-omission fault in $\mathcal{B}_z$, $P_j \in R \uplus S_i$ given that we only add send-omitted messages to processes in $R \uplus S_i$. Hence, $P_j \in \mathcal{F}'$.
        In this case, omission-validity is satisfied.

        \item Let $P_j$ commit a receive-omission fault in $\mathcal{B}_j'$.
        Note that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z$, which implies that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z'$ (as our construction does not add receive-omitted messages to any process).
        
        Moreover, $P_i$ does not commit a receive-omission fault in $\mathcal{B}_i'$ as (1) it does not commit any receive-omission faults in any round $k' \in [1, k - 1]$ in $\mathcal{B}_i$ (due to \Cref{definition:isolation}), and (2) all receive-omitted messages in any round $k' \in [k, \infty]$ are removed by the step (3)(b).
        Therefore, $P_j \in R \uplus (Q \setminus{\{P_i\}})$, which means that omission-validity holds in this case as well.
    \end{compactitem}
    Omission-validity is satisfied in $\mathcal{E}'_i$.
\end{compactitem}

Thus, $\mathcal{E}'_i$ is indeed an execution of $\mathcal{A}$.
\fi
Since $|P|>t_S$, $|S_i|\leq t_S$, $\exists P_j \in P \setminus S_i \neq \emptyset$.

Observe that $P_i$ and $P_j$ are correct in $\mathcal{E}'_i$, and $\mathcal{B}'_j = \mathcal{B}_j$.
Hence, they both decide the same value $b$.

Moreover (1) $P_i$'s states in $\mathcal{B}_i'$ and $\mathcal{B}_i$ are identical, and (2) $P_j$'s states in $\mathcal{B}_j'$ and $\mathcal{B}_j$ are identical.
Therefore, $P_i$ decides $b$ in $\mathcal{E}$.
Thus, every process in $Q'$ decides $b$ in $\mathcal{E}$.
Hence, the lemma holds.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%
%% end formal proof %%
%%%%%%%%%%%%%%%%%%%%%%

We partition all processes into three disjoint groups: (1) group $A$ with $|A| = n - \frac{t}{2}$ processes, (2) group $B$ with $|B| = \frac{t}{4}$ processes, and (3) group $C$ with $|C| = \frac{t}{4}$ processes, where (i) every process in $A$ is always correct and (ii) the set $B$ (resp.  $C$) is either a group of receive-isolated processes from some round or a group of correct processes.

\begin{lemma}[Some isolated processes must agree]\label{lemma:0bis}
Let $\mathcal{E}$ be an infinite execution of $\mathcal{A}$ such that every process in $A$ decides $b_A' \in \{0,1\}$. 
Then,  either the communication complexity of $\mathcal{A}$ is greater than $\frac{t^2}{16}$ or $\exists (B', C') \subset B \times C$, $|B'|,|C'| \geq \frac{t}{8}$, such that every process in $B' \cup C'$ decides $b_A'$.
\end{lemma}

\begin{proof}
We apply \Cref{lemma:0} with $(P,Q,R)=(A,B,C)$ (resp. $(P,Q,R)=(A,C, B)$, resp.  $(P,Q,R)=(A\cup B,C, \emptyset)$, resp.  $(P,Q,R)=(A\cup C,B, \emptyset)$), $t_S = \frac{t}{2}, t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$. 
\end{proof}

The \Cref{lemma:0bis} can be seen as a simple generalization of the Dolev-Reischuk result. Before applying it to prove the main lemma of the paper (lemma \ref{lemma:combining_receive_isolation}), we will define a simple construction that describes the correct behavior of a group ($A$ in practice) when the received messages are given.


\iffalse
\begin{corollary}
If $t_Q = 2t_{Q'}$, and the communication complexity of $\mathcal{A}$ is less than $t_{Q'} \cdot t_S$, then $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{corollary}

\begin{corollary}
If $|P|=n-\frac{t}{4}$, $|Q| = \frac{t}{4}$, $|R|=0$ and the communication complexity of $\mathcal{A}$ is less than $\frac{3nt}{32}$, then $\exists Q' \subset Q$, $|Q| = \frac{t}{8}$, such that every process in $Q'$ decides $b_P$.
\end{corollary}


\begin{lemma}\label{lemma:forced_termination_new}
Lemma \ref{lemma:forced_termination}
Consider an infinite execution $\mathcal{E}$ such that (1) some group $X$ of $|X| = \frac{t}{4}$ processes is receive-isolated from some round $k \geq 1$, and (2) all processes in $\Bar{X}$ are correct.
At least $\frac{|X|}{2}$ processes from $X$ decide in $\mathcal{E}$.
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $|R|=0$, $P = \bar{X}$, $Q = X$ with $t_S = t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$.
\end{proof}


\begin{lemma}\label{lemma:disagreement_quadratic_messages_new}
Lemma \ref{lemma:disagreement_quadratic_messages}
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $(Q,R)=(B,C)$ (resp. $(Q,R)=(C,B)$), $P = A$, $t_S = \frac{t}{2}, t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$. We verify $|R| = \frac{t}{4} \leq t-t_S - t_Q+1 = \frac{t}{4} +1$. 
\end{proof}


\begin{corollary}
If $|P|=n-\frac{t}{2}$, $|Q| = |R| = \frac{t}{4}$, $|R|=0$, while $R$ is also receive-isolated after some round and the communication complexity of $\mathcal{A}$ is less than $\frac{t^2}{16}$, then $\exists Q' \subset Q$, $|Q| = \frac{t}{8}$, such that every process in $Q'$ decides $b_P$.
\end{corollary}

\fi




\begin{definition}
Let $P = \{P_{i_1}, ..., P_{i_{\ell}}\}$ be a set of correct processes.
Let $\bar{b} : P \rightarrow \{0, 1\}$ that maps each process $P_i \in P$ to a proposal bit $\bar{b}(P_i) \in \{0,1\}$.
Let $M$ be a set of messages not sent by processes in $P$, i.e. $\forall m \in M, m.\mathit{sender} \notin P$.
For every $k \in \mathbb{N} \cup \{\infty\}$,
We define $\mathsf{correct}(P, \bar{b},M,k) \triangleq [\mathcal{B}_{i_1}, ..., \mathcal{B}_{i_{\ell}}]$,  where each $\mathcal{B}_{i} \triangleq \langle \mathcal{F}^1_i, ..., \mathcal{F}^k_i\rangle$ is a $k$-round behavior of process $P_i$ and each $\mathcal{F}^j_i \triangleq (\state{i}{j}, \msgs{i}{j}, \emptyset, \msgr{i}{j}, \emptyset)$ as follows.

\begin{compactenum}
    \item (Initialization) $\forall P_i \in P$:
\begin{itemize}
\item  (correct proposal) $\pstate{i}{1}.\mathit{proposal} = \bar{b}(P_i)$, $  \msgs{i}{1} = \mathcal{M}^{b_i}_i$
\item (received message) $\msgr{i}{1} = \{m \in M \cup (\bigcup_{i \in \{i_{1}, ..., i_{\ell}\}} \msgs{i}{1}) | m.\mathit{round} = 1 \wedge m.\mathit{receiver} = P_i\}$
\end{itemize}    
    \item (Induction) $\forall P_i \in P, \forall j \in [1:k]$:
    \begin{itemize}
\item  (correct transition) if $j<k$, $(\pstate{i}{j+1}, \msgs{i}{j+1}) = \mathcal{A}(\pstate{i}{j}, \msgr{i}{j})$
\item (received message) $\msgr{i}{j} = \{m \in M \cup (\bigcup_{i \in \{i_{1}, ..., i_{\ell}\}} \msgs{i}{j}) | m.\mathit{round} = j \wedge m.\mathit{receiver} = P_i\}$
\end{itemize}    
\end{compactenum}
\end{definition}

\iffalse
%%%%%%%%%%%%
%% useless lemma %%
%%%%%%%%%%%%
\begin{lemma}
Let $P = \{P_{i_1}, ..., P_{i_{\ell}}\}$ be a set of correct processes.
Let $\bar{b} : P \rightarrow \{0, 1\}$ that maps each process $P_i \in P$ to a proposal bit $\bar{b}(P_i) \in \{0,1\}$. Let $(k',k) \in \mathbb{N} \times (\mathbb{N} \cup \{\infty\})$ with $k' < k$.
Let $M = M_{\leq k'} \uplus M_{>k'}$ be a set of messages not sent by processes in $P$ (i.e. $\forall m \in M, m.\mathit{sender} \notin P$), such that (1) $\forall m \in M_{\leq k'}$, $m.\mathsf{round} \leq k'$ and $\forall m \in M_{> k'}$, $m.\mathsf{round} > k'$.

Let $[\mathcal{B}_{i_1}, ..., \mathcal{B}_{i_{\ell}}] = \mathsf{correct}(P, \bar{b},M,k)$ and $[\mathcal{B}'_{i_1}, ..., \mathcal{B}'_{i_{\ell}}] = \mathsf{correct}(P, \bar{b},M_{\leq k'},k')$.

For every $P_i \in P$, we note $\mathcal{B}'_{i} = \langle \mathcal{F}_{i}^{\prime 1}, ...,  \mathcal{F}_{i}^{\prime k'}\rangle$ and $\mathcal{B}_{i} = \langle \mathcal{F}_{i}^{1}, ...,  \mathcal{F}_{i}^{k}\rangle$.

Then, $\forall P_i \in P$,  $\forall j \in [1:k']$, $\mathcal{F}^{j}_{i} = \mathcal{F}^{\prime j}_{i} $
\end{lemma}

\begin{proof}
It is trivial to realise that the construction are the same ones until round $k'$.
\end{proof}

%%%%%%%%%%%%%%
%% end useless lemma %%
%%%%%%%%%%%%%%
\fi

Now, we are ready to prove the key lemma of the paper.

\begin{lemma}[Combining receive-isolation]\label{lemma:combining_receive_isolation}
Let  $\bar{b}^u, \bar{b}^v: \Pi \rightarrow \{0,1\}$.
Let $\mathcal{A}$ be an agreement algorithm.
Let $\mathcal{E}^{u}$ and $\mathcal{E}^{v}$ be two infinite executions of $\mathcal{A}$ such that:
\begin{compactitem}
\item $\forall P_i \in \Pi$, $P_i$ proposes $\bar{b}^u(P_i)$ (resp.  $\bar{b}^v(P_i)$) in $\mathcal{E}^{u}$ (resp.  $\mathcal{E}^{v}$).
\item in $\mathcal{E}^{u}$: $A \cup B $ are correct,  while $C$ is receive-isolated from some round $k^u$ onward. 
\item in $\mathcal{E}^{v}$: $A \cup C $ are correct,  while $B$ is receive-isolated from some round $k^v$ onward.
\item $A$ decides $b'_u$ in $\mathcal{E}^{u}$ and $b'_v$ in $\mathcal{E}^{v}$
\end{compactitem}
If either (1) $k^u = k^v = 1$ or (2) $|k^u-k^v| \leq 1$ and $\bar{b}^u = \bar{b}^v$. \newline
Then,  either (3) the message-complexity of $\mathcal{A}$ is greater than $\frac{t^2}{16}$, or (4) $b'_u = b'_v$.
\end{lemma}

\begin{proof}[formal proof] (see figure \ref{figure:lemma_343} for case (1) and \ref{figure:lemma_343} for case (2) )
By contradiction, let us assume than both the message-complexity of $\mathcal{A}$ is lower than $\frac{t^2}{16}$, and $b'_u \neq b'_v$.

We note $\mathcal{E}^u = [\mathcal{F}^u, \mathcal{B}^{u}_1, ...,  \mathcal{B}^{u}_n]$ and $\mathcal{E}^v = [\mathcal{F}^v, \mathcal{B}^{v}_1, ...,  \mathcal{B}^{v}_n]$.
By lemma \ref{lemma:0bis}, there exists a set $B' \subset B$ of $|B'| = \frac{t}{8}$ processes that decide $b'_u$ in $\mathcal{E}^u$ and there exists a set $C' \subset C$ of $|C'| = \frac{t}{8}$ processes that decide $b'_v$ in $\mathcal{E}^v$.
Let's construct a new infinite execution $\mathcal{E}^{*} = [\mathcal{F}^{*}, \mathcal{B}^{*}_1, ...,  \mathcal{B}^{*}_n]$, as follows:
\begin{compactenum}

\item (Message naming) We note:

\begin{compactitem}
\item $k^{-} = \mathsf{min}(k^u, k^{w})$ and $k^{+} = \mathsf{max}(k^u, k^{w})$.

\item  $M^{S(B,C)} = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{v}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{u}_i}{k'} \big)$.

%\item  $M^{S(B,C)}_{\leq k^{-}}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k^{-}]}  \fmsgs{\mathcal{B}^{v}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k^{-}]}  \fmsgs{\mathcal{B}^{u}_i}{k'} \big)$.

%\item $M^{S(B,C)}_{> k^{-}}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [k^{-}+1:k]}  \fmsgs{\mathcal{B}^{v}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [k^{-}+1:k]}  \fmsgs{\mathcal{B}^{u}_i}{k'} \big)$.

%\item  $M^{S(B,C)} = M^{S(B,C)}_{\leq k^{-}} \uplus M^{S(B,C)}_{> k^{-}}$

\end{compactitem}



\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A : A  \rightarrow \{0,1\}$ with $\forall P_i \in A, \bar{b}_A(P_i) = \bar{b}^{u}(P_i)$.  We define
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

\item Let $P_i \in B\cup C$. We note $ \mathcal{B}_{i} =  \mathcal{B}^{v}_{i}$ if $P_i \in B$ and $ \mathcal{B}_{i} =  \mathcal{B}^{u}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}^{*}_{i} \gets \mathcal{B}_{i}$. \label{item:init_behaviours_receive_isolated_groups_in_combined_execution}

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], $

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup C} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in B$, and  

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup B} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in C$\label{item:replace_receive_omission_in_combined_execution}

\item $\mathcal{F}^{*} \subseteq \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}^{*}_i}{k'} \neq \emptyset\}$

\end{compactenum}


Let us show that $\mathcal{E}^{*}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} = B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior. Let $P_i \in \Pi$. If $P_i \in A$,  $\mathcal{B}_i^{*}$ is an infinite behavior of process $P_i$ by construction of $\mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.  If $P_i \in B \cup B$, $\mathcal{B}_i^{*}$ is   is an infinite behavior of process by \ref{lemma:behavior_receive_omitted} applied to the infinite behavior $\mathcal{B}_i$.  
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $ \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $ \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

\item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgr{\mathcal{B}_r}{j}$ by send-validity of $\mathcal{E}^u$ and $\mathcal{E}^v$ so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_in_combined_execution}.

\item If $(P_s, P_r) \in A \times (B \cup C) \cup (B \times C) \cup (C \times B)$, $m \in \fmsgro{\mathcal{B}^{*}_r}{j}$ is ensured by step \ref{item:replace_receive_omission_in_combined_execution} of the construction of $\mathcal{E}^{*}$, while no step modifies $\fmsgro{\mathcal{B}^{*}_r}{j}$ afterwards.

\end{compactitem}
    
    
    
    Send-validity is satisfied in $\mathcal{E}^{*}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r^{*}}{j} \cup \fmsgro{\mathcal{B}_r^{*}}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

 \item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgs{\mathcal{B}_s}{j}$ by send-validity of $\mathcal{E}^u$ and $\mathcal{E}^v$, so $m \in \fmsgs{\mathcal{B}_r}{j}$, since $\fmsgs{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_in_combined_execution}.

\item If $(P_s, P_r) \in (A \times (B \cup C)) \cup (B \times C) \cup (C \times B)$,  $m \notin \fmsgr{\mathcal{B}_r}{j}$. 
If $m \in \fmsgro{\mathcal{B}^{*}_r}{j}$, then
$m \in \fmsgs{\mathcal{B}^{*}_s}{j}$,   by step \ref{item:replace_receive_omission_in_combined_execution}, while no step modifies neither $\fmsgs{\mathcal{B}^{*}_s}{j}$ or $ \fmsgro{\mathcal{B}^{*}_r}{j}$ afterwards.

So let us assume $m \in \fmsgr{\mathcal{B}^{*}_r}{j}$. 

In that case, $j \leq k^{-}$. Indeed, $B$ (resp. $C$) is receive-isolated from the round $k^v$ (resp. $k^u$) in execution $\mathcal{E}^u$ (resp.  $\mathcal{E}^v$), so $j > k^{-}$ would imply $m \notin \fmsgr{\mathcal{B}_r}{k^{-}}$. Finally, it would imply $m \notin \fmsgr{\mathcal{B}_r^{*}}{k^{-}}$ by step \ref{item:init_behaviours_receive_isolated_groups_in_combined_execution}, while no step modifies $ \fmsgr{\mathcal{B}^{*}_r}{j}$ afterwards.

Moreoever, the condition $k^{u} = k^{v}=1$ does not hold, since $B \cup C$ would be receive-isolated from the first round of the execution $\mathcal{E}^{*}$. Hence, in addition of $j \leq k^{-}$, the condition $|k^u-k^v| \leq 1 \wedge \bar{b}^u = \bar{b}^v$
necessarily holds, to satisfy the precondition of the lemma.

Since no group of processes is receive-isolated before $k^{-}$,  and $\bar{b}^u = \bar{b}^v$, the executions $\mathcal{E}^{u}$, $\mathcal{E}^{v}$,  and $\mathcal{E}^{*}$ share a common prefix until round $k^{-}-1$ and messages sent in round $k^{-}$, which means that $\forall k' \in [1:k^{-}] $, $\bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{*}}{k'} = \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{u}}{k'} = \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{v}}{'}$.
Hence, $ \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{*}}{j} =  \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{u}}{j} =  \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{v}}{j} \triangleq M_{j}$.

By receive-validity of $\mathcal{E}^{u}$ and $\mathcal{E}^{v}$, $m \in M_{j}$ and so $m \in  \fmsgs{\mathcal{B}^{*}_s}{j}$.

\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}^{*}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}^{*}$ since no process in $A$ commits any omission fault by construction of $ \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.
\end{compactitem}
Thus, $\mathcal{E}^{*}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $b'_u$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $b'_v$ in $\mathcal{E}^*$.
By \Cref{lemma:0bis}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.

Thus, the lemma holds.

\end{proof}

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/lemma_343.eps}
\caption{Lemma \ref{lemma:combining_receive_isolation}, case (1) }
\label{figure:lemma_343}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/lemma_344.eps}
\caption{Lemma \ref{lemma:combining_receive_isolation}, case (2)}
\label{figure:lemma_344}
\end{figure}

In the rest of the proof, we assume the message complexity of $\mathcal{A}$ is lower than $\frac{t^2}{16}$. Moreover, we rely on the following two infinite executions:
\begin{compactitem}
    \item $\mathcal{E}_0$: 
    The group $B$ is receive-isolated from round $1$; all other processes are correct.
    Every process proposes $0$. 

    \item $\mathcal{E}_1$:
    The group $C$ is receive-isolated from round $1$; all other processes are correct.
    Every process proposes $1$.
\end{compactitem}

\begin{lemma}
Let $\mathcal{E}_0$ and $\mathcal{E}_1$ as defined above and presented in figure \ref{figure:lemma_3}.
There exists a pair of sets $(B', C') \subset B \times C$ of size $|B'| = |C'| = \frac{t}{8}$ such that processes  in $A \cup C \cup B'$ decide $b \in \{0, 1 \}$ in $\mathcal{E}_0$ and $A \cup B \cup C'$ decide $b' \in \{0, 1 \}$ in $\mathcal{E}_1$.
Moreover either $b = 1$ or $b'=0$.
\end{lemma}

\begin{proof}%[New proof]
We apply \Cref{lemma:combining_receive_isolation} to executions $\mathcal{E}^u=\mathcal{E}_0$ and $\mathcal{E}^v = \mathcal{E}_1$ and $k^{u} = k^{v} = 1$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}[proof sketch]
(see figure \ref{figure:lemma_3})
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{8}$ processes that decide $b$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{8}$ processes that decide $b'$ in $\mathcal{E}_1$.
%\pierre{it seems to me we can avoid the set of size $\frac{|B|}{4}$ (resp. $\frac{|C|}{4}$ invoked in the proof of lemma \ref{lemma:either} (lemma 3). The remaining part is the same.}
By contratiction, assume $b=0$ and $b'=1$. Let's construct a new infinite execution $\mathcal{E}^{*}$, such that $\mathcal{E}^{*}|_{B} \equiv \mathcal{E}_0|_{B}$ and $\mathcal{E}^{*}|_{C} \equiv \mathcal{E}_1|_{C}$:

\begin{compactenum}
    \item In $\mathcal{E}^*$, all processes from $A \cup B$ propose $0$, whereas all processes from $C$ propose $1$.

    \item All processes from $A$ are correct, whereas all processes from $B \cup C$ are faulty.
    Note that $|B \cup C| < t$.

    \item Every process from $B$ exhibits the exact same behavior as in $\mathcal{E}_0$.
    Note that this step implies that $B$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    \item Every process from $C$ exhibits the exact same behavior as in $\mathcal{E}_1$.
    Note that this step implies that $C$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    % \item Both groups $B$ and $C$ are receive-isolated from round $1$.
\end{compactenum}
Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages}, correct processes send at least $\frac{t^2}{32}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{32}$ (or even $\frac{t^2}{16}$) messages in every execution.
Thus, the lemma holds.
\end{proof}

\begin{proof}[formal proof]
We note $\mathcal{E}_0 = [\mathcal{F}_0, \mathcal{B}^{0}_1, ...,  \mathcal{B}^{0}_n]$ and $\mathcal{E}_1 = [\mathcal{F}_1, \mathcal{B}^{1}_1, ...,  \mathcal{B}^{1}_n]$.
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{4}$ processes that decide $b$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{4}$ processes that decide $b'$ in $\mathcal{E}_1$.
By contratiction, assume $b=0$ and $b'=1$. Let's construct a new infinite execution $\mathcal{E}^{*} = [\mathcal{F}^{*}, \mathcal{B}^{*}_1, ...,  \mathcal{B}^{*}_n]$, as follows:
\begin{compactenum}
\item $\mathcal{F}^{*} = B \cup C$

\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{0}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{1}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M,k)$.

\item $\forall P_i \in B\cup C$, we note $ \mathcal{B}_{i} =  \mathcal{B}^{0}_{i}$ if $P_i \in B$ and $ \mathcal{B}_{i} =  \mathcal{B}^{1}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}^{*}_{i} \gets \mathcal{B}_{i}$.

%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], $

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup C} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in B$, and  

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup B} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in C$\label{item:replace_receive_omission_in_e_star}

\item $\mathcal{F} \subseteq \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}^{*}_i}{k'} \neq \emptyset\}$

\end{compactenum}


Let us show that $\mathcal{E}^{*}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} = B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times (B \cup C)$, $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ is ensured by step \ref{item:replace_receive_omission_in_e_star} of the construction of $\mathcal{E}^{*}$.
\end{compactitem}
    
    
    
    Send-validity is satisfied in $\mathcal{E}^{*}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r^{*}}{j} \cup \fmsgro{\mathcal{B}_r^{*}}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times (B \cup C)$, $m \in \fmsgro{\mathcal{B}_r^{*}}{j}$, since $\fmsgr{\mathcal{B}_r^{*}}{j} = \emptyset$ by construction, because $\fmsgr{\mathcal{B}_r}{j} = \emptyset$ and no additional received messages are added during the contruction of $\mathcal{B}_r^{*}$.
Thus, $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ is ensured by step \ref{item:replace_receive_omission_in_e_star} of the construction of $\mathcal{E}^{*}$.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}^{*}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}^{*}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}^{*}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Hence, the assumption $b=0$ and $b'=1$ is false, which means that either $b=1$ or $b'=0$.
Thus, the lemma holds.

\end{proof}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end  lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/lemma_5.eps}
\caption{Lemma \ref{lemma:either_or}}
\label{figure:lemma_3}
\end{figure}

Then, we define the execution $\mathcal{E}^{k^{*}}$, and $\mathcal{E}^{k^{*}+1}$ as in \Cref{lemma:final}, and illustrated in figure \ref{figure:execution_C}. Without loss of generality, it has been assumed that processes in $A$ decide $b=1$ in execution $\mathcal{E}_0$.

Next, let $\mathcal{E}^*_0$ denote the fully-correct infinite execution in which all processes propose $0$.
Note that, in order to satisfy \emph{Weak Validity}, all processes decide $0$ in $\mathcal{E}_0^*$.
Let $k_0^* \in \mathbb{N}^+$ denote the first round in which (at least) $\frac{t}{8}$ processes from $B$ decide the same bit in $\mathcal{E}_0^*$.

For every round $k \in [1, k_0^*]$, we perform the following actions:
\begin{compactenum}
    \item We consider the infinite execution $\mathcal{E}^k$ such that (1) every process proposes $0$, (2) every process behaves correctly until (and including) round $k - 1$ (i.e., no omission faults occur), (3) group $B$ is receive-isolated from round $k$, and (4) processes in $A \cup C$ are correct.

    \item By \Cref{lemma:0bis}, at least $\frac{t}{8}$ processes from $B$ decide the same bit $b_k$ in $\mathcal{E}^k$.
\end{compactenum}
Importantly, $b_1 = 1$ (due to the assumption) and $b_{k_0^*} = 0$ (due to the execution $\mathcal{E}_0^*$).
Hence, there exists a round $k^* \geq 1$ such that $b_{k^*} = 1$ and $b_{k^* + 1} = 0$.

Now, consider an infinite execution $\mathcal{E}_C$ such that (1) every process proposes $0$, (2) every process behaves correctly until (and including) round $k^* - 1$, (3) group $C$ is receive-isolated from round $k^*$, and (4) processes in $A \cup B$ are correct.
By \Cref{lemma:0bis}, at least $\frac{t}{8}$ processes from $C$ decide the same bit $b_C$.

Finally, we are ready to prove a contradiction with the assumed non-existence of an execution of $\mathcal{A}$ with (at least) $\frac{t^2}{16}$ messages sent by correct processes.

\iffalse

Let $\mathcal{E}^{k^*} = [\mathcal{F}^{k^*} = B, \mathcal{B}^{k^*}_1, ..., \mathcal{B}^{k^*}_n]$, let $\mathcal{E}^{k^* + 1} = [\mathcal{F}^{k^* + 1} = B, \mathcal{B}^{k^* + 1}_1, ..., \mathcal{B}^{k^* + 1}_n]$ and let $\mathcal{E}^C = [\mathcal{F}^C = C, \mathcal{B}_1^C, ..., \mathcal{B}_n^C]$.
The following holds:
\begin{compactitem}
    \item At least $\frac{t}{8}$ processes from $B$ decide the $1$ in $\mathcal{E}^{k^*}$.

    \item At least $\frac{t}{8}$ processes from $B$ decide the $0$ in $\mathcal{E}^{k^* + 1}$.
    
    \item At least $\frac{|C|}{4}$ processes from $C$ decide the same bit $b_C$ in $\mathcal{E}^C$.

    \item Until (and including) round $k^* - 1$, $\mathcal{B}_i^{k^*} = \mathcal{B}_i^{k^* + 1} = \mathcal{B}_i^C$, for every process $P_i$.
\end{compactitem}

\fi

\begin{figure}[!t]
\centering
\includegraphics[clip, trim=0cm 6.5cm 0cm 0cm, width=13cm]{figures/quadratic_lower_bound_execution_C.eps}
\caption{Executions $\mathcal{E}^{k^{*}}$ and $\mathcal{E}^{k^{*}+1}$}
\label{figure:execution_C}
\end{figure}

\begin{lemma}
There exists an execution of $\mathcal{A}$ in which correct processes send (at least) $\frac{t^2}{16}$ messages.
\end{lemma}

\begin{proof}%[New proof]
We apply lemma \ref{lemma:combining_receive_isolation}, case (2),  twice, to executions $\mathcal{E}^u=\mathcal{E}_C$ and $\mathcal{E}^v = \mathcal{E}^{k^{*}}$ in case $b_C=0$ and  $\mathcal{E}^v = \mathcal{E}^{k^{*}+1}$ in case $b_C=1$,  where $(k^{u}, k^{v}) = (k^{*}, k^{*}+1)$, and $\forall P_i \in \Pi$, $\bar{b}^{u}(P_i) = \bar{b}^{v}(P_i) = 0$.  Since $b_{k^{*}} = 1$ and $b_{k^{*}+1} = 1$, either $b_C \neq b_{k^{*}}$ or $b_C \neq b_{k^{*}+1} = 1$.  Thus, there exists an execution of $\mathcal{A}$ in which correct processes send (at least) $\frac{t^2}{16}$ messages. (see figure \ref{figure:lemma_final})
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}[proof sketch]
(see figure \ref{figure:lemma_4})
We consider two possible cases:
\begin{compactitem}
    \item Let $b_C = 0$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Both groups $B$ and $C$ are receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^*}$ (from round $k^*$ onward).
        Note that this step implies that $B$ is receive-isolated from round $k^*$.

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item From (and including) round $k^*$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.

% this is pointless, by item 4. not really, will change something more
        % \item From (and including) round $k^*$ onward, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$ in $\mathcal{E}^k$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$ in $\mathcal{E}_C$.
    \end{compactenum}
    
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $1$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $0$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.

    \item Let $b_C = 1$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}+1}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Group $C$ is receive-isolated from round $k^*$, whereas group $B$ is receive-isolated from round $k^*+1$

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^* + 1}$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^* + 1$.
        \add{Note that the message received in round $k^{*}$ from processes in $C$ are indeed the same ones than in execution $\mathcal{E}^{k^* + 1}$, since the receive-omission at round $k^*$ has no impact of the messages at the same round $k^*$.} 

        \item In round $k^*$, all messages from $C$ are received, which means that processes in $B$ successfully receive messages sent by $C$.

        \item From (and including) round $k^* + 1$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.
        
        
        % we send-omit (1) all messages sent by processes in $C$ to processes in $A$ in $\mathcal{E}_C$.
        % Note that, in round $k^*$, messages sent by processes in $C$ to processes in $B$ are successfully sent and successfully received.

        % \item From round $k^* + 1$, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$.
    \end{compactenum}
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $0$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $1$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.
\end{compactitem}
As the statement of the lemma holds in both possible cases, the proof is concluded.
\end{proof}

\begin{proof}[formal proof]
We note $\mathcal{E}_C = [\mathcal{F}_C, \mathcal{B}^{C}_1, ...,  \mathcal{B}^{C}_n]$, $\mathcal{E}^{k^{*}} = [\mathcal{F}_{k^{*}}, \mathcal{B}^{k^{*}}_1, ...,  \mathcal{B}^{k^{*}}_n]$ and $\mathcal{E}^{k^{*}+1} = [\mathcal{F}_{k^{*}+1}, \mathcal{B}^{k^{*}+1}_1, ...,  \mathcal{B}^{k^{*}+1}_n]$.

Case $b_C = 0$.

Let's construct a new infinite execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ...,  \mathcal{B}_n]$, as follows:
\begin{compactenum}

\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{k^{*}}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{C}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M^S_{(B,C)},k)$.

\item $\forall P_i \in B\cup C$, we note $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{k^{*}}_{i}$ if $P_i \in B$ and $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{C}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}_{i} \gets \tilde{\mathcal{B}}_{i}$. \label{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}

%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], $

$\fmsgro{\mathcal{B}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup C} \fmsgs{\mathcal{B}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in B$, and  

$\fmsgro{\mathcal{B}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup B} \fmsgs{\mathcal{B}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in C$\label{item:replace_receive_omission_when_bc_equal_0}

\item $\mathcal{F} = \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}_i}{k'} \neq \emptyset\}$
\end{compactenum}


Let us show that $\mathcal{E}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} \subseteq B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgr{\tilde{\mathcal{B}}_r}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.

\item If $(P_s, P_r) \in A \times (B \cup C) \cup (B \times C) \cup (C \times B)$, $m \in \fmsgro{\mathcal{B}_r}{j}$ is ensured by step \ref{item:replace_receive_omission_when_bc_equal_0} of the construction of $\mathcal{E}$, while no step modifies $\fmsgro{\mathcal{B}_r}{j}$ afterwards.
\end{compactitem}
    

    Send-validity is satisfied in $\mathcal{E}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.

\item If $(P_s, P_r) \in (A \times (B \cup C)) \cup (B \times C) \cup (C \times B)$,  $m \notin \fmsgr{\tilde{\mathcal{B}}_r}{j}$ since both $B$ and $C$ are receive isolated in $\mathcal{E}^{k^{*}}$ and $\mathcal{E}^C$ respectively.  Moreover, $\fmsgr{\mathcal{B}_r}{j} = \fmsgr{\tilde{\mathcal{B}}_r}{j}$ because no step modifies $\fmsgr{\mathcal{B}_r}{j}$ after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}. Hence, $m \notin \fmsgr{\mathcal{B}_r}{j}$,  and so $m \in \fmsgro{\mathcal{B}_r}{j}$.
Finally, 
$m \in \fmsgs{\mathcal{B}_s}{j}$,   by step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}, while no step modifies neither $\fmsgs{\mathcal{B}_s}{j}$ or $ \fmsgro{\mathcal{B}_r}{j}$ afterwards.

 \item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgs{\tilde{\mathcal{B}}_s}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}$, the following holds: (1) all processes from $B'$ decide $1$ in $\mathcal{E}$, and (2) all processes from $C'$ decide $0$ in $\mathcal{E}$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}$.
%which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Thus, the lemma holds.

Case $b_C = 1$.

Let's construct a new infinite execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ...,  \mathcal{B}_n]$, as follows:
\begin{compactenum}


\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{k^{*}+1}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{C}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M^S_{(B,C)},k)$.

\item $\forall P_i \in B\cup C$, we note $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{k^{*}+1}_{i}$ if $P_i \in B$ and $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{C}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}_{i} \gets \tilde{\mathcal{B}}_{i}$.
\label{item:init_behaviours_receive_isolated_groups_when_bc_equal_1}
%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], \fmsgro{\mathcal{B}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in \Pi \setminus \{P_i\}} \fmsgs{\mathcal{B}_j}{k'} | m.\mathsf{receiver} = P_i\}$ \label{item:replace_receive_omission_when_bc_equal_1}

\item $\mathcal{F} = \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}_i}{k'} \neq \emptyset\}$
\end{compactenum}

Let us show that $\mathcal{E}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} \subseteq B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgr{\tilde{\mathcal{B}}_r}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.

\item If $(P_s, P_r) \in A \times (B \cup C) \cup (B \times C) \cup (C \times B)$, $m \in \fmsgro{\mathcal{B}_r}{j}$ is ensured by step \ref{item:replace_receive_omission_when_bc_equal_0} of the construction of $\mathcal{E}$, while no step modifies $\fmsgro{\mathcal{B}_r}{j}$ afterwards.
\end{compactitem}
    

    Send-validity is satisfied in $\mathcal{E}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (A \times (B \cup C)) \cup (B \times C) \cup (C \times B)$,  $m \notin \fmsgr{\tilde{\mathcal{B}}_r}{j}$ since both $B$ and $C$ are receive isolated in $\mathcal{E}^{k^{*}+1}$ and $\mathcal{E}^C$ respectively.  Moreover, $\fmsgr{\mathcal{B}_r}{j} = \fmsgr{\tilde{\mathcal{B}}_r}{j}$ because no step modifies $\fmsgr{\mathcal{B}_r}{j}$ after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}. Hence, $m \notin \fmsgr{\mathcal{B}_r}{j}$,  and so $m \in \fmsgro{\mathcal{B}_r}{j}$.
Finally, 
$m \in \fmsgs{\mathcal{B}_s}{j}$,   by step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}, while no step modifies neither $\fmsgs{\mathcal{B}_s}{j}$ or $ \fmsgro{\mathcal{B}_r}{j}$ afterwards.

 \item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgs{\tilde{\mathcal{B}}_s}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}$.
%which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Thus, the lemma holds.
\end{proof}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end  lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/final_lemma.eps}
\caption{Lemma \ref{lemma:final}}
\label{figure:lemma_final}
\end{figure}







==> sections/lower_bound.tex <==
\section{Lower Bound on Message Complexity of Synchronous Consensus}

In this section, we show the quadratic lower bound on message complexity for any synchronous algorithm solving the Byzantine consensus problem with any non-trivial (and solvable) validity property.

\paragraph{Events.}
An \emph{event} is a pair $e = [P, a]$, where $P \in \Pi$ is a process and $a \in \{ \mathsf{propose}(v \in \mathcal{V}_I), \mathsf{decide}(v' \in \mathcal{V}_O), \mathsf{send}(m \in \mathcal{M}), \mathsf{receive}(m' \in \mathcal{M}) \}$.
Intuitively, an event describes an action of a process.
For instance, $e = [P, \mathsf{decide}(v')]$ means that the process $P$ decides a value $v'$.

\paragraph{Process' behavior.}
A \emph{round behavior} of a process $P$ is a sequence of events $e' = [P, \cdot]$, i.e., all events are associated with $P$.
A \emph{$k$-round behavior} of a process $P$ is a sequence of $k$ round behaviors of $P$.
Given a $k$-round behavior $\beta_P^k$ of a process $P$ and a set of processes $S \subset \Pi$ with $P \notin S$, $\mathsf{ignorance}(S, \beta_P^k)$ denotes a $k$-round behavior $\gamma_P^k$ such that $\gamma_P^k$ is identical to $\beta_P^k$ except that all events $[P, \mathsf{receive}(m)]$ with $\mathsf{sender}(m) \in S$ are removed.
We say that a $k$-round behavior of a process is \emph{valid} according to an algorithm is correct if and only if the behavior follows the state transitions imposed by the algorithm.

\paragraph{Notation \& definitions.}
We start by stating the notation and a few definitions we use throughout the entire proof.





\begin{definition}
Consider any $k$-round execution $\mathcal{E}_k$.
A set of processes $S$ is said to \emph{become ignorant} at round $r < k$ in $\mathcal{E}_k$ if and only if (1) all processes in $S$ are faulty in $\mathcal{E}_k$, and (2) 
\end{definition}

\begin{theorem} \label{theorem:lower_bound}
The message complexity of any synchronous algorithm solving the Byzantine consensus problem with Weak Validity is $\Omega(t^2)$.
\end{theorem}

We prove the theorem by contradiction.
Hence, we fix any synchronous algorithm $\mathcal{A}$ which solves Byzantine consensus with \emph{Weak Validity} and exchanges $o(t^2)$ messages.
In order to prove \Cref{theorem:lower_bound}, we prove that there exists an execution in which $\mathcal{A}$ violates \emph{Agreement}.

\begin{lemma} 
Let $S \subset \Pi$ be any subset of $|S| = t / 4$ processes.
Consider any execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ such that (1) processes in $S$ are faulty, whereas all other processes are correct, and (2) in some round $R \geq 0$, processes in $S$ become ignorant.
There exists an execution $\mathcal{E}' \in \mathit{execs}(\mathcal{A})$ such that (1)


\begin{compactitem}
    \item Processes in $S$ are faulty, whereas all other processes are correct.

    \item In some round $R$, processes in $S$ become ignorant.
\end{compactitem}




Consider any execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ such that (1) there exists a set $S \subset \Pi$ of $|S| = t / 4$ processes faulty in $\mathcal{E}$, and (2) from some round $r$ onward, all 

\end{lemma}

==> sections/lower_bound_algorithm.tex <==
% \newpage
\section{Lower Bound \& General Algorithm}
\label{section:lower_upper_bounds}

This section is devoted to the cost of solving  consensus.
Specifically, we first show that any non-trivial and solvable validity property requires $\Omega(t^2)$ messages to be exchanged (\Cref{subsection:lower_bound}).
Then, we present \general, a general algorithm which, if $n > 3t$, solves consensus  with any validity property which satisfies $\mathcal{C}_S$ (\Cref{subsection:general_algorithm}).
Thus, \general proves the sufficiency of $\mathcal{C}_S$ when $n > 3t$.
% \footnote{Recall that, if $n \leq 3t$, any solvable validity property is trivial (see \Cref{subsection:triviality_main}).}

\subsection{Lower Bound on Message Complexity}
\label{subsection:lower_bound}

In this subsection, we prove the following theorem:

\begin{theorem} \label{theorem:lower_bound_main}
If an algorithm solves consensus  with a non-trivial validity property, the message complexity of the algorithm is $\Omega(t^2)$.
\end{theorem}

% This subsection proves that any algorithm which solves the Byzantine consensus problem with a non-trivial and solvable validity property incurs $\Omega(t^2)$ message complexity.
\Cref{theorem:lower_bound_main} extends the seminal Dolev-Reischuk bound~\cite{dolev1985bounds}, proven only for consensus algorithms with \emph{Strong Validity}, to all non-trivial variants of consensus.
% validity properties.
To prove \Cref{theorem:lower_bound_main}, we intertwine the idea of the original proof~\cite{dolev1985bounds} with the canonical similarity result (\Cref{subsection:similarity}).

% The proof of \Cref{theorem:lower_bound_main} follows the idea of the original proof~\cite{dolev1985bounds}.
% However, as \Cref{theorem:lower_bound_main} focuses on \emph{all} validity properties, our proof neatly conn

\paragraph{Proof of \Cref{theorem:lower_bound_main}.}
In our proof, we show that any algorithm which solves the Byzantine consensus problem with a non-trivial validity property has a synchronous execution ($\text{GST} = 0$) in which correct processes send 
more than $(\frac{t}{2})^2$ messages.
Hence, throughout the entire subsection, we fix a non-trivial and solvable validity property $\mathit{val}$.
Moreover, we fix $\mathcal{A}$, an algorithm which solves Byzantine consensus with $\mathit{val}$.
As $\mathit{val}$ is a non-trivial validity property, $n > 3t$ (\Cref{subsection:triviality_main}).


% Throughout the entire subsection, we fix a non-trivial and solvable validity property $\mathit{val}$.
% Moreover, we fix $\mathcal{A}$, an algorithm which solves the Byzantine consensus problem with $\mathit{val}$.
% Finally, $n > 3t$ as $\mathit{val}$ is non-trivial (see \Cref{subsection:triviality_main}).

% \paragraph{Overview of the proof.}
% We prove the lower bound by the means of contradiction.
% Hence, suppose that the message complexity of $\mathcal{A}$ is $o(t^2)$.
% Our proof consists of two steps: 
% \begin{compactenum}
%     \item We identify a process $Q$ such that $\mathcal{A}$ allows $Q$ to decide some value $v_Q \in \mathcal{V}_O$ without receiving any message (from any other processes).
%     The first step of our proof is identical to the first step of the original Dolev-Reischuk proof~\cite{dolev1985bounds,DBLP:conf/podc/AbrahamCDNP0S19}.
    
%     \item We show that there exists an execution of $\mathcal{A}$ such that (1) $Q$ is faulty and silent, and (2) other processes decide some value $v \neq v_Q$.
%     Hence, we can then ``merge'' this execution with a correct behavior of $Q$ in which $Q$ decides $v_Q$ without having received any message, thus constructing an execution in which \emph{Agreement} is violated.
    
%     The original proof of the Dolev-Reischuk bound follows the same idea.
%     However, given that the original bound concerns only \emph{Strong Validity}, the second step in the original proof is straightforward.
%     Conversely, as our bound considers \emph{all} non-trivial and solvable validity properties, completing the second step proved more challenging.
% \end{compactenum}
% In this subsection, we give an informal proof of our lower bound; the formal treatment is delegated to \Cref{section:lower_bound_appendix}.

% \paragraph{Execution $\mathcal{E}_{\mathit{base}}$ of $\mathcal{A}$.}
Next, we define a specific infinite execution $\mathcal{E}_{\mathit{base}} \in \mathit{execs}(\mathcal{A})$ in the following manner:
\begin{compactenum}
     \item $\text{GST} = 0$.
     That is, the system is synchronous throughout the entire execution.
     
     \item All processes are separated into two disjoint groups: (1) group $A$, with $|A| = n - \lceil \frac{t}{2} \rceil$, and (2) group $B$, with $|B| = \lceil \frac{t}{2} \rceil$.
     
     \item All processes in the group $A$ are correct, whereas all processes in the group $B$ are faulty.
     
     \item We fix any value $v^* \in \mathcal{V}_I$.
     For every correct process $P_A \in A$, the proposal of $P_A$ in $\mathcal{E}_{\mathit{base}}$ is $v^*$.
     
     \item For every faulty process $P_B \in B$, $P_B$ behaves correctly in $\mathcal{E}_{\mathit{base}}$ with its proposal being $v^*$, except that (1) $P_B$ ignores the first $\lceil \frac{t}{2} \rceil$ messages received from other processes, and (2) $P_B$ omits sending messages to other processes in $B$. 
\end{compactenum}
% \paragraph{Proof of the lower bound.}
To prove \Cref{theorem:lower_bound_main}, it suffices to show that the message complexity of $\mathcal{E}_{\mathit{base}}$ is greater than $ (\lceil \frac{t}{2} \rceil)^2$.
By contradiction, let the correct processes (processes in $A$) send $\leq (\lceil \frac{t}{2} \rceil)^2$ messages in $\mathcal{E}_{\mathit{base}}$.

The first step of our proof shows that, given that correct processes send $\leq (\lceil \frac{t}{2} \rceil)^2$ messages in $\mathcal{E}_{\mathit{base}}$, there must exist a process $Q \in B$ which can correctly decide some value $v_Q \in \mathcal{V}_O$ without receiving \emph{any} message from any other process.
We prove this claim using the pigeonhole principle.

\begin{lemma} \label{lemma:behavior_without_receptions}
There exist a value $v_Q \in \mathcal{V}_O$ and a process $Q \in B$ such that $Q$ has a correct 
local behavior $\beta_Q$ in which (1) $Q$ decides $v_Q$, and (2) $Q$ receives no messages from other processes.
% can correctly decide $v$ without having received any message from any other process.
\end{lemma}
\begin{proof}
By assumption, correct processes (i.e., processes in the group $A$) send $\leq (\lceil \frac{t}{2} \rceil)^2$ messages in $\mathcal{E}_{\mathit{base}}$.
Therefore, due to the pigeonhole principle, there exists a process $Q \in B$ which receives at most $\lceil \frac{t}{2} \rceil$ messages (from other processes) in $\mathcal{E}_{\mathit{base}}$.
Recall that $Q$ behaves correctly in $\mathcal{E}_{\mathit{base}}$ with its proposal being $v^* \in \mathcal{V}_I$, except that (1) $Q$ ignores the first $\lceil \frac{t}{2} \rceil$ messages received from other processes, and (2) $Q$ does not send any messages to other processes in the group $B$.
We denote by $S_Q$ the set of processes, not including $Q$, which send messages to $Q$ in $\mathcal{E}_{\mathit{base}}$; $|S_Q| \leq \lceil \frac{t}{2} \rceil$.

Next, we construct an infinite execution $\mathcal{E}_{\mathit{base}}'$.
Execution $\mathcal{E}_{\mathit{base}}'$ is identical to $\mathcal{E}_{\mathit{base}}$, except that we introduce the following modifications:
\begin{compactenum}
    % \item $\text{GST}_{\mathit{core}}' = 0$, i.e., the system is synchronous from the beginning.
    
    \item Processes in $(A \cup \{Q\}) \setminus{S_Q}$ are correct; other processes are faulty.
    That is, we make $Q$ correct in $\mathcal{E}'_{\mathit{base}}$, and we make all processes in $S_Q$ faulty in $\mathcal{E}'_{\mathit{base}}$.
    
    \item Processes in $B \setminus{\{Q\}}$ behave exactly as in $\mathcal{E}_{\mathit{base}}$.
    Moreover, processes in $S_Q$ behave exactly as in $\mathcal{E}_{\mathit{base}}$, except that they \emph{do not} send any message to $Q$.
\end{compactenum}
% Importantly, there exists a process $P \in A \setminus{S_Q}$ (as $n > 3t$) such that $P$ cannot distinguish $\mathcal{E}_{\mathit{base}}'$ from $\mathcal{E}_{\mathit{base}}$.
% Hence, as $P$ decides some value $v_Q \in \mathcal{V}_O$ in $\mathcal{E}_{\mathit{base}}$ (as $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{\mathit{base}}$ is infinite), $P$ decides the same value $v_Q$ in $\mathcal{E}_{\mathit{base}}'$.
Due to the construction of $\mathcal{E}_{\mathit{base}}'$, process $Q$ does not receive any message (from any other process) in $\mathcal{E}_{\mathit{base}}'$.
As $Q$ is correct in $\mathcal{E}_{\mathit{base}}'$ and $\mathcal{A}$ satisfies \emph{Termination}, $Q$ decides some value $v_Q \in \mathcal{V}_O$ in $\mathcal{E}_{\mathit{base}}'$.
Thus, $Q$ indeed has a correct local behavior $\beta_Q$ in which it decides $v_Q \in \mathcal{V}_O$ without having received messages from other processes. 
\end{proof}
% \jovan{Is this proof ok? Please, try to attack is much as possible. Can there be any problems with timers or I don't know what.
% I am not seeing any problems. Just want us to be very careful!}

In the second step of our proof, we show that there exists an infinite execution in which (1) $Q$ is faulty and silent, and (2) correct processes decide some value $v \neq v_Q$.
% As $\mathit{val}$ is a non-trivial validity property, there exists some input configuration $c_{\notni v_Q} \in \mathcal{I}$ where $v_Q$ is not an admissible value, i.e., $v_Q\notin \mathit{val}(c_{\notni v_Q})$; recall that $v_Q$ is the value that $Q$ can correctly decide without having received any message from any other process (by \Cref{lemma:behavior_without_receptions}).
% The following lemma shows that $Q \in \processes{c_{\notni v_Q}}$; otherwise, $Q$ could be faulty and \emph{Agreement} would not necessarily be violated.

\begin{lemma} \label{lemma:conflicting_execution}
There exists an infinite execution $\mathcal{E}_{v}$ such that (1) $Q$ is faulty and silent in $\mathcal{E}_{v}$, and (2) a value $v \neq v_Q$ is decided by a correct process.
\end{lemma}
\begin{proof}
As $\mathit{val}$ is a non-trivial validity property, there exists an input configuration $c_{\notni v_Q} \in \mathcal{I}$ such that $v_Q \notin \mathit{val}(c_{\notni v_Q})$; recall that $v_Q$ is the value that $Q$ can correctly decide without having received any message from any other process (\Cref{lemma:behavior_without_receptions}).
We consider two possible cases:
\begin{compactitem}
     \item Let $Q \notin \processes{c_{\notni v_Q}}$.
     Thus, $\mathcal{E}_v$ is any infinite canonical execution which corresponds to $c_{\notni v_Q}$.
     As $v_Q \notin \mathit{val}(c_{\notni v_Q})$, the value decided in $\mathcal{E}_v$ must be different from $v_Q$ (as $\mathcal{A}$ satisfies $\mathit{val}$).
     
     \item Let $Q \in \processes{c_{\notni v_Q}}$.
     We construct an input configuration $c_{\notni Q} \in \mathcal{I}$ such that $Q \notin \processes{c_{\notni Q}}$:
     \begin{compactenum}
        \item Let $c_{\notni Q} \gets c_{\notni v_Q}$.

        \item We remove $(Q, \cdot)$ from $c_{\notni Q}$.
        That is, we remove $Q$'s process-proposal pair from $c_{\notni Q}$.

        \item If $|\processes{c_{\notni v_Q}}| = n - t$, we add $(Z, \text{any proposal})$ to $c_{\notni Q}$, where $Z$ is any process such that $Z \notin \processes{c_{\notni v_Q}}$; note that such a process $Z$ exists as $t > 0$.
    \end{compactenum}
    Due to the construction of $c_{\notni Q}$, $c_{\notni Q} \sim c_{\notni v_Q}$.
    Indeed, (1) $\processes{c_{\notni Q}} \cap \processes{c_{\notni v_Q}} \neq \emptyset$ (as $n - t - 1 > 0$ when $n > 3t$ and $t > 0$), and (2) for every process $P \in \processes{c_{\notni Q}} \cap \processes{c_{\notni v_Q}}$, the proposal of $P$ is identical in $c_{\notni Q}$ and $c_{\notni v_Q}$.
    
    In this case, $\mathcal{E}_v$ is any infinite canonical execution such that $\mathsf{input\_conf}(\mathcal{E}_{v}) = c_{\notni Q}$.
    As $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{v}$ is infinite, some value $v \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_{v}$.
    As $c_{\notni Q} \sim c_{\notni v_Q}$, $v \in \mathit{val}(c_{\notni v_Q})$ (by canonical similarity; \Cref{lemma:helper_main}).
    Finally, $v \neq v_Q$ as (1) $v \in \mathit{val}(c_{\notni v_Q})$, and (2) $v_Q \notin \mathit{val}(c_{\notni v_Q})$.
\end{compactitem}
The lemma holds as its statement is true in both possible cases.
\end{proof}

\iffalse
\begin{lemma} \label{lemma:q_in_c}
$Q \in \processes{c_{\notni v_Q}}$.
\end{lemma}
\begin{proof}
By contradiction, let $Q \notin \processes{c_{\notni v_Q}}$.
We fix any infinite canonical execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}) = c_{\notni v_Q}$.
Observe that $Q$ takes no computational steps in $\mathcal{E}$.
% as $Q \notin \processes{c}$.
As $v_Q \notin \mathit{val}(c_{\notni v_Q})$, $\mathcal{E}$ is infinite and $\mathcal{A}$ satisfies \emph{Termination} and $\mathit{val}$, some value $v' \neq v_Q$ is decided in $\mathcal{E}$.
Let $t_c$ denote the time at which a correct process decides $v'$ in $\mathcal{E}$.
Moreover, let $t_Q$ denote the time at which $Q$ decides $v_Q$ in $\beta_Q$ (see \Cref{lemma:behavior_without_receptions}).

We now construct another execution $\mathcal{E}'$ such that $\mathcal{E}' \in \mathit{execs}(\mathcal{A})$ is identical to $\mathcal{E}$, except that:
\begin{compactenum}
    \item Process $Q$ is correct in $\mathcal{E}'$.
    
    \item All messages sent by and to $Q$ are delayed until after $\max(t_c, t_Q)$.
    
    \item Process $Q$ exhibits the behavior $\beta_Q$ (see \Cref{lemma:behavior_without_receptions}).
    
    \item Until $\max(t_c, t_Q)$, no process in $\processes{c}$ can distinguish $\mathcal{E}'$ from $\mathcal{E}$.
    % in which (1) it receives no messages by other processes (until some time as in-flight messages must eventually be received by $Q$), and (2) $Q$ decides $v_Q$.
    % Such a behavior of the process $Q$ exists due to \Cref{lemma:behavior_without_receptions}.
    
    % \item All messages sent by and to $Q$ are delayed until $Q$ decides $v_Q$ and some other correct process decides $v' \neq v_Q$.
    
    \item GST is set to after $\max(t_c, t_Q)$.
    % $Q$ decides $v_Q$ and some other correct process decides $v'$.
\end{compactenum}
As no process in $\processes{c_{\notni v_Q}}$ can distinguish $\mathcal{E}'$ from $\mathcal{E}$ until $\max(t_c, t_Q)$, $v' \neq v_Q$ is decided by a correct process in $\mathcal{E}'$.
Moreover, $Q$ decides $v_Q$ in $\mathcal{E}'$ (due to the step 3).
% As messages from $Q$ are delayed in $\mathcal{E}'$, all other correct processes cannot distinguish $\mathcal{E}'$ from $\mathcal{E}_c$ (until some time); hence, all other correct processes decide $v' \neq v_Q$ in $\mathcal{E}'$.
Therefore, there is a disagreement in $\mathcal{E}'$, which contradicts the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Thus, $Q \in \processes{c_{\notni v_Q}}$.
\end{proof}

The previous lemma shows that $Q \in \processes{c_{\notni v_Q}}$; recall that $v_Q \notin \mathit{val}(c_{\notni v_Q})$.
Let us construct an input configuration $c_{\notni Q} \in \mathcal{I}$ such that $Q \notin \processes{c_{\notni Q}}$:
\begin{compactenum}
    \item Let $c_{\notni Q} \gets c_{\notni v_Q}$.

    \item We remove $(Q, \cdot)$ from $c_{\notni Q}$.
    That is, we remove $Q$'s process-proposal pair from $c_{\notni Q}$.

    \item If $|\processes{c_{\notni v_Q}}| = n - t$, we add $(Z, \text{any value})$ to $c_{\notni Q}$, where $Z$ is any process such that $Z \notin \processes{c_{\notni v_Q}}$; note that such a process $Z$ exists as $t > 0$.
\end{compactenum}
Due to the construction of $c_{\notni Q}$, $c_{\notni Q} \sim c_{\notni v_Q}$.
Indeed, (1) $\processes{c_{\notni Q}} \cap \processes{c_{\notni v_Q}} \neq \emptyset$ (as $n - t - 1 > 0$ when $n > 3t$ and $t > 0$), and (2) for every process $P \in \processes{c_{\notni Q}} \cap \processes{c_{\notni v_Q}}$, the proposal of $P$ is identical in $c_{\notni Q}$ and $c_{\notni v_Q}$ (by the step 1 of the construction).

The lemma below shows that there exists a canonical execution $\mathcal{E}_{c_{\notni Q}}$ such that (1) $\mathcal{E}_{c_{\notni Q}}$ corresponds to $c_{\notni Q}$, and (2) some value $v \neq v_Q$ is decided in $\mathcal{E}_{c_{\notni Q}}$.

\begin{lemma} \label{lemma:another_execution}
There exists a canonical execution $\mathcal{E}_{c_{\notni Q}} \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_{c_{\notni Q}}) = c_{\notni Q}$, and (2) a value $v \neq v_Q$ is decided by a correct process in $\mathcal{E}_{c_{\notni Q}}$.
\end{lemma}
\begin{proof}
We fix any infinite canonical execution $\mathcal{E}_{c_{\notni Q}} \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}_{c_{\notni Q}}) = c_{\notni Q}$.
As $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{c_{\notni Q}}$ is infinite, some value $v \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_{c_{\notni Q}}$.
As $c_{\notni Q} \sim c_{\notni v_Q}$, $v \in \mathit{val}(c_{\notni v_Q})$ (by \Cref{lemma:helper_main}).
Finally, $v \neq v_Q$ as (1) $v \in \mathit{val}(c_{\notni v_Q})$, and (2) $v_Q \notin \mathit{val}(c_{\notni v_Q})$.
% , which concludes the proof.
% Thus, xthe lemma.
\end{proof}
\fi

As we have shown the existence of $\mathcal{E}_{v}$ (\Cref{lemma:conflicting_execution}), we can ``merge'' $\mathcal{E}_{v}$ with the valid local behavior $\beta_Q$ in which $Q$ decides $v_Q$ without having received any message (\Cref{lemma:behavior_without_receptions}).
Hence, we can construct an execution in which $\mathcal{A}$ violates \emph{Agreement}.
%, which represents a contradiction with the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Thus, correct processes must send more than $(\lceil \frac{t}{2} \rceil)^2 \in \Omega(t^2)$ messages in $\mathcal{E}_{\mathit{base}}$.
% , which implies an $\Omega(t^2)$ message complexity of $\mathcal{A}$.
% The formal proof of the following lemma, from which the lower bound on message complexity (\Cref{theorem:lower_bound_main}) follows directly, is given in \Cref{section:lower_bound_appendix}.

\begin{lemma} \label{lemma:final_lemma_lower_bound}
The message complexity of $\mathcal{E}_{\mathit{base}}$ is greater than $(\lceil \frac{t}{2} \rceil)^2$.
\end{lemma}
\begin{proof}
By \Cref{lemma:behavior_without_receptions}, there exists a local behavior $\beta_Q$ of process $Q$ in which $Q$ decides a value $v_Q$ without having received any message (from any other process).
Let $t_Q$ denote the time at which $Q$ decides $v_Q$ in $\beta_Q$.
Moreover, there exists an infinite execution $\mathcal{E}_{v}$ in which (1) $Q$ is faulty and silent, and (2) correct processes decide a value $v \neq v_Q$ (by \Cref{lemma:conflicting_execution}).
Let $t_{v}$ denote the time at which a correct process decides $v \neq v_Q$ in $\mathcal{E}_{v}$.

We now construct an execution $\mathcal{E}$ in the following way:
\begin{compactenum}
    \item Processes in $\mathit{Corr}_{\mathcal{A}}(\mathcal{E}_{v}) \cup \{Q\}$ are correct in $\mathcal{E}$.
    All other processes are faulty.
    
    \item All messages from and to $Q$ are delayed until after $\max(t_Q, t_{v})$.
    
    \item Process $Q$ exhibits the local behavior $\beta_Q$.
    
    \item Until $\max(t_Q, t_{v})$, no process in $\mathit{Corr}_{\mathcal{A}}(\mathcal{E}_{v})$ can distinguish $\mathcal{E}$ from $\mathcal{E}_{v}$.
    
    \item GST is set to after $\max(t_Q, t_{v})$ (and after all correct processes from the $\mathit{Corr}_{\mathcal{A}}(\mathcal{E}_v) \cup \{Q\}$ set have taken a computational step).
\end{compactenum}
As no process in $\mathit{Corr}_{\mathcal{A}}(\mathcal{E}_{v})$ can distinguish $\mathcal{E}$ from $\mathcal{E}_{v}$ until $\max(t_Q, t_{v})$, $v \neq v_Q$ is decided by a correct process in $\mathcal{E}$.
Moreover, $Q$ decides $v_Q$ in $\mathcal{E}$ as it exhibits $\beta_Q$ (step 3 of the construction).
Thus, \emph{Agreement} is violated in $\mathcal{E}$, which contradicts the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Hence, the starting assumption is not correct: in $\mathcal{E}_{\mathit{base}}$, correct processes send more than $(\lceil \frac{t}{2} \rceil)^2$ messages.
% , which concludes the proof.
% implies that the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
\end{proof}

The following subsection shows that the quadratic bound on message complexity is tight with $t \in \Omega(n)$: \general exchanges $O(n^2)$ messages by relying on a threshold signature scheme (as all of the previous work on optimal consensus in partial synchrony~\cite{civit2022byzantine,lewis2022quadratic}).
We underline that our lower bound holds even for algorithms which employ threshold signatures.
Achieving the optimal quadratic message complexity without relying on threshold signatures (or any other signature variants) remains an important open question.

% Finally, as each message contains at least one word, \Cref{theorem:lower_bound_main} implies the $\Omega(t^2)$ lower bound on the communication complexity for any consensus algorithm with a non-trivial validity property.

% As \Cref{lemma:final_lemma_lower_bound} proves that the message complexity of $\mathcal{A}$ is $\Omega(t^2)$, the proof of \Cref{theorem:lower_bound_main} is concluded.

% With \Cref{lemma:final_lemma_lower_bound}, the proof of \Cref{theorem:lower_bound_main} is concluded.


% Observe that, as each message contains at least one word, \Cref{theorem:lower_bound_main} implies an $\Omega(t^2)$ lower bound on the communication complexity, as well.

% \newpage
\subsection{General Algorithm \general: Similarity Condition is Sufficient if $n > 3t$} \label{subsection:general_algorithm}

In this subsection, we show that $\mathcal{C}_S$ is sufficient for a validity property to be solvable when $n > 3t$.
Furthermore, we prove that, assuming a threshold signature scheme, the quadratic lower bound (\Cref{subsection:lower_bound}) is tight with $t \in \Omega(n)$.
In brief, we prove the following theorem:

\begin{theorem} \label{theorem:general}
Let $n > 3t$, and let $\mathit{val}$ be any validity property which satisfies $\mathcal{C}_S$.
Then, $\mathit{val}$ is solvable.
Moreover, assuming a threshold signature scheme, there exists an algorithm which solves Byzantine consensus with $\mathit{val}$, and has $O(n^2)$ message complexity.
\end{theorem}

To prove \Cref{theorem:general}, we present \general, an algorithm which solves the Byzantine consensus problem with \emph{any} validity property satisfying $\mathcal{C}_S$, given that $n > 3t$.
In other words, \general solves consensus with any solvable and non-trivial validity property.
Notably, assuming a threshold signature scheme, \general achieves $O(n^2)$ message complexity, making it optimal (when $t \in \Omega(n)$) according to our lower bound.

To construct \general, we rely on vector consensus~\cite{neves2005solving,vaidya2013byzantine,Doudou1998,correia2006consensus} (see \Cref{subsubsection:interactive_consistency}), a problem which requires correct processes to agree on the proposals of $n - t$ processes.
Specifically, when a correct process decides a vector $\mathit{vec}$ of $n - t$ proposals (from vector consensus), it decides (from \general) the common admissible value for all input configurations similar to $\mathit{vec}$, i.e., the process decides $\Lambda(\mathit{vec})$.
Note that the idea of solving consensus from vector consensus is not novel~\cite{Ben-Or94,CGL18,mostefaoui2000binary}.
For some validity properties it is even natural, such as \emph{Strong Validity}  (choose the most common value) or \emph{Weak Validity} (choose any value).
However, thanks to the necessity of $\mathcal{C}_S$ (\Cref{subsection:necessary_condition}), \emph{any} solvable  consensus variant can reuse this simple algorithmic design.

In this subsection, we first recall vector consensus (\Cref{subsubsection:interactive_consistency}).
% , a problem which requires correct processes to agree on the proposals of $n - t$ processes.
Then, we utilize vector consensus to construct \general (\Cref{subsubsection:Complete}).
Throughout the entire subsection, $n > 3t$.

% \newpage
\subsubsection{Vector Consensus.} \label{subsubsection:interactive_consistency}
In essence, vector consensus allows each correct process to infer the proposals of $n - t$ (correct or faulty) processes.
Formally, correct processes agree on input configurations (of vector consensus) with exactly $n - t$ process-proposal pairs: $\mathcal{V}_O = \mathcal{I}_{n - t}$. 
Let us precisely define \emph{Vector Validity}, the validity property of vector consensus:
\begin{compactitem}
     \item \emph{Vector Validity:} Let a correct process decide $\mathit{vector} \in \mathcal{V}_O$, which contains exactly $n - t$ process-proposal pairs, such that (1) $(P, v)$ belongs to $\mathit{vector}$, for some process $P \in \Pi$ and some value $v \in \mathcal{V}_I$, and (2) $P$ is a correct process.
     Then, $P$ proposed $v$ to vector consensus.
\end{compactitem}
Intuitively, \emph{Vector Validity} states that, if a correct process ``concludes'' that a value $v$ was proposed by a process $P$ and $P$ is correct, then $P$'s proposal was indeed $v$.

We provide two implementations of vector consensus: (1) a non-authenticated implementation (without any cryptographic primitives), and (2) an authenticated implementation (with threshold signatures).
% \pierre{I think this claim is controversial. A lot of similar (if not identical) reductions have been proposed  \cite{Ben-Or94} \cite{CGL18}}\manuel{We're just saying we provide implementations, not that we're solving the problem for the first time. We can maybe add a footnote: ``For alternative non-authenticated implementations of vector consensus, see~\cite{Ben-Or94, CGL18}''}\pierre{But can we say what is the difference between our proposal and \cite{CGL18} ?}\jovan{We discussed this already; will remove it.}
We give the pseudocode of the non-authenticated version in \Cref{subsection:nonauthenticated_vector}.
The pseudocode of the authenticated version is presented in \Cref{algorithm:interactive_consistency}.
This version relies on \textsc{Quad}, a Byzantine consensus algorithm recently introduced in~\cite{civit2022byzantine}; we briefly discuss \textsc{Quad} below.

% The pseudocode of \wic is presented in \Cref{algorithm:interactive_consistency}.
% \wic achieves $O(n^2)$ message complexity.
% % The \emph{communication complexity of \wic, the number of bits sent by correct processes, is $O(n^3)$.
% % , and $O(n^3)$ communication complexity.
% We construct \wic by relying on \textsc{Quad}, a Byzantine consensus algorithm introduced by Civit \emph{et al.}~\cite{civit2022byzantine}; we give a brief description of \textsc{Quad} below.


\paragraph{\textsc{Quad}.}
In essence, \textsc{Quad} is a partially-synchronous, ``leader-based'' Byzantine consensus algorithm, which achieves $O(n^2)$ message complexity.
Internally, \textsc{Quad} relies on a threshold signature scheme.
% \textsc{Quad} owes its complexity to its quadratic view synchronization~\cite{lewis2022quadratic, civit2022byzantine,naor2019cogsworth,naor2020expected} algorithm.
Formally, \textsc{Quad} is concerned with two sets: (1) $\mathcal{V}_{\textsc{Quad}}$, a set of values, and (2) $\mathcal{P}_{\textsc{Quad}}$, a set of proofs.
In \textsc{Quad}, processes propose and decide value-proof pairs.
There exists a function $\mathsf{verify}: \mathcal{V}_{\textsc{Quad}} \times \mathcal{P}_{\textsc{Quad}} \to \{ \mathit{true}, \mathit{false} \}$.
Importantly, $\mathcal{P}_{\textsc{Quad}}$ is not known a-priori: it is only assumed that, if a correct process proposes a pair $(v \in \mathcal{V}_{\textsc{Quad}}, \Sigma \in \mathcal{P}_{\textsc{Quad}})$, then $\mathsf{verify}(v, \Sigma) = \mathit{true}$.
\textsc{Quad} guarantees the following: if a correct process decides a pair $(v, \Sigma)$, then $\mathsf{verify}(v, \Sigma) = \mathit{true}$.
In other words, correct processes decide only valid value-proof pairs.
(See~\cite{civit2022byzantine} for full details on \textsc{Quad}.)

% As for the validity property, $\textsc{Quad}$ satisfies \emph{External Validity}:
% \begin{compactitem}
%      \item \emph{External Validity:} If a correct process decides a pair $(v, \Sigma)$, then $\mathsf{verify}(v, \Sigma) = \mathit{true}$.
% \end{compactitem}
% \textsc{Quad} achieves $O(n^2)$ message complexity, which enables the $O(n^2)$ message complexity of \wic, by relying on threshold signatures~\cite{libert2014born}.
% % The \emph{communication complexity}, the number of bits sent in messages by correct processes, of \textsc{Quad} is $O(n^2 \cdot x)$, where $x$ denotes the maximum size of a proof.
% (See the paper~\cite{civit2022byzantine} for more details on \textsc{Quad}.)
% For completeness, we provide a detailed explanation of \textsc{Quad} in \Cref{section:quad_appendix}; 

In our authenticated implementation of vector consensus
(\Cref{algorithm:interactive_consistency}), we rely on a specific instance of \textsc{Quad} where (1) $\mathcal{V}_{\textsc{Quad}} = \mathcal{I}_{n - t}$ (processes propose to \textsc{Quad} the input configurations of vector consensus), and (2) $\mathcal{P}_{\textsc{Quad}}$ is a set of $n - t$ \textsc{proposal} messages (sent by processes in vector consensus).
Finally, given an input configuration $\mathit{vector} \in \mathcal{V}_{\textsc{Quad}}$ and a set of messages $\Sigma \in \mathcal{P}_{\textsc{Quad}}$, $\mathsf{verify}(\mathit{vector}, \Sigma) = \mathit{true}$ if and only if, for every process-proposal pair $(P_j, v_j)$ which belongs to $\mathit{vector}$, $\langle \textsc{proposal}, v_j \rangle_{\sigma_j} \in \Sigma$ (i.e., every process-proposal pair of $\mathit{vector}$ is accompanied by a properly signed \textsc{proposal} message).

\paragraph{Description of authenticated vector consensus (\Cref{algorithm:interactive_consistency}).}
When a correct process $P_i$ proposes a value $v \in \mathcal{V}_I$ to vector consensus (line~\ref{line:propose}), the process broadcasts a signed \textsc{proposal} message (line~\ref{line:broadcast_proposal}).
Once $P_i$ receives $n - t$ \textsc{proposal} messages (line~\ref{line:received_n_t_proposals}), $P_i$ constructs an input configuration $\mathit{vector}$ (line~\ref{line:construct_input_configuration}), and a proof $\Sigma$ (line~\ref{line:construct_proof}) from the received \textsc{proposal} messages.
Moreover, $P_i$ proposes $(\mathit{vector}, \Sigma)$ to \textsc{Quad} (line~\ref{line:propose_quad}).
Finally, when $P_i$ decides a pair $(\mathit{vector}', \Sigma')$ from \textsc{Quad} (line~\ref{line:decide_quad}), $P_i$ decides $\mathit{vector}'$ from vector consensus (line~\ref{line:decide}).

\begin{algorithm}
\caption{Authenticated Vector Consensus: Pseudocode (for process $P_i$)}
\label{algorithm:interactive_consistency}
\footnotesize
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Best-Effort Broadcast~\cite{cachin2011introduction}, \textbf{instance} $\mathit{beb}$ \BlueComment{broadcast with no guarantees if the sender is faulty}
\State \hskip2em \textsc{Quad}~\cite{civit2022byzantine}, \textbf{instance} $\mathit{quad}$

\medskip
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\mathsf{Integer}$ $\mathit{received\_proposals}_i \gets 0$ \BlueComment{the number of received proposals}
\State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathcal{V}_I)$ $\mathit{proposals}_i \gets \text{empty}$ \BlueComment{received proposals}
\State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathsf{Message})$ $\mathit{messages}_i \gets \text{empty}$ \BlueComment{received \textsc{proposal} messages}

\medskip
\State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$: \label{line:propose}
\State \hskip2em \textbf{invoke} $\mathit{beb}.\mathsf{broadcast}\big( \langle \textsc{proposal}, v \rangle_{\sigma_i} \big)$ \BlueComment{broadcast a signed proposal} \label{line:broadcast_proposal}

\medskip
\State \textbf{upon} reception of $\mathsf{Message}$ $m = \langle \textsc{proposal}, v_j \in \mathcal{V}_I \rangle_{\sigma_j}$ from process $P_j$ and $\mathit{received\_proposals}_i < n - t$:
\State \hskip2em $\mathit{received\_proposals}_i \gets \mathit{received\_proposals}_i + 1$
\State \hskip2em $\mathit{proposals}_i[P_j] \gets v_j$
\State \hskip2em $\mathit{messages}_i[P_j] \gets m$

\State \hskip2em \textbf{if} $\mathit{received\_proposals}_i = n - t$: \label{line:received_n_t_proposals} \BlueComment{received $n - t$ proposals; can propose to \textsc{Quad}}
\State \hskip4em $\mathsf{Input\_Configuration}$ $\mathit{vector} \gets $ input configuration constructed from $\mathit{proposals}_i$ \label{line:construct_input_configuration}
\State \hskip4em $\mathsf{Proof}$ $\Sigma \gets $ set of messages containing all \textsc{proposal} messages from $\mathit{messages}_i$ \label{line:construct_proof}
\State \hskip4em \textbf{invoke} $\mathit{quad}.\mathsf{propose}\big( (\mathit{vector}, \Sigma) \big)$ \label{line:propose_quad}

\medskip
\State \textbf{upon} $\mathit{quad}.\mathsf{decide}\big( (\mathsf{Input\_Configuration} \text{ } \mathit{vector}', \mathsf{Proof} \text{ } \Sigma') \big)$: \label{line:decide_quad}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{vector}')$ \label{line:decide}

\end{algorithmic}
\end{algorithm}

%\medskip
The message complexity of \Cref{algorithm:interactive_consistency} is $O(n^2)$ as (1) processes only broadcast \textsc{proposal} messages, and (2) the message complexity of \textsc{Quad} is $O(n^2)$.
We underline that the \emph{communication complexity} of \Cref{algorithm:interactive_consistency}, the number of bits sent by correct processes, is $O(n^3)$ as the communication complexity of \textsc{Quad} is $O(n^2 \cdot x) = O(n^3)$ (see~\cite{civit2022byzantine}), where $x$ is the size of a \textsc{Quad} proposal (in our case, $x \in \Theta(n)$).
% Lastly, the latency of \Cref{algorithm:interactive_consistency}, the time until processes decide (measured from GST), is linear (due to the linear latency of \textsc{Quad}; see~\cite{civit2022byzantine}).
We delegate the full proof of the correctness and complexity of \Cref{algorithm:interactive_consistency} to \Cref{subsection:authenticated_vector_proof}.
% , where we also include a solution to the vector consensus problem in the \emph{non-authenticated} setting (\Cref{algorithm:interactive_consistency} above relies on cryptographic signatures).
%Observe that \wic (\Cref{algorithm:interactive_consistency}) utilizes cryptographic signatures (\textsc{proposal} messages are signed, and \textsc{Quad} uses threshold signatures internally).
%We underline that the Byzantine consensus problem with \emph{Vector Validity} (i.e., vector consensus) can be solved even in a \emph{non-authenticated} setting, although with a higher cost; we provide such an algorithm in \Cref{section:algorithm_appendix}.
% Thus, the solvability of validity properties is \emph{independent} of the assumptions on authentication (as we show in \Cref{subsubsection:Complete}).

% \begin{theorem} [\textsc{Icon} is correct] \label{theorem:icon}
% \textsc{Icon} (\Cref{algorithm:interactive_consistency}) is a Byzantine consensus algorithm with Interactive-Consistency Validity.
% The message complexity of \textsc{Icon} is $O(n^2)$, whereas its communication complexity is $O(n^3)$.
% \end{theorem}
% \begin{proof}
% \emph{Agreement} follows directly from \emph{Agreement} of \textsc{Quad}.
% Moreover, as there are (at least) $n - t$ correct processes, every correct process eventually proposes to \textsc{Quad} (line~\ref{line:propose_quad}).
% Due to \emph{Termination} of \textsc{Quad}, every correct process eventually decides.
% Therefore, \Cref{algorithm:interactive_consistency} satisfies \emph{Termination}.

% It is left to prove that \textsc{Icon} satisfies \emph{Interactive-Consistency Validity}.
% Let $\mathit{vector}' \in \mathcal{I}_{n - t}$ be an input configuration decided by a correct process.
% Due to \emph{External Validity} of \textsc{Quad}, if a process-proposal pair $(P_j, v_j)$ belongs to $\mathit{vector}'$, for some value $v_j \in \mathcal{V}_I$, $P_j$ has sent a properly signed \textsc{proposal} message for $v_j$.
% If $P_j$ is correct, $v_j$ is its proposal as correct processes send \textsc{proposal} messages only for their proposals (line~\ref{line:broadcast_proposal}).
% Thus, \Cref{algorithm:interactive_consistency} satisfies \emph{Interactive-Consistency Validity}.

% The $O(n^2)$ message complexity of \textsc{Icon} follows from the following two facts: (1) correct processes only broadcast \textsc{proposal} messages (line~\ref{line:broadcast_proposal}) before proposing to \textsc{Quad}, and (2) the message complexity of \textsc{Quad} is $O(n^2)$.
% As for the communication complexity of \textsc{Icon}, it is indeed $O(n^3)$ as (1) correct processes only broadcast $O(n^2)$ words (via the \textsc{proposal} messages; line~\ref{line:broadcast_proposal}) before proposing to \textsc{Quad}, and (2) the communication complexity of \textsc{Quad} is $O(n^3)$ (because the maximum size of a proof is $O(n)$ words).
% Thus, the theorem.
% \end{proof}

% Observe that \textsc{Icon} (\Cref{algorithm:interactive_consistency}) utilizes cryptographic signatures (\textsc{proposal} messages are signed).
% We underline that a Byzantine consensus algorithm with \emph{Interactive-Consistency Validity} can be obtained even in a \emph{non-authenticated} setting; we provide such an algorithm in \Cref{section:appendix_non_authenticated}.

\subsubsection{\general.} \label{subsubsection:Complete}
We construct \general (\Cref{algorithm:general}) directly from vector consensus (\Cref{subsubsection:interactive_consistency}).
When a correct process $P_i$ proposes to \general (line~\ref{line:propose_general}), the proposal is forwarded to vector consensus (line~\ref{line:propose_ic}).
Once $P_i$ decides an input configuration $\mathit{vector}$ from vector consensus (line~\ref{line:decide_ic}), $P_i$ decides $\Lambda(\mathit{vector})$ (line~\ref{line:decide_general}).

Note that our implementation of \general (\Cref{algorithm:general}) is independent of the actual implementation of vector consensus.
Thus, by employing our authenticated implementation of vector consensus (\Cref{algorithm:interactive_consistency}), we obtain a general consensus algorithm with $O(n^2)$ message complexity.
% : both authenticated and non-authenticated vector consensus implementations can be used in \Cref{algorithm:general}.
On the other hand, by employing a non-authenticated implementation of vector consensus (see \Cref{subsection:nonauthenticated_vector}), we obtain a non-authenticated version of \general, which implies that any validity property which satisfies $\mathcal{C}_S$ is solvable even in a non-authenticated setting (if $n > 3t$).

\begin{algorithm} [ht]
\caption{\general: Pseudocode for process $P_i$}
\label{algorithm:general}
\footnotesize
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Vector Consensus, \textbf{instance} $\mathit{vec\_cons}$

\medskip
\State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$: \label{line:propose_general}
\State \hskip2em \textbf{invoke} $\mathit{vec\_cons}.\mathsf{propose}(v)$ \label{line:propose_ic}

\medskip
\State \textbf{upon} $\mathit{vec\_cons}.\mathsf{decide}(\mathsf{Input\_Configuration} \text{ } \mathit{vector})$: \label{line:decide_ic}
\State \hskip2em \textbf{trigger} $\mathsf{decide}\big( \Lambda(\mathit{vector}) \big)$ \label{line:decide_general}
\end{algorithmic}
\end{algorithm}

% Magical vspace
% \vspace{-5pt}

Finally, we show that \general (\Cref{algorithm:general}) is a general Byzantine consensus algorithm and that its authenticated variant achieves $O(n^2)$ message complexity, which proves \Cref{theorem:general}.

\begin{lemma} \label{theorem:general_algorithm}
Let $\mathit{val}$ be any validity property which satisfies $\mathcal{C}_S$, and let $n > 3t$.
\general solves Byzantine consensus with $\mathit{val}$.
Moreover, if \general employs \Cref{algorithm:interactive_consistency} as its vector consensus building block, the message complexity of \general is $O(n^2)$.
% , whereas its communication complexity is $O(n^3)$.
% , whereas its communication complexity is $O(n^3)$.
\end{lemma}
\begin{proof}
\emph{Termination} and \emph{Agreement} of \general follow from \emph{Termination} and \emph{Agreement} of vector consensus, respectively.
Moreover, the message complexity of \general is identical to the message complexity of its vector consensus building block.

Finally, we prove that \general satisfies $\mathit{val}$.
Consider any execution $\mathcal{E}$ of \general; let $\mathsf{input\_conf}(\mathcal{E}) = c^*$, for some input configuration $c^* \in \mathcal{I}$.
Moreover, let $\mathit{vector} \in \mathcal{I}_{n - t}$ be the input configuration correct processes decide from vector consensus in $\mathcal{E}$ (line~\ref{line:decide_ic}).
As vector consensus satisfies \emph{Vector Validity}, we have that, for every process $P \in \processes{c^*} \cap \processes{\mathit{vector}}$, $P$'s proposals in $c^*$ and $\mathit{vector}$ are identical.
Hence, $\mathit{vector} \sim c^*$.
Therefore, $\Lambda(\mathit{vector}) \in \mathit{val}(c^*)$ (by the definition of the $\Lambda$ function).
Thus, $\mathit{val}$ is satisfied by \general.
\end{proof}

As \general (\Cref{algorithm:general}) solves the Byzantine consensus problem with any validity property which satisfies $\mathcal{C}_S$ (\Cref{theorem:general_algorithm}) if $n > 3t$, $\mathcal{C}_S$ is sufficient for solvable validity properties when $n > 3t$.
Lastly, as \general relies on vector consensus, we conclude that \emph{Vector Validity} is a \emph{strongest} validity property.
That is, a consensus solution to any solvable variant of the validity property can be obtained (with no additional cost) from vector consensus.

\paragraph{A note on the communication complexity of vector consensus.}
While the version of \general which employs \Cref{algorithm:interactive_consistency} (as its vector consensus building block) has optimal message complexity, its communication complexity is $O(n^3)$.
% (measured as total bits sent by all correct processes from GST to infinity).
This presents a linear gap to the lower bound for communication complexity (also $\Omega(n^2)$, implied by \Cref{theorem:lower_bound_main}), and to known optimal solutions for some validity properties (e.g., \emph{Strong Validity}, proven to be $\Theta(n^2)$ \cite{civit2022byzantine,lewis2022quadratic}).
At first glance, this seems like an issue inherent to vector consensus: the decided vectors are linear in size, suggesting that the linear gap could be inevitable.
However, this is not the case.
In~\Cref{subsection:better_communication}, we give a vector consensus algorithm with $O(n^2\log n)$ communication complexity, albeit with exponential latency.\footnote{Both our authenticated (\Cref{algorithm:interactive_consistency}) and our non-authenticated (see \Cref{subsection:nonauthenticated_vector}) variants of vector consensus have linear latency, which implies linear latency of \general when employing any of these two algorithms.}
Is it possible to construct vector consensus with subcubic communication and polynomial latency?
This is an important open question, as positive answers would lead to (practical) performance improvements of all consensus variants.

==> sections/model_preliminaries.tex <==
% \newpage
\section{Preliminaries} \label{section:preliminaries}

In this section, we present the computational model (\Cref{subsection:computational_model_main}), recall the  consensus problem (\Cref{subsection:byzantine_consensus}), formally define validity properties (\Cref{subsection:specifying_validity}), and introduce canonical similarity (\Cref{subsection:similarity}).

\subsection{Computational Model} \label{subsection:computational_model_main}

\paragraph{Processes.}
We consider a system $\allprocesses = \{P_1, P_2, ..., P_n\}$ of $n$ processes; each process is a deterministic state machine.
% Each process is polynomially-bounded.
% \add{For simplicity, we consider a \emph{static adversary} which corrupts up to $t$ ($0 < t < n$) processes before the start of the algorithm; these processes are \emph{faulty}, and can exhibit arbitrary behavior.\footnote{Note that all negative results proven against a static adversary extend to an adaptive one, which can corrupt processes at any point. Moreover, \Cref{section:algorithm_appendix} proves that \general (our positive result) is resilient to an adaptive adversary.}}
At most $t$ ($0 < t < n$) processes can be \emph{faulty}: those processes can exhibit arbitrary behavior.
A non-faulty process is said to be \emph{correct}.
Processes communicate by exchanging messages over an authenticated point-to-point network.
The communication network is \emph{reliable}: if a correct process sends a message to a correct process, the message is eventually received.
Each process has its own local clock, and no process can take infinitely many computational steps in finite time.
% Finally, we assume that local steps of processes take zero time, as the time needed for local computation is negligible in comparison with message delays. 

\paragraph{Executions.}
Given an algorithm $\mathcal{A}$, $\mathit{execs}(\mathcal{A})$ denotes the set of all executions of $\mathcal{A}$.
Furthermore, $\mathit{Corr}_{\mathcal{A}}(\mathcal{E})$ denotes the set of correct processes in an execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$.
We say that an execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ is \emph{canonical} if and only if no faulty process takes any computational step in $\mathcal{E}$; note that faulty processes do not send any message in a canonical execution.

\paragraph{Partial synchrony.}
We consider the standard partially synchronous model~\cite{DLS88}. 
For every execution of the system, there exists a Global Stabilization Time (GST) and a positive duration $\delta$ such that message delays are bounded by $\delta$ after GST.
GST is not known to the processes, whereas $\delta$ is.
We assume that all correct processes start executing their local algorithm before or at GST.
Local clocks may drift arbitrarily before GST, but do not drift thereafter.

We remark that (almost) all results presented in the paper hold even if $\delta$ is unknown.
The only result that is not preserved is the message complexity of \general: if $\delta$ is unknown, \general may send arbitrarily many messages after GST (while processes are trying to estimate the message delays).
In fact, this subtle point is the main reason we consider the standard model in which $\delta$ is known since it provides a fair chance of designing \general with a quadratic number of exchanged messages, as is done in other consensus algorithms geared towards low complexity~\cite{civit2022byzantine,lewis2022quadratic,yin2019hotstuff}.

\paragraph{Cryptographic primitives.}
In one variant of the \general algorithm, we assume a $(k, n)$-threshold signature scheme~\cite{libert2014born} (see \Cref{subsection:general_algorithm}).
In fact, this variant relies on a closed-box consensus algorithm which internally utilizes threshold signatures.
In a threshold signature scheme, each process holds a distinct private key, and there exists a single public key.
Each process $P_i$ can use its private key to produce a (partial) signature of a message $m$; we denote by $\langle m \rangle_{\sigma_i}$ a message $m$ (partially) signed by the process $P_i$.
Moreover, a signature can be verified by other processes.
Finally, a set of signatures for a message $m$ from $k$ (the threshold) distinct processes can be combined into a single threshold signature for $m$, which proves that $k$ processes have signed $m$.
% , which proves that $k$ processes have signed the message.


% by invoking $\mathit{ShareSign}_i(m)$.
% A partial signature $\mathit{tsignature}$ of a message $m$ produced by a process $P_i$ can be verified by $\mathit{ShareVerify}_i(m, \mathit{tsignature})$.
% Finally, set $S = \{\mathit{tsignature}_i\}$ of partial signatures, where $|S| = k$ and, for each $\mathit{tsignature}_i \in S$, $\mathit{tsignature}_i = \mathit{ShareSign}_i(m)$, can be combined into a \emph{single} (threshold) signature by invoking $\mathit{Combine}(S)$; a combined signature $\mathit{tcombined}$ of message $m$ can be verified by $\mathit{CombinedVerify}(m, \mathit{tcombined})$.
% Where appropriate, invocations of $\mathit{ShareVerify}(\cdot)$ and $\mathit{CombinedVerify}(\cdot)$ are implicit in our descriptions of protocols.


% For \general, our general algorithm with $O(n^2)$ message complexity, we assume an idealized \emph{public-key infrastructure} (PKI): each process is associated with its public/private key pair which is used to (1) sign messages, and (2) verify signatures of other processes.
% The adversary is computationally bounded, i.e., faulty processes cannot forge signatures of correct processes.
% We denote by $\langle m \rangle_{\sigma_i}$ a message $m$ which is properly signed by the process $P_i$.
% Moreover, \general utilizes, as a closed-box, an algorithm which internally relies on a threshold signature scheme~\cite{libert2014born} (see \Cref{subsection:general_algorithm}).
% We emphasize that 
% Add a comment about threshold signatures

% \paragraph{Message \& communication complexities.}
% A \emph{word} contains a constant number of signatures and values.
% Each message contains at least a single word.
% Let $\mathcal{A}$ be any algorithm and let $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ be any execution of $\mathcal{A}$.
% The message complexity of $\mathcal{E}$ is the number of messages sent by correct processes during $[\text{GST}, \infty]$.
% The communication complexity of $\mathcal{E}$ is the number of words sent in messages by correct processes during $[\text{GST}, \infty]$.

% The \emph{message complexity} of $\mathcal{A}$ is defined as
% \begin{equation*}
%     \max_{\mathcal{E} \in \mathit{execs}(\mathcal{A})}\bigg\{\text{message complexity of } \mathcal{E} \bigg\}.
% \end{equation*}

% The \emph{communication complexity} of $\mathcal{A}$ is defined as
% \begin{equation*}
%     \max_{\mathcal{E} \in \mathit{execs}(\mathcal{A})}\bigg\{\text{communication complexity of } \mathcal{E} \bigg\}.
% \end{equation*}

\paragraph{Message complexity.}
% A \emph{word} contains a constant number of signatures and values.
% Each message contains at least a single word.
Let $\mathcal{A}$ be any algorithm and let $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ be any execution of $\mathcal{A}$.
The message complexity of $\mathcal{E}$ is the number of messages sent by correct processes during $[\text{GST}, \infty)$.
% The communication complexity of $\mathcal{E}$ is the number of words sent in messages by correct processes during $[\text{GST}, \infty]$.

The \emph{message complexity} of $\mathcal{A}$ is defined as
\begin{equation*}
    \max_{\mathcal{E} \in \mathit{execs}(\mathcal{A})}\bigg\{\text{message complexity of } \mathcal{E} \bigg\}.
\end{equation*}

% The \emph{communication complexity} of $\mathcal{A}$ is defined as
% \begin{equation*}
%     \max_{\mathcal{E} \in \mathit{execs}(\mathcal{A})}\bigg\{\text{communication complexity of } \mathcal{E} \bigg\}.
% \end{equation*}

\subsection{Consensus} \label{subsection:byzantine_consensus}

% In the Byzantine consensus problem, all processes start with their proposal and aim to agree on a common value despite Byzantine failures.
We denote by $\mathcal{V}_I$ the (potentially infinite) set of values processes can propose, and by $\mathcal{V}_O$ the (potentially infinite) set of values processes can decide.
% We underline that $\mathcal{V}_I$ might not be in
% Sometimes, we refer to $\mathcal{V}_I$ (resp., $\mathcal{V}_O$) as input (resp., output) space.
% We assume that $\mathcal{V}_I$ and $\mathcal{V}_O$ are known to all processes.
% \footnote{Our extended formalism, which can be found in \Cref{section:extended_formalim_appendix}, removes this assumption, thus making itself more expressive.}
The consensus\footnote{Throughout the paper, we use ``consensus'' and ``Byzantine consensus'' interchangeably.} problem exposes the following interface:
\begin{compactitem}
    \item \textbf{request} $\mathsf{propose}(v \in \mathcal{V}_I)$: a process proposes a value $v$.
    
    \item \textbf{indication} $\mathsf{decide}(v' \in \mathcal{V}_O)$: a process decides a value $v'$.
\end{compactitem}
A correct process proposes exactly once, and it decides at most once.
Consensus requires the following properties:
\begin{compactitem}
    \item \emph{Termination:} Every correct process eventually decides.
    
    \item \emph{Agreement:} No two correct processes decide different values.
\end{compactitem}
If the  consensus problem was completely defined by \emph{Termination} and \emph{Agreement}, a trivial solution would exist: processes decide on a default value.
Therefore, the specification of consensus additionally includes a validity property, which connects the proposals of correct processes to admissible decisions, precluding the aforementioned trivial solutions.

\subsection{Validity} \label{subsection:specifying_validity}
In a nutshell, our specification of a validity property includes a set of assignments of proposals to correct processes, and, for each such assignment, a corresponding set of admissible decisions.
% We provide a formal definition of a validity property below.

% \paragraph{Input configurations.}
We start by defining a \emph{process-proposal} pair as a pair $(P, v)$, where (1) $P \in \allprocesses$ is a process, and (2) $v \in \mathcal{V}_I$ is a proposal.
Given a process-proposal pair $\mathit{pp} = (P, v)$, $\mathsf{proposal}(\mathit{pp}) = v$ denotes the proposal associated with $\mathit{pp}$.
% $\process{\mathit{pp}} = P$ denotes the process associated with $\mathit{pp}$, and $\mathsf{proposal}(\mathit{pp}) = v$ denotes the proposal associated with $\mathit{pp}$.

An \emph{input configuration} is a tuple $\big[ \mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_x \big]$ of $x$ process-proposal pairs, where (1) $n - t \leq x \leq n$, and (2) every process-proposal pair is associated with a distinct process.
Intuitively, an input configuration represents an assignment of proposals to correct processes.
For example, an input configuration $\big[ (P_1, v), (P_2, v), (P_3, v), (P_4, v), (P_5, v) \big]$ describes an execution in which (1) only processes $P_1$, $P_2$, $P_3$, $P_4$ and $P_5$ are correct, and (2) all of them propose the same value $v$.

We denote by $\mathcal{I}$ the set of all input configurations.
Furthermore, for every $x \in [n - t, n]$, $\mathcal{I}_x \subset \mathcal{I}$ denotes the set of input configurations with \emph{exactly} $x$ process-proposal pairs.
For every input configuration $c \in \mathcal{I}$, we denote by $c[i]$ the process-proposal pair associated with process $P_i$; if such a process-proposal pair does not exist, $c[i] = \bot$.
Lastly, $\process{c} = \{ P_i \in \Pi \,|\, c[i] \neq \bot\}$ denotes the set of all processes included in $c$.

% \medskip
Given (1) an execution $\mathcal{E}$ of an algorithm $\mathcal{A}$, where $\mathcal{A}$ exposes the $\mathsf{propose}(\cdot)/\mathsf{decide}(\cdot)$ interface, and (2) an input configuration $c \in \mathcal{I}$, we say that $\mathcal{E}$ \emph{corresponds} to $c$ ($\mathsf{input\_conf}(\mathcal{E}) = c$) if and only if (1) $\process{c} = \mathit{Corr}_{\mathcal{A}}(\mathcal{E})$, and (2) for every process $P_i \in \processes{c}$, $P_i$'s proposal in $\mathcal{E}$ is $\mathsf{proposal}(c[i])$.
% We denote by \add{$\mathsf{input\_conf}(\mathcal{E}) = c$} the input configuration to which $\mathcal{E}$ corresponds.

Finally, we define a validity property $\mathit{val}$ as a function $\mathit{val}: \allconfigurations \to 2^{\mathcal{V}_O}$ such that, for every input configuration $c \in \allconfigurations$, $\mathit{val}(\mathit{c}) \neq \emptyset$.
An algorithm $\mathcal{A}$, where $\mathcal{A}$ exposes the $\mathsf{propose}(\cdot)/\mathsf{decide}(\cdot)$ interface, \emph{satisfies} a validity property $\mathit{val}$ if and only if, in any execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$, no correct process decides a value $v' \notin \mathit{val}\big( \mathsf{input\_conf}(\mathcal{E}) \big)$.
% if a correct process decides a value $v' \in \mathcal{V}_O$, then $v' \in \mathit{val}(\mathsf{input\_conf}(\mathcal{E}))$.
That is, an algorithm satisfies a validity property if and only if correct processes decide only admissible values.

\paragraph{Traditional properties in our formalism.}
% Let us take a look at two well-established validity properties, and how they can be expressed using the formalism above.
% \begin{compactitem}
%     \item \emph{Weak Validity}~\cite{milosevic2009unifying,lynch1996distributed,lamport1983weak}: If all processes are correct and propose the same value, only that value can be decided.
%     \item \emph{Strong Validity}~\cite{CGL18,civit2022byzantine,Momose2021,lamport2019byzantine}: If all correct processes propose the same value, only that value can be decided.
% \end{compactitem}
% Note that, 
To illustrate the expressiveness of our formalism, we describe how it can be used for \emph{Strong Validity}, \emph{Weak Validity} and \emph{Correct-Proposal Validity}.
For all of them, $\mathcal{V}_I = \mathcal{V}_O$.
\emph{Weak Validity} can be expressed as
\[
    \mathit{val}(c) =\begin{cases}
            \{v\}, & \text{if } (\processes{c} = \allprocesses) \land (\forall P_i \in \processes{c}: \mathsf{proposal}(c[i]) = v) \\
            \mathcal{V}_O, & \text{otherwise,}
    \end{cases}
\]

whereas \emph{Strong Validity} can be expressed as
\[
    \mathit{val}(c) =\begin{cases}
            \{v\}, & \text{if } \forall P_i \in \processes{c}: \mathsf{proposal}(c[i]) = v \\
            \mathcal{V}_O, & \text{otherwise.}
    \end{cases}
\]
Finally, \emph{Correct-Proposal Validity} can be expressed as
\[
    \mathit{val}(c) = \{v \,|\, \exists P_i \in \processes{c}: \mathsf{proposal}(c[i]) = v\}\text{.}
\]

% It is interesting to note how the difference between these two properties (and their relative ``strength'') is evident when expressed this way.
% The set of configurations for which \emph{Strong Validity} allows any value ($\mathcal{V}$) is strictly less than for \emph{Weak Validity}, as it lacks the $\processes{c} = \allprocesses$ term in the first case.

\paragraph{Consensus algorithms.}
An algorithm $\mathcal{A}$ solves consensus with a validity property $\mathit{val}$ if and only if the following holds:
\begin{compactitem}
    \item $\mathcal{A}$ exposes the $\mathsf{propose}(\cdot)/\mathsf{decide}(\cdot)$ interface, and
    
    \item $\mathcal{A}$ satisfies \emph{Termination}, \emph{Agreement} and $\mathit{val}$.
\end{compactitem}

Lastly, we formally define the notion of a solvable validity property.
% solvable validity properties.

\begin{definition} [Solvable validity property]
We say that a validity property $\mathit{val}$ is \emph{solvable} if and only if there exists an algorithm which solves  consensus 
with $\mathit{val}$.
\end{definition} 

\input{sections/similarity_lemma}

==> sections/probabilistic_extension.tex <==
\clearpage

\section{The hurdle in extending the reasoning to randomized protocols}

The extension of the quadratic lower bounds à la Dolev-Reischuk, which were initially conceived for deterministic protocols, to encompass randomized protocols against an adaptive adversary capable of after-the-fact message removal (called strongly adaptive adversary), as seen in Byzantine Broadcast \cite{Abraham2019c,Abraham2023revisited} and Crusader Broadcast \cite{AbrahamStern22}, might seem immediate. 

In the randomized protocol context, the discourse shifts from specific executions to the concept of \emph{worlds}. A world is formally defined as a pair $(Adv, X)$, where $Adv$ represents an adversarial strategy, inclusive of the input choices for honest processes, and $X$ is an event (a.k.a. fact or predicate), technically a binary random variable over executions. Thus, a world corresponds to a probabilistic measure over executions, defined by the adversarial strategy and the randomized protocol, given the realization of an event $X$. For instance, a world $W_0$ (resp. $W_1$) may denote the probability distribution over executions under an adversary that assigns the input $0$ (resp. $1$), on the condition that a predetermined process receives fewer than $t$ messages from so-for-honest processes. Conceptually, a world can be regarded as a 'randomized' execution or, alternatively, as a probability distribution over executions with certain shared characteristics.

A quadratic lower bound  à la Dolev-Reischuk is based on the observation that unless $\Omega(t^2)$ messages are
exchanged, there necessarily exists an execution $\mathcal{E}_0$ (resp., $\mathcal{E}_1$) in which a correct process $p$ (resp.,
$q \neq p$) decides 0 (resp., 1) without receiving any message (by some application of the pigeonhole). Importantly, the existence of executions $\mathcal{E}_0$ and $\mathcal{E}_1$ follows directly from the (non-weak) validity property.
To conclude the, it then suffices to “merge” $\mathcal{E}_0$ and $\mathcal{E}_1$, thus creating an execution that violates Agreement as $p$ and $q$ disagree, which proves that no correct algorithm with $o(t^2)$ exchanged messages exists.

In the probabilistic framework, the adversary cannot deterministically anticipate which processes may become isolated. Nevertheless, the adversary can wager with a probability of success approaching certainty ($1-O(1)$). In such scenarios, within the constructs of worlds $W_0$ and $W_1$—analogous to the deterministic executions $\mathcal{E}_0$ and $\mathcal{E}_1$—the adversary uniformly selects processes $p$ and $q$ at random, hoping that they receive an insufficient number of messages in $W_0$ and $W_1$, respectively. A straightforward Markov inequality demonstrates that for protocols with a message complexity below $o(t^2)$, this event occurs with a probability of $1-O(1)$. Subsequently, in each round, if a process attempts to communicate with $p$ (or $q$), the adversary intervenes, corrupting the process and eliminating the message sent, exploiting the critical capability of after-the-fact message removal. This strategy allows the adversary to execute the attack with a probability that is arbitrarily close to one, mirroring the structure of the deterministic proof.

However, as previously indicated, there are no pairs of conflicting executions $\mathcal{E}_0$ and $\mathcal{E}_1$, or equivalently, conflicting worlds $W_0$ and $W_1$. This necessitates a comprehensive extension of the proof's aspects. With reference to \Cref{lemma:lower_bound_helper}, this part of the proof is complete, but what about the remaining part ?

The proof frequently manipulates scenarios where a subset of processes becomes isolated from a certain round $k$ onwards, while the remainder agree on a particular bit $b$. One might presume that this bit $b$ is determined in a quasi-deterministic fashion; otherwise, an isolated process attempting to deduce $b$ faces a constant probability of error. Yet, the reality is more subtle. The determination of bit $b$ must be quasi-deterministic, contingent upon the events leading up to round $k$. In other words, for each adversary strategy $Adv$, there should be a partitioning of the executions of exactly $k$ rounds, denoted as $(E^0_{k}, E^1_{k})$, where the probability, as dictated by $Adv$, of agreeing on $1$ (resp. $0$) given the continuation of an execution in $E^0_{k}$ (resp. $E^1_{k}$) is approximately $1$. We would write $\mathbb{P}r_{\mathsf{Adv}}(\text{agreeing on } b \; | \; \mathsf{Cone}(E_b^k)) = 1-O(1)$. However, this does not address the probability of the executions extending from either $E^0_{k}$ or $E^1_{k}$, i.e. $\mathbb{P}r_{\mathsf{Adv}}(\mathsf{Cone}(E_b^k))$ is not restricted a priori.

The original proof strategy encounters a significant obstacle when we consider the probabilistic nature of the argument. Specifically, \Cref{lemma:R} loses its applicability. This is because the probability associated with an adversary strategy $Adv_0^{B(k)}$, which assigns the input $0$ to all and isolates a set of processes $B$ from round $k$ onwards, must see the probability of the set $E^0_{k}$ transition from $0$ to $1$ when $k$ goes from $1$ to $k^{*}_0$ (a round where decision must occur with overwhelming probability in a failure-free world where each process receives $0$ as input). Unlike the deterministic scenario, this transition may occur gradually (see \Cref{figure:proba_extension}). Consequently, the precise methodology of the original proof does not hold in probabilistic version.
Let us note that all the probabilistic measures mentioned in the progressive shift are different since they are defined by different adversaries of the form $\mathsf{Adv}_0^{B(k)}$ Nevertheless, the events occurring up to round $k$ are not influenced by what will be done by the adversary after round $k$, formally: $\mathbb{P}r_{\mathsf{Adv}_0^{B(k_1)}}(\mathsf{Cone}(E_b^k)) = \mathbb{P}r_{\mathsf{Adv}_0^{B(k_2)}}(\mathsf{Cone}(E_b^k)))$ if $k \leq \mathit{min}(k_1,k_2)$.

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/proba/probabilistic_lower_bound.eps}
\caption{The hurdle in extending the reasoning to randomized protocols. \newline$\mathsf{Cone}(\mathcal{E}) \triangleq \{\mathcal{E}' | \mathcal{E} \text{ is a prefix of } \mathcal{E}'\} $, and $\mathsf{Cone}(E) \triangleq \bigcup_{\mathcal{E} \in \mathcal{E}} \mathsf{Cone}(\mathcal{E})$}
\label{figure:proba_extension}
\end{figure}





\iffalse








In the extended version of this argument for randomized protocols facing a strongly adaptive adversary, the adversary cannot know in advance who are the processes that are susceptible to be isolated. However, he can bet with arbitrarily high probability $1-O(1)$. 
That is, in the worlds $W_0$ and $W_1$ (corresponding to the executions $\mathcal{E}_0$ and $\mathcal{E}_1$ in the deterministic case), he will uniformly pick up processes $p$ and $q$, cross the fingers such that they do not receive too many messages in $\mathcal{W}_0$ and $\mathcal{W}_1$ respectively (a simple Markov inequality allows to show it will be the case with probability $1-O(1)$ for protocol with $o(t^2)$ message complexity), and at each round, when a process send a message to $p$ (resp. $q$), the adversary corrupt it and remove its sent message (thanks to the crucial after-the-fact removal capability). Hence, the attack can be performed with arbitrarily high probability, following the exact same structure than for the deterministic proof.

However, as mentioned before, there is no such pair of conflicting executions $\mathcal{E}_0$ and $\mathcal{E}_1$ (resp. conflicting worlds $W_0$ and $W_1$). So we need to extend to all the aspects of the proof. Fair enough, let's do this. So for \Cref{lemma:lower_bound_helper}, we are done.

During the proof, we highly play with executions (res. worlds) where a group of processes is isolated from some round $k$ onward, while the other processes will agree on some common bit $b$. We might think that such a bit should be decided quasi-determinsitically, since otherwise, an isolated process should guess the bit $b$, and will have a constant probability to fail. However, the correct version of this intuition is slightly more subtle than that. The bit $b$ must be decided quasi-determinsitically conditioned to what happen until round $k$ (and this remark makes a big difference). To reformulate, for each adversary $Adv$, there must exist a partition of the executions of size $k$, $(E^0_{k}, E^1_{k})$, such that the probability (defined by $Adv$) to decide $1$ (resp. $0$) conditioned to be in the set of executions prolonging an execution in $E^0_{k}$ (resp. $E^0_{k}$) is approximately $1$. However, nothing is said about the probability to be in the set of executions prolonging an execution in $E^0_{k}$ (resp. $E^1_{k}$)

Now, what happens to the original proof strategy ? Well, \Cref{lemma:R} cannot be applied anymore. Indeed, the probability (for an adversary $Adv_0^{B(k)}$ that gives $0$ as input to everyone and isolate processes in $B$ from some round $k$ onward) of the set  $E^0_{k}$ must evolve from $0$ to $1$, but, conversely of the deterministic case, it can be progressive ! And thus the (exact) original proof collapses.
\fi





==> sections/randomized_version.tex <==

\section{Randomized Version}

In this section, we extend our results to randomized protocols in the presence of a strongly adaptive adversary with after-the-fact removal capabilities.

\subsection{Proof Intuition}

\paragraph*{Randomized Isolation with Arbitrarily High Probability}

Similar to the deterministic result, it is always feasible to isolate certain processes from a linear-sized set $Y'$, with $|Y'| = \Theta(t)$. Here, the probability of such isolation is $1-c$, for any arbitrary constant $c \in \Theta(1)$. The procedure involves uniformly selecting a process $P_u$ in $Y'$, and a specific round $k_u$ for isolation. Post round $k_u$, if a message is received, its sender is (adaptively) corrupted if not already so; the message is subsequently removed (after-the-fact removal) and marked as send-omitted. If the expected message complexity is below $c_e n^2$, it can be demonstrated through a straightforward application of Markov's inequality that the probability of this attack occurring is $1-c_e \cdot c_{\text{attack}}$, where $c_{\text{attack}}$ is a constant. Therefore, reducing $c_e$ suffices to achieve an arbitrarily high probability of success.

\paragraph*{Quasi-deterministic Output Requirement for $1$-isolated $B$ and $C$}

We extend the same indistinguishability argument to demonstrate that in both worlds $W_{1,1,\bar{b}_0}$ and $W_{1,1,\bar{b}_1}$, wherein (i) all processes unanimously propose the same bit $b \in \{0,1\}$, and (ii) $B$ and $C$ are $1$-isolated, the processes in $A$ must agree on the same bit $b'$ quasi-deterministically (i.e., with probability $1-c_g$, where $c_g$ is a suitably low constant). Otherwise, a third scenario $W_{1,1,\bar{b}_2}$ can be constructed, where $B$ and $C$ propose differing bits. Due to indistinguishability, they will yield identical outputs with the same probability as in $W_{1,1,\bar{b}_0}$ and $W_{1,1,\bar{b}_1}$ respectively. Hence, a constant probability exists for a disagreement to arise (the only resolution being a quasi-deterministic agreement on the same bit). Consequently, with a certain probability, $A$ will disagree with either $B$ or $C$. We can further perform an isolation to construct a fourth scenario $\hat{W}_{1,1,\bar{b}_2}$, such that $W_{1,1,\bar{b}_2}$ and $\hat{W}_{1,1,\bar{b}_2}$ are indistinguishable, and a process $P_u$ (isolated) remains correct but disagrees with $A$.

\paragraph*{Isolate a process in a fully-correct world}

Without loss of generality, we assume that the quasi-deterministic bit agreed upon in both worlds $W_{1,1,\bar{b}_0}$ and $W_{1,1,\bar{b}_1}$ is $1$ (a symmetric argument holds otherwise). 
In world $W_{*,*,\bar{b}_0}$, the processes propose $0$, behave correctly and must agree on $0$ quasi-deterministically to satisfy consensus with weak validity. Moreoevr, the termination has to be ensured with good probability by some round $k_0^{*}$. Hence, the same applies to world $W_{k_0^{*},k_0^{*},\bar{b}_0}$, where processes in $B$ and $C$ are $k_0^{*}$-isolated.

We now examine a sequence of scenarios of the form $W_{k, k',\bar{b}_0}$, where $k' \in \{k,k+1\}$, (1) $B$ is $k$-isolated, while $C$ is $k'$-isolated, and (2) every process proposes $0$. 
The sequence must go from a high probability to decide $1$ to a high probability to decide $0$. There are two possibilities:
\begin{itemize}
    \item Sharp Case: there exists an integer $k \in [1,k^{*}-1]$ such that processes decide with high probability $1$ in world $W_{k, k,\bar{b}_0}$ and $0$ in in world $W_{k+1, k+1,\bar{b}_0}$. This case is similar to deterministic case, and we can apply an indistinguishable argument between $W_{k, k,\bar{b}_0}$, $W_{k, k+1,\bar{b}_0}$ and $W_{k+1, k+1,\bar{b}_0}$ to show a contradiction.
    
    \item Smooth Case: With a similar isolation-based argument, we can show that in world $W_{k, k,\bar{b}_0}$, processes must decide an output quasi-deterministically, conditioned to what they observed in $W_{k, k,\bar{b}_0}$, that is, for every $k$, we can partition executions of $k-1$ rounds into 2 subsets $E^{0}_{k,\bar{b}}$ and $E^{1}_{k,\bar{b}}$, where $\prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\text{agreeing on 0} | E^{0}_{k,\bar{b}} ) \simeq 1 $ and $\prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\text{agreeing on 1} | E^{1}_{k,\bar{b}} ) \simeq 1$.
    Crucially, it is a priori possible to have $\prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\mathsf{Cone}(E^{0}_{k,\bar{b}} )) \simeq \prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\mathsf{Cone}(E^{1}_{k,\bar{b}} )) \simeq \frac{1}{2}$. Hence, the probability to \emph{a priori} agree on $0$ (roughly $\prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\mathsf{Cone}(E^{0}_{k,\bar{b}} ))$) can progressively move from $0$ to $1$ while $k$ moves from $1$ to $k^{*}_0$, even if the the probability to agree on a bit $b$ \emph{conditioned to what happened in the first $k-1$ rounds} is close to 1.
\end{itemize}


%We note $Z_{(k+k')} = S_{(k,k')}$.The sequence $Z_2, ..., Z_{2k^{*}}$ will be studied. We will show that in each scenario $Z_q$, processes must output 



\subsection{Model's Extension}

The model is enhanced as follows:

The set of messages is denoted by $ \mathscr{M} $. Let $ \mathcal{M} \subset \mathcal{P}(\mathscr{M}) $ represent the sets of messages that can be sent in a single round by a correct process. The state-transition function $ \mathcal{A} $ now maps each pair $ (s,M^R) \in \mathcal{S} \times \mathcal{P}(\mathscr{M}) $ to a probabilistic measure $ \mathcal{A}(s,M^R) $ on $\mathcal{S} \times \mathcal{M}, \mathscr{F}_{\mathcal{S} \times \mathcal{M}} $, where $\mathscr{F}_{\mathcal{S} \times \mathcal{M}}$ is a sigma-algebra over $\mathcal{S} \times \mathcal{M}$.

The behavior definition remains unchanged, except for condition (\ref{item:deterministic_transition}), which now requires $ \mathcal{A}(s^j,M^{R(j)})(s^{j+1},M^{S(j+1)} \cup M^{SO(j+1)}) > 0 $.

To define a probabilistic measure over executions, the adversary's strategy must be specified to resolve pure non-determinism. To account for after-the-fact removal, we introduce additional terms to the formalism.

A \emph{$ k $-round pseudo-fragment} for some $ k \in \mathbb{N}^{+} $ of process $ P_i $,  is a tuple $ \mathcal{F} = (s,M^S, M^{SO}) $ such that there exists a pair of message sets $ (M^R, M^{RO}) $ where $ \mathcal{F}' = (s,M^S, M^{SO},M^R, M^{RO}) $ is a $ k $-round fragment for $ k $ of process $ P_i $. Here, $ \mathcal{F}' $ is termed a \emph{completion} of $ \mathcal{F} $.

A $ k $-round pseudo-behavior $ \mathcal{B} = (\mathcal{F}^1, \ldots, \mathcal{F}^k) $ is a sequence such that: (i) $ \mathcal{F}^k $ is a pseudo-fragment, and (ii) for any completion $ \mathcal{F}^{\prime k} $ of $ \mathcal{F}^k $, $ \mathcal{B}' = (\mathcal{F}^1, \ldots, \mathcal{F}') $ is a $ k $-round behavior for $ k $ of process $ P_i $. In this context, $ \mathcal{B}' $ is termed a \emph{completion} of $ \mathcal{B} $.

A $ k $-round pseudo-execution $ \mathcal{E} = [\mathcal{F},\mathcal{B}^1, \ldots, \mathcal{B}^n] $ is a sequence such that: (i) each $ \mathcal{B}^j $ is a pseudo-behavior, and (ii) for any tuple of completions $ (\mathcal{B}^{\prime 1}, \ldots, \mathcal{B}^{\prime n}) $ of $ (\mathcal{B}^{1}, \ldots, \mathcal{B}^{n}) $, $ \mathcal{E}' = [\mathcal{F},\mathcal{B}^{\prime 1}, \ldots, \mathcal{B}^{\prime n}] $ is a $ k $-round execution. Here, $ \mathcal{E}' $ is termed a \emph{completion} of $ \mathcal{E} $.

For every $ k $-round execution $ \mathcal{E} = [\mathcal{F},\mathcal{B}^1, \ldots, \mathcal{B}^n] $, we naturally extend $ \mathcal{A} $ to produce the corresponding probabilistic distribution over $ k+1 $-round pseudo-executions. Specifically, for every $ k+1 $-round pseudo-execution $ \mathcal{E}' $, $ \mathcal{A}(\mathcal{E})(\mathcal{E}') = \Pi_{i \in [1:n]} \mathcal{A}(s^k_i,M_i^{R(k)})(s^{k+1}_i,M_i^{S(k+1)} \cup M_i^{SO(k+1)}) $.

An adversary is an algorithm that: (1) selects the initial correct states for all processes, and (2) for every $ k \in \mathbb{N}^{+} $, takes a $ k $-round pseudo-execution $ \mathcal{E} = [\mathcal{F},\mathcal{B}^1, \ldots, \mathcal{B}^n] $ and randomly outputs an execution $ \mathcal{E}' = [\mathcal{F}',\mathcal{B}^{\prime 1}, \ldots, \mathcal{B}^{\prime n}] $ that differs only in: (i) the final pseudo-fragments/fragment, and (ii) $ \mathcal{F} \subseteq \mathcal{F}' $. This definition encapsulates the adversary's capability to observe messages sent at round $ k $, corrupt new processes in $ \mathcal{F}' \setminus \mathcal{F} $, remove messages sent by corrupted processes in the last round of $ \mathcal{F}' $, and replace them with new messages.

\subsection{Sigma-algebra over executions and behaviours}

We now define the measurable space of executions. For every execution $ \mathcal{E}' = [\mathcal{F},\mathcal{B}^{\prime 1}, \ldots, \mathcal{B}^{\prime n}] $, an execution $ \mathcal{E} = [\mathcal{F},\mathcal{B}^1, \ldots, \mathcal{B}^n] $ is a prefix of $ \mathcal{E}' $ if every $ \mathcal{B}^j $ is a prefix of $ \mathcal{B}^{\prime j} $ and $ \mathcal{F} \subseteq \mathcal{F}' $. For each $ k $-round execution $ \mathcal{E} $ with $ k \in \mathbb{N}^{+} $, we denote $ \mathsf{Cone}(\mathcal{E}) $ as the set of executions $ \mathcal{E}' $ such that $ \mathcal{E} $ is a prefix of $ \mathcal{E}' $ (we define the tuple of initial states as the unique 0-round execution). Additionally, we denote $ \mathsf{Cones}_{\mathsf{Execs}} $ as the set of execution cones.


Given an adversary $ \mathsf{Adv} $, we can define the probabilistic measure over executions determined by the adversary. We denote $ \bar{\eta}_{\mathsf{Adv}} $ as the measure over $ \mathsf{Cones}_{\mathsf{Execs}} $, defined as follows: For every $ k' $-round execution $ \mathcal{E}' $, $ \bar{\eta}_{\mathsf{Adv}}(\mathsf{Cone}(\mathcal{E}'))= $
\begin{itemize}
    \item $1$ if $ k'=0 $
    \item $ \bar{\eta}_{\mathsf{Adv}}(\mathsf{Cone}(\mathcal{E})) \cdot \sum_{\mathcal{E}''}[\mathcal{A}(\mathcal{E})(\mathcal{E}'') \cdot \mathsf{Adv}(\mathcal{E}'')(\mathcal{E}')] $ if $ \mathcal{E} $ is the $ k'-1 $-round prefix of $ \mathcal{E}' $.
\end{itemize}

This equation represents a straightforward conditional probability for $ \mathcal{E}' $. The probability of having an execution in $ \mathsf{Cone}(\mathcal{E}') $ is the probability of the conjunction of: (1) having an execution in $ \mathsf{Cone}(\mathcal{E}) $ and reaching $ \mathsf{Cone}(\mathcal{E}') $ from $ \mathcal{E} $ through all the weighted possibilities defined by the algorithm $ \mathcal{A} $ and the adversary's strategy $ \mathsf{Adv} $.

Using standard measure-theoretic arguments, we can extend $ \bar{\eta}_{\mathsf{Adv}} $ to a probabilistic measure $ \prob_{\mathsf{Adv}} $ over sigma-field $ \mathscr{F}_{\mathsf{Execs}} $ over executions generated by $ \mathsf{Cones}_{\mathsf{Execs}} $. It suffices to first extend $ \bar{\eta}_{\mathsf{Adv}} $ on the field $ F_{\mathsf{Execs}} $ generated by $ \mathsf{Cones}_{\mathsf{Execs}} $ and then apply Carathéodory's extension theorem for a second extension on the sigma-algebra $ \mathscr{F}_{\mathsf{Execs}} $ generated by $ F_{\mathsf{Execs}} $.

With a similar construction, it is possible to define the set of cones of behaviours for each process $P_i$: for every behaviour $\mathcal{B}_i$ of process $P_i$, $\mathsf{Cone}(\mathcal{B}_i)$ is the set of behaviours $\mathcal{B}_i'$ such that $\mathcal{B}_i$ is a prefix of $\mathcal{B}_i'$. Similarly, $ \mathsf{Cones}_{\mathsf{Beh}^{i}} $ denotes the set of cones of behaviours of process $P_i$, while $ \mathscr{F}_{\mathsf{Beh}^{i}} $ denotes the sigma-algebra generated by $ \mathsf{Cones}_{\mathsf{Beh}^{i}} $.


We will deal with random variables of the form (of measurable function) $X : (\mathsf{Execs}, \mathscr{F}_{\mathsf{Execs}}, \prob_{\mathsf{Adv}}) \rightarrow (E, \mathscr{F}_{E}, \prob^{X})$, where $\prob^{X}$ is the image measure of $X$ under $\prob_{\mathsf{Adv}}$.

Clearly, the function $\mathsf{proj}_i : (\mathsf{Execs}, \mathscr{F}_{\mathsf{Execs}} ,  \prob_{\mathsf{Adv}}) \rightarrow (\mathsf{Beh}^i, \mathscr{F}_{\mathsf{Beh}^i})$ that maps each execution $ \mathcal{E} = [\mathcal{F},\mathcal{B}^1, \ldots, \mathcal{B}^n] $ to the behaviour $\mathcal{B}^i$ of the corresponding process is a measurable function.
Thus, we can define $\prob_{\mathsf{Adv}}^{i}$ as the image measure of $\prob_{\mathsf{Adv}}$ under $\mathsf{proj}_i$.
 
For any (measurable) predicate we use the classical notations:

$\prob_{\mathsf{Adv}}(\mathsf{predicate}(X)) \triangleq \prob_{\mathsf{Adv}}(\{\mathcal{E} | \mathsf{predicate}(X(\mathcal{E}))\}) $ and 

$\prob_{\mathsf{Adv}}(\mathsf{predicate}(X) | \mathsf{predicate}'(Y)) \triangleq \frac{1}{Pr_Y} \cdot \prob_{\mathsf{Adv}}(\{\mathcal{E} | \mathsf{predicate}(X(\mathcal{E})) \wedge \mathsf{predicate}'(Y(\mathcal{E}))\}) $ if $Pr_Y \triangleq \prob_{\mathsf{Adv}}(\{\mathcal{E} | \mathsf{predicate}'(Y(\mathcal{E}))\}) \neq 0$ and $0$ otherwise.

The random variables defined on $(\mathsf{Execs}, \mathscr{F}_{\mathsf{Execs}} ,  \prob_{\mathsf{Adv}})$ that we will use will be:
\begin{itemize}
    \item "message complexity" that maps each execution to the number of messages sent by forever-honest processes in this execution.
\end{itemize}

and some binary random variables (with output in $\{\mathit{true},\mathit{false}\}$):
\begin{itemize}
    \item "agreement holds"
    \item "process $P_i$ receives less than a certain number of messages from a certain subset of processes" 
\end{itemize}

A \emph{world} is a pair $(\mathsf{Adv},X)$ where $\mathsf{Adv}$ is an adversary's strategy and $X$ is a binary random variable defined on $(\mathsf{Execs}, \mathscr{F}_{\mathsf{Execs}})$.
Two worlds $W=(\mathsf{Adv},X)$ and $W'=(\mathsf{Adv}',X')$ are said indistinguishable for a process $P_i$, noted $W \overset{i}{\sim} W'$, if $\prob^{i}_{\mathsf{Adv}}(\cdotp | X) =$ $\prob^{i}_{\mathsf{Adv}'}(\cdotp | X')$. Similarly, $W$ and $W'$ are said indistinguishable for a set of processes $S$, noted $W \overset{S}{\sim} W'$, if $\forall P_i \in S$, $W \overset{i}{\sim} W'$. Obviously, $\overset{i}{\sim}$ is an equivalence relationship.



%A \emph{world} $W$ is a pair $(E,\mathsf{Adv})$ where $E$ is a subset of executions and $\mathsf{Adv}$ is an adversary strategy. 
%Now, we can say that two adversary worlds $(E,\mathsf{Adv})$ and $(E',\mathsf{Adv}')$ are indistinguishable for a process $P_i$ if the restriction of $\eta_{\mathsf{Adv}}^{i} = \eta_{\mathsf{Adv}'}^{i}$ (same support and same valuation for each element of the support).

\subsection{The proof}

Here, a protocol and an adversary strategy is parameterized with $n \in \mathbb{N}$. We assume that $\mathcal{A}$ is a synchronous protocol with subquadratic expected message complexity, i.e. for every (allowed) adversary $\mathsf{Adv}$, $\expe_{Adv}(\text{message complexity}) \leq c_e\cdot t^2$, where $c_e$ is some positive real constant.

\iffalse
\begin{lemma}[trivial isolation]
Let $c_m$ be a constant positive real numbers.
Then, for every sets $\Pi_s, \Pi_r \subseteq \Pi$ of processes, the processes in $\Pi_r$ will receive less than $c_m \cdot t^2$ messages from correct processes in $\Pi_s$ with probability $c_p \geq \frac{c_m-c_e}{c_m}$.
\end{lemma}

\begin{proof}
    Let's fix an adversary strategy $\mathsf{Adv}$. Let $R_{\Pi_r}$ be the random variable that maps each execution to the number of messages received from so-far-correct processes by processes in $\Pi'$. By Markov's inequality, $ \forall a \in \mathbb{R}^{>0}$, $\prob_{\mathsf{Adv}}(R_{\Pi'} \geq a) \leq  \frac{\expe_{\mathsf{Adv}}(R_{\Pi'})}{a} $, i.e. $\prob_{\mathsf{Adv}}(R_{\Pi'} \leq a) \geq 1 - \frac{\expe_{\mathsf{Adv}}(R_{\Pi'})}{a} $, and so $\prob_{\mathsf{Adv}}(R_{\Pi'} \leq c_m \cdot t^2) \geq 1 - \frac{c_e}{c_m} \geq  \frac{c_m-c_e}{c_m}$.  
\end{proof}

\begin{lemma}[isolation bet]
Let $c'_m, \tilde{c}_m, c_r$ be constant positive real numbers with $c'_m = \frac{\tilde{c}_m}{c_r}$.
Let $\Pi_s, \Pi_r \subseteq \Pi$ such that $|\Pi_r| = c_r \cdot t$ and $\mathbb{U}_r$ be the uniform distribution over $\Pi_r$.
Then, a process uniformly chosen among processes in $\Pi_r$ (according to $\mathbb{U}_r$)  will receive less than $c'_m \cdot t$ messages from correct processes in $\Pi_s$ with constant probability $c'_p = 1 - \frac{c_e}{\tilde{c}_m} = \frac{\tilde{c}_m-c_e}{\tilde{c}_m}$.
\end{lemma}

\begin{proof}
    Let's fix an adversary strategy $\mathsf{Adv}$. Let $R_{u}$ be the random variable that maps each execution to the number of messages received from so-far-correct processes by process $P_u$ uniformly picked in $\Pi'$. By Markov's inequality, $ \forall a \in \mathbb{R}^{>0}$, $\prob_{\mathsf{Adv}}(R_{u} \geq a) \leq  \frac{\expe_{\mathsf{Adv}}(R_{u})}{a} $, i.e. $\prob_{\mathsf{Adv}}(R_{u} \leq a) \geq 1 - \frac{\expe_{\mathsf{Adv}}(R_{u})}{a} $, and so $\prob_{\mathsf{Adv}}(R_{u} \leq c'_m \cdot t) \geq 1 - \frac{c_e \cdot t^2}{c_r \cdot t} \cdot \frac{1}{c'_m \cdot t} \geq 1 - \frac{c_e}{c_r \cdot c'_m} \geq \frac{c_r \cdot c'_m-c_e}{c_r \cdot c'_m}$.  
\end{proof}

\begin{lemma}[probabilistic indistinguishability by substitution]
Let $(X, Y, Z)$ represent any partition of $\Pi$ such that (1) $|X| = n - |Y| - |Z|$, (2) $|Y| = \frac{t}{4}$, and (3) $|Z| \leq \frac{t}{4}$.
Let $Y'$ be any group of processes such that (1) $Y' \subseteq Y$, and (2) $|Y'| \geq \frac{|Y|}{4} = \frac{t}{16}$. 

Let $\mathsf{Adv}$ be any adversary's strategy such that:
\begin{compactitem}
    \item processes from $X$ are forever-correct, whereas processes from $Y \cup Z$ are initially corrupted; and

    \item group $Y$ is isolated from some round $k \in \mathbb{N}$.
\end{compactitem}

For every process $P_u \in Y'$, we define $R_u$ as the random variable that maps each execution to the number of messages received by process $P_u$ from processes in $X$ and the adversary strategy $\widehat{\mathsf{Adv}}^{u}$ as follows:
\begin{compactitem}
    \item processes from $X \cup \{P_u\}$ are initially-correct, whereas processes from $Y \cup Z \setminus \{P_u\}$ are initially corrupted; and

    \item group $Y \setminus \{P_u\}$ is isolated from some round $k \in \mathbb{N}$.

    \item  $\widehat{\mathsf{Adv}}^{u}$ behaves as $\mathsf{Adv}$ except that, as long as $R_u < t - |Y \cup Z \setminus \{P_u\}| \leq t/2$, every time a process $P \in X \cup Z \setminus \{P_u\}$ sends a message $m$ to process $P_u$ at round $k' \geq k$, $\widehat{\mathsf{Adv}}^{u}$ (i) corrupts $P$ if it was not already the case, (ii) moves $m$ from sent messages of $P_x$ to sent-omitted messages of $P_x$.
\end{compactitem}

 
%Let $P_v$ be the process from $Y'$ that receive messages from the smaller subset of $X$ in expectation, according to the probabilistic distribution defined by $\mathsf{Adv}$, that is $v = \mathit{arg \; min}_{u} \expe_{\mathsf{Adv}}(R_u)$, where $R_u$ is the random variable that maps each execution to the number of messages received by process $P_u \in Y'$ from processes in $X$. 
Let $W^u = (\mathsf{Adv}, \{R_u \leq \frac{t}{2}\})$ and $\widehat{W}^u = (\widehat{\mathsf{Adv}}^{u}, \{R_u \leq \frac{t}{2}\})$.

Then, $\forall P_i \in \Pi$, $W^u \overset{i}{\sim} \widehat{W}^{u}$.

It means the two adversaries $\mathsf{Adv}$ and $\widehat{\mathsf{Adv}}^{u}$, conditioned to the fact that $P_u$ receives messages from less than $\frac{t}{2}$ members of $X$ after round $k$ (for the success of the attack), are indistinguishable for the processes.

%Moreover, for every process $P_x \in X$, we note $S_{x \nrightarrow v}$ the binary random variable that maps each execution to $\mathit{true}$ if $P_x$ does not send a message to $P_v$ and $\mathit{false}$ otherwise. Furthermore, we note $\mathsf{Hit}_x$ the binary random variable that maps each execution $\mathcal{E}$ to $\mathit{true}$ if $S_{x \nrightarrow v}(\mathcal{E}) \wedge R_v(\mathcal{E}) \leq \frac{t}{2}$ and $\mathit{false}$ otherwise. 
\end{lemma}
\fi
%%%
%%%
\begin{definition}[partition]
We fix $(A, B, C)$ a partition of $\Pi$ such that (1) $|A| = n - |B| - |C| \geq n/2$, (2) $|B| = |C| = \frac{t}{4}$.
\end{definition}

\begin{definition}[basic adversary $\mathsf{Adv}_{(k,k',\bar{b})}$]
For every $(k,k',\bar{b}) \in \mathbb{N}^{>0} \times \mathbb{N}^{>0} \times (\Pi \mapsto \{0,1\})$, we note $\mathsf{Adv}_{(k,k',\bar{b})}$ the adversary strategy such that:
\begin{compactitem}
    \item processes from $A$ are forever-correct, whereas processes from $B \cup C$ are initially corrupted; and

    \item group $B$ and $C$ are isolated from some round $k \in \mathbb{N}$ and $k' \in \mathbb{N}$ respectively.

    \item Every process $P_i$ initially proposes the bit $\bar{b}(P_i)$.
\end{compactitem}
\end{definition}

\begin{definition}[substitution adversary]
Let $(k,k',\bar{b}) \in \mathbb{N}^{>0} \times \mathbb{N}^{>0} \times (\Pi \mapsto \{0,1\})$.
Let $P_u \in \Pi$ and $k_u \in \mathbb{N}$.%$P_u \in B$ (resp. $P_u \in C$). 
We define $R_u$ as the random variable that maps each execution to the number of members of set $A$ whose he receives a message and the adversary strategy $\widehat{\mathsf{Adv}}^{u,k_u}_{(k,k',\bar{b})}$ as follows:
\begin{compactitem}
    \item processes from $A \cup \{P_u\}$ are initially-correct, whereas processes from $B \cup C \setminus \{P_u\}$ are initially corrupted; and

    \item group $B \setminus \{P_u\}$ and $C \setminus \{P_u\}$ are isolated from some round $k \in \mathbb{N}$ and $k' \in \mathbb{N}$ respectively.

    \item Every process $P_i$ initially proposes the bit $\bar{b}(P_i)$.
    
    \item  $\widehat{\mathsf{Adv}}^{u,k_u}_{(k,k',\bar{b})}$ behaves as $\mathsf{Adv}$ except that, as long as $R_u < t - |B \cup C \setminus \{P_u\}| \leq t/2$, every time a process $P \neq P_u$ sends a message $m$ to process $P_u$ at round $k'' \geq k_u$, $\widehat{\mathsf{Adv}}^{u}$ (i) corrupts $P$ if it was not already the case, (ii) moves $m$ from sent messages of $P$ to sent-omitted messages of $P$.
\end{compactitem}

Moreover, we note $\widehat{W}^{u,k_u}_{(k,k',\bar{b})} = (\widehat{\mathsf{Adv}}^{u,k_u}_{(k,k',\bar{b})}, R_u)$ and $W^u_{(k,k',\bar{b})} = (\mathsf{Adv}_{(k,k',\bar{b})}, R_u)$.
\end{definition}

\begin{lemma}[indistinguishability by substitution]
    Let $(k,k',k_u,\bar{b}) \in (\mathbb{N}^{>0})^3 \times (\Pi \mapsto \{0,1\})$.
Let $P_u \in \Pi$. If $k_u \geq min(k,k')$, then $\widehat{W}^{u,k_u}_{(k,k',\bar{b})}  \overset{\Pi}{\sim} W^u_{(k,k',\bar{b})} $ 
\end{lemma}

\begin{lemma}[$W^u_{(k,k,\bar{b})} \overset{u}{\sim} W^u_{(k,k-1,\bar{b})}$ \& $W^v_{(k,k,\bar{b})} \overset{v}{\sim} W^v_{(k+1,k,\bar{b})}$]
    Let $(k,\bar{b}) \in \mathbb{N}^{>0} \times \mathbb{N}^{>0} \times (\Pi \mapsto \{0,1\})$. Let $(P_u, P_v) \in B \times C$.
We always have $W^u_{(k,k,\bar{b})} \overset{u}{\sim} W^u_{(k,k-1,\bar{b})}$ (if $k>1$) and $W^v_{(k,k,\bar{b})} \overset{v}{\sim} W^v_{(k+1,k,\bar{b})}$.
\end{lemma}

\begin{lemma}[double isolation]
    Let $(k,\bar{b}) \in \mathbb{N}^{>0} \times \mathbb{N}^{>0} \times (\Pi \mapsto \{0,1\})$.
\end{lemma}

\begin{lemma}[binding]
    Assume $\mathcal{A}$ solves agreement with probability $\tilde{\rho}$.
    Let $(k,\bar{b}) \in \mathbb{N}^{>0} \times (\Pi \mapsto \{0,1\})$. 
    There is a partition of the executions of $k-1$ rounds $(E^0_{k,\bar{b}}, E^1_{k,\bar{b}}, E^2_{k,\bar{b}})$.% and a triplet of probabilities $(\rho^0_{k}, \rho^1_{k}, \rho^2_{k})$ with $\rho^0_{k} + \rho^1_{k} + \rho^2_{k} = 1$, such that:
    \begin{itemize}
        \item $\prob_{\mathsf{Adv}_{(k,k,\bar{b})}}(\mathsf{Cone}(E^0_{k,\bar{b}})) = \rho^0_{min} $
        \item $\prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\mathsf{Cone}(E^1_{k,\bar{b}})) = \rho^1_{min} $
        \item $\prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\mathsf{Cone}(E^2_{k,\bar{b}})) = \rho^2_{min} \simeq 0$.
        \item processes in $A$ reach agreement on $0$ in $\mathsf{Cone}(E^0_{k,\bar{b}})$ with probability $\tilde{\rho}^0_{(k,k',\bar{b})}$ under $\mathsf{Adv}_{(k,k',\bar{b})}$
        \item processes in $A$ reach agreement on $1$ in $\mathsf{Cone}(E^1_{k,\bar{b}})$ with probability $\tilde{\rho}^1_{(k,k',\bar{b})}$ under $\mathsf{Adv}_{(k,k',\bar{b})}$
        \item $\tilde{\rho}^1_{(k,k',\bar{b})} \cdot \rho^1_{(k,k',\bar{b})} + \tilde{\rho}^0_{(k,k',\bar{b})} \cdot \rho^0_{min} \geq \tilde{\rho} - cste$ 
    \end{itemize}
\end{lemma}

\iffalse
\begin{lemma}[binding]
    Assume $\mathcal{A}$ solves agreement with probability $\tilde{\rho}$.
    Let $(k,k',\bar{b}) \in \mathbb{N}^{>0} \times \mathbb{N}^{>0} \times (\Pi \mapsto \{0,1\})$. Let $k_{min} = \mathsf{min}(k,k')$. There is a partition of the executions of $k_{min}$ rounds $(E^0_{k_{min}}, E^1_{k_{min}}, E^2_{k_{min}})$ and a triplet of probabilities $(\rho^0_{min}, \rho^1_{min}, \rho^2_{min})$ with $\rho^0_{min} + \rho^1_{min} + \rho^2_{min} = 1$, such that:
    \begin{itemize}
        \item $\prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\mathsf{Cone}(E^0_{k_{min}})) = \rho^0_{min} $
        \item $\prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\mathsf{Cone}(E^1_{k_{min}})) = \rho^1_{min} $
        \item $\prob_{\mathsf{Adv}_{(k,k',\bar{b})}}(\mathsf{Cone}(E^2_{k_{min}})) = \rho^2_{min} $ close to $0$
        \item processes in $A$ reach agreement on $0$ in $\mathsf{Cone}(E^0_{k_{min}})$ with probability $\tilde{\rho}^0_{min}$ under $\mathsf{Adv}_{(k,k',\bar{b})}$
        \item processes in $A$ reach agreement on $1$ in $\mathsf{Cone}(E^1_{k_{min}})$ with probability $\tilde{\rho}^1_{min}$ under $\mathsf{Adv}_{(k,k',\bar{b})}$
        \item $\tilde{\rho}^1_{min} \cdot \rho^1_{min} + \tilde{\rho}^0_{min} \cdot \rho^0_{min} \geq \tilde{\rho} - cste$ 
    \end{itemize}
\end{lemma}

\begin{proof}[sketch]
    Without loss of generality, assume $k \leq k'$. 
    The idea is to perform the attack $\widehat{\mathsf{Adv}}^{u}_{(k,k',\bar{b})}$ with $P_u$ well-chosen (or uniformly chosen) in $B$, that can succeed with an arbitrary big probability $1-O(1)$. In such an attack, $P_u$ cannot see what happen after round $k$ (by isolation). So, if the bit to decide is not decided, he will have to decide it randomly, and so he will face an important probability to fail.
\end{proof}
\fi
%%%
%%%

\begin{lemma}
    Let $(X, Y, Z)$ represent any partition of $\Pi$ such that (1) $|X| = n - |Y| - |Z|$, (2) $|Y| = \frac{t}{4}$, and (3) $|Z| \leq \frac{t}{4}$.
Let $Y'$ be any group of processes such that (1) $Y' \subseteq Y$, and (2) $|Y'| \geq \frac{|Y|}{4} = \frac{t}{16}$. 

Let $\mathsf{Adv}$ be any adversary's strategy such that:
\begin{compactitem}
    \item processes from $X$ are forever-correct, whereas processes from $Y \cup Z$ are initially corrupted; and

    \item group $Y$ is isolated from some round $k \in \mathbb{N}$.
\end{compactitem}

For every process $P_u \in Y'$, we define $R_u$ as the random variable that maps each execution to the number of messages received by process $P_u$ from processes in $X$.

Let $P_v$ be the process from $Y'$ that receive messages from the smaller subset of $X$ in expectation, according to the probabilistic distribution defined by $\mathsf{Adv}$, that is $v = \mathit{arg \; min}_{u} \expe_{\mathsf{Adv}}(R_u)$.
Then $\prob_{\mathsf{Adv}}(R_v \leq t/2) \geq c_s$ for some constant $c_s = 1 - 8c_e$.
\end{lemma}

\begin{proof}
    By Markov inequality, $ \forall a \in \mathbb{R}^{>0}$, $\prob_{\mathsf{Adv}}(R_{v} \geq a) \leq  \frac{\expe_{\mathsf{Adv}}(R_{v})}{a} $, i.e. $\prob_{\mathsf{Adv}}(R_{v} \leq a) \geq 1 - \frac{\expe_{\mathsf{Adv}}(R_{v})}{a} $, and so $\prob_{\mathsf{Adv}}(R_{v} \leq \frac{t}{2}) \geq 1 - \frac{4}{t} \cdot (c_e \cdot t^2) \cdot \frac{2}{ t} \geq 1 - 8 c_e $.  
\end{proof}

\begin{lemma}[Combining receive-isolation]\label{lemma:combining_receive_isolation}
Let  $\bar{b}^u, \bar{b}^v: \Pi \rightarrow \{0,1\}$.
Let $\mathsf{Adv}^{u}$ and $\mathsf{Adv}^{v}$ be two adversarial strategies such that:
\begin{compactitem}
\item $\forall P_i \in \Pi$, $P_i$ proposes $\bar{b}^u(P_i)$ (resp.  $\bar{b}^v(P_i)$) with $\mathsf{Adv}^{u}$ (resp.  $\mathsf{Adv}^{v}$).
\item With $\mathsf{Adv}^{u}$: $A \cup B $ are forever-correct,  while $C$ is initially-corrupted and receive-isolated from some round $k^u$ onward. 
\item With $\mathsf{Adv}^{v}$: $A \cup C $ are forever-correct,  while $B$ is initially-corrupted and receive-isolated from some round $k^v$ onward.
\item \begin{itemize}
    \item with  $\mathsf{Adv}^{u}$, processes in $A \cup B$: 
    $\left\{
\begin{array}{l}
\mbox{agree on 0 with probability } \rho_0^u\\ 
\mbox{agree on 1 with probability } \rho_1^u 
% \\ \mbox{do not agree with probability } 1-\rho_1^u-\rho_0^u
\end{array}
\right.$
 \item with  $\mathsf{Adv}^{v}$, processes in $A \cup C$: 
    $\left\{
\begin{array}{l}
\mbox{agree on 0 with probability } \rho_0^v\\ 
\mbox{agree on 1 with probability } \rho_1^v 
%\\ \mbox{do not agree with probability } 1-\rho_1^v-\rho_0^v
\end{array}
\right.$
\end{itemize}
\end{compactitem}
If either (1) $k^u = k^v = 1$ or (2) $|k^u-k^v| \leq 1$ and $\bar{b}^u = \bar{b}^v$. \newline
Then, $b'_u = b'_v$.
\end{lemma}

\begin{proof}
   
    We define $\mathsf{Adv}^{*}$, such that processes in $A$ are forever-correct,  while processes in $B$ (resp. $C$) behave exactly as with adversary $\mathsf{Adv}^{u}$ (resp. $\mathsf{Adv}^v$), i.e. are initially-corrupted, receive-isolated from some round $k^v$ (resp. $k^u$) onward and propose $\bar{b}^{u}$ (resp. $\bar{b}^{v}$).
    Let $b'_w$ be the bit such that
    $A$ decides $b'_w$  with the highest probability $\rho_w$ with  $\mathsf{Adv}^{*}$.
    

    As in former lemma, we note $P_i$ (resp. $P_j$), the process in $C$ (resp. $B$)
    that receive messages after round $k^u$ (resp. $k^v$) from the smaller subset of $A$ in expectation, according to the probabilistic distribution defined by $\mathsf{Adv}^{*}$.
    Then, we define the adversary $\tilde{\mathsf{Adv}}^{*}_i$ (resp. $\tilde{\mathsf{Adv}}^{*}_j$) that isolates process $P_i$ (resp. $P_j$) exactly as in former lemma.

    %%
    We note:
    \begin{itemize}
         \item $\mathsf{Hit} = \{R_i \leq t/2\} \wedge \{R_j \leq t/2\}$
        \item  $W^{*} = (\mathsf{Adv}^{*}, \mathsf{Hit})$
        \item  $W^{u} = (\mathsf{Adv}^{u}, \mathsf{Hit})$
        \item  $W^{v} = (\mathsf{Adv}^{v}, \mathsf{Hit})$
        \item $\tilde{W}^{*}_i = (\tilde{\mathsf{Adv}}^{*}_i, \mathsf{Hit})$
        \item $\tilde{W}^{*}_j = (\tilde{\mathsf{Adv}}^{*}_j, \mathsf{Hit})$
    \end{itemize}
    
    We have:
    \begin{itemize}
        \item $W^u \overset{A,i}{\sim} W^{*} \overset{A,i}{\sim} \tilde{W}^{*}_i$
        \item $W^v \overset{A,j}{\sim} W^{*} \overset{A,j}{\sim} \tilde{W}^{*}_j$
    \end{itemize}

    

\end{proof}
%%%%%%%%%%%%%
%%%%%%%%%%%%%





==> sections/related_validity_paper.tex <==
\section{Related work}
\label{section:related_work}

\paragraph{Solvability of consensus.}
The consensus problem has been thoroughly investigated in a variety of system settings and failure models.
It has been known (for long) that consensus can be solved in a synchronous setting, both with crash~\cite{lynch1996distributed,cachin2011introduction,raynal2002consensus} and arbitrary failures~\cite{abraham2017brief,kowalski2013synchronous,schmid2004synchronous,raynal2002consensus,Momose2021}.
% Moreover, the celebrated Dolev-Reischuk bound~\cite{dolev1985bounds} shows that any synchronous solution to the Byzantine consensus problem requires $\Omega(n^2)$ exchanged messages.
% Recently, this bound was shown to be tight by Momose and Ren~\cite{Momose2021}.
In an asynchronous environment, however, consensus cannot be solved deterministically even if a single process can fail, and it does so only by crashing; this is the seminal FLP impossibility result~\cite{fischer1985impossibility}.

A traditional way of circumventing the FLP impossibility result is \emph{randomization}~\cite{B83,aspnes2003randomized,abraham2019asymptotically,LL0W20,ezhilchelvan2001randomized}, where termination of consensus is not ensured deterministically.
Another well-established approach to bypass the FLP impossibility is to strengthen the communication model with \emph{partial synchrony}~\cite{DLS88}: the communication is asynchronous until some unknown time, and then it becomes synchronous.
The last couple of decades have produced many partially synchronous consensus algorithms~\cite{yin2019hotstuff,CGL18,CGG21,CL02,DLS88,BKM19,lynch1996distributed,lamport2001paxos,civit2022byzantine,lewis2022quadratic}.
% Recently, the aforementioned Dolev-Reischuk bound was shown to be tight even in partial synchrony~\cite{civit2022byzantine,lewis2022quadratic}.

Another line of research has consisted in weakening the definition of  consensus  to make it deterministically solvable under asynchrony.
In the \emph{condition-based} approach~\cite{mostefaoui2003conditions}, 
the specification of consensus is relaxed to require termination only if the assignment of proposals satisfies some predetermined conditions.
The efficiency of this elegant approach has been studied further in~\cite{mostefaoui2001hierarchy}.
Moreover, the approach is extended to the synchronous setting~\cite{mostefaoui2003using,zibin2003condition}, as well as  to the $k$-set agreement problem~\cite{hagit2002wait,mostefaoui2002condition}.

\paragraph{Solvability of general decision problems.}
% The question of which problems are solvable under which assumptions is crucial in distributed computing.
% Traditionally, 
A distributed decision problem has been defined in~\cite{crime_punishment,MendesTH14,HerlihyS99} 
as a mapping from input assignments to admissible decisions. 
Our validity formalism is of the same nature, and it is inspired by the aforementioned specification of decision problems.

The solvability of decision problems has been thoroughly studied in asynchronous, crash-prone settings.
It was shown in~\cite{moran1987extended} that the FLP impossibility result~\cite{fischer1985impossibility} can be extended to many decision problems.
In~\cite{biran1990combinatorial}, the authors defined the necessary and sufficient conditions for a decision problem to be asynchronously solvable with a single crash failure.
% the aforementioned work from Moran and Wolfstahl~\cite{moran1987extended}.
The asynchronous solvability of problems in which crash failures occur at the very beginning of an execution was studied in~\cite{taubenfeld1989initial}.
%using the game-theoretical approach, authors give necessary and sufficient conditions for a problem to be solvable in such a setting. 
The necessary and sufficient conditions for a decision problem to be asynchronously solvable (assuming a crash-prone setting) in a randomized manner were given in ~\cite{Chor1989}. 
The topology-based approach on studying the solvability of decision problems in asynchrony has proven to be extremely effective, both for crash~\cite{HerlihyS93,SaraphHG18,Herlihy2013} and arbitrary failures~\cite{MendesTH14,Herlihy2013}.
% \jovan{Pierre, please add some citations for topology (if you know them).} \pierre{Classically, results from algebraic topology address deterministic asynchronous computation (e.g. approximate agreement, $k$-set agreement, etc). I do no think they are topology-based results for consensus. I will take a look.}
Our results follow the same spirit as many of these approaches; however, we study the deterministic solvability and complexity of all consensus variants in a partially synchronous environment.

\paragraph{Validity of consensus.}
Various validity properties have been  associated with the consensus problem (beyond the aforementioned \emph{Strong Validity} and \emph{Weak Validity}).
\emph{Correct-Proposal Validity}~\cite{fitzi2003efficient,siu1998reaching} states that  a value decided by a correct process must have been proposed by a correct process. 
% (The consensus problem with \emph{Correct Proposal Validity} is usually referred to as strong Byzantine consensus.)
\emph{Median Validity}~\cite{stolz2016byzantine} is a validity property proposed in the context of synchronous consensus,  requiring the decision to be close to the median of the proposals of correct processes. \emph{Interval Validity}~\cite{melnyk2018byzantine}, on the other hand, requires the  decision to be close to the $k$-th smallest proposal of correct processes.
The advent of blockchain technologies has resurged the concept of \emph{External Validity}~\cite{Cachin2001,BKM19,yin2019hotstuff}.
This property requires the decided value to satisfy a predetermined predicate, typically asserting whether the decided value follows the rules of a blockchain system (e.g., no double-spending).
(This paper considers a simple formalism to express basic validity properties and derive our results. To express \emph{External Validity}, which is out of the scope of the paper, we propose an (incomplete) extension of our formalism in \Cref{section:extended_formalim_appendix}, and leave its full realization for future work.)
\emph{Convex-Hull Validity}, which states that the decision must belong to the convex hull of the proposals made by the correct processes, is employed in approximate agreement~\cite{AbrahamAD04,MendesH13,GhineaLW22,ghinea2023multidimensional}.
We underline that the approximate agreement problem is not covered in this paper since the problem allows correct processes to disagree as long as their decisions are ``close'' to each other.
However, this paper does study (in a general manner) the utilization of \emph{Convex-Hull Validity} in the classical consensus problem (in which the correct processes are required to ``exactly'' agree).


In interactive consistency~\cite{maneas2021achieving,fischer1981lower,ben2003resilient},  correct processes agree on the proposals of all correct processes. Given that the problem is  impossible in a non-synchronous setting, a weaker variant has been considered: vector consensus~\cite{neves2005solving,vaidya2013byzantine,Doudou1998,correia2006consensus,duan2023practical,Ben-Or94}. Here, processes need to agree on a vector of proposals which does not necessarily include the proposals of \emph{all} correct processes. Interactive consistency and vector consensus can be seen as specific consensus problems with a validity property requiring that, if a decided vector contains a proposal $v$ of a correct process, that correct process has indeed proposed $v$.
% which requires the decided vector to contain all the proposals of correct processes.
The design of \general, our general consensus algorithm for any solvable (and non-trivial) validity property, demonstrates that any non-trivial flavor of consensus which is solvable in partial synchrony can be solved using vector consensus (see \Cref{subsection:general_algorithm}).



==> sections/similarity_lemma.tex <==
\subsection{Canonical Similarity} \label{subsection:similarity}

In this subsection, we introduce \emph{canonical similarity}, a crucial intermediate result.
In order to do so, we first establish an important relation between input configurations, that of \emph{similarity}.

\paragraph{Similarity.}

We define the similarity relation (``$\sim$'') between input configurations:
\begin{equation*}
    \forall c_1, c_2 \in \allconfigurations: c_1 \sim c_2 \iff (\processes{c_1} \cap \processes{c_2} \neq \emptyset) \land (\forall P_i \in \processes{c_1} \cap \processes{c_2}: c_1[i] = c_2[i]).
\end{equation*}

In other words, $c_1$ is similar to $c_2$ if and only if (1) $c_1$ and $c_2$ have (at least) one process in common, and (2) for every common process, the process's proposal is identical in both input configurations.
For example, when $n = 3$ and $t = 1$, $c = \big[ (P_1, 0), (P_2, 1), (P_3, 0) \big]$ is similar to $\big[ (P_1, 0), (P_3, 0) \big]$, whereas $c$ is not similar to $\big[ (P_1, 0), (P_2, 0), (P_3, 0) \big]$.
Note that the similarity relation is symmetric (for every pair $c_1, c_2 \in \mathcal{I}$, $c_1 \sim c_2 \Leftrightarrow c_2 \sim c_1$) and reflexive (for every $c \in \mathcal{I}$, $c \sim c$).

For every input configuration $c \in \mathcal{I}$, we define its \emph{similarity set}, denoted by $\mathit{sim}(c)$:
\begin{equation*}
    \mathit{sim}(c) = \{ c' \in \mathcal{I} \,|\, c' \sim c \}.
\end{equation*}

% We rely on the similarity relation to define canonical simi larity (\Cref{subsection:intermediate_results}), and the similarity condition (\Cref{subsection:necessary_condition}).

% We later rely on the similarity relation in defining the similarity condition, which we prove to be a necessary condition for a validity property to be solvable (see \Cref{subsection:necessary_condition}).
% utilize to classify validity properties.

\paragraph{The result.}
Let $\mathcal{A}$ be an algorithm which solves  consensus  with some validity property $\mathit{val}$.
Our canonical similarity result states that $\mathcal{A}$, in any canonical execution which corresponds to some input configuration $c$, can only decide a value which is admissible for \emph{all} input configurations similar to $c$.
Informally, the reason is that correct processes cannot distinguish silent faulty processes from slow correct ones.

\begin{lemma}[Canonical similarity] \label{lemma:helper_main}
Let $\mathit{val}$ be any solvable validity property and let $\mathcal{A}$ be any algorithm which solves the consensus problem with $\mathit{val}$.
Let $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ be any (potentially infinite) canonical execution and let $\mathsf{input\_conf}(\mathcal{E}) = c$, for some input configuration $c \in \mathcal{I}$.
If a value $v' \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}$, then $v' \in \bigcap\limits_{c' \in \mathit{sim}(c)} \mathit{val}(c')$.
\end{lemma}
\begin{proof}
We prove the lemma by contradiction.
Suppose that $v' \notin \bigcap\limits_{c' \in \mathit{sim}(c)} \mathit{val}(c')$.
Hence, there exists an input configuration $c' \in \mathit{sim}(c)$ such that $v' \notin \mathit{val}(c')$.
If $\mathcal{E}$ is infinite, let $\mathcal{E}_P \gets \mathcal{E}$.
Otherwise, let $\mathcal{E}_P$ denote any infinite continuation of $\mathcal{E}$ such that (1) $\mathcal{E}_P$ is canonical, and (2) $\mathsf{input\_conf}(\mathcal{E}_P) = c$.
Let $P$ be any process such that $P \in \processes{c'} \cap \processes{c}$; such a process exists as $c' \sim c$.
As $\mathcal{A}$ satisfies \emph{Termination} and \emph{Agreement}, $\mathcal{E}_P$ is an infinite execution, and $P$ is correct in $\mathcal{E}_P$, $P$ decides $v'$ in $\mathcal{E}_P$.
Let $\mathcal{S}$ denote the set of all processes which take a computational step in $\mathcal{E}_P$ until $P$ decides $v'$; note that $\mathcal{S} \subseteq \processes{c}$ and $P \in \mathcal{S}$.

In the next step, we construct another execution $\mathcal{E}' \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}') = c'$:
\begin{compactenum}
    \item $\mathcal{E}'$ is identical to $\mathcal{E}_P$ until process $P$ decides $v'$.
    
    \item All processes not in $\processes{c'}$ are faulty in $\mathcal{E}'$ (they might behave correctly until $P$ has decided), and all processes in $\processes{c'}$ are correct in $\mathcal{E}'$.
    % Observe that processes behave correctly in $\mathcal{E}'$ until $P$ has decided.
    
    \item After $P$ has decided, processes in $\processes{c'} \setminus{\mathcal{S}}$ ``wake up'' with the proposals specified in $c'$.
    
    \item GST is set to after all processes in $\processes{c'}$ have taken a computational step.
\end{compactenum}
For every process $P_i \in \mathcal{S} \cap \processes{c'}$, the proposal of $P_i$ in $\mathcal{E}'$ is $\mathsf{proposal}(c'[i])$; recall that $c'[i] = c[i]$ as $c' \sim c$ and $\mathcal{S} \subseteq \processes{c}$.
Moreover, for every process $P_j \in \processes{c'} \setminus{\mathcal{S}}$, the proposal of $P_j$ in $\mathcal{E}'$ is $\mathsf{proposal}(c'[j])$ (due to the step 3 of the construction).
Hence, $\mathsf{input\_conf}(\mathcal{E}') = c'$.
Furthermore, process $P$, which is correct in $\mathcal{E}'$, decides a value $v' \notin \mathit{val}(c')$ (due to the step 1 of the construction).
Thus, we reach a contradiction with the fact that $\mathcal{A}$ satisfies $\mathit{val}$, which proves the lemma.
\end{proof}

We underline that \Cref{lemma:helper_main} does not rely on \emph{any} assumptions on $n$ and $t$.
In other words, \Cref{lemma:helper_main} is applicable to any algorithm irrespectively of the parameters $n$ and $t$ (as long as $0 < t < n$).

% We construct another execution $\mathcal{E}' \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}') = c'$:
% \begin{compactenum}
%     \item $\mathcal{E}'$ is identical to $\mathcal{E}_P$ until process $P$ decides $v'$.
    
%     \item All processes in $\Pi \setminus{\processes{c'}}$ are faulty in $\mathcal{E}'$ (they behave correctly until $P$ has decided), and all processes in $\processes{c'}$ are correct.
%     % Observe that processes behave correctly in $\mathcal{E}'$ until $P$ has decided.
    
%     \item After $P$ has decided, processes in $\processes{c'} \setminus{\processes{c}}$ ``wake up'' with the proposals specified in $c'$.
    
%     \item GST is set to after all processes in $\processes{c'}$ have taken a computational step.
% \end{compactenum}
% For every process $P_i \in \processes{c'} \cap \processes{c}$, the proposal of $P_i$ in $\mathcal{E}'$ is $\mathsf{proposal}(c'[i])$; recall that $c'[i] = c[i]$ as $c' \sim c$.
% Moreover, for every process $P_j \in \processes{c'} \setminus{\processes{c}}$, the proposal of $P_j$ in $\mathcal{E}'$ is $\mathsf{proposal}(c'[j])$ (due to the step 3 of the construction).

==> sections/suggestions.tex <==
\section{Suggestions (Pierre)}

\subsection{Lemma 1 and lemma 2 as a consequence of a more general lemma}

Let's fix
\begin{itemize}
    \item $(P,Q,R)$ is a partition of the processes
    \item $t_S, t_Q \in \mathbb{N}, t_S + t_Q \leq t + 1$
    \item $|P|> t_S $
    \item $|Q| \geq t_Q$
    \item $|R|\leq t-t_S-t_Q+1$
    
    \item $\mathcal{A}$ is a synchronous protocol that solves non-uniform weak agreement in the omission model
\end{itemize}

Let $\mathcal{E}$ be an execution of $\mathcal{A}$ such that:
\begin{itemize}
    \item Every process in $P$ is correct and eventually decides $b_P$.
    \item Every process in $Q$ is receive-isolated after some round $k$.
    \item Every process in $R$ is faulty.
\end{itemize}

\begin{lemma}\label{lemma:0}
If there exists $t_{Q'} \in \mathbb{N}$, such that the communication complexity of $\mathcal{A}$ is less than $(t_Q -t_{Q'}) \cdot t_S$, then $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{lemma}

\begin{proof}[proof sketch] (see figure \ref{figure:lemma_0})
First, we can remark that (*) $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$. By contradiction, assume the opposite. There exists a set $Q''$ of $|Q''|= |Q|-t_{Q'}+1 > t_Q -t_{Q'}$ processes that would receive more than $t_S$ messages. Thus, the communication complexity of $\mathcal{A}$ would be strictly greater than $(t_Q -t_{Q'}) \cdot t_S$.

Let $q_i \in Q'$.
Let $S_i$ be the set of processes in $P$ that have sent at least 1 message after round $k$ (including) to process $q_i$ in execution $\mathcal{E}$.
By (*), $|S_i| \leq t_S$.
We can construct an execution $\mathcal{E}_i$ s.t. behaviour of every process except the ones in $R \cup S_i \cup \{q_i\}$ are unchanged. Every message receive-omitted by process $q_i$ in execution $\mathcal{E}$ is now send-omitted by $R \cup S_i$. the rest remains unchanged. By agreement, termination, and correctness, $q_i$ must decide in $\mathcal{E}_i$ the same value than $P \setminus S_i \neq \emptyset$, that is $b_P$.
Since, the behaviours of $q_i$ in $\mathcal{E}$ and $\mathcal{E}_i$ are equivalent, $q_i$ must decide $b_P$ in $\mathcal{E}$.

Hence, every process $q_j \in Q'$ decides $b_P$ in $\mathcal{E}$.
\end{proof}


\begin{figure}[!t]
\centering
\includegraphics[width=15cm]{figures/quadratic_lower_bound_lemma_0_vector.eps}
\caption{Lemma \ref{lemma:0}}
\label{figure:lemma_0}
\end{figure}

%%%%%%%%%%%%%%%%%%
%% formal proof %%
%%%%%%%%%%%%%%%%%%
\begin{proof}[formal proof]
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Due to the statement of the lemma, $\mathcal{F} = Q \uplus R$.
Moreover, no process in $P \uplus Q$ commits any send-omission failure in $\mathcal{E}$: for every process $P_i \in P \uplus Q$ and every round $j \in \mathbb{N}^+ \cup \{+\infty\}$, $\mathsf{send\_omitted}(\mathcal{B}_i, j) = \emptyset$.

For every set of processes $U$, we note $M_{U} = \bigcup\limits_{P_i \in U} \big( \bigcup\limits_{k' \geq k}  \fmsgs{\mathcal{B}_i}{k'} \big)$ to denote the set of messages sent by processes in $U$ from (and including) round $k$ onward in $\mathcal{E}$.

For every pair of sets of processes $(U, V)$, we define $M_{U \to V}$ as the set containing all messages sent to a process in $V$ by processes in $U$ from (and including) round $k$ onward of $\mathcal{E}$:
\begin{equation*}
    M_{U \to V} = \{ m \,|\, m \in M_{U} \land m.\mathsf{receiver} \in V \}.
\end{equation*}
Note that, for every $P_i \in Q$, each message $m \in M_{(P \uplus R) \to \{P_i\}}$ is receive-omitted in $\mathcal{B}_i$.

First, we will prove by contradiction that $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$ from processes in $P$. Therefore, assume that there exists a subset $Q'' \subseteq Q$ of $|Q''| > |Q|-t_Q \geq t_Q-t_{Q'}$ processes which receive more than $t_S$ messages in $\mathcal{E}$ from processes in $P$.
As $\mathcal{A}$ sends less than $(t_Q-t_{Q'})\cdot t_S$ messages in execution $\mathcal{E}$, less than $(t_Q-t_{Q'})\cdot t_S$ messages are sent in $\mathcal{E}$ by correct processes (i.e., processes in $P$), which implies $|M_{P \to \tilde{Q}'}| < (t_Q-t_{Q'})\cdot t_S$, thus we reach a contradiction. Hence, $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$ from processes in $P$, i.e. $\forall P_i \in Q', |M_{P \to \{P_i\}}| \leq t_S$.

Let $P_i \in Q'$.
Let $S_i$ denote the set of processes in $P$ whose messages $P_i$ receive-omits from (and including) round $k$ onward in $\mathcal{B}_i$:
\begin{equation*}
    S_i = \{ P_j \in P \,|\, \exists j \in [k, \infty], \exists m \in \fmsgro{\mathcal{B}_i}{j}: m.\mathsf{sender} = P_j \}.
\end{equation*}
Note that $P_i \notin S_i$ (as no process ever sends messages to itself).
Moreover, as $|M_{P \to \{P_i\}}| \leq t_S$, $|S_i| \leq t_S$.
We now create another execution $\mathcal{E}'_i = [\mathcal{F}', \mathcal{B}_1', ..., \mathcal{B}_n']$:
\begin{compactenum}
    \item $\mathcal{F}' \gets S_i \uplus R \uplus (Q \setminus{ \{P_i\}})$.

    \item For every process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, let $\mathcal{B}_j' \gets \mathcal{B}_j$, i.e., $P_j$'s behavior in $\mathcal{E}'$ is identical to $P_j$'s behavior in $\mathcal{E}_i$.

    \item For the process $P_i$, we build $\mathcal{B}_i'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_i' \gets \mathcal{B}_i$.

        \item For every round $k' \in [k, \infty]$ such that $\fmsgro{\mathcal{B}_i}{k'} \neq \emptyset$, we remove all messages from $\fmsgro{\mathcal{B}'_i}{k'}$: $\fmsgro{\mathcal{B}'_i}{k'} \gets \emptyset$.
        Note that all messages removed from $\fmsgro{\mathcal{B}'_i}{k'}$ are sent by processes in $S_i \uplus R$.
    \end{compactenum}
    Note that $P_i$ does not commit any omission faults in $\mathcal{B}_i'$: (1) it does not commit any send-omission faults due to the statement of the lemma, and (2) it does not commit any receive-omission faults due to the step (3)(b). 

    \item For every process $P_j \in S_i \uplus R$, we build $\mathcal{B}_j'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_j' \gets \mathcal{B}_j$.

        \item For every message $m$ such that there exists a round $k' \geq [k, \infty]$ with (1) $m \in \fmsgs{\mathcal{B}_j}{k'}$, and (2) $m \in \fmsgro{\mathcal{B}_i}{k'}$, we perform the following steps:
        \begin{compactenum}
            \item We remove $m$ from sent messages: $\fmsgs{\mathcal{B}_j'}{k'} \gets \fmsgs{\mathcal{B}_j'}{k'} \setminus{\{m\}}$.

            \item We add $m$ to send-omitted messages:
            $\fmsgso{\mathcal{B}_j'}{k'} \gets \fmsgso{\mathcal{B}_j'}{k'} \cup \{m\}$.
        \end{compactenum}
    \end{compactenum}
\end{compactenum}

Let us prove that $\mathcal{E}_i'$ is indeed an execution:
\begin{compactitem}
    \item Faulty processes: As $\mathcal{F}' \subseteq S_i \uplus R \uplus (Q \setminus{\{ P_i \}})$ and $|R| \leq t-t_S-t_Q+1$, thus $|\mathcal{F}'| \leq t$. Potentially, some processes in $R$ are now correct.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore:
    \begin{compactitem}
        \item For any process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ since $\mathcal{B}_j' = \mathcal{B}_j$. 
        \item For process $P_i$, $\mathcal{B}_i'$ is an infinite behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
        \item For any process $P_j \in R \uplus S_i$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ due to \Cref{lemma:behavior_send_transfer}. 
    \end{compactitem}
    

    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$).
    We consider two possibilities:
    \begin{compactitem}
        \item If $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (3)(b), then $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ as $m$ is included in step (3)(a).

        \item Otherwise, $m$ is excluded by step (3)(b).
        This implies that $j \geq k$, $P_r = P_i$, $P_s \in S_i \uplus R$, $m \in \fmsgro{\mathcal{B}_r}{j}$ and $m \in \fmsgs{\mathcal{B}_s}{j}$.
        Then, by step (4)(b)(i), $m \notin \fmsgs{\mathcal{B}_s'}{j}$ making this case impossible.
    \end{compactitem}
    Send-validity is satisfied in $\mathcal{E}'_i$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $j \geq k$ and $P_r = P_i$ and $m \in \fmsgro{\mathcal{B}_r}{j}$.
        However, this case is impossible as $m \notin \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ due to the step (3)(b).

        \item Otherwise, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
        Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (4)(b)(i) while constructing $\mathcal{B}_s'$.
    \end{compactitem}
    Receive-validity is satisfied in $\mathcal{E}'_i$.

    \item Omission-validity:
    Consider a process $P_j$ which commits an omission-fault in $\mathcal{B}_j'$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $P_j$ commit a send-omission fault in $\mathcal{B}_j'$.
        As no process $P_z \in \Pi \setminus R$ commits a send-omission fault in $\mathcal{B}_z$, $P_j \in R \uplus S_i$ given that we only add send-omitted messages to processes in $R \uplus S_i$. Hence, $P_j \in \mathcal{F}'$.
        In this case, omission-validity is satisfied.

        \item Let $P_j$ commit a receive-omission fault in $\mathcal{B}_j'$.
        Note that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z$, which implies that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z'$ (as our construction does not add receive-omitted messages to any process).
        
        Moreover, $P_i$ does not commit a receive-omission fault in $\mathcal{B}_i'$ as (1) it does not commit any receive-omission faults in any round $k' \in [1, k - 1]$ in $\mathcal{B}_i$ (due to \Cref{definition:isolation}), and (2) all receive-omitted messages in any round $k' \in [k, \infty]$ are removed by the step (3)(b).
        Therefore, $P_j \in R \uplus (Q \setminus{\{P_i\}})$, which means that omission-validity holds in this case as well.
    \end{compactitem}
    Omission-validity is satisfied in $\mathcal{E}'_i$.
\end{compactitem}
Thus, $\mathcal{E}'_i$ is indeed an execution of $\mathcal{A}$.

Since $|P|>t_S$, $|S_i|\leq t_S$, $\exists P_j \in P \setminus S_i \neq \emptyset$.

Observe that $P_i$ and $P_j$ are correct in $\mathcal{E}'_i$, and $\mathcal{B}'_j = \mathcal{B}_j$.
Hence, they both decide the same value $b$.

Moreover (1) $P_i$'s states in $\mathcal{B}_i'$ and $\mathcal{B}_i$ are identical, and (2) $P_j$'s states in $\mathcal{B}_j'$ and $\mathcal{B}_j$ are identical.
Therefore, $P_i$ decides $b$ in $\mathcal{E}$.
Thus, every process in $Q'$ decides $b$ in $\mathcal{E}$.
Hence, the lemma holds.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%
%% end formal proof %%
%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}
If $t_Q = 2t_{Q'}$, and the communication complexity of $\mathcal{A}$ is less than $t_{Q'} \cdot t_S$, then $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{corollary}

\begin{lemma}
Lemma \ref{lemma:forced_termination}
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $|R|=0$, $P = \bar{X}$, $Q = X$ with $t_S = t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$.
\end{proof}

\begin{lemma}
Lemma \ref{lemma:disagreement_quadratic_messages}
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $(Q,R)=(B,C)$ (resp. $(Q,R)=(C,B)$), $P = A$, $t_S = \frac{t}{2}, t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$. We verify $|R| = \frac{t}{4} \leq t-t_S - t_Q+1 = \frac{t}{4} +1$. 

\end{proof}

\begin{lemma}
Lemma \ref{lemma:either} (lemma 3):
Let $\mathcal{E}_0$ and $\mathcal{E}_1$ as presented in figure \ref{figure:lemma_3}.
There exists a set $B' \subset B$ of $|B'| = \frac{t}{4}$ processes that decide $1$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{4}$ processes that decide $0$ in $\mathcal{E}_1$.
\end{lemma}

\begin{proof}
(see figure \ref{figure:lemma_3})
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{4}$ processes that decide $b$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{4}$ processes that decide $b'$ in $\mathcal{E}_1$.
\pierre{it seems to me we can avoid the set of size $\frac{|B|}{4}$ (resp. $\frac{|C|}{4}$ invoked in the proof of lemma \ref{lemma:either} (lemma 3). The remaining part is the same.}
By contratiction, assume $b=0$ and $b'=1$. Let's construct a new infinite execution $\mathcal{E}^{*}$, such that $\mathcal{E}^{*}|_{B} = \mathcal{E}_0|_{B}$ and $\mathcal{E}^{*}|_{C} = \mathcal{E}_1|_{C}$:

\begin{compactenum}
    \item In $\mathcal{E}^*$, all processes from $A \cup B$ propose $0$, whereas all processes from $C$ propose $1$.

    \item All processes from $A$ are correct, whereas all processes from $B \cup C$ are faulty.
    Note that $|B \cup C| < t$.

    \item Every process from $B$ exhibits the exact same behavior as in $\mathcal{E}_0$.
    Note that this step implies that $B$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    \item Every process from $C$ exhibits the exact same behavior as in $\mathcal{E}_1$.
    Note that this step implies that $C$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    % \item Both groups $B$ and $C$ are receive-isolated from round $1$.
\end{compactenum}
Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages}, correct processes send at least $\frac{t^2}{32}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{32}$ (or even $\frac{t^2}{16}$) messages in every execution.
Thus, the lemma holds.
\end{proof}

\begin{figure}[!t]
\centering
\includegraphics[width=15cm]{figures/quadratic_lower_bound_lemma_3.eps}
\caption{Lemma \ref{lemma:either}}
\label{figure:lemma_3}
\end{figure}

Then, we define the execution $\mathcal{E}_C, \mathcal{E}^{k^{*}}$, and $\mathcal{E}^{k^{*}+1}$ as in the prologue of lemma \ref{lemma:final} (lemma 4), and illustrated in figure \ref{figure:execution_C}.

\begin{figure}[!t]
\centering
\includegraphics[width=15cm]{figures/quadratic_lower_bound_execution_C.eps}
\caption{Execution $\mathcal{E}_C$}
\label{figure:execution_C}
\end{figure}

\begin{lemma} Lemma \ref{lemma:final} (lemma 4).
There exists an execution of $\mathcal{A}$ in which correct processes send (at least) $\frac{t^2}{32}$ messages.
\end{lemma}
\begin{proof}
(see figure \ref{figure:lemma_4})
We consider two possible cases:
\begin{compactitem}
    \item Let $b_C = 0$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Both groups $B$ and $C$ are receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^*}$ (from round $k^*$ onward).
        Note that this step implies that $B$ is receive-isolated from round $k^*$.

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item From (and including) round $k^*$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.

% this is pointless, by item 4. not really, will change something more
        % \item From (and including) round $k^*$ onward, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$ in $\mathcal{E}^k$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$ in $\mathcal{E}_C$.
    \end{compactenum}
    
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $1$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $0$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.

    \item Let $b_C = 1$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}+1}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Group $C$ is receive-isolated from round $k^*$, whereas group $B$ is receive-isolated from round $k^*+1$

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^* + 1}$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^* + 1$.
        \add{Note that the message received in round $k^{*}$ from processes in $C$ are indeed the same ones than in execution $\mathcal{E}^{k^* + 1}$, since the receive-omission at round $k^*$ has no impact of the messages at the same round $k^*$.} 

        \item In round $k^*$, all messages from $C$ are received, which means that processes in $B$ successfully receive messages sent by $C$.

        \item From (and including) round $k^* + 1$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.
        
        
        % we send-omit (1) all messages sent by processes in $C$ to processes in $A$ in $\mathcal{E}_C$.
        % Note that, in round $k^*$, messages sent by processes in $C$ to processes in $B$ are successfully sent and successfully received.

        % \item From round $k^* + 1$, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$.
    \end{compactenum}
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $0$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $1$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.
\end{compactitem}
As the statement of the lemma holds in both possible cases, the proof is concluded.
\end{proof}

\begin{figure}[!t]
\centering
\includegraphics[width=15cm]{figures/quadratic_lower_bound_lemma_4.eps}
\caption{Lemma \ref{lemma:final}}
\label{figure:lemma_4}
\end{figure}

\iffalse
\subsection{Formalism}

It seems to me that it would be easier to see a (valid) execution as a \emph{consistent} set of $n$ (valid) \emph{behaviours}.
I would see a \emph{(valid) round-behaviour} as a tuple $(s, M^{r/o}, M^{r}, s', M^{s/o}, M^{s})$, such that $(s', M^{s/o} \uplus M^{s}) = \mathcal{A}(s, M^{r})$, while $M^{s/o}$ represents the send-omitted messages, $M^{o/r}$ represents the receive-omitted messages, $M^{s}$ represents the sent messages, $M^{r}$ represents the received messages. 
I would see a \emph{(valid) behaviour} as a sequence of valid behaviours, with the obvious properties (e.g. $s_{k+1} = s'_k$).
A process would be correct if its behaviour only counts round-behaviours of the form $(s_k, \emptyset, M^{r}_{k}, s_k', \emptyset, M^{s}_{k})$.
For any set of messages $M$ concerning one round of one execution, we note $M|_{i \rightarrow j}$ the message sent by $i$ to $j$, if it exists, $\bot$ otherwise.
I would see a valid execution as a set of valid behaviours such that:
\begin{itemize}
    \item A message $m$ can be receive-omitted or received only if has been sent in the same round.
    \item If a message is sent at round $k$, it is necessarily either received or receive-omitted at round $k$.
\end{itemize}
These two last properties can be written for every pair of process $(i,j)$, for every round $k$, $M^{s}_k|_{i \rightarrow j} = (M^{r}_k \uplus M^{r/o}_k)|_{i \rightarrow j}$.
We can also write $M^{s}_k|_{. \rightarrow j} = (M^{r}_k \uplus M^{r/o}_k)|_{. \rightarrow j}$ with the obvious meaning.


%for every pair of behavior $(\beta_i, \beta_j)$, for every round $r$, for the corresponding round-behaviours $(\gamma_i, \gamma_j) \triangleq ((s_i, M^{o}_{in, i}, M^{r}_{in, i}, s_i', M^{o}_{out, i}, M^{s}_{out, i}), (s_j, M^{o}_{in, j}, M^{r}_{in, j}, s_j', M^{o}_{out, j}, M^{s}_{out, j})) \triangleq (\beta_i[r], \beta_j[r]) $, 
\fi

\paragraph*{Modularity in proofs}

\begin{definition}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
We note $\mathcal{E}^{M \rightleftarrows} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$ the execution such that, for every process $P_i \in \Pi$:
\begin{compactenum}
    \item $\mathcal{B}'_i \gets \mathcal{B}_i$
    
    \item $\forall j \in [1:k]$, $\fmsgro{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgro{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_receive_omission}
    
    \item $\forall j \in [1:k]$, $\fmsgso{\mathcal{B}'_i}{j}$ $ \gets \fmsgso{\mathcal{B}'_i}{j} $ $\cup \{m \in M | m.\mathit{round} = j \wedge m.\mathit{sender} = P_i\}$ \label{item:add_send_omission}

    \item $\forall j \in [1:k]$, $\fmsgs{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgs{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_send}
    
    \item $\mathcal{F}' = \{P_i \in \Pi \; | \bigcup\limits_{k' \in [1:k]} ( \fmsgso{\mathcal{B}_i}{k'} \cup \fmsgro{\mathcal{B}_i}{k'} ) \neq \emptyset\}$ \label{item:faulty_processes}
\end{compactenum}
\end{definition}

Intuitively, $\mathcal{E}^{M \rightleftarrows}$ corresponds to the execution $\mathcal{E}$, where every receive-omitted message is send-omitted instead.

\begin{lemma}
    .Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
Let $\fswitcho{\mathcal{E}}{M} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$. 
If $|\mathcal{F}'| \leq t$, then $\mathcal{E}^{M \rightleftarrows}$ is a valid execution.
\end{lemma}

\begin{proof}
$\;$
\begin{compactitem}
 \item Faulty processes: $|\mathcal{F}'| \leq t$ is a precondition of the lemma.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$). Necessarily $m \notin M$ by step (\ref{item:remove_send}). Thus, $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and so $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ by Send-Validity of $\mathcal{E}$.
    
    Send-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$. Necessarily, $m \notin M$. Indeed, if $m \in M$, $m \in \fmsgro{\mathcal{B}_r}{j} \setminus \fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and $m \notin \in \fmsgr{\mathcal{B}'_r}{j}$, since $\fmsgr{\mathcal{B}'_r}{j} = \fmsgr{\mathcal{B}_r}{j}$ by construction and $\fmsgr{\mathcal{B}_r}{j} \cap \fmsgro{\mathcal{B}_r}{j} = \emptyset$, since $\mathcal{B}_r$ is a behavior of process $P_r$.

    Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (\ref{item:remove_send}) while constructing $\mathcal{B}_s'$.
    
    Receive-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.
    
    \item Omission-validity is obviously satisfied in $\fswitcho{\mathcal{E}}{M}$. by step (\ref{item:faulty_processes}).
\end{compactitem}
Thus, $\fswitcho{\mathcal{E}}{M}$. is indeed an execution of $\mathcal{A}$. 
\end{proof}

\pierre{TO DO}

\begin{definition}
Let $P = \{P_{i_1}, ..., P_{i_{\ell}}\}$ be a set of correct processes and $M$ be a set of messages not sent by processes in $P$, i.e. $\forall m \in M, m.\mathit{sender} \notin P$.
For every $k \in \mathbb{N} \cup \{\infty\}$,
We define $\mathit{correct}(P,M,k) \triangleq [\mathcal{B}_{i_1}, ..., \mathcal{B}_{i_{\ell}}]$, as follows.

\begin{compactenum}
    \item (Initialisation)

    \item $\mathcal{B}_{i}[j+1] = (s_{j+1}, M_{j+1}^{s},\emptyset, M^{r}_{j+1}, \emptyset)$ s.t. (1) $M^{r}_{j+1} = \{m \in M | m.\mathit{round} = j+1, m.\mathit{receiver} = P_i\} \cup \{m \in \bigcup_{i} M^{s,i}_{j+1} | m.\mathit{receiver} = P_i\}$ and (2) $(s_{j+1}, M_{j+1}^{s}) = \mathcal{A}(s'_{j}, M_{j}^{r})$
\end{compactenum}
\end{definition}

\begin{lemma}
Let $P = \{P_{i_1}, ..., P_{i_{\ell}}\}$ be a set of correct processes and $M$ be a set of messages not sent by processes in $P$, i.e. $\forall m \in M, m.\mathit{sender} \notin P$.
For every $k \in \mathbb{N} \cup \{\infty\}$, $\mathit{correct}(P,M,k) \triangleq [\mathcal{B}_{i_1}, ..., \mathcal{B}_{i_{\ell}}]$, is a tuple of correct behaviours.
\end{lemma}

==> sections/suggestions_2.tex <==
\section{Suggestions (Pierre)}

\cite{dolev1985bounds}

\subsection{Lemma 1 and lemma 2 as a consequence of a more general lemma}

\begin{definition}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
We note $\mathcal{E}^{M \rightleftarrows} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$ the execution such that, for every process $P_i \in \Pi$:
\begin{compactenum}
    \item $\mathcal{B}'_i \gets \mathcal{B}_i$
    
    \item $\forall j \in [1:k]$, $\fmsgro{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgro{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_receive_omission}
    
    \item $\forall j \in [1:k]$, $\fmsgso{\mathcal{B}'_i}{j}$ $ \gets \fmsgso{\mathcal{B}'_i}{j} $ $\cup \{m \in M | m.\mathit{round} = j \wedge m.\mathit{sender} = P_i\}$ \label{item:add_send_omission}

    \item $\forall j \in [1:k]$, $\fmsgs{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgs{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_send}
    
    \item $\mathcal{F}' = \{P_i \in \Pi \; | \bigcup\limits_{k' \in [1:k]} ( \fmsgso{\mathcal{B}_i}{k'} \cup \fmsgro{\mathcal{B}_i}{k'} ) \neq \emptyset\}$ \label{item:faulty_processes}
\end{compactenum}
\end{definition}

Intuitively, $\mathcal{E}^{M \rightleftarrows}$ corresponds to the execution $\mathcal{E}$, where every receive-omitted message is send-omitted instead.

\begin{lemma}\label{lemma:switch_omission}
    .Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
Let $\fswitcho{\mathcal{E}}{M} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$. 
If $|\mathcal{F}'| \leq t$, then $\mathcal{E}^{M \rightleftarrows}$ is a valid execution.
\end{lemma}

\begin{proof}
$\;$
\begin{compactitem}
 \item Faulty processes: $|\mathcal{F}'| \leq t$ is a precondition of the lemma.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$). Necessarily $m \notin M$ by step (\ref{item:remove_send}). Thus, $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and so $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ by Send-Validity of $\mathcal{E}$.
    
    Send-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$. Necessarily, $m \notin M$. Indeed, if $m \in M$, $m \in \fmsgro{\mathcal{B}_r}{j} \setminus \fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and $m \notin \in \fmsgr{\mathcal{B}'_r}{j}$, since $\fmsgr{\mathcal{B}'_r}{j} = \fmsgr{\mathcal{B}_r}{j}$ by construction and $\fmsgr{\mathcal{B}_r}{j} \cap \fmsgro{\mathcal{B}_r}{j} = \emptyset$, since $\mathcal{B}_r$ is a behavior of process $P_r$.

    Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (\ref{item:remove_send}) while constructing $\mathcal{B}_s'$.
    
    Receive-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.
    
    \item Omission-validity is obviously satisfied in $\fswitcho{\mathcal{E}}{M}$. by step (\ref{item:faulty_processes}).
\end{compactitem}
Thus, $\fswitcho{\mathcal{E}}{M}$. is indeed an execution of $\mathcal{A}$. 
\end{proof}



\begin{lemma}\label{lemma:0}
Let's fix
\begin{itemize}
    \item $(P,Q,R)$ is a partition of the processes
    \item $t_S, t_Q \in \mathbb{N}, t_S + t_Q \leq t + 1$
    \item $|P|> t_S $
    \item $|Q| \geq t_Q$
    \item $|R|\leq t-t_S-t_Q+1$
    
    \item $\mathcal{A}$ is a synchronous protocol that solves non-uniform weak agreement in the omission model
\end{itemize}

Let $\mathcal{E}$ be an execution of $\mathcal{A}$ such that:
\begin{itemize}
    \item Every process in $P$ is correct and eventually decides $b_P$.
    \item Every process in $Q$ is receive-isolated after some round $k$.
    \item Every process in $R$ is faulty.
\end{itemize}

If there exists $t_{Q'} \in \mathbb{N}$, such that the communication complexity of $\mathcal{A}$ is less than $(t_Q -t_{Q'}) \cdot t_S$, then $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{lemma}

\begin{proof}[proof sketch] (see figure \ref{figure:lemma_0})
First, we can remark that (*) $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$. By contradiction, assume the opposite. There exists a set $Q''$ of $|Q''|= |Q|-t_{Q'}+1 > t_Q -t_{Q'}$ processes that would receive more than $t_S$ messages. Thus, the communication complexity of $\mathcal{A}$ would be strictly greater than $(t_Q -t_{Q'}) \cdot t_S$.

Let $q_i \in Q'$.
Let $S_i$ be the set of processes in $P$ that have sent at least 1 message after round $k$ (including) to process $q_i$ in execution $\mathcal{E}$.
By (*), $|S_i| \leq t_S$.
We can construct an execution $\mathcal{E}_i$ s.t. behaviour of every process except the ones in $R \cup S_i \cup \{q_i\}$ are unchanged. Every message receive-omitted by process $q_i$ in execution $\mathcal{E}$ is now send-omitted by $R \cup S_i$. the rest remains unchanged. By agreement, termination, and correctness, $q_i$ must decide in $\mathcal{E}_i$ the same value than $P \setminus S_i \neq \emptyset$, that is $b_P$.
Since, the behaviours of $q_i$ in $\mathcal{E}$ and $\mathcal{E}_i$ are equivalent, $q_i$ must decide $b_P$ in $\mathcal{E}$.

Hence, every process $q_j \in Q'$ decides $b_P$ in $\mathcal{E}$.
\end{proof}


\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_0_vector.eps}
\caption{Lemma \ref{lemma:0}}
\label{figure:lemma_0}
\end{figure}

%%%%%%%%%%%%%%%%%%
%% formal proof %%
%%%%%%%%%%%%%%%%%%
\begin{proof}[formal proof]
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Due to the statement of the lemma, $\mathcal{F} = Q \uplus R$.
Moreover, no process in $P \uplus Q$ commits any send-omission failure in $\mathcal{E}$: for every process $P_i \in P \uplus Q$ and every round $j \in \mathbb{N}^+ \cup \{+\infty\}$, $\mathsf{send\_omitted}(\mathcal{B}_i, j) = \emptyset$.

For every set of processes $U$, we note $M_{U} = \bigcup\limits_{P_i \in U} \big( \bigcup\limits_{k' \geq k}  \fmsgs{\mathcal{B}_i}{k'} \big)$ to denote the set of messages sent by processes in $U$ from (and including) round $k$ onward in $\mathcal{E}$.

For every pair of sets of processes $(U, V)$, we define $M_{U \to V}$ as the set containing all messages sent to a process in $V$ by processes in $U$ from (and including) round $k$ onward of $\mathcal{E}$:
\begin{equation*}
    M_{U \to V} = \{ m \,|\, m \in M_{U} \land m.\mathsf{receiver} \in V \}.
\end{equation*}
Note that, for every $P_i \in Q$, each message $m \in M_{(P \uplus R) \to \{P_i\}}$ is receive-omitted in $\mathcal{B}_i$.

First, we will prove by contradiction that $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$ from processes in $P$. Therefore, assume that there exists a subset $Q'' \subseteq Q$ of $|Q''| > |Q|-t_Q \geq t_Q-t_{Q'}$ processes which receive more than $t_S$ messages in $\mathcal{E}$ from processes in $P$.
As $\mathcal{A}$ sends less than $(t_Q-t_{Q'})\cdot t_S$ messages in execution $\mathcal{E}$, less than $(t_Q-t_{Q'})\cdot t_S$ messages are sent in $\mathcal{E}$ by correct processes (i.e., processes in $P$), which implies $|M_{P \to \tilde{Q}'}| < (t_Q-t_{Q'})\cdot t_S$, thus we reach a contradiction. Hence, $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$ from processes in $P$, i.e. $\forall P_i \in Q', |M_{P \to \{P_i\}}| \leq t_S$.

Let $P_i \in Q'$.
Let $S_i$ denote the set of processes in $P$ whose messages $P_i$ receive-omits from (and including) round $k$ onward in $\mathcal{B}_i$:
\begin{equation*}
    S_i = \{ P_j \in P \,|\, \exists j \in [k, \infty], \exists m \in \fmsgro{\mathcal{B}_i}{j}: m.\mathsf{sender} = P_j \}.
\end{equation*}
Note that $P_i \notin S_i$ (as no process ever sends messages to itself).
Moreover, as $|M_{P \to \{P_i\}}| \leq t_S$, $|S_i| \leq t_S$.
We now create another execution $\mathcal{E}'_i = [\mathcal{F}', \mathcal{B}_1', ..., \mathcal{B}_n'] = \fswitcho{\mathcal{E}}{\tilde{M}_i}$ where $\tilde{M}_i = M_{(P \uplus R) \to \{P_i\}}$.
We can observe that $P_i$ is correct in $\mathcal{E}'_i$.
Hence, $\mathcal{F}' \subseteq S_i \uplus R \uplus (Q \setminus{\{ P_i \}})$ and $|R| \leq t-t_S-t_Q+1$, thus $|\mathcal{F}'| \leq t$. 
Let us note that some processes in $R$ might be now correct.
By lemma \ref{lemma:switch_omission}, $\mathcal{E}'_i$ is an execution of $\mathcal{A}$.
\iffalse
:
\begin{compactenum}
    \item $\mathcal{F}' \gets S_i \uplus R \uplus (Q \setminus{ \{P_i\}})$.

    \item For every process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, let $\mathcal{B}_j' \gets \mathcal{B}_j$, i.e., $P_j$'s behavior in $\mathcal{E}'$ is identical to $P_j$'s behavior in $\mathcal{E}_i$.

    \item For the process $P_i$, we build $\mathcal{B}_i'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_i' \gets \mathcal{B}_i$.

        \item For every round $k' \in [k, \infty]$ such that $\fmsgro{\mathcal{B}_i}{k'} \neq \emptyset$, we remove all messages from $\fmsgro{\mathcal{B}'_i}{k'}$: $\fmsgro{\mathcal{B}'_i}{k'} \gets \emptyset$.
        Note that all messages removed from $\fmsgro{\mathcal{B}'_i}{k'}$ are sent by processes in $S_i \uplus R$.
    \end{compactenum}
    Note that $P_i$ does not commit any omission faults in $\mathcal{B}_i'$: (1) it does not commit any send-omission faults due to the statement of the lemma, and (2) it does not commit any receive-omission faults due to the step (3)(b). 

    \item For every process $P_j \in S_i \uplus R$, we build $\mathcal{B}_j'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_j' \gets \mathcal{B}_j$.

        \item For every message $m$ such that there exists a round $k' \geq [k, \infty]$ with (1) $m \in \fmsgs{\mathcal{B}_j}{k'}$, and (2) $m \in \fmsgro{\mathcal{B}_i}{k'}$, we perform the following steps:
        \begin{compactenum}
            \item We remove $m$ from sent messages: $\fmsgs{\mathcal{B}_j'}{k'} \gets \fmsgs{\mathcal{B}_j'}{k'} \setminus{\{m\}}$.

            \item We add $m$ to send-omitted messages:
            $\fmsgso{\mathcal{B}_j'}{k'} \gets \fmsgso{\mathcal{B}_j'}{k'} \cup \{m\}$.
        \end{compactenum}
    \end{compactenum}
\end{compactenum}

Let us prove that $\mathcal{E}_i'$ is indeed an execution:
\begin{compactitem}
    \item Faulty processes: As $\mathcal{F}' \subseteq S_i \uplus R \uplus (Q \setminus{\{ P_i \}})$ and $|R| \leq t-t_S-t_Q+1$, thus $|\mathcal{F}'| \leq t$. Potentially, some processes in $R$ are now correct.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore:
    \begin{compactitem}
        \item For any process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ since $\mathcal{B}_j' = \mathcal{B}_j$. 
        \item For process $P_i$, $\mathcal{B}_i'$ is an infinite behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
        \item For any process $P_j \in R \uplus S_i$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ due to \Cref{lemma:behavior_send_transfer}. 
    \end{compactitem}
    

    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$).
    We consider two possibilities:
    \begin{compactitem}
        \item If $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (3)(b), then $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ as $m$ is included in step (3)(a).

        \item Otherwise, $m$ is excluded by step (3)(b).
        This implies that $j \geq k$, $P_r = P_i$, $P_s \in S_i \uplus R$, $m \in \fmsgro{\mathcal{B}_r}{j}$ and $m \in \fmsgs{\mathcal{B}_s}{j}$.
        Then, by step (4)(b)(i), $m \notin \fmsgs{\mathcal{B}_s'}{j}$ making this case impossible.
    \end{compactitem}
    Send-validity is satisfied in $\mathcal{E}'_i$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $j \geq k$ and $P_r = P_i$ and $m \in \fmsgro{\mathcal{B}_r}{j}$.
        However, this case is impossible as $m \notin \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ due to the step (3)(b).

        \item Otherwise, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
        Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (4)(b)(i) while constructing $\mathcal{B}_s'$.
    \end{compactitem}
    Receive-validity is satisfied in $\mathcal{E}'_i$.

    \item Omission-validity:
    Consider a process $P_j$ which commits an omission-fault in $\mathcal{B}_j'$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $P_j$ commit a send-omission fault in $\mathcal{B}_j'$.
        As no process $P_z \in \Pi \setminus R$ commits a send-omission fault in $\mathcal{B}_z$, $P_j \in R \uplus S_i$ given that we only add send-omitted messages to processes in $R \uplus S_i$. Hence, $P_j \in \mathcal{F}'$.
        In this case, omission-validity is satisfied.

        \item Let $P_j$ commit a receive-omission fault in $\mathcal{B}_j'$.
        Note that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z$, which implies that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z'$ (as our construction does not add receive-omitted messages to any process).
        
        Moreover, $P_i$ does not commit a receive-omission fault in $\mathcal{B}_i'$ as (1) it does not commit any receive-omission faults in any round $k' \in [1, k - 1]$ in $\mathcal{B}_i$ (due to \Cref{definition:isolation}), and (2) all receive-omitted messages in any round $k' \in [k, \infty]$ are removed by the step (3)(b).
        Therefore, $P_j \in R \uplus (Q \setminus{\{P_i\}})$, which means that omission-validity holds in this case as well.
    \end{compactitem}
    Omission-validity is satisfied in $\mathcal{E}'_i$.
\end{compactitem}

Thus, $\mathcal{E}'_i$ is indeed an execution of $\mathcal{A}$.
\fi
Since $|P|>t_S$, $|S_i|\leq t_S$, $\exists P_j \in P \setminus S_i \neq \emptyset$.

Observe that $P_i$ and $P_j$ are correct in $\mathcal{E}'_i$, and $\mathcal{B}'_j = \mathcal{B}_j$.
Hence, they both decide the same value $b$.

Moreover (1) $P_i$'s states in $\mathcal{B}_i'$ and $\mathcal{B}_i$ are identical, and (2) $P_j$'s states in $\mathcal{B}_j'$ and $\mathcal{B}_j$ are identical.
Therefore, $P_i$ decides $b$ in $\mathcal{E}$.
Thus, every process in $Q'$ decides $b$ in $\mathcal{E}$.
Hence, the lemma holds.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%
%% end formal proof %%
%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}
If $t_Q = 2t_{Q'}$, and the communication complexity of $\mathcal{A}$ is less than $t_{Q'} \cdot t_S$, then $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{corollary}

\begin{lemma}\label{lemma:forced_termination_new}
Lemma \ref{lemma:forced_termination}
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $|R|=0$, $P = \bar{X}$, $Q = X$ with $t_S = t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$.
\end{proof}

\begin{lemma}\label{lemma:disagreement_quadratic_messages_new}
Lemma \ref{lemma:disagreement_quadratic_messages}
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $(Q,R)=(B,C)$ (resp. $(Q,R)=(C,B)$), $P = A$, $t_S = \frac{t}{2}, t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$. We verify $|R| = \frac{t}{4} \leq t-t_S - t_Q+1 = \frac{t}{4} +1$. 

\end{proof}




\begin{definition}
Let $P = \{P_{i_1}, ..., P_{i_{\ell}}\}$ be a set of correct processes proposing $b =(b_{i_1}, ..., b_{i_{\ell}}) \in \{0, 1\}^{\ell}$ and $M$ be a set of messages not sent by processes in $P$, i.e. $\forall m \in M, m.\mathit{sender} \notin P$.
For every $k \in \mathbb{N} \cup \{\infty\}$,
We define $\mathit{correct}(P, b,M,k) \triangleq [\mathcal{B}_{i_1}, ..., \mathcal{B}_{i_{\ell}}]$,  where each $\mathcal{B}_{i} \triangleq \langle \mathcal{F}^1_i, ..., \mathcal{F}^k_i\rangle$ is a $k$-round behavior of process $P_i$ and each $\mathcal{F}^j_i \triangleq (\state{i}{j}, \msgs{i}{j}, \emptyset, \msgr{i}{j}, \emptyset)$ as follows.

\begin{compactenum}
    \item (Initialization) $\forall P_i \in P$:
\begin{itemize}
\item  (correct proposal) $\pstate{i}{1}.\mathit{proposal} = b_i, \msgs{i}{1} = \mathcal{M}^{b_i}_i$
\item (received message) $\msgr{i}{1} = \{m \in M \cup (\bigcup_{i \in \{i_{1}, ..., i_{\ell}\}} \msgs{i}{1}) | m.\mathit{round} = 1 \wedge m.\mathit{receiver} = P_i\}$
\end{itemize}    
    \item (Induction) $\forall P_i \in P, \forall j \in [1:k]$:
    \begin{itemize}
\item  (correct transition) if $j<k$, $(\pstate{i}{j+1}, \msgs{i}{j+1}) = \mathcal{A}(\pstate{i}{j}, \msgr{i}{j})$
\item (received message) $\msgr{i}{j} = \{m \in M \cup (\bigcup_{i \in \{i_{1}, ..., i_{\ell}\}} \msgs{i}{j}) | m.\mathit{round} = j \wedge m.\mathit{receiver} = P_i\}$
\end{itemize}    
\end{compactenum}
\end{definition}

\begin{lemma}
Lemma \ref{lemma:either} (lemma 3):
Let $\mathcal{E}_0$ and $\mathcal{E}_1$ as presented in figure \ref{figure:lemma_3}.
There exists a set $B' \subset B$ of $|B'| = \frac{t}{8}$ processes that decide $1$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{8}$ processes that decide $0$ in $\mathcal{E}_1$.
\end{lemma}

\begin{proof}[proof sketch]
(see figure \ref{figure:lemma_3})
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{8}$ processes that decide $b$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{8}$ processes that decide $b'$ in $\mathcal{E}_1$.
%\pierre{it seems to me we can avoid the set of size $\frac{|B|}{4}$ (resp. $\frac{|C|}{4}$ invoked in the proof of lemma \ref{lemma:either} (lemma 3). The remaining part is the same.}
By contratiction, assume $b=0$ and $b'=1$. Let's construct a new infinite execution $\mathcal{E}^{*}$, such that $\mathcal{E}^{*}|_{B} = \mathcal{E}_0|_{B}$ and $\mathcal{E}^{*}|_{C} = \mathcal{E}_1|_{C}$:

\begin{compactenum}
    \item In $\mathcal{E}^*$, all processes from $A \cup B$ propose $0$, whereas all processes from $C$ propose $1$.

    \item All processes from $A$ are correct, whereas all processes from $B \cup C$ are faulty.
    Note that $|B \cup C| < t$.

    \item Every process from $B$ exhibits the exact same behavior as in $\mathcal{E}_0$.
    Note that this step implies that $B$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    \item Every process from $C$ exhibits the exact same behavior as in $\mathcal{E}_1$.
    Note that this step implies that $C$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    % \item Both groups $B$ and $C$ are receive-isolated from round $1$.
\end{compactenum}
Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages}, correct processes send at least $\frac{t^2}{32}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{32}$ (or even $\frac{t^2}{16}$) messages in every execution.
Thus, the lemma holds.
\end{proof}

\begin{proof}[formal proof]
We note $\mathcal{E}_0 = [\mathcal{F}_0, \mathcal{B}^{0}_1, ...,  \mathcal{B}^{0}_n]$ and $\mathcal{E}_1 = [\mathcal{F}_1, \mathcal{B}^{1}_1, ...,  \mathcal{B}^{1}_n]$.
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{4}$ processes that decide $b$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{4}$ processes that decide $b'$ in $\mathcal{E}_1$.
By contratiction, assume $b=0$ and $b'=1$. Let's construct a new infinite execution $\mathcal{E}^{*} = [\mathcal{F}^{*}, \mathcal{B}^{*}_1, ...,  \mathcal{B}^{*}_n]$, as follows:
\begin{compactenum}
\item $\mathcal{F}^{*} = B \cup C$

\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{0}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{1}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M,k)$.

\item $\forall P_i \in B\cup C$, we note $ \mathcal{B}_{i} =  \mathcal{B}^{0}_{i}$ if $P_i \in B$ and $ \mathcal{B}_{i} =  \mathcal{B}^{1}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}^{*}_{i} \gets \mathcal{B}_{i}$.

%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], \fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in \Pi \setminus \{P_i\}} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ \label{item:replace_receive_omission_in_e_star}
\end{compactenum}


Let us show that $\mathcal{E}^{*}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} = B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times (B \cup C)$, $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ is ensured by step \ref{item:replace_receive_omission_in_e_star} of the construction of $\mathcal{E}^{*}$.
\end{compactitem}
    
    
    
    Send-validity is satisfied in $\mathcal{E}^{*}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r^{*}}{j} \cup \fmsgro{\mathcal{B}_r^{*}}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times (B \cup C)$, $m \in \fmsgro{\mathcal{B}_r^{*}}{j}$, since $\fmsgr{\mathcal{B}_r^{*}}{j} = \emptyset$ by construction, because $\fmsgr{\mathcal{B}_r}{j} = \emptyset$ and no additional received messages are added during the contruction of $\mathcal{B}_r^{*}$.
Thus, $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ is ensured by step \ref{item:replace_receive_omission_in_e_star} of the construction of $\mathcal{E}^{*}$.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}^{*}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}^{*}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}^{*}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Hence, the assumption $b=0$ and $b'=1$ is false, which means that either $b=1$ or $b'=0$.
Thus, the lemma holds.

\end{proof}

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_3.eps}
\caption{Lemma \ref{lemma:either}}
\label{figure:lemma_3}
\end{figure}

Then, we define the execution $\mathcal{E}_C, \mathcal{E}^{k^{*}}$, and $\mathcal{E}^{k^{*}+1}$ as in the prologue of lemma \ref{lemma:final} (lemma 4), and illustrated in figure \ref{figure:execution_C}.

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_execution_C.eps}
\caption{Execution $\mathcal{E}_C$}
\label{figure:execution_C}
\end{figure}

\begin{lemma}[proof sketch] Lemma \ref{lemma:final} (lemma 4).
There exists an execution of $\mathcal{A}$ in which correct processes send (at least) $\frac{t^2}{32}$ messages.
\end{lemma}
\begin{proof}
(see figure \ref{figure:lemma_4})
We consider two possible cases:
\begin{compactitem}
    \item Let $b_C = 0$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Both groups $B$ and $C$ are receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^*}$ (from round $k^*$ onward).
        Note that this step implies that $B$ is receive-isolated from round $k^*$.

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item From (and including) round $k^*$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.

% this is pointless, by item 4. not really, will change something more
        % \item From (and including) round $k^*$ onward, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$ in $\mathcal{E}^k$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$ in $\mathcal{E}_C$.
    \end{compactenum}
    
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $1$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $0$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.

    \item Let $b_C = 1$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}+1}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Group $C$ is receive-isolated from round $k^*$, whereas group $B$ is receive-isolated from round $k^*+1$

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^* + 1}$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^* + 1$.
        \add{Note that the message received in round $k^{*}$ from processes in $C$ are indeed the same ones than in execution $\mathcal{E}^{k^* + 1}$, since the receive-omission at round $k^*$ has no impact of the messages at the same round $k^*$.} 

        \item In round $k^*$, all messages from $C$ are received, which means that processes in $B$ successfully receive messages sent by $C$.

        \item From (and including) round $k^* + 1$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.
        
        
        % we send-omit (1) all messages sent by processes in $C$ to processes in $A$ in $\mathcal{E}_C$.
        % Note that, in round $k^*$, messages sent by processes in $C$ to processes in $B$ are successfully sent and successfully received.

        % \item From round $k^* + 1$, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$.
    \end{compactenum}
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $0$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $1$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.
\end{compactitem}
As the statement of the lemma holds in both possible cases, the proof is concluded.
\end{proof}

\begin{proof}[formal proof]

\end{proof}

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_4.eps}
\caption{Lemma \ref{lemma:final}}
\label{figure:lemma_4}
\end{figure}







==> sections/suggestions_3.tex <==
\section{Suggestions (Pierre)}

\begin{figure}[!t]
\centering
\includegraphics[width=6cm]{figures/lemma_map.drawio.png}
\caption{Lemma Map (A draft to show what I would expect)}
\label{figure:lemma_map}
\end{figure}


\subsection{Lemma 1 and lemma 2 as a consequence of a more general lemma}

\begin{definition}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
We note $\mathcal{E}^{M \rightleftarrows} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$ the execution such that, for every process $P_i \in \Pi$:
\begin{compactenum}
    \item $\mathcal{B}'_i \gets \mathcal{B}_i$
    
    \item $\forall j \in [1:k]$, $\fmsgro{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgro{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_receive_omission}
    
    \item $\forall j \in [1:k]$, $\fmsgso{\mathcal{B}'_i}{j}$ $ \gets \fmsgso{\mathcal{B}'_i}{j} $ $\cup \{m \in M | m.\mathit{round} = j \wedge m.\mathit{sender} = P_i\}$ \label{item:add_send_omission}

    \item $\forall j \in [1:k]$, $\fmsgs{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgs{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_send}
    
    \item $\mathcal{F}' = \{P_i \in \Pi \; | \bigcup\limits_{k' \in [1:k]} ( \fmsgso{\mathcal{B}_i}{k'} \cup \fmsgro{\mathcal{B}_i}{k'} ) \neq \emptyset\}$ \label{item:faulty_processes}
\end{compactenum}
\end{definition}

Intuitively, $\mathcal{E}^{M \rightleftarrows}$ corresponds to the execution $\mathcal{E}$, where every receive-omitted message is send-omitted instead.

\begin{lemma}\label{lemma:switch_omission}
    .Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
Let $\fswitcho{\mathcal{E}}{M} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$. 
If $|\mathcal{F}'| \leq t$, then $\mathcal{E}^{M \rightleftarrows}$ is a valid execution.
\end{lemma}

\begin{proof}
$\;$
\begin{compactitem}
 \item Faulty processes: $|\mathcal{F}'| \leq t$ is a precondition of the lemma.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$). Necessarily $m \notin M$ by step (\ref{item:remove_send}). Thus, $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and so $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ by Send-Validity of $\mathcal{E}$.
    
    Send-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$. Necessarily, $m \notin M$. Indeed, if $m \in M$, $m \in \fmsgro{\mathcal{B}_r}{j} \setminus \fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and $m \notin \in \fmsgr{\mathcal{B}'_r}{j}$, since $\fmsgr{\mathcal{B}'_r}{j} = \fmsgr{\mathcal{B}_r}{j}$ by construction and $\fmsgr{\mathcal{B}_r}{j} \cap \fmsgro{\mathcal{B}_r}{j} = \emptyset$, since $\mathcal{B}_r$ is a behavior of process $P_r$.

    Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (\ref{item:remove_send}) while constructing $\mathcal{B}_s'$.
    
    Receive-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.
    
    \item Omission-validity is obviously satisfied in $\fswitcho{\mathcal{E}}{M}$. by step (\ref{item:faulty_processes}).
\end{compactitem}
Thus, $\fswitcho{\mathcal{E}}{M}$. is indeed an execution of $\mathcal{A}$. 
\end{proof}



\begin{lemma}\label{lemma:0}
Let's fix
\begin{itemize}
    \item $(P,Q,R)$ is a partition of the processes
    \item $t_S, t_Q \in \mathbb{N}, t_S + t_Q \leq t + 1$
    \item $|P|> t_S $
    \item $|Q| \geq t_Q$
    \item $|R|\leq t-t_S-t_Q+1$
    
    \item $\mathcal{A}$ is a synchronous protocol that solves non-uniform weak agreement in the omission model
\end{itemize}

Let $\mathcal{E}$ be an execution of $\mathcal{A}$ such that:
\begin{itemize}
    \item Every process in $P$ is correct and eventually decides $b_P$.
    \item Every process in $Q$ is receive-isolated after some round $k$.
    \item Every process in $R$ is faulty.
\end{itemize}

If there exists $t_{Q'} \in \mathbb{N}$, such that the communication complexity of $\mathcal{A}$ is less than $(t_Q -t_{Q'}) \cdot t_S$, then $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{lemma}

\begin{proof}[proof sketch] (see figure \ref{figure:lemma_0})
First, we can remark that (*) $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$. By contradiction, assume the opposite. There exists a set $Q''$ of $|Q''|= |Q|-t_{Q'}+1 > t_Q -t_{Q'}$ processes that would receive more than $t_S$ messages. Thus, the communication complexity of $\mathcal{A}$ would be strictly greater than $(t_Q -t_{Q'}) \cdot t_S$.

Let $q_i \in Q'$.
Let $S_i$ be the set of processes in $P$ that have sent at least 1 message after round $k$ (including) to process $q_i$ in execution $\mathcal{E}$.
By (*), $|S_i| \leq t_S$.
We can construct an execution $\mathcal{E}_i$ s.t. behaviour of every process except the ones in $R \cup S_i \cup \{q_i\}$ are unchanged. Every message receive-omitted by process $q_i$ in execution $\mathcal{E}$ is now send-omitted by $R \cup S_i$. the rest remains unchanged. By agreement, termination, and correctness, $q_i$ must decide in $\mathcal{E}_i$ the same value than $P \setminus S_i \neq \emptyset$, that is $b_P$.
Since, the behaviours of $q_i$ in $\mathcal{E}$ and $\mathcal{E}_i$ are equivalent, $q_i$ must decide $b_P$ in $\mathcal{E}$.

Hence, every process $q_j \in Q'$ decides $b_P$ in $\mathcal{E}$.
\end{proof}


\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_0_vector.eps}
\caption{Lemma \ref{lemma:0}}
\label{figure:lemma_0}
\end{figure}

%%%%%%%%%%%%%%%%%%
%% formal proof %%
%%%%%%%%%%%%%%%%%%
\begin{proof}[formal proof]
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Due to the statement of the lemma, $\mathcal{F} = Q \uplus R$.
Moreover, no process in $P \uplus Q$ commits any send-omission failure in $\mathcal{E}$: for every process $P_i \in P \uplus Q$ and every round $j \in \mathbb{N}^+ \cup \{+\infty\}$, $\mathsf{send\_omitted}(\mathcal{B}_i, j) = \emptyset$.

For every set of processes $U$, we note $M_{U} = \bigcup\limits_{P_i \in U} \big( \bigcup\limits_{k' \geq k}  \fmsgs{\mathcal{B}_i}{k'} \big)$ to denote the set of messages sent by processes in $U$ from (and including) round $k$ onward in $\mathcal{E}$.

For every pair of sets of processes $(U, V)$, we define $M_{U \to V}$ as the set containing all messages sent to a process in $V$ by processes in $U$ from (and including) round $k$ onward of $\mathcal{E}$:
\begin{equation*}
    M_{U \to V} = \{ m \,|\, m \in M_{U} \land m.\mathsf{receiver} \in V \}.
\end{equation*}
Note that, for every $P_i \in Q$, each message $m \in M_{(P \uplus R) \to \{P_i\}}$ is receive-omitted in $\mathcal{B}_i$.

First, we will prove by contradiction that $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$ from processes in $P$. Therefore, assume that there exists a subset $Q'' \subseteq Q$ of $|Q''| > |Q|-t_Q \geq t_Q-t_{Q'}$ processes which receive more than $t_S$ messages in $\mathcal{E}$ from processes in $P$.
As $\mathcal{A}$ sends less than $(t_Q-t_{Q'})\cdot t_S$ messages in execution $\mathcal{E}$, less than $(t_Q-t_{Q'})\cdot t_S$ messages are sent in $\mathcal{E}$ by correct processes (i.e., processes in $P$), which implies $|M_{P \to \tilde{Q}'}| < (t_Q-t_{Q'})\cdot t_S$, thus we reach a contradiction. Hence, $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$ from processes in $P$, i.e. $\forall P_i \in Q', |M_{P \to \{P_i\}}| \leq t_S$.

Let $P_i \in Q'$.
Let $S_i$ denote the set of processes in $P$ whose messages $P_i$ receive-omits from (and including) round $k$ onward in $\mathcal{B}_i$:
\begin{equation*}
    S_i = \{ P_j \in P \,|\, \exists j \in [k, \infty], \exists m \in \fmsgro{\mathcal{B}_i}{j}: m.\mathsf{sender} = P_j \}.
\end{equation*}
Note that $P_i \notin S_i$ (as no process ever sends messages to itself).
Moreover, as $|M_{P \to \{P_i\}}| \leq t_S$, $|S_i| \leq t_S$.
We now create another execution $\mathcal{E}'_i = [\mathcal{F}', \mathcal{B}_1', ..., \mathcal{B}_n'] = \fswitcho{\mathcal{E}}{\tilde{M}_i}$ where $\tilde{M}_i = M_{(P \uplus R) \to \{P_i\}}$.
We can observe that $P_i$ is correct in $\mathcal{E}'_i$.
Hence, $\mathcal{F}' \subseteq S_i \uplus R \uplus (Q \setminus{\{ P_i \}})$ and $|R| \leq t-t_S-t_Q+1$, thus $|\mathcal{F}'| \leq t$. 
Let us note that some processes in $R$ might be now correct.
By lemma \ref{lemma:switch_omission}, $\mathcal{E}'_i$ is an execution of $\mathcal{A}$.
\iffalse
:
\begin{compactenum}
    \item $\mathcal{F}' \gets S_i \uplus R \uplus (Q \setminus{ \{P_i\}})$.

    \item For every process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, let $\mathcal{B}_j' \gets \mathcal{B}_j$, i.e., $P_j$'s behavior in $\mathcal{E}'$ is identical to $P_j$'s behavior in $\mathcal{E}_i$.

    \item For the process $P_i$, we build $\mathcal{B}_i'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_i' \gets \mathcal{B}_i$.

        \item For every round $k' \in [k, \infty]$ such that $\fmsgro{\mathcal{B}_i}{k'} \neq \emptyset$, we remove all messages from $\fmsgro{\mathcal{B}'_i}{k'}$: $\fmsgro{\mathcal{B}'_i}{k'} \gets \emptyset$.
        Note that all messages removed from $\fmsgro{\mathcal{B}'_i}{k'}$ are sent by processes in $S_i \uplus R$.
    \end{compactenum}
    Note that $P_i$ does not commit any omission faults in $\mathcal{B}_i'$: (1) it does not commit any send-omission faults due to the statement of the lemma, and (2) it does not commit any receive-omission faults due to the step (3)(b). 

    \item For every process $P_j \in S_i \uplus R$, we build $\mathcal{B}_j'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_j' \gets \mathcal{B}_j$.

        \item For every message $m$ such that there exists a round $k' \geq [k, \infty]$ with (1) $m \in \fmsgs{\mathcal{B}_j}{k'}$, and (2) $m \in \fmsgro{\mathcal{B}_i}{k'}$, we perform the following steps:
        \begin{compactenum}
            \item We remove $m$ from sent messages: $\fmsgs{\mathcal{B}_j'}{k'} \gets \fmsgs{\mathcal{B}_j'}{k'} \setminus{\{m\}}$.

            \item We add $m$ to send-omitted messages:
            $\fmsgso{\mathcal{B}_j'}{k'} \gets \fmsgso{\mathcal{B}_j'}{k'} \cup \{m\}$.
        \end{compactenum}
    \end{compactenum}
\end{compactenum}

Let us prove that $\mathcal{E}_i'$ is indeed an execution:
\begin{compactitem}
    \item Faulty processes: As $\mathcal{F}' \subseteq S_i \uplus R \uplus (Q \setminus{\{ P_i \}})$ and $|R| \leq t-t_S-t_Q+1$, thus $|\mathcal{F}'| \leq t$. Potentially, some processes in $R$ are now correct.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore:
    \begin{compactitem}
        \item For any process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ since $\mathcal{B}_j' = \mathcal{B}_j$. 
        \item For process $P_i$, $\mathcal{B}_i'$ is an infinite behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
        \item For any process $P_j \in R \uplus S_i$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ due to \Cref{lemma:behavior_send_transfer}. 
    \end{compactitem}
    

    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$).
    We consider two possibilities:
    \begin{compactitem}
        \item If $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (3)(b), then $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ as $m$ is included in step (3)(a).

        \item Otherwise, $m$ is excluded by step (3)(b).
        This implies that $j \geq k$, $P_r = P_i$, $P_s \in S_i \uplus R$, $m \in \fmsgro{\mathcal{B}_r}{j}$ and $m \in \fmsgs{\mathcal{B}_s}{j}$.
        Then, by step (4)(b)(i), $m \notin \fmsgs{\mathcal{B}_s'}{j}$ making this case impossible.
    \end{compactitem}
    Send-validity is satisfied in $\mathcal{E}'_i$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $j \geq k$ and $P_r = P_i$ and $m \in \fmsgro{\mathcal{B}_r}{j}$.
        However, this case is impossible as $m \notin \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ due to the step (3)(b).

        \item Otherwise, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
        Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (4)(b)(i) while constructing $\mathcal{B}_s'$.
    \end{compactitem}
    Receive-validity is satisfied in $\mathcal{E}'_i$.

    \item Omission-validity:
    Consider a process $P_j$ which commits an omission-fault in $\mathcal{B}_j'$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $P_j$ commit a send-omission fault in $\mathcal{B}_j'$.
        As no process $P_z \in \Pi \setminus R$ commits a send-omission fault in $\mathcal{B}_z$, $P_j \in R \uplus S_i$ given that we only add send-omitted messages to processes in $R \uplus S_i$. Hence, $P_j \in \mathcal{F}'$.
        In this case, omission-validity is satisfied.

        \item Let $P_j$ commit a receive-omission fault in $\mathcal{B}_j'$.
        Note that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z$, which implies that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z'$ (as our construction does not add receive-omitted messages to any process).
        
        Moreover, $P_i$ does not commit a receive-omission fault in $\mathcal{B}_i'$ as (1) it does not commit any receive-omission faults in any round $k' \in [1, k - 1]$ in $\mathcal{B}_i$ (due to \Cref{definition:isolation}), and (2) all receive-omitted messages in any round $k' \in [k, \infty]$ are removed by the step (3)(b).
        Therefore, $P_j \in R \uplus (Q \setminus{\{P_i\}})$, which means that omission-validity holds in this case as well.
    \end{compactitem}
    Omission-validity is satisfied in $\mathcal{E}'_i$.
\end{compactitem}

Thus, $\mathcal{E}'_i$ is indeed an execution of $\mathcal{A}$.
\fi
Since $|P|>t_S$, $|S_i|\leq t_S$, $\exists P_j \in P \setminus S_i \neq \emptyset$.

Observe that $P_i$ and $P_j$ are correct in $\mathcal{E}'_i$, and $\mathcal{B}'_j = \mathcal{B}_j$.
Hence, they both decide the same value $b$.

Moreover (1) $P_i$'s states in $\mathcal{B}_i'$ and $\mathcal{B}_i$ are identical, and (2) $P_j$'s states in $\mathcal{B}_j'$ and $\mathcal{B}_j$ are identical.
Therefore, $P_i$ decides $b$ in $\mathcal{E}$.
Thus, every process in $Q'$ decides $b$ in $\mathcal{E}$.
Hence, the lemma holds.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%
%% end formal proof %%
%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}
If $t_Q = 2t_{Q'}$, and the communication complexity of $\mathcal{A}$ is less than $t_{Q'} \cdot t_S$, then $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{corollary}

\begin{lemma}\label{lemma:forced_termination_new}
Lemma \ref{lemma:forced_termination}
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $|R|=0$, $P = \bar{X}$, $Q = X$ with $t_S = t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$.
\end{proof}

\begin{lemma}\label{lemma:disagreement_quadratic_messages_new}
Lemma \ref{lemma:disagreement_quadratic_messages}
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $(Q,R)=(B,C)$ (resp. $(Q,R)=(C,B)$), $P = A$, $t_S = \frac{t}{2}, t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$. We verify $|R| = \frac{t}{4} \leq t-t_S - t_Q+1 = \frac{t}{4} +1$. 

\end{proof}




\begin{definition}
Let $P = \{P_{i_1}, ..., P_{i_{\ell}}\}$ be a set of correct processes.
Let $\bar{b} : P \rightarrow \{0, 1\}$ that maps each process $P_i \in P$ to a proposal bit $\bar{b}(P_i) \in \{0,1\}$.
Let $M$ be a set of messages not sent by processes in $P$, i.e. $\forall m \in M, m.\mathit{sender} \notin P$.
For every $k \in \mathbb{N} \cup \{\infty\}$,
We define $\mathsf{correct}(P, \bar{b},M,k) \triangleq [\mathcal{B}_{i_1}, ..., \mathcal{B}_{i_{\ell}}]$,  where each $\mathcal{B}_{i} \triangleq \langle \mathcal{F}^1_i, ..., \mathcal{F}^k_i\rangle$ is a $k$-round behavior of process $P_i$ and each $\mathcal{F}^j_i \triangleq (\state{i}{j}, \msgs{i}{j}, \emptyset, \msgr{i}{j}, \emptyset)$ as follows.

\begin{compactenum}
    \item (Initialization) $\forall P_i \in P$:
\begin{itemize}
\item  (correct proposal) $\pstate{i}{1}.\mathit{proposal} = \bar{b}(P_i)$, $  \msgs{i}{1} = \mathcal{M}^{b_i}_i$
\item (received message) $\msgr{i}{1} = \{m \in M \cup (\bigcup_{i \in \{i_{1}, ..., i_{\ell}\}} \msgs{i}{1}) | m.\mathit{round} = 1 \wedge m.\mathit{receiver} = P_i\}$
\end{itemize}    
    \item (Induction) $\forall P_i \in P, \forall j \in [1:k]$:
    \begin{itemize}
\item  (correct transition) if $j<k$, $(\pstate{i}{j+1}, \msgs{i}{j+1}) = \mathcal{A}(\pstate{i}{j}, \msgr{i}{j})$
\item (received message) $\msgr{i}{j} = \{m \in M \cup (\bigcup_{i \in \{i_{1}, ..., i_{\ell}\}} \msgs{i}{j}) | m.\mathit{round} = j \wedge m.\mathit{receiver} = P_i\}$
\end{itemize}    
\end{compactenum}
\end{definition}

\iffalse
%%%%%%%%%%%%
%% useless lemma %%
%%%%%%%%%%%%
\begin{lemma}
Let $P = \{P_{i_1}, ..., P_{i_{\ell}}\}$ be a set of correct processes.
Let $\bar{b} : P \rightarrow \{0, 1\}$ that maps each process $P_i \in P$ to a proposal bit $\bar{b}(P_i) \in \{0,1\}$. Let $(k',k) \in \mathbb{N} \times (\mathbb{N} \cup \{\infty\})$ with $k' < k$.
Let $M = M_{\leq k'} \uplus M_{>k'}$ be a set of messages not sent by processes in $P$ (i.e. $\forall m \in M, m.\mathit{sender} \notin P$), such that (1) $\forall m \in M_{\leq k'}$, $m.\mathsf{round} \leq k'$ and $\forall m \in M_{> k'}$, $m.\mathsf{round} > k'$.

Let $[\mathcal{B}_{i_1}, ..., \mathcal{B}_{i_{\ell}}] = \mathsf{correct}(P, \bar{b},M,k)$ and $[\mathcal{B}'_{i_1}, ..., \mathcal{B}'_{i_{\ell}}] = \mathsf{correct}(P, \bar{b},M_{\leq k'},k')$.

For every $P_i \in P$, we note $\mathcal{B}'_{i} = \langle \mathcal{F}_{i}^{\prime 1}, ...,  \mathcal{F}_{i}^{\prime k'}\rangle$ and $\mathcal{B}_{i} = \langle \mathcal{F}_{i}^{1}, ...,  \mathcal{F}_{i}^{k}\rangle$.

Then, $\forall P_i \in P$,  $\forall j \in [1:k']$, $\mathcal{F}^{j}_{i} = \mathcal{F}^{\prime j}_{i} $
\end{lemma}

\begin{proof}
It is trivial to realise that the construction are the same ones until round $k'$.
\end{proof}

%%%%%%%%%%%%%%
%% end useless lemma %%
%%%%%%%%%%%%%%
\fi

\pierre{I realize that the lemma 3 and lemma 4 can be proved by a generic lemma with the exact same structure}

\begin{lemma}[Combining receive-isolation]\label{lemma:combining_receive_isolation}
Let  $\bar{b}^u, \bar{b}^v: \Pi \rightarrow \{0,1\}$.
Let $\mathcal{A}$ be an agreement algorithm.
Let $\mathcal{E}^{u}$ and $\mathcal{E}^{v}$ be two executions of $\mathcal{A}$ such that:
\begin{compactitem}
\item $\forall P_i \in \Pi$, $P_i$ proposes $\bar{b}^u(P_i)$ (resp.  $\bar{b}^v(P_i)$) in $\mathcal{E}^{u}$ (resp.  $\mathcal{E}^{v}$).
\item in $\mathcal{E}^{u}$: $A \cup B $ are correct,  while $C$ is receive-isolated from some round $k^u$ onward. 
\item in $\mathcal{E}^{v}$: $A \cup C $ are correct,  while $B$ is receive-isolated from some round $k^v$ onward.
\item $A$ decides $b'_u$ in $\mathcal{E}^{u}$ and $b'_v$ in $\mathcal{E}^{v}$
\end{compactitem}
If either (1) $k^u = k^v = 1$ or (2) $|k^u-k^v| \leq 1$ and $\bar{b}^u = \bar{b}^v$. \newline
Then,  either (3) the message-complexity of $\mathcal{A}$ is greater than $\frac{t^2}{16}$, or (4) $b'_u = b'_v$.
\end{lemma}

\begin{proof}[formal proof] (see figure \ref{figure:lemma_343} for case (1) and \ref{figure:lemma_343} for case (2) )
By contradiction, let us assume than both the message-complexity of $\mathcal{A}$ is lower than $\frac{t^2}{16}$, and $b'_u \neq b'_v$.

We note $\mathcal{E}^u = [\mathcal{F}^u, \mathcal{B}^{u}_1, ...,  \mathcal{B}^{u}_n]$ and $\mathcal{E}^v = [\mathcal{F}^v, \mathcal{B}^{v}_1, ...,  \mathcal{B}^{v}_n]$.
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{8}$ processes that decide $b'_u$ in $\mathcal{E}^u$ and there exists a set $C' \subset C$ of $|C'| = \frac{t}{8}$ processes that decide $b'_v$ in $\mathcal{E}^v$.
Let's construct a new infinite execution $\mathcal{E}^{*} = [\mathcal{F}^{*}, \mathcal{B}^{*}_1, ...,  \mathcal{B}^{*}_n]$, as follows:
\begin{compactenum}

\item (Message naming) We note:

\begin{compactitem}
\item $k^{-} = \mathsf{min}(k^u, k^{w})$ and $k^{+} = \mathsf{max}(k^u, k^{w})$.

\item  $M^{S(B,C)}_{\leq k^{-}}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k^{-}]}  \fmsgs{\mathcal{B}^{v}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k^{-}]}  \fmsgs{\mathcal{B}^{u}_i}{k'} \big)$.

\item $M^{S(B,C)}_{> k^{-}}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [k^{-}+1:k]}  \fmsgs{\mathcal{B}^{v}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [k^{-}+1:k]}  \fmsgs{\mathcal{B}^{u}_i}{k'} \big)$.

\item  $M^{S(B,C)} = M^{S(B,C)}_{\leq k^{-}} \uplus M^{S(B,C)}_{> k^{-}}$

\end{compactitem}



\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A : A  \rightarrow \{0,1\}$ with $\bar{b}_A(P_i) = \bar{b}^{u}(P_i)$. For every $P_i \in A$., we define

$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

\item Let $P_i \in B\cup C$. We note $ \mathcal{B}_{i} =  \mathcal{B}^{v}_{i}$ if $P_i \in B$ and $ \mathcal{B}_{i} =  \mathcal{B}^{u}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}^{*}_{i} \gets \mathcal{B}_{i}$. \label{item:init_behaviours_receive_isolated_groups_in_combined_execution}

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], $

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup C} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in B$, and  

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup B} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in C$\label{item:replace_receive_omission_in_combined_execution}

\item $\mathcal{F}^{*} \subseteq \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}^{*}_i}{k'} \neq \emptyset\}$

\end{compactenum}


Let us show that $\mathcal{E}^{*}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} = B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $ \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $ \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

\item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgr{\mathcal{B}_r}{j}$ by send-validity of $\mathcal{E}^u$ and $\mathcal{E}^v$ so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_in_combined_execution}.

\item If $(P_s, P_r) \in A \times (B \cup C) \cup (B \times C) \cup (C \times B)$, $m \in \fmsgro{\mathcal{B}^{*}_r}{j}$ is ensured by step \ref{item:replace_receive_omission_in_combined_execution} of the construction of $\mathcal{E}^{*}$, while no step modifies $\fmsgro{\mathcal{B}^{*}_r}{j}$ afterwards.

\end{compactitem}
    
    
    
    Send-validity is satisfied in $\mathcal{E}^{*}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r^{*}}{j} \cup \fmsgro{\mathcal{B}_r^{*}}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

 \item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgs{\mathcal{B}_s}{j}$ by send-validity of $\mathcal{E}^u$ and $\mathcal{E}^v$, so $m \in \fmsgs{\mathcal{B}_r}{j}$, since $\fmsgs{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.

\item If $(P_s, P_r) \in (A \times (B \cup C)) \cup (B \times C) \cup (C \times B)$,  $m \notin \fmsgr{\mathcal{B}_r}{j}$. 
If $m \in \fmsgro{\mathcal{B}^{*}_r}{j}$, then
$m \in \fmsgs{\mathcal{B}^{*}_s}{j}$,   by step \ref{item:replace_receive_omission_in_combined_execution}, while no step modifies neither $\fmsgs{\mathcal{B}^{*}_s}{j}$ or $ \fmsgro{\mathcal{B}^{*}_r}{j}$ afterwards.

So let us assume $m \in \fmsgr{\mathcal{B}^{*}_r}{j}$. 

In that case, $j \leq k^{-}$. Indeed, $B$ (resp. $C$) is receive-isolated from the round $k^v$ (resp. $k^u$) in execution $\mathcal{E}^u$ (resp.  $\mathcal{E}^v$), so $j > k^{-}$ would imply $m \notin \fmsgr{\mathcal{B}_r}{k^{-}}$. Finally, it would imply $m \notin \fmsgr{\mathcal{B}_r^{*}}{k^{-}}$ by step \ref{item:init_behaviours_receive_isolated_groups_in_combined_execution}, while no step modifies $ \fmsgr{\mathcal{B}^{*}_r}{j}$ afterwards.

Moreoever, the condition $k^{u} = k^{v}=1$ does not hold, since $B \cup C$ would be receive-isolated from the first round of the execution $\mathcal{E}^{*}$. Hence, in addition of $j \leq k^{-}$, the condition $|k^u-k^v| \leq 1 \wedge \bar{b}^u = \bar{b}^v$
necessarily holds, to satisfy the precondition of the lemma.

The fact that $\bar{b}^u = \bar{b}^v$ implies that executions $\mathcal{E}^{u}$, $\mathcal{E}^{v}$,  and $\mathcal{E}^{*}$ are identical up to round $k^{-}-1$.   \pierre{to make formal}
Moreover, $\bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{*}}{k^{-}} = \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{u}}{k^{-}} = \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{v}}{k^{-}}$ \pierre{to prove}.
Hence, $ \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{*}}{j} =  \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{u}}{j} =  \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{v}}{j} \triangleq M_{j}$.

By receive-validity of $\mathcal{E}^{u}$ and $\mathcal{E}^{v}$, $m \in M_{j}$ and so $m \in  \fmsgs{\mathcal{B}^{*}_s}{j}$.

\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}^{*}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}^{*}$ since no process in $A$ commits any omission fault by construction of $ \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.
\end{compactitem}
Thus, $\mathcal{E}^{*}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $b'_u$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $b'_v$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.

Thus, the lemma holds.

\end{proof}

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/lemma_343.eps}
\caption{Lemma \ref{lemma:combining_receive_isolation}, case (1) }
\label{figure:lemma_343}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/lemma_344.eps}
\caption{Lemma \ref{lemma:combining_receive_isolation}, case (2)}
\label{figure:lemma_344}
\end{figure}

\begin{lemma}
Lemma \ref{lemma:either} (lemma 3):
Let $\mathcal{E}_0$ and $\mathcal{E}_1$ as presented in figure \ref{figure:lemma_3}.
There exists a pair of sets $(B', C') \subset B \times C$ of size $|B'| = |C'| = \frac{t}{8}$ such that processes  in $A \cup C \cup B'$ decide $b \in \{0, 1 \}$ in $\mathcal{E}_0$ and $A \cup B \cup C'$ decide $b' \in \{0, 1 \}$ in $\mathcal{E}_1$.
Moreover either $b = 1$ or $b'=0$.
\end{lemma}

\begin{proof}[New proof]
Directly by lemma \ref{lemma:combining_receive_isolation} applied to executions $\mathcal{E}^u=\mathcal{E}_0$ and $\mathcal{E}^v = \mathcal{E}_1$ and $k^{u} = k^{v} = 1$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}[proof sketch]
(see figure \ref{figure:lemma_3})
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{8}$ processes that decide $b$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{8}$ processes that decide $b'$ in $\mathcal{E}_1$.
%\pierre{it seems to me we can avoid the set of size $\frac{|B|}{4}$ (resp. $\frac{|C|}{4}$ invoked in the proof of lemma \ref{lemma:either} (lemma 3). The remaining part is the same.}
By contratiction, assume $b=0$ and $b'=1$. Let's construct a new infinite execution $\mathcal{E}^{*}$, such that $\mathcal{E}^{*}|_{B} \equiv \mathcal{E}_0|_{B}$ and $\mathcal{E}^{*}|_{C} \equiv \mathcal{E}_1|_{C}$:

\begin{compactenum}
    \item In $\mathcal{E}^*$, all processes from $A \cup B$ propose $0$, whereas all processes from $C$ propose $1$.

    \item All processes from $A$ are correct, whereas all processes from $B \cup C$ are faulty.
    Note that $|B \cup C| < t$.

    \item Every process from $B$ exhibits the exact same behavior as in $\mathcal{E}_0$.
    Note that this step implies that $B$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    \item Every process from $C$ exhibits the exact same behavior as in $\mathcal{E}_1$.
    Note that this step implies that $C$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    % \item Both groups $B$ and $C$ are receive-isolated from round $1$.
\end{compactenum}
Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages}, correct processes send at least $\frac{t^2}{32}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{32}$ (or even $\frac{t^2}{16}$) messages in every execution.
Thus, the lemma holds.
\end{proof}

\begin{proof}[formal proof]
We note $\mathcal{E}_0 = [\mathcal{F}_0, \mathcal{B}^{0}_1, ...,  \mathcal{B}^{0}_n]$ and $\mathcal{E}_1 = [\mathcal{F}_1, \mathcal{B}^{1}_1, ...,  \mathcal{B}^{1}_n]$.
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{4}$ processes that decide $b$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{4}$ processes that decide $b'$ in $\mathcal{E}_1$.
By contratiction, assume $b=0$ and $b'=1$. Let's construct a new infinite execution $\mathcal{E}^{*} = [\mathcal{F}^{*}, \mathcal{B}^{*}_1, ...,  \mathcal{B}^{*}_n]$, as follows:
\begin{compactenum}
\item $\mathcal{F}^{*} = B \cup C$

\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{0}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{1}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M,k)$.

\item $\forall P_i \in B\cup C$, we note $ \mathcal{B}_{i} =  \mathcal{B}^{0}_{i}$ if $P_i \in B$ and $ \mathcal{B}_{i} =  \mathcal{B}^{1}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}^{*}_{i} \gets \mathcal{B}_{i}$.

%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], $

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup C} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in B$, and  

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup B} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in C$\label{item:replace_receive_omission_in_e_star}

\item $\mathcal{F} \subseteq \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}^{*}_i}{k'} \neq \emptyset\}$

\end{compactenum}


Let us show that $\mathcal{E}^{*}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} = B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times (B \cup C)$, $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ is ensured by step \ref{item:replace_receive_omission_in_e_star} of the construction of $\mathcal{E}^{*}$.
\end{compactitem}
    
    
    
    Send-validity is satisfied in $\mathcal{E}^{*}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r^{*}}{j} \cup \fmsgro{\mathcal{B}_r^{*}}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times (B \cup C)$, $m \in \fmsgro{\mathcal{B}_r^{*}}{j}$, since $\fmsgr{\mathcal{B}_r^{*}}{j} = \emptyset$ by construction, because $\fmsgr{\mathcal{B}_r}{j} = \emptyset$ and no additional received messages are added during the contruction of $\mathcal{B}_r^{*}$.
Thus, $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ is ensured by step \ref{item:replace_receive_omission_in_e_star} of the construction of $\mathcal{E}^{*}$.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}^{*}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}^{*}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}^{*}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Hence, the assumption $b=0$ and $b'=1$ is false, which means that either $b=1$ or $b'=0$.
Thus, the lemma holds.

\end{proof}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end  lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_3.eps}
\caption{Lemma \ref{lemma:either}}
\label{figure:lemma_3}
\end{figure}

Then, we define the execution $\mathcal{E}_C, \mathcal{E}^{k^{*}}$, and $\mathcal{E}^{k^{*}+1}$ as in the prologue of lemma \ref{lemma:final} (lemma 4), and illustrated in figure \ref{figure:execution_C}. Without loss of generality, it has been assumed that processes in $A$ decide $b=1$ in execution $\mathcal{E}_0$.

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_execution_C.eps}
\caption{Execution $\mathcal{E}_C$}
\label{figure:execution_C}
\end{figure}

\begin{lemma} Lemma \ref{lemma:final} (lemma 4).
There exists an execution of $\mathcal{A}$ in which correct processes send (at least) $\frac{t^2}{32}$ messages.
\end{lemma}

\begin{proof}[New proof]
Directly by lemma \ref{lemma:combining_receive_isolation} applied to executions $\mathcal{E}^u=\mathcal{E}_C$ and $\mathcal{E}^v = \mathcal{E}^{k^{*}}$ in case $b_C=0$ and  $\mathcal{E}^v = \mathcal{E}^{k^{*}+1}$ in case $b_C=1$ and $|k^{u} - k^{v}| \leq 1$, where $\forall P_i \in \Pi$, $\bar{b}^{u}(P_i) = \bar{b}^{v}(P_i) = 0$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}[proof sketch]
(see figure \ref{figure:lemma_4})
We consider two possible cases:
\begin{compactitem}
    \item Let $b_C = 0$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Both groups $B$ and $C$ are receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^*}$ (from round $k^*$ onward).
        Note that this step implies that $B$ is receive-isolated from round $k^*$.

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item From (and including) round $k^*$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.

% this is pointless, by item 4. not really, will change something more
        % \item From (and including) round $k^*$ onward, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$ in $\mathcal{E}^k$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$ in $\mathcal{E}_C$.
    \end{compactenum}
    
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $1$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $0$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.

    \item Let $b_C = 1$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}+1}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Group $C$ is receive-isolated from round $k^*$, whereas group $B$ is receive-isolated from round $k^*+1$

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^* + 1}$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^* + 1$.
        \add{Note that the message received in round $k^{*}$ from processes in $C$ are indeed the same ones than in execution $\mathcal{E}^{k^* + 1}$, since the receive-omission at round $k^*$ has no impact of the messages at the same round $k^*$.} 

        \item In round $k^*$, all messages from $C$ are received, which means that processes in $B$ successfully receive messages sent by $C$.

        \item From (and including) round $k^* + 1$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.
        
        
        % we send-omit (1) all messages sent by processes in $C$ to processes in $A$ in $\mathcal{E}_C$.
        % Note that, in round $k^*$, messages sent by processes in $C$ to processes in $B$ are successfully sent and successfully received.

        % \item From round $k^* + 1$, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$.
    \end{compactenum}
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $0$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $1$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.
\end{compactitem}
As the statement of the lemma holds in both possible cases, the proof is concluded.
\end{proof}

\begin{proof}[formal proof]
We note $\mathcal{E}_C = [\mathcal{F}_C, \mathcal{B}^{C}_1, ...,  \mathcal{B}^{C}_n]$, $\mathcal{E}^{k^{*}} = [\mathcal{F}_{k^{*}}, \mathcal{B}^{k^{*}}_1, ...,  \mathcal{B}^{k^{*}}_n]$ and $\mathcal{E}^{k^{*}+1} = [\mathcal{F}_{k^{*}+1}, \mathcal{B}^{k^{*}+1}_1, ...,  \mathcal{B}^{k^{*}+1}_n]$.

Case $b_C = 0$.

Let's construct a new infinite execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ...,  \mathcal{B}_n]$, as follows:
\begin{compactenum}

\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{k^{*}}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{C}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M^S_{(B,C)},k)$.

\item $\forall P_i \in B\cup C$, we note $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{k^{*}}_{i}$ if $P_i \in B$ and $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{C}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}_{i} \gets \tilde{\mathcal{B}}_{i}$. \label{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}

%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], $

$\fmsgro{\mathcal{B}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup C} \fmsgs{\mathcal{B}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in B$, and  

$\fmsgro{\mathcal{B}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup B} \fmsgs{\mathcal{B}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in C$\label{item:replace_receive_omission_when_bc_equal_0}

\item $\mathcal{F} = \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}_i}{k'} \neq \emptyset\}$
\end{compactenum}


Let us show that $\mathcal{E}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} \subseteq B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgr{\tilde{\mathcal{B}}_r}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.

\item If $(P_s, P_r) \in A \times (B \cup C) \cup (B \times C) \cup (C \times B)$, $m \in \fmsgro{\mathcal{B}_r}{j}$ is ensured by step \ref{item:replace_receive_omission_when_bc_equal_0} of the construction of $\mathcal{E}$, while no step modifies $\fmsgro{\mathcal{B}_r}{j}$ afterwards.
\end{compactitem}
    

    Send-validity is satisfied in $\mathcal{E}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.

\item If $(P_s, P_r) \in (A \times (B \cup C)) \cup (B \times C) \cup (C \times B)$,  $m \notin \fmsgr{\tilde{\mathcal{B}}_r}{j}$ since both $B$ and $C$ are receive isolated in $\mathcal{E}^{k^{*}}$ and $\mathcal{E}^C$ respectively.  Moreover, $\fmsgr{\mathcal{B}_r}{j} = \fmsgr{\tilde{\mathcal{B}}_r}{j}$ because no step modifies $\fmsgr{\mathcal{B}_r}{j}$ after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}. Hence, $m \notin \fmsgr{\mathcal{B}_r}{j}$,  and so $m \in \fmsgro{\mathcal{B}_r}{j}$.
Finally, 
$m \in \fmsgs{\mathcal{B}_s}{j}$,   by step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}, while no step modifies neither $\fmsgs{\mathcal{B}_s}{j}$ or $ \fmsgro{\mathcal{B}_r}{j}$ afterwards.

 \item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgs{\tilde{\mathcal{B}}_s}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}$, the following holds: (1) all processes from $B'$ decide $1$ in $\mathcal{E}$, and (2) all processes from $C'$ decide $0$ in $\mathcal{E}$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}$.
%which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Thus, the lemma holds.

Case $b_C = 1$.

Let's construct a new infinite execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ...,  \mathcal{B}_n]$, as follows:
\begin{compactenum}


\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{k^{*}+1}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{C}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M^S_{(B,C)},k)$.

\item $\forall P_i \in B\cup C$, we note $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{k^{*}+1}_{i}$ if $P_i \in B$ and $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{C}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}_{i} \gets \tilde{\mathcal{B}}_{i}$.
\label{item:init_behaviours_receive_isolated_groups_when_bc_equal_1}
%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], \fmsgro{\mathcal{B}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in \Pi \setminus \{P_i\}} \fmsgs{\mathcal{B}_j}{k'} | m.\mathsf{receiver} = P_i\}$ \label{item:replace_receive_omission_when_bc_equal_1}

\item $\mathcal{F} = \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}_i}{k'} \neq \emptyset\}$
\end{compactenum}

Let us show that $\mathcal{E}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} \subseteq B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgr{\tilde{\mathcal{B}}_r}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.

\item If $(P_s, P_r) \in A \times (B \cup C) \cup (B \times C) \cup (C \times B)$, $m \in \fmsgro{\mathcal{B}_r}{j}$ is ensured by step \ref{item:replace_receive_omission_when_bc_equal_0} of the construction of $\mathcal{E}$, while no step modifies $\fmsgro{\mathcal{B}_r}{j}$ afterwards.
\end{compactitem}
    

    Send-validity is satisfied in $\mathcal{E}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (A \times (B \cup C)) \cup (B \times C) \cup (C \times B)$,  $m \notin \fmsgr{\tilde{\mathcal{B}}_r}{j}$ since both $B$ and $C$ are receive isolated in $\mathcal{E}^{k^{*}+1}$ and $\mathcal{E}^C$ respectively.  Moreover, $\fmsgr{\mathcal{B}_r}{j} = \fmsgr{\tilde{\mathcal{B}}_r}{j}$ because no step modifies $\fmsgr{\mathcal{B}_r}{j}$ after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}. Hence, $m \notin \fmsgr{\mathcal{B}_r}{j}$,  and so $m \in \fmsgro{\mathcal{B}_r}{j}$.
Finally, 
$m \in \fmsgs{\mathcal{B}_s}{j}$,   by step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}, while no step modifies neither $\fmsgs{\mathcal{B}_s}{j}$ or $ \fmsgro{\mathcal{B}_r}{j}$ afterwards.

 \item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgs{\tilde{\mathcal{B}}_s}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}$.
%which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Thus, the lemma holds.
\end{proof}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end  lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_4.eps}
\caption{Lemma \ref{lemma:final}}
\label{figure:lemma_4}
\end{figure}







==> sections/suggestions_4.tex <==
\section{Suggestions (DONE)}

In this section, we provide a formal proof of the quadratic lower bound for the worst case complexity of weak agreement (see figure \ref{figure:lemma_map}). 

\begin{figure}[!t]
\centering
\includegraphics[width=6cm]{figures/lemma_map.eps}
\caption{Lemma Map (A draft to show what I would expect). The "lemma 21" in the figure corresponds to \Cref{lemma:0bis}, while "lemma 21" in the figure corresponds to \Cref{lemma:combining_receive_isolation}.}
\label{figure:lemma_map}
\end{figure}

First, we define a function that takes an execution and replace some receive-omitted messages by send-omitted messages.

\begin{definition}\label{definition:permutation_receive_omission_to_send_omission}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
We denote by $\mathcal{E}^{M \rightleftarrows} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$ the execution such that, for every process $P_i \in \Pi$:
\begin{compactenum}
    \item $\mathcal{B}'_i \gets \mathcal{B}_i$
    
    \item $\forall j \in [1:k]$, $\fmsgro{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgro{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_receive_omission}
    
    \item $\forall j \in [1:k]$, $\fmsgso{\mathcal{B}'_i}{j}$ $ \gets \fmsgso{\mathcal{B}'_i}{j} $ $\cup \{m \in M | m.\mathit{round} = j \wedge m.\mathit{sender} = P_i\}$ \label{item:add_send_omission}

    \item $\forall j \in [1:k]$, $\fmsgs{\mathcal{B}'_i}{j}$ $\gets$ $\fmsgs{\mathcal{B}_i}{j}$ $\setminus M$ \label{item:remove_send}
    
    \item $\mathcal{F}' = \{P_i \in \Pi \; | \bigcup\limits_{k' \in [1:k]} ( \fmsgso{\mathcal{B}_i}{k'} \cup \fmsgro{\mathcal{B}_i}{k'} ) \neq \emptyset\}$ \label{item:faulty_processes}
\end{compactenum}
\end{definition}

Intuitively, $\mathcal{E}^{M \rightleftarrows}$ corresponds to the execution $\mathcal{E}$, where every receive-omitted message is send-omitted instead.

\begin{lemma}\label{lemma:switch_omission}
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$ be an execution of size $k \in \mathbb{N} \cup \{\infty\}$ and $M$ be a set of receive-omitted messages only, i.e. $\forall m \in M$, $\exists (P_i, j) \in \Pi \times [1:k]$, $m \in \fmsgro{\mathcal{B}_i}{j}$.
Let $\fswitcho{\mathcal{E}}{M} = [\mathcal{F}', \mathcal{B}'_1, ..., \mathcal{B}'_n]$. 
If $|\mathcal{F}'| \leq t$, then $\mathcal{E}^{M \rightleftarrows}$ is a valid execution.
\end{lemma}

\begin{proof}
$\;$
\begin{compactitem}
 \item Faulty processes: $|\mathcal{F}'| \leq t$ is a precondition of the lemma.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$). Necessarily $m \notin M$ by step (\ref{item:remove_send}). Thus, $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and so $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ by Send-Validity of $\mathcal{E}$.
    
    Send-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$. Necessarily, $m \notin M$. Indeed, if $m \in M$, $m \in \fmsgro{\mathcal{B}_r}{j} \setminus \fmsgro{\mathcal{B}_r'}{j}$ by step (\ref{item:remove_receive_omission}), and $m \notin \in \fmsgr{\mathcal{B}'_r}{j}$, since $\fmsgr{\mathcal{B}'_r}{j} = \fmsgr{\mathcal{B}_r}{j}$ by construction and $\fmsgr{\mathcal{B}_r}{j} \cap \fmsgro{\mathcal{B}_r}{j} = \emptyset$, since $\mathcal{B}_r$ is a behavior of process $P_r$.

    Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (\ref{item:remove_send}) while constructing $\mathcal{B}_s'$.
    
    Receive-validity is satisfied in $\fswitcho{\mathcal{E}}{M}$.
    
    \item Omission-validity is obviously satisfied in $\fswitcho{\mathcal{E}}{M}$. by step (\ref{item:faulty_processes}).
\end{compactitem}
Thus, $\fswitcho{\mathcal{E}}{M}$. is indeed an execution of $\mathcal{A}$. 
\end{proof}



\begin{lemma}[Some isolated processes must agree]\label{lemma:0}
Let's fix
\begin{itemize}
    \item $(P,Q,R)$ is a partition of the processes
    \item $t_S, t_Q \in \mathbb{N}, t_S + t_Q \leq t + 1$
    \item $|P|> t_S $
    \item $|Q| \geq t_Q$
    \item $|R|\leq t-t_S-t_Q+1$
    
    \item $\mathcal{A}$ is a synchronous protocol that solves non-uniform weak agreement in the omission model
\end{itemize}

Let $\mathcal{E}$ be an execution of $\mathcal{A}$ such that:
\begin{itemize}
    \item Every process in $P$ is correct and eventually decides $b_P$.
    \item Every process in $Q$ is receive-isolated after some round $k$.
    \item Every process in $R$ is faulty.
\end{itemize}

If there exists $t_{Q'} \in \mathbb{N}$, such that the communication complexity of $\mathcal{A}$ is less than $(t_Q -t_{Q'}) \cdot t_S$, then $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{lemma}

\begin{proof}[proof sketch] (see figure \ref{figure:lemma_0})
First, we can remark that (*) $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$. By contradiction, assume the opposite. There exists a set $Q''$ of $|Q''|= |Q|-t_{Q'}+1 > t_Q -t_{Q'}$ processes that would receive more than $t_S$ messages. Thus, the communication complexity of $\mathcal{A}$ would be strictly greater than $(t_Q -t_{Q'}) \cdot t_S$.

Let $q_i \in Q'$.
Let $S_i$ be the set of processes in $P$ that have sent at least 1 message after round $k$ (including) to process $q_i$ in execution $\mathcal{E}$.
By (*), $|S_i| \leq t_S$.
We can construct an execution $\mathcal{E}_i$ s.t. behaviour of every process except the ones in $R \cup S_i \cup \{q_i\}$ are unchanged. Every message receive-omitted by process $q_i$ in execution $\mathcal{E}$ is now send-omitted by $R \cup S_i$. the rest remains unchanged. By agreement, termination, and correctness, $q_i$ must decide in $\mathcal{E}_i$ the same value than $P \setminus S_i \neq \emptyset$, that is $b_P$.
Since, the behaviours of $q_i$ in $\mathcal{E}$ and $\mathcal{E}_i$ are equivalent, $q_i$ must decide $b_P$ in $\mathcal{E}$.

Hence, every process $q_j \in Q'$ decides $b_P$ in $\mathcal{E}$.
\end{proof}


\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_0_vector.eps}
\caption{Lemma \ref{lemma:0}}
\label{figure:lemma_0}
\end{figure}

%%%%%%%%%%%%%%%%%%
%% formal proof %%
%%%%%%%%%%%%%%%%%%
\begin{proof}[formal proof]
Let $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ..., \mathcal{B}_n]$.
Due to the statement of the lemma, $\mathcal{F} = Q \uplus R$.
Moreover, no process in $P \uplus Q$ commits any send-omission failure in $\mathcal{E}$: for every process $P_i \in P \uplus Q$ and every round $j \in \mathbb{N}^+ \cup \{+\infty\}$, $\mathsf{send\_omitted}(\mathcal{B}_i, j) = \emptyset$.

For every set of processes $U$, we note $M_{U} = \bigcup\limits_{P_i \in U} \big( \bigcup\limits_{k' \geq k}  \fmsgs{\mathcal{B}_i}{k'} \big)$ to denote the set of messages sent by processes in $U$ from (and including) round $k$ onward in $\mathcal{E}$.

For every pair of sets of processes $(U, V)$, we define $M_{U \to V}$ as the set containing all messages sent to a process in $V$ by processes in $U$ from (and including) round $k$ onward of $\mathcal{E}$:
\begin{equation*}
    M_{U \to V} = \{ m \,|\, m \in M_{U} \land m.\mathsf{receiver} \in V \}.
\end{equation*}
Note that, for every $P_i \in Q$, each message $m \in M_{(P \uplus R) \to \{P_i\}}$ is receive-omitted in $\mathcal{B}_i$.

First, we will prove by contradiction that $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ receives less than $t_S$ messages in $\mathcal{E}$ from processes in $P$. Therefore, assume that there exists a subset $Q'' \subseteq Q$ of $|Q''| > |Q|-t_{Q'} \geq t_Q-t_{Q'}$ processes which receive more than $t_S$ messages in $\mathcal{E}$ from processes in $P$.
As $\mathcal{A}$ sends less than $(t_Q-t_{Q'})\cdot t_S$ messages in execution $\mathcal{E}$, less than $(t_Q-t_{Q'})\cdot t_S$ messages are sent in $\mathcal{E}$ by correct processes (i.e., processes in $P$), which implies $|M_{P \to \tilde{Q}'}| < (t_Q-t_{Q'})\cdot t_S$, thus we reach a contradiction. Hence, $\exists Q' \subset Q$, $|Q'| = t_{Q'}$, such that every process in $Q'$ receive less than $t_S$ messages in $\mathcal{E}$ from processes in $P$, i.e. $\forall P_i \in Q', |M_{P \to \{P_i\}}| \leq t_S$.

Let $P_i \in Q'$.
Let $S_i$ denote the set of processes in $P$ whose messages $P_i$ receive-omits from (and including) round $k$ onward in $\mathcal{B}_i$:
\begin{equation*}
    S_i = \{ P_j \in P \,|\, \exists j \in [k, \infty], \exists m \in \fmsgro{\mathcal{B}_i}{j}: m.\mathsf{sender} = P_j \}.
\end{equation*}
Note that $P_i \notin S_i$ (as no process ever sends messages to itself).
Moreover, as $|M_{P \to \{P_i\}}| \leq t_S$, $|S_i| \leq t_S$.
We now create another execution $\mathcal{E}'_i = [\mathcal{F}', \mathcal{B}_1', ..., \mathcal{B}_n'] = \fswitcho{\mathcal{E}}{\tilde{M}_i}$ where $\tilde{M}_i = M_{(P \uplus R) \to \{P_i\}}$.
We can observe that $P_i$ is correct in $\mathcal{E}'_i$.
Hence, $\mathcal{F}' \subseteq S_i \uplus R \uplus (Q \setminus{\{ P_i \}})$ and $|R| \leq t-t_S-t_Q+1$, thus $|\mathcal{F}'| \leq t$. 
Let us note that some processes in $R$ might be now correct.
By lemma \ref{lemma:switch_omission}, $\mathcal{E}'_i$ is an execution of $\mathcal{A}$.
\iffalse
:
\begin{compactenum}
    \item $\mathcal{F}' \gets S_i \uplus R \uplus (Q \setminus{ \{P_i\}})$.

    \item For every process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, let $\mathcal{B}_j' \gets \mathcal{B}_j$, i.e., $P_j$'s behavior in $\mathcal{E}'$ is identical to $P_j$'s behavior in $\mathcal{E}_i$.

    \item For the process $P_i$, we build $\mathcal{B}_i'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_i' \gets \mathcal{B}_i$.

        \item For every round $k' \in [k, \infty]$ such that $\fmsgro{\mathcal{B}_i}{k'} \neq \emptyset$, we remove all messages from $\fmsgro{\mathcal{B}'_i}{k'}$: $\fmsgro{\mathcal{B}'_i}{k'} \gets \emptyset$.
        Note that all messages removed from $\fmsgro{\mathcal{B}'_i}{k'}$ are sent by processes in $S_i \uplus R$.
    \end{compactenum}
    Note that $P_i$ does not commit any omission faults in $\mathcal{B}_i'$: (1) it does not commit any send-omission faults due to the statement of the lemma, and (2) it does not commit any receive-omission faults due to the step (3)(b). 

    \item For every process $P_j \in S_i \uplus R$, we build $\mathcal{B}_j'$ in the following manner:
    \begin{compactenum}
        \item Let $\mathcal{B}_j' \gets \mathcal{B}_j$.

        \item For every message $m$ such that there exists a round $k' \geq [k, \infty]$ with (1) $m \in \fmsgs{\mathcal{B}_j}{k'}$, and (2) $m \in \fmsgro{\mathcal{B}_i}{k'}$, we perform the following steps:
        \begin{compactenum}
            \item We remove $m$ from sent messages: $\fmsgs{\mathcal{B}_j'}{k'} \gets \fmsgs{\mathcal{B}_j'}{k'} \setminus{\{m\}}$.

            \item We add $m$ to send-omitted messages:
            $\fmsgso{\mathcal{B}_j'}{k'} \gets \fmsgso{\mathcal{B}_j'}{k'} \cup \{m\}$.
        \end{compactenum}
    \end{compactenum}
\end{compactenum}

Let us prove that $\mathcal{E}_i'$ is indeed an execution:
\begin{compactitem}
    \item Faulty processes: As $\mathcal{F}' \subseteq S_i \uplus R \uplus (Q \setminus{\{ P_i \}})$ and $|R| \leq t-t_S-t_Q+1$, thus $|\mathcal{F}'| \leq t$. Potentially, some processes in $R$ are now correct.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$.
    Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    Therefore:
    \begin{compactitem}
        \item For any process $P_j \in \Pi \setminus{ (R \uplus S_i \uplus \{P_i\}) }$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ since $\mathcal{B}_j' = \mathcal{B}_j$. 
        \item For process $P_i$, $\mathcal{B}_i'$ is an infinite behavior of $P_i$ due to \Cref{lemma:behavior_receive_omitted}.
        \item For any process $P_j \in R \uplus S_i$, $\mathcal{B}_j'$ is an infinite behavior of $P_j$ due to \Cref{lemma:behavior_send_transfer}. 
    \end{compactitem}
    

    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s'}{j}$.
    Note that $m \in \fmsgs{\mathcal{B}_s}{j}$ (as no sent messages are added to $\mathcal{B}_s'$).
    Therefore, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$ (due to the send-validity of $\mathcal{E}$).
    We consider two possibilities:
    \begin{compactitem}
        \item If $m$ is not excluded from $\fmsgro{\mathcal{B}_r'}{j}$ by step (3)(b), then $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ as $m$ is included in step (3)(a).

        \item Otherwise, $m$ is excluded by step (3)(b).
        This implies that $j \geq k$, $P_r = P_i$, $P_s \in S_i \uplus R$, $m \in \fmsgro{\mathcal{B}_r}{j}$ and $m \in \fmsgs{\mathcal{B}_s}{j}$.
        Then, by step (4)(b)(i), $m \notin \fmsgs{\mathcal{B}_s'}{j}$ making this case impossible.
    \end{compactitem}
    Send-validity is satisfied in $\mathcal{E}'_i$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $j \geq k$ and $P_r = P_i$ and $m \in \fmsgro{\mathcal{B}_r}{j}$.
        However, this case is impossible as $m \notin \fmsgr{\mathcal{B}_r'}{j} \cup \fmsgro{\mathcal{B}_r'}{j}$ due to the step (3)(b).

        \item Otherwise, $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$.
        Therefore, $m \in \fmsgs{\mathcal{B}_s}{j}$ (as $\mathcal{E}$ satisfies receive-validity), which implies that $m \in \fmsgs{\mathcal{B}_s'}{j}$ as the sending of $m$ is not removed by step (4)(b)(i) while constructing $\mathcal{B}_s'$.
    \end{compactitem}
    Receive-validity is satisfied in $\mathcal{E}'_i$.

    \item Omission-validity:
    Consider a process $P_j$ which commits an omission-fault in $\mathcal{B}_j'$.
    We consider two possibilities:
    \begin{compactitem}
        \item Let $P_j$ commit a send-omission fault in $\mathcal{B}_j'$.
        As no process $P_z \in \Pi \setminus R$ commits a send-omission fault in $\mathcal{B}_z$, $P_j \in R \uplus S_i$ given that we only add send-omitted messages to processes in $R \uplus S_i$. Hence, $P_j \in \mathcal{F}'$.
        In this case, omission-validity is satisfied.

        \item Let $P_j$ commit a receive-omission fault in $\mathcal{B}_j'$.
        Note that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z$, which implies that no process $P_z \in P$ commits a receive-omission fault in $\mathcal{B}_z'$ (as our construction does not add receive-omitted messages to any process).
        
        Moreover, $P_i$ does not commit a receive-omission fault in $\mathcal{B}_i'$ as (1) it does not commit any receive-omission faults in any round $k' \in [1, k - 1]$ in $\mathcal{B}_i$ (due to \Cref{definition:isolation}), and (2) all receive-omitted messages in any round $k' \in [k, \infty]$ are removed by the step (3)(b).
        Therefore, $P_j \in R \uplus (Q \setminus{\{P_i\}})$, which means that omission-validity holds in this case as well.
    \end{compactitem}
    Omission-validity is satisfied in $\mathcal{E}'_i$.
\end{compactitem}

Thus, $\mathcal{E}'_i$ is indeed an execution of $\mathcal{A}$.
\fi
Since $|P|>t_S$, $|S_i|\leq t_S$, $\exists P_j \in P \setminus S_i \neq \emptyset$.

Observe that $P_i$ and $P_j$ are correct in $\mathcal{E}'_i$, and $\mathcal{B}'_j = \mathcal{B}_j$.
Hence, they both decide the same value $b$.

Moreover (1) $P_i$'s states in $\mathcal{B}_i'$ and $\mathcal{B}_i$ are identical, and (2) $P_j$'s states in $\mathcal{B}_j'$ and $\mathcal{B}_j$ are identical.
Therefore, $P_i$ decides $b$ in $\mathcal{E}$.
Thus, every process in $Q'$ decides $b$ in $\mathcal{E}$.
Hence, the lemma holds.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%
%% end formal proof %%
%%%%%%%%%%%%%%%%%%%%%%

We partition all processes into three disjoint groups: (1) group $A$ with $|A| = n - \frac{t}{2}$ processes, (2) group $B$ with $|B| = \frac{t}{4}$ processes, and (3) group $C$ with $|C| = \frac{t}{4}$ processes, where (i) every process in $A$ is always correct and (ii) the set $B$ (resp.  $C$) is either a group of receive-isolated processes from some round or a group of correct processes.

\begin{lemma}[Some isolated processes must agree]\label{lemma:0bis}
Let $\mathcal{E}$ be an infinite execution of $\mathcal{A}$ such that every process in $A$ decides $b_A' \in \{0,1\}$. 
Then,  either the communication complexity of $\mathcal{A}$ is greater than $\frac{n t}{16}$ or $\exists (B', C') \subset B \times C$, $|B'|,|C'| \geq \frac{t}{8}$, such that every process in $B' \cup C'$ decides $b_A'$.
\end{lemma}

\begin{proof}
We apply \Cref{lemma:0} with $(P,Q,R)=(A,B,C)$ (resp. $(P,Q,R)=(A,C, B)$, resp.  $(P,Q,R)=(A\cup B,C, \emptyset)$, resp.  $(P,Q,R)=(A\cup C,B, \emptyset)$), $t_S = \frac{t}{2}, t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$. 
\end{proof}

The \Cref{lemma:0bis} can be seen as a simple generalization of the Dolev-Reischuk result. Before applying it to prove the main lemma of the paper (lemma \ref{lemma:combining_receive_isolation}), we will define a simple construction that describes the correct behavior of a group ($A$ in practice) when the received messages are given.


\iffalse
\begin{corollary}
If $t_Q = 2t_{Q'}$, and the communication complexity of $\mathcal{A}$ is less than $t_{Q'} \cdot t_S$, then $\exists Q' \subset Q$, $|Q| = t_{Q'}$, such that every process in $Q'$ decides $b_P$.
\end{corollary}

\begin{corollary}
If $|P|=n-\frac{t}{4}$, $|Q| = \frac{t}{4}$, $|R|=0$ and the communication complexity of $\mathcal{A}$ is less than $\frac{3nt}{32}$, then $\exists Q' \subset Q$, $|Q| = \frac{t}{8}$, such that every process in $Q'$ decides $b_P$.
\end{corollary}


\begin{lemma}\label{lemma:forced_termination_new}
Lemma \ref{lemma:forced_termination}
Consider an infinite execution $\mathcal{E}$ such that (1) some group $X$ of $|X| = \frac{t}{4}$ processes is receive-isolated from some round $k \geq 1$, and (2) all processes in $\Bar{X}$ are correct.
At least $\frac{|X|}{2}$ processes from $X$ decide in $\mathcal{E}$.
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $|R|=0$, $P = \bar{X}$, $Q = X$ with $t_S = t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$.
\end{proof}


\begin{lemma}\label{lemma:disagreement_quadratic_messages_new}
Lemma \ref{lemma:disagreement_quadratic_messages}
\end{lemma}

\begin{proof}
Apply lemma \ref{lemma:0} with $(Q,R)=(B,C)$ (resp. $(Q,R)=(C,B)$), $P = A$, $t_S = \frac{t}{2}, t_Q = \frac{t}{4}$, $t_{Q'} = \frac{t_Q}{2} = \frac{t}{8}$. We verify $|R| = \frac{t}{4} \leq t-t_S - t_Q+1 = \frac{t}{4} +1$. 
\end{proof}


\begin{corollary}
If $|P|=n-\frac{t}{2}$, $|Q| = |R| = \frac{t}{4}$, $|R|=0$, while $R$ is also receive-isolated after some round and the communication complexity of $\mathcal{A}$ is less than $\frac{nt}{16}$, then $\exists Q' \subset Q$, $|Q| = \frac{t}{8}$, such that every process in $Q'$ decides $b_P$.
\end{corollary}

\fi




\begin{definition}
Let $P = \{P_{i_1}, ..., P_{i_{\ell}}\}$ be a set of correct processes.
Let $\bar{b} : P \rightarrow \{0, 1\}$ that maps each process $P_i \in P$ to a proposal bit $\bar{b}(P_i) \in \{0,1\}$.
Let $M$ be a set of messages not sent by processes in $P$, i.e. $\forall m \in M, m.\mathit{sender} \notin P$.
For every $k \in \mathbb{N} \cup \{\infty\}$,
We define $\mathsf{correct}(P, \bar{b},M,k) \triangleq [\mathcal{B}_{i_1}, ..., \mathcal{B}_{i_{\ell}}]$,  where each $\mathcal{B}_{i} \triangleq \langle \mathcal{F}^1_i, ..., \mathcal{F}^k_i\rangle$ is a $k$-round behavior of process $P_i$ and each $\mathcal{F}^j_i \triangleq (\state{i}{j}, \msgs{i}{j}, \emptyset, \msgr{i}{j}, \emptyset)$ as follows.

\begin{compactenum}
    \item (Initialization) $\forall P_i \in P$:
\begin{itemize}
\item  (correct proposal) $\pstate{i}{1}.\mathit{proposal} = \bar{b}(P_i)$, $  \msgs{i}{1} = \mathcal{M}^{b_i}_i$
\item (received message) $\msgr{i}{1} = \{m \in M \cup (\bigcup_{i \in \{i_{1}, ..., i_{\ell}\}} \msgs{i}{1}) | m.\mathit{round} = 1 \wedge m.\mathit{receiver} = P_i\}$
\end{itemize}    
    \item (Induction) $\forall P_i \in P, \forall j \in [1:k]$:
    \begin{itemize}
\item  (correct transition) if $j<k$, $(\pstate{i}{j+1}, \msgs{i}{j+1}) = \mathcal{A}(\pstate{i}{j}, \msgr{i}{j})$
\item (received message) $\msgr{i}{j} = \{m \in M \cup (\bigcup_{i \in \{i_{1}, ..., i_{\ell}\}} \msgs{i}{j}) | m.\mathit{round} = j \wedge m.\mathit{receiver} = P_i\}$
\end{itemize}    
\end{compactenum}
\end{definition}

\iffalse
%%%%%%%%%%%%
%% useless lemma %%
%%%%%%%%%%%%
\begin{lemma}
Let $P = \{P_{i_1}, ..., P_{i_{\ell}}\}$ be a set of correct processes.
Let $\bar{b} : P \rightarrow \{0, 1\}$ that maps each process $P_i \in P$ to a proposal bit $\bar{b}(P_i) \in \{0,1\}$. Let $(k',k) \in \mathbb{N} \times (\mathbb{N} \cup \{\infty\})$ with $k' < k$.
Let $M = M_{\leq k'} \uplus M_{>k'}$ be a set of messages not sent by processes in $P$ (i.e. $\forall m \in M, m.\mathit{sender} \notin P$), such that (1) $\forall m \in M_{\leq k'}$, $m.\mathsf{round} \leq k'$ and $\forall m \in M_{> k'}$, $m.\mathsf{round} > k'$.

Let $[\mathcal{B}_{i_1}, ..., \mathcal{B}_{i_{\ell}}] = \mathsf{correct}(P, \bar{b},M,k)$ and $[\mathcal{B}'_{i_1}, ..., \mathcal{B}'_{i_{\ell}}] = \mathsf{correct}(P, \bar{b},M_{\leq k'},k')$.

For every $P_i \in P$, we note $\mathcal{B}'_{i} = \langle \mathcal{F}_{i}^{\prime 1}, ...,  \mathcal{F}_{i}^{\prime k'}\rangle$ and $\mathcal{B}_{i} = \langle \mathcal{F}_{i}^{1}, ...,  \mathcal{F}_{i}^{k}\rangle$.

Then, $\forall P_i \in P$,  $\forall j \in [1:k']$, $\mathcal{F}^{j}_{i} = \mathcal{F}^{\prime j}_{i} $
\end{lemma}

\begin{proof}
It is trivial to realise that the construction are the same ones until round $k'$.
\end{proof}

%%%%%%%%%%%%%%
%% end useless lemma %%
%%%%%%%%%%%%%%
\fi

Now, we are ready to prove the key lemma of the paper.

\begin{lemma}[Combining receive-isolation]\label{lemma:combining_receive_isolation}
Let  $\bar{b}^u, \bar{b}^v: \Pi \rightarrow \{0,1\}$.
Let $\mathcal{A}$ be an agreement algorithm.
Let $\mathcal{E}^{u}$ and $\mathcal{E}^{v}$ be two infinite executions of $\mathcal{A}$ such that:
\begin{compactitem}
\item $\forall P_i \in \Pi$, $P_i$ proposes $\bar{b}^u(P_i)$ (resp.  $\bar{b}^v(P_i)$) in $\mathcal{E}^{u}$ (resp.  $\mathcal{E}^{v}$).
\item in $\mathcal{E}^{u}$: $A \cup B $ are correct,  while $C$ is receive-isolated from some round $k^u$ onward. 
\item in $\mathcal{E}^{v}$: $A \cup C $ are correct,  while $B$ is receive-isolated from some round $k^v$ onward.
\item $A$ decides $b'_u$ in $\mathcal{E}^{u}$ and $b'_v$ in $\mathcal{E}^{v}$
\end{compactitem}
If either (1) $k^u = k^v = 1$ or (2) $|k^u-k^v| \leq 1$ and $\bar{b}^u = \bar{b}^v$. \newline
Then,  either (3) the message-complexity of $\mathcal{A}$ is greater than $\frac{t^2}{16}$, or (4) $b'_u = b'_v$.
\end{lemma}

\begin{proof}[formal proof] (see figure \ref{figure:lemma_343} for case (1) and \ref{figure:lemma_343} for case (2) )
By contradiction, let us assume than both the message-complexity of $\mathcal{A}$ is lower than $\frac{t^2}{16}$, and $b'_u \neq b'_v$.

We note $\mathcal{E}^u = [\mathcal{F}^u, \mathcal{B}^{u}_1, ...,  \mathcal{B}^{u}_n]$ and $\mathcal{E}^v = [\mathcal{F}^v, \mathcal{B}^{v}_1, ...,  \mathcal{B}^{v}_n]$.
By lemma \ref{lemma:0bis}, there exists a set $B' \subset B$ of $|B'| = \frac{t}{8}$ processes that decide $b'_u$ in $\mathcal{E}^u$ and there exists a set $C' \subset C$ of $|C'| = \frac{t}{8}$ processes that decide $b'_v$ in $\mathcal{E}^v$.
Let's construct a new infinite execution $\mathcal{E}^{*} = [\mathcal{F}^{*}, \mathcal{B}^{*}_1, ...,  \mathcal{B}^{*}_n]$, as follows:
\begin{compactenum}

\item (Message naming) We note:

\begin{compactitem}
\item $k^{-} = \mathsf{min}(k^u, k^{w})$ and $k^{+} = \mathsf{max}(k^u, k^{w})$.

\item  $M^{S(B,C)} = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{v}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{u}_i}{k'} \big)$.

%\item  $M^{S(B,C)}_{\leq k^{-}}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k^{-}]}  \fmsgs{\mathcal{B}^{v}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k^{-}]}  \fmsgs{\mathcal{B}^{u}_i}{k'} \big)$.

%\item $M^{S(B,C)}_{> k^{-}}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [k^{-}+1:k]}  \fmsgs{\mathcal{B}^{v}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [k^{-}+1:k]}  \fmsgs{\mathcal{B}^{u}_i}{k'} \big)$.

%\item  $M^{S(B,C)} = M^{S(B,C)}_{\leq k^{-}} \uplus M^{S(B,C)}_{> k^{-}}$

\end{compactitem}



\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A : A  \rightarrow \{0,1\}$ with $\forall P_i \in A, \bar{b}_A(P_i) = \bar{b}^{u}(P_i)$.  We define
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

\item Let $P_i \in B\cup C$. We note $ \mathcal{B}_{i} =  \mathcal{B}^{v}_{i}$ if $P_i \in B$ and $ \mathcal{B}_{i} =  \mathcal{B}^{u}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}^{*}_{i} \gets \mathcal{B}_{i}$. \label{item:init_behaviours_receive_isolated_groups_in_combined_execution}

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], $

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup C} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in B$, and  

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup B} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in C$\label{item:replace_receive_omission_in_combined_execution}

\item $\mathcal{F}^{*} \subseteq \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}^{*}_i}{k'} \neq \emptyset\}$

\end{compactenum}


Let us show that $\mathcal{E}^{*}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} = B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior. Let $P_i \in \Pi$. If $P_i \in A$,  $\mathcal{B}_i^{*}$ is an infinite behavior of process $P_i$ by construction of $\mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.  If $P_i \in B \cup B$, $\mathcal{B}_i^{*}$ is   is an infinite behavior of process by \ref{lemma:behavior_receive_omitted} applied to the infinite behavior $\mathcal{B}_i$.  
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $ \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $ \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

\item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgr{\mathcal{B}_r}{j}$ by send-validity of $\mathcal{E}^u$ and $\mathcal{E}^v$ so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_in_combined_execution}.

\item If $(P_s, P_r) \in A \times (B \cup C) \cup (B \times C) \cup (C \times B)$, $m \in \fmsgro{\mathcal{B}^{*}_r}{j}$ is ensured by step \ref{item:replace_receive_omission_in_combined_execution} of the construction of $\mathcal{E}^{*}$, while no step modifies $\fmsgro{\mathcal{B}^{*}_r}{j}$ afterwards.

\end{compactitem}
    
    
    
    Send-validity is satisfied in $\mathcal{E}^{*}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r^{*}}{j} \cup \fmsgro{\mathcal{B}_r^{*}}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.

 \item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgs{\mathcal{B}_s}{j}$ by send-validity of $\mathcal{E}^u$ and $\mathcal{E}^v$, so $m \in \fmsgs{\mathcal{B}_r}{j}$, since $\fmsgs{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_in_combined_execution}.

\item If $(P_s, P_r) \in (A \times (B \cup C)) \cup (B \times C) \cup (C \times B)$,  $m \notin \fmsgr{\mathcal{B}_r}{j}$. 
If $m \in \fmsgro{\mathcal{B}^{*}_r}{j}$, then
$m \in \fmsgs{\mathcal{B}^{*}_s}{j}$,   by step \ref{item:replace_receive_omission_in_combined_execution}, while no step modifies neither $\fmsgs{\mathcal{B}^{*}_s}{j}$ or $ \fmsgro{\mathcal{B}^{*}_r}{j}$ afterwards.

So let us assume $m \in \fmsgr{\mathcal{B}^{*}_r}{j}$. 

In that case, $j \leq k^{-}$. Indeed, $B$ (resp. $C$) is receive-isolated from the round $k^v$ (resp. $k^u$) in execution $\mathcal{E}^u$ (resp.  $\mathcal{E}^v$), so $j > k^{-}$ would imply $m \notin \fmsgr{\mathcal{B}_r}{k^{-}}$. Finally, it would imply $m \notin \fmsgr{\mathcal{B}_r^{*}}{k^{-}}$ by step \ref{item:init_behaviours_receive_isolated_groups_in_combined_execution}, while no step modifies $ \fmsgr{\mathcal{B}^{*}_r}{j}$ afterwards.

Moreoever, the condition $k^{u} = k^{v}=1$ does not hold, since $B \cup C$ would be receive-isolated from the first round of the execution $\mathcal{E}^{*}$. Hence, in addition of $j \leq k^{-}$, the condition $|k^u-k^v| \leq 1 \wedge \bar{b}^u = \bar{b}^v$
necessarily holds, to satisfy the precondition of the lemma.

Since no group of processes is receive-isolated before $k^{-}$,  and $\bar{b}^u = \bar{b}^v$, the executions $\mathcal{E}^{u}$, $\mathcal{E}^{v}$,  and $\mathcal{E}^{*}$ share a common prefix until round $k^{-}-1$ and messages sent in round $k^{-}$, which means that $\forall k' \in [1:k^{-}] $, $\bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{*}}{k'} = \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{u}}{k'} = \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{v}}{'}$.
Hence, $ \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{*}}{j} =  \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{u}}{j} =  \bigcup_{P_i \in \Pi} \fmsgs{\mathcal{B}_i^{v}}{j} \triangleq M_{j}$.

By receive-validity of $\mathcal{E}^{u}$ and $\mathcal{E}^{v}$, $m \in M_{j}$ and so $m \in  \fmsgs{\mathcal{B}^{*}_s}{j}$.

\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}^{*}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}^{*}$ since no process in $A$ commits any omission fault by construction of $ \mathsf{correct}(A, \bar{b}_A,M^{S(B,C)},k)$.
\end{compactitem}
Thus, $\mathcal{E}^{*}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $b'_u$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $b'_v$ in $\mathcal{E}^*$.
By \Cref{lemma:0bis}, correct processes send at least $\frac{nt}{16}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{nt}{16}$ messages in every execution.

Thus, the lemma holds.

\end{proof}

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/lemma_343.eps}
\caption{Lemma \ref{lemma:combining_receive_isolation}, case (1) }
\label{figure:lemma_343}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/lemma_344.eps}
\caption{Lemma \ref{lemma:combining_receive_isolation}, case (2)}
\label{figure:lemma_344}
\end{figure}

In the rest of the proof, we assume the message complexity of $\mathcal{A}$ is lower than $\frac{n t}{16}$. Moreover, we rely on the following two infinite executions:
\begin{compactitem}
    \item $\mathcal{E}_0$: 
    The group $B$ is receive-isolated from round $1$; all other processes are correct.
    Every process proposes $0$. 

    \item $\mathcal{E}_1$:
    The group $C$ is receive-isolated from round $1$; all other processes are correct.
    Every process proposes $1$.
\end{compactitem}

\begin{lemma}
Let $\mathcal{E}_0$ and $\mathcal{E}_1$ as defined above and presented in figure \ref{figure:lemma_3}.
There exists a pair of sets $(B', C') \subset B \times C$ of size $|B'| = |C'| = \frac{t}{8}$ such that processes  in $A \cup C \cup B'$ decide $b \in \{0, 1 \}$ in $\mathcal{E}_0$ and $A \cup B \cup C'$ decide $b' \in \{0, 1 \}$ in $\mathcal{E}_1$.
Moreover either $b = 1$ or $b'=0$.
\end{lemma}

\begin{proof}%[New proof]
We apply \Cref{lemma:combining_receive_isolation} to executions $\mathcal{E}^u=\mathcal{E}_0$ and $\mathcal{E}^v = \mathcal{E}_1$ and $k^{u} = k^{v} = 1$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}[proof sketch]
(see figure \ref{figure:lemma_3})
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{8}$ processes that decide $b$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{8}$ processes that decide $b'$ in $\mathcal{E}_1$.
%\pierre{it seems to me we can avoid the set of size $\frac{|B|}{4}$ (resp. $\frac{|C|}{4}$ invoked in the proof of lemma \ref{lemma:either} (lemma 3). The remaining part is the same.}
By contratiction, assume $b=0$ and $b'=1$. Let's construct a new infinite execution $\mathcal{E}^{*}$, such that $\mathcal{E}^{*}|_{B} \equiv \mathcal{E}_0|_{B}$ and $\mathcal{E}^{*}|_{C} \equiv \mathcal{E}_1|_{C}$:

\begin{compactenum}
    \item In $\mathcal{E}^*$, all processes from $A \cup B$ propose $0$, whereas all processes from $C$ propose $1$.

    \item All processes from $A$ are correct, whereas all processes from $B \cup C$ are faulty.
    Note that $|B \cup C| < t$.

    \item Every process from $B$ exhibits the exact same behavior as in $\mathcal{E}_0$.
    Note that this step implies that $B$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    \item Every process from $C$ exhibits the exact same behavior as in $\mathcal{E}_1$.
    Note that this step implies that $C$ is receive-isolated from round $1$ in $\mathcal{E}^*$.

    % \item Both groups $B$ and $C$ are receive-isolated from round $1$.
\end{compactenum}
Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages}, correct processes send at least $\frac{t^2}{32}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{32}$ (or even $\frac{t^2}{16}$) messages in every execution.
Thus, the lemma holds.
\end{proof}

\begin{proof}[formal proof]
We note $\mathcal{E}_0 = [\mathcal{F}_0, \mathcal{B}^{0}_1, ...,  \mathcal{B}^{0}_n]$ and $\mathcal{E}_1 = [\mathcal{F}_1, \mathcal{B}^{1}_1, ...,  \mathcal{B}^{1}_n]$.
By lemma \ref{lemma:0} applied twice, there exists a set $B' \subset B$ of $|B'| = \frac{t}{4}$ processes that decide $b$ in $\mathcal{E}_0$ or there exists a set $C' \subset C$ of $|C'| = \frac{t}{4}$ processes that decide $b'$ in $\mathcal{E}_1$.
By contratiction, assume $b=0$ and $b'=1$. Let's construct a new infinite execution $\mathcal{E}^{*} = [\mathcal{F}^{*}, \mathcal{B}^{*}_1, ...,  \mathcal{B}^{*}_n]$, as follows:
\begin{compactenum}
\item $\mathcal{F}^{*} = B \cup C$

\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{0}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{1}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M,k)$.

\item $\forall P_i \in B\cup C$, we note $ \mathcal{B}_{i} =  \mathcal{B}^{0}_{i}$ if $P_i \in B$ and $ \mathcal{B}_{i} =  \mathcal{B}^{1}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}^{*}_{i} \gets \mathcal{B}_{i}$.

%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], $

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup C} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in B$, and  

$\fmsgro{\mathcal{B}^{*}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup B} \fmsgs{\mathcal{B}^{*}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in C$\label{item:replace_receive_omission_in_e_star}

\item $\mathcal{F} \subseteq \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}^{*}_i}{k'} \neq \emptyset\}$

\end{compactenum}


Let us show that $\mathcal{E}^{*}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} = B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j'$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times (B \cup C)$, $m \in \fmsgr{\mathcal{B}_r^{*}}{j}$ is ensured by step \ref{item:replace_receive_omission_in_e_star} of the construction of $\mathcal{E}^{*}$.
\end{compactitem}
    
    
    
    Send-validity is satisfied in $\mathcal{E}^{*}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r^{*}}{j} \cup \fmsgro{\mathcal{B}_r^{*}}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times (B \cup C)$, $m \in \fmsgro{\mathcal{B}_r^{*}}{j}$, since $\fmsgr{\mathcal{B}_r^{*}}{j} = \emptyset$ by construction, because $\fmsgr{\mathcal{B}_r}{j} = \emptyset$ and no additional received messages are added during the contruction of $\mathcal{B}_r^{*}$.
Thus, $m \in \fmsgs{\mathcal{B}_s^{*}}{j}$ is ensured by step \ref{item:replace_receive_omission_in_e_star} of the construction of $\mathcal{E}^{*}$.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}^{*}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}^{*}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}^{*}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}^*$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}^*$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}^*$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}^*$, which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Hence, the assumption $b=0$ and $b'=1$ is false, which means that either $b=1$ or $b'=0$.
Thus, the lemma holds.

\end{proof}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end  lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_3.eps}
\caption{Lemma \ref{lemma:either}}
\label{figure:lemma_3}
\end{figure}

Then, we define the execution $\mathcal{E}^{k^{*}}$, and $\mathcal{E}^{k^{*}+1}$ as in the prologue of lemma \ref{lemma:final} (lemma 4), and illustrated in figure \ref{figure:execution_C}. Without loss of generality, it has been assumed that processes in $A$ decide $b=1$ in execution $\mathcal{E}_0$.

Next, let $\mathcal{E}^*_0$ denote the fully-correct infinite execution in which all processes propose $0$.
Note that, in order to satisfy \emph{Weak Validity}, all processes decide $0$ in $\mathcal{E}_0^*$.
Let $k_0^* \in \mathbb{N}^+$ denote the first round in which (at least) $\frac{t}{8}$ processes from $B$ decide the same bit in $\mathcal{E}_0^*$.

For every round $k \in [1, k_0^*]$, we perform the following actions:
\begin{compactenum}
    \item We consider the infinite execution $\mathcal{E}^k$ such that (1) every process proposes $0$, (2) every process behaves correctly until (and including) round $k - 1$ (i.e., no omission faults occur), (3) group $B$ is receive-isolated from round $k$, and (4) processes in $A \cup C$ are correct.

    \item By \Cref{lemma:0bis}, at least $\frac{t}{8}$ processes from $B$ decide the same bit $b_k$ in $\mathcal{E}^k$.
\end{compactenum}
Importantly, $b_1 = 1$ (due to the assumption) and $b_{k_0^*} = 0$ (due to the execution $\mathcal{E}_0^*$).
Hence, there exists a round $k^* \geq 1$ such that $b_{k^*} = 1$ and $b_{k^* + 1} = 0$.

Now, consider an infinite execution $\mathcal{E}_C$ such that (1) every process proposes $0$, (2) every process behaves correctly until (and including) round $k^* - 1$, (3) group $C$ is receive-isolated from round $k^*$, and (4) processes in $A \cup B$ are correct.
By \Cref{lemma:0bis}, at least $\frac{t}{8}$ processes from $C$ decide the same bit $b_C$.

Finally, we are ready to prove a contradiction with the assumed non-existence of an execution of $\mathcal{A}$ with (at least) $\frac{nt}{16}$ messages sent by correct processes.

\iffalse

Let $\mathcal{E}^{k^*} = [\mathcal{F}^{k^*} = B, \mathcal{B}^{k^*}_1, ..., \mathcal{B}^{k^*}_n]$, let $\mathcal{E}^{k^* + 1} = [\mathcal{F}^{k^* + 1} = B, \mathcal{B}^{k^* + 1}_1, ..., \mathcal{B}^{k^* + 1}_n]$ and let $\mathcal{E}^C = [\mathcal{F}^C = C, \mathcal{B}_1^C, ..., \mathcal{B}_n^C]$.
The following holds:
\begin{compactitem}
    \item At least $\frac{t}{8}$ processes from $B$ decide the $1$ in $\mathcal{E}^{k^*}$.

    \item At least $\frac{t}{8}$ processes from $B$ decide the $0$ in $\mathcal{E}^{k^* + 1}$.
    
    \item At least $\frac{|C|}{4}$ processes from $C$ decide the same bit $b_C$ in $\mathcal{E}^C$.

    \item Until (and including) round $k^* - 1$, $\mathcal{B}_i^{k^*} = \mathcal{B}_i^{k^* + 1} = \mathcal{B}_i^C$, for every process $P_i$.
\end{compactitem}

\fi

\begin{figure}[!t]
\centering
\includegraphics[clip, trim=0cm 6.5cm 0cm 0cm, width=13cm]{figures/quadratic_lower_bound_execution_C.eps}
\caption{Executions $\mathcal{E}^{k^{*}}$ and $\mathcal{E}^{k^{*}+1}$}
\label{figure:execution_C}
\end{figure}

\begin{lemma}
There exists an execution of $\mathcal{A}$ in which correct processes send (at least) $\frac{n t}{16}$ messages.
\end{lemma}

\begin{proof}%[New proof]
We apply lemma \ref{lemma:combining_receive_isolation}, case (2),  twice, to executions $\mathcal{E}^u=\mathcal{E}_C$ and $\mathcal{E}^v = \mathcal{E}^{k^{*}}$ in case $b_C=0$ and  $\mathcal{E}^v = \mathcal{E}^{k^{*}+1}$ in case $b_C=1$,  where $(k^{u}, k^{v}) = (k^{*}, k^{*}+1)$, and $\forall P_i \in \Pi$, $\bar{b}^{u}(P_i) = \bar{b}^{v}(P_i) = 0$.  Since $b_{k^{*}} = 1$ and $b_{k^{*}+1} = 1$, either $b_C \neq b_{k^{*}}$ or $b_C \neq b_{k^{*}+1} = 1$.  Thus, there exists an execution of $\mathcal{A}$ in which correct processes send (at least) $\frac{n t}{16}$ messages. (see figure \ref{figure:lemma_final})
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}[proof sketch]
(see figure \ref{figure:lemma_4})
We consider two possible cases:
\begin{compactitem}
    \item Let $b_C = 0$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Both groups $B$ and $C$ are receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^*}$ (from round $k^*$ onward).
        Note that this step implies that $B$ is receive-isolated from round $k^*$.

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item From (and including) round $k^*$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.

% this is pointless, by item 4. not really, will change something more
        % \item From (and including) round $k^*$ onward, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$ in $\mathcal{E}^k$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$ in $\mathcal{E}_C$.
    \end{compactenum}
    
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $1$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $0$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.

    \item Let $b_C = 1$.
    We now construct an execution $\mathcal{E}$ such that $\mathcal{E}|_B \equiv \mathcal{E}^{k^{*}+1}|_B$ and $\mathcal{E}|_C \equiv \mathcal{E}_C|_C$ (the receive-omitted messages are not necessarily equals) in the following manner:
    \begin{compactenum}
        \item Processes in $A$ are correct, whereas all other processes are faulty.

        \item All processes propose $0$.

        \item Until (and including) round $k^* - 1$, $\mathcal{E}$ is identical to $\mathcal{E}_0$, i.e., every process behaves correctly until round $k^* - 1$.

        % \item Group $C$ is receive-isolated from round $k^*$, whereas group $B$ is receive-isolated from round $k^*+1$

        \item For every process $c \in C$, $c$'s behavior in the continuation of $\mathcal{E}$ is identical to $c$'s behavior in $\mathcal{E}_C$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^*$.

        \item For every process $b \in B$, $b$'s behavior in the continuation of $\mathcal{E}$ is identical to $b$'s behavior in $\mathcal{E}^{k^* + 1}$ (from round $k^*$ onward).
        Note that this step implies that $C$ is receive-isolated from round $k^* + 1$.
        \add{Note that the message received in round $k^{*}$ from processes in $C$ are indeed the same ones than in execution $\mathcal{E}^{k^* + 1}$, since the receive-omission at round $k^*$ has no impact of the messages at the same round $k^*$.} 

        \item In round $k^*$, all messages from $C$ are received, which means that processes in $B$ successfully receive messages sent by $C$.

        \item From (and including) round $k^* + 1$ onward, we receive-omit (1) all messages sent by processes in $B$ to $C$ in $\mathcal{E}^{k^*}$, and (2) all messages sent by processes in $C$ to $B$ in $\mathcal{E}_C$.
        
        
        % we send-omit (1) all messages sent by processes in $C$ to processes in $A$ in $\mathcal{E}_C$.
        % Note that, in round $k^*$, messages sent by processes in $C$ to processes in $B$ are successfully sent and successfully received.

        % \item From round $k^* + 1$, we send-omit (1) all messages successfully sent by processes in $B$ to processes in $\bar{B}$, and (2) all messages successfully sent by processes in $C$ to processes in $\bar{C}$.
    \end{compactenum}
    Hence, the following holds for $\mathcal{E}$: (1) at least \replace{$\frac{|B|}{4}$}{$\frac{|B|}{2}$} processes from $B$ decide $0$, and (2) at least \replace{$\frac{|C|}{4}$}{$\frac{|C|}{2}$} processes \add{from $C$} decide $1$. 
    By \Cref{lemma:disagreement_quadratic_messages}, correct processes send (at least) $\frac{t^2}{32}$ messages in $\mathcal{E}$, which concludes the lemma in this case.
\end{compactitem}
As the statement of the lemma holds in both possible cases, the proof is concluded.
\end{proof}

\begin{proof}[formal proof]
We note $\mathcal{E}_C = [\mathcal{F}_C, \mathcal{B}^{C}_1, ...,  \mathcal{B}^{C}_n]$, $\mathcal{E}^{k^{*}} = [\mathcal{F}_{k^{*}}, \mathcal{B}^{k^{*}}_1, ...,  \mathcal{B}^{k^{*}}_n]$ and $\mathcal{E}^{k^{*}+1} = [\mathcal{F}_{k^{*}+1}, \mathcal{B}^{k^{*}+1}_1, ...,  \mathcal{B}^{k^{*}+1}_n]$.

Case $b_C = 0$.

Let's construct a new infinite execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ...,  \mathcal{B}_n]$, as follows:
\begin{compactenum}

\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{k^{*}}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{C}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M^S_{(B,C)},k)$.

\item $\forall P_i \in B\cup C$, we note $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{k^{*}}_{i}$ if $P_i \in B$ and $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{C}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}_{i} \gets \tilde{\mathcal{B}}_{i}$. \label{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}

%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], $

$\fmsgro{\mathcal{B}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup C} \fmsgs{\mathcal{B}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in B$, and  

$\fmsgro{\mathcal{B}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in A \cup B} \fmsgs{\mathcal{B}_j}{k'} | m.\mathsf{receiver} = P_i\}$ if $P_i \in C$\label{item:replace_receive_omission_when_bc_equal_0}

\item $\mathcal{F} = \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}_i}{k'} \neq \emptyset\}$
\end{compactenum}


Let us show that $\mathcal{E}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} \subseteq B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgr{\tilde{\mathcal{B}}_r}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.

\item If $(P_s, P_r) \in A \times (B \cup C) \cup (B \times C) \cup (C \times B)$, $m \in \fmsgro{\mathcal{B}_r}{j}$ is ensured by step \ref{item:replace_receive_omission_when_bc_equal_0} of the construction of $\mathcal{E}$, while no step modifies $\fmsgro{\mathcal{B}_r}{j}$ afterwards.
\end{compactitem}
    

    Send-validity is satisfied in $\mathcal{E}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.

\item If $(P_s, P_r) \in (A \times (B \cup C)) \cup (B \times C) \cup (C \times B)$,  $m \notin \fmsgr{\tilde{\mathcal{B}}_r}{j}$ since both $B$ and $C$ are receive isolated in $\mathcal{E}^{k^{*}}$ and $\mathcal{E}^C$ respectively.  Moreover, $\fmsgr{\mathcal{B}_r}{j} = \fmsgr{\tilde{\mathcal{B}}_r}{j}$ because no step modifies $\fmsgr{\mathcal{B}_r}{j}$ after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}. Hence, $m \notin \fmsgr{\mathcal{B}_r}{j}$,  and so $m \in \fmsgro{\mathcal{B}_r}{j}$.
Finally, 
$m \in \fmsgs{\mathcal{B}_s}{j}$,   by step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}, while no step modifies neither $\fmsgs{\mathcal{B}_s}{j}$ or $ \fmsgro{\mathcal{B}_r}{j}$ afterwards.

 \item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgs{\tilde{\mathcal{B}}_s}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}$, the following holds: (1) all processes from $B'$ decide $1$ in $\mathcal{E}$, and (2) all processes from $C'$ decide $0$ in $\mathcal{E}$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}$.
%which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Thus, the lemma holds.

Case $b_C = 1$.

Let's construct a new infinite execution $\mathcal{E} = [\mathcal{F}, \mathcal{B}_1, ...,  \mathcal{B}_n]$, as follows:
\begin{compactenum}


\item We note $M^S_{(B,C)}  = \bigcup\limits_{P_i \in B} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{k^{*}+1}_i}{k'} \big) \cup \bigcup\limits_{P_i \in C} \big( \bigcup\limits_{k' \in [1:k]}  \fmsgs{\mathcal{B}^{C}_i}{k'} \big)$.


\item Let $A = \{P_{i_1}, ..., P_{i_{\ell}}\}$.  Let $\bar{b}_A = (0, ..., 0)$ with $|\bar{b}_A| = \ell$. 
$ [\mathcal{B}^{*}_{i_1}, ..., \mathcal{B}^{*}_{i_{\ell}}] \gets \mathit{correct}(A, b,M^S_{(B,C)},k)$.

\item $\forall P_i \in B\cup C$, we note $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{k^{*}+1}_{i}$ if $P_i \in B$ and $ \tilde{\mathcal{B}}_{i} =  \mathcal{B}^{C}_{i}$ if $P_i \in C$.  Moreover,  $\mathcal{B}_{i} \gets \tilde{\mathcal{B}}_{i}$.
\label{item:init_behaviours_receive_isolated_groups_when_bc_equal_1}
%\item $\forall P_i \in B, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{0}_{i}$ and $\forall P_i \in C, \mathcal{B}^{*}_{i} \gets \mathcal{B}^{1}_{i}$.

\item $\forall P_i \in B \cup C, \forall k' \in [1:k], \fmsgro{\mathcal{B}_{i}}{k'} \gets \{ m \in \bigcup\limits_{P_j \in \Pi \setminus \{P_i\}} \fmsgs{\mathcal{B}_j}{k'} | m.\mathsf{receiver} = P_i\}$ \label{item:replace_receive_omission_when_bc_equal_1}

\item $\mathcal{F} = \{P_i \in  B \cup C | \exists k' \in [1:k], \fmsgro{\mathcal{B}_i}{k'} \neq \emptyset\}$
\end{compactenum}

Let us show that $\mathcal{E}$ is a valid execution of $\mathcal{A}$
\begin{compactitem}
 \item Faulty processes: $\mathcal{F}^{*} \subseteq B \cup C$, thus $ |\mathcal{F}^{*}| \leq t$.

    \item Composition: Holds due to the construction of each behavior $\mathcal{B}_j$. \pierre{TO DO}
    
    
    %Since $\mathcal{E}$ is an execution, then, for every process $P_j$, $\mathcal{B}_j$ is a infinite behavior of $P_j$.
    %Therefore, for every process $P_j$, $\mathcal{B}'_j$ is a infinite behavior of $P_j$ by successive application of \Cref{lemma:behavior_receive_omitted} and \Cref{lemma:behavior_send_transfer}.
    
    \item Send-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgs{\mathcal{B}_s}{j}$.
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgr{\tilde{\mathcal{B}}_r}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.

\item If $(P_s, P_r) \in A \times (B \cup C) \cup (B \times C) \cup (C \times B)$, $m \in \fmsgro{\mathcal{B}_r}{j}$ is ensured by step \ref{item:replace_receive_omission_when_bc_equal_0} of the construction of $\mathcal{E}$, while no step modifies $\fmsgro{\mathcal{B}_r}{j}$ afterwards.
\end{compactitem}
    

    Send-validity is satisfied in $\mathcal{E}$.

    \item Receive-validity:
    Consider any message $m$, where $P_s = m.\mathsf{sender}$, $P_r = m.\mathsf{receiver}$ and $j = m.\mathsf{round}$, such that $m \in \fmsgr{\mathcal{B}_r}{j} \cup \fmsgro{\mathcal{B}_r}{j}$. 
\begin{compactitem}
\item If $(P_s, P_r) \in A \times A$,  $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (B \cup C) \times A$, $m \in M^{S}_{(B, C)}$ and so $m \in \fmsgs{\mathcal{B}_s}{j}$ by construction of $\mathit{correct}(A, b,M,k)$.
\item If $(P_s, P_r) \in (A \times (B \cup C)) \cup (B \times C) \cup (C \times B)$,  $m \notin \fmsgr{\tilde{\mathcal{B}}_r}{j}$ since both $B$ and $C$ are receive isolated in $\mathcal{E}^{k^{*}+1}$ and $\mathcal{E}^C$ respectively.  Moreover, $\fmsgr{\mathcal{B}_r}{j} = \fmsgr{\tilde{\mathcal{B}}_r}{j}$ because no step modifies $\fmsgr{\mathcal{B}_r}{j}$ after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}. Hence, $m \notin \fmsgr{\mathcal{B}_r}{j}$,  and so $m \in \fmsgro{\mathcal{B}_r}{j}$.
Finally, 
$m \in \fmsgs{\mathcal{B}_s}{j}$,   by step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}, while no step modifies neither $\fmsgs{\mathcal{B}_s}{j}$ or $ \fmsgro{\mathcal{B}_r}{j}$ afterwards.

 \item If $(P_s, P_r) \in (B \times B) \cup (C \times C)$,  $m \in \fmsgs{\tilde{\mathcal{B}}_s}{j}$ by send-validity of $\tilde{\mathcal{B}}_r$ and so $m \in \fmsgr{\mathcal{B}_r}{j}$, since $\fmsgr{\mathcal{B}_r}{j}$ is not modified after step \ref{item:init_behaviours_receive_isolated_groups_when_bc_equal_0}.
\end{compactitem}    
Receive-validity is satisfied in $\mathcal{E}$.
    
    \item Omission-validity is obviously satisfied in $\mathcal{E}$ since no process in $A$ commits any omission fault by construction of $\mathit{correct}(A, b,M,k)$.
\end{compactitem}
Thus, $\mathcal{E}$ is indeed an execution of $\mathcal{A}$. 

Due to the construction of $\mathcal{E}$, the following holds: (1) all processes from $B'$ decide $0$ in $\mathcal{E}$, and (2) all processes from $C'$ decide $1$ in $\mathcal{E}$.
By \Cref{lemma:disagreement_quadratic_messages_new}, correct processes send at least $\frac{t^2}{16}$ messages in $\mathcal{E}$.
%which contradicts the fact that $\mathcal{A}$ sends less than $\frac{t^2}{16}$ messages in every execution.
Thus, the lemma holds.
\end{proof}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end  lemma proof removed by more general lemma on combined receive isolation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
\centering
\includegraphics[width=13cm]{figures/quadratic_lower_bound_lemma_4.eps}
\caption{Lemma \ref{lemma:final}}
\label{figure:lemma_final}
\end{figure}






